Foundations of Work-Systems Modeling

In 2006, the course "Modeling of Organizations" is taught for the third time. This third time will be the second time we will use the new lecture notes "Work Systems Modelling" from the DA VINCI series. These lecture notes, however, will be evolved further hand-in-hand with the actual process of lecturing. In the academic year 2005/2006, a second incarnation of these lecture notes will be created, where the aim is to deliver these lecture notes in three increments. An important step that will be taken in this academic year is the integration of the ICIS Work Systems Modelling lecture notes with the NICI course on Organisational Dynamics. The first results of this integration will start to appear in the second and third trimester.

==> courses/agent-based-information-systems/description.tex <==
\Course{Agent-based Information Systems}

\Synopsis
The purpose of this course is to introduce the paradigm of intelligent agency.
Intelligent agents are software programs that can autonomously perform tasks
for users. The ideal agent can perceive its environment, communicate with other
agents, and take a series of actions to achieve a complex goal. The potential
applications of agents are numerous: including web search assistants, travel
advisors, electronic secretaries, and bidders in on-line auctions. The course
will cover the underlying theory of agents, the common agent architectures, the
potential applications for agents, and will let students construct their own
agents. 

\Goals
\begin{enumerate}
   \item design and construct intelligent agents, 
   \item apply formal models and logic of rational agency, 
   \item determine in which situations agent architectures should be used. 
\end{enumerate}

\Topics
Planning, plan recognition, logic of beliefs, desires and intentions, game
theory, autonomy, adaptation, reactivity and proactivity, knowledge
representation (tasks, environment), bounded rationality, Sense-Plan-Act cycle,
agent architectures, uncertainty reasoning, communication and coordination,
multi-agent systems Leerdoelen



==> courses/architecture-driven-information-systems-engineering/description.tex <==
\Course{Architecture-driven Information Systems Engineering}
\Version{18-07-05}

\Synopsis
This course comprises three parts. It starts (part 1) by revisiting the
modeling of information systems, were we provide an overview of the courses on
\emph{Domain Modeling} and \emph{Work-Systems Modeling} from the perspective of
information systems modeling. We then continue by considering information
systems engineering from an abstract point of view (part 2). As such, it ties
the courses of the previous courses in the \DaVinci\ series together. This
abstract view translates to taking a system theoretical perspective on
information systems, their engineering and the role of architecture in
bounding/guiding the engineering processes.

We then move on to the architecture level (part 3), by discussing both the
definition of architecture in an information systems engineering context, its
need, as well as its potential role as a means of negotiation and
communication.  Special attention will be paid to the mechanism of
\emph{architecture principles} as a mechanism to guide/bound the engineering
processes.  We also consider the process of architecting information systems,
in particular communication strategies and negotiation between different
stakeholders. An information system involves organisational, human and
technological issues, leading to a plethora of stakes and stakeholders. These
stakes need to be balanced during the development of an information system's
architecture.

\Goals
After this course, students are able to:
\begin{enumerate}
   \item argue about the different aspects of information system engineering
   and position the methods \& techniques as presented in the other courses in
   the \DaVinci\ series relative to these aspects,
   \item reason about organisations, information systems, and computerised
   information systems at an abstract (system theoretical) level,
   \item argue the need, and potential role, for architecture in the context of
   information systems engineering,
   \item discuss and relate different definitions of architecture,
   \item reason about different levels of abstraction at which an information
   system, and its context, can be modelled/designed/architected, as well as
   identify situations for which these levels are relevant,
   \item reason about the selection of modelling techniques, for given goals and
   situations during information systems engineering, that are most apt to the
   situation at hand,
   \item develop, and reason about, communication and negotiation strategies 
   relevant to information systems engineering.
\end{enumerate}

\Topics
\begin{enumerate}
   \item Information systems modeling
   \item System theory
   \item Information systems engineering
   \item Architecture
   \item Viewpoints
   \item Architecture principles
   \item Stakeholders
   \item Communication \& negotiation
\end{enumerate}


==> courses/architecture-driven-information-systems-engineering/outline.tex <==
\Outline
\Version{28-07-05}

\Part{Introduction}
\begin{itemize}
   \item The digital era

   \item Enablers of the digital era

   \item The information systems area:

	 computerized information systems, information systems, organizational
	 systems, work-systems, systems
	 
   \item Information systems engineering

         Triangle: Define, Design, Construct, Deploy
   
         Approaches: Linear, evolutionary, etc.

   \item Challenges for information systems engineering in the digital era.

   \item Architecture-driven information system engineering
\end{itemize}

\Part{Model-driven Information Systems Engineering}
\begin{itemize}
   \item Enduring challenge for ISE: optimizing the desirability of an
   information-systems behavior as perceived by the stakeholders.

   \item ISE as a communicative, model-driven, knowledge transformation process.
   
   Really: a second order Information System!!
   
   Stakeholders and their stakes, information needs of stakeholders, goals of
   development team, best means to achieve this, communication strategies, etc.
   This raise the question: which languages to use to express different aspects
   (to whom, for what reason) of the information system being developed? 

   \item Methodological perspective.

   Method of working: ways-of framework

   Key concepts: viewing frameworks, viewpoints, methods, techniques

   See: WSML.

   \item Viewing frameworks:
         \begin{itemize}
            \item Dimensions for viewpoints
         
	    \item Example viewing frameworks for information systems: 4+1,
	    RM-ODP, E-Tom, ArchiMate, ...

	    \item Leading framework in this part: definition, design,
	    deployment.
         \end{itemize}
   
   \item Definition of information systems, and their engineering process.
    
         High-level recap of the course \emph{definition of information systems}.

         Fundamental discussion of qualities. Qualities not only of the product,
	 but also of the process.

   \item Design of information systems, and their engineering processes
         \begin{itemize} 
            \item High-level recap of design parts of \emph{(advanced) modeling
            and design of information systems}.

            \item Design of product and process

	    \item Vitruvius perspectives on design of IS. See Daan's inaugural
	    speech.

            \item Tradeoff between resource use and qualities of product (oratie Mario)

            \item Design rationale: From \emph{what} + \emph{why} to \emph{how}.
            
	          A research methodological perspective: 
                  \begin{itemize}
                     \item Requirements are assumptions
                     \item Design is hypothesis
		     \item How do you test/validate/verify: design follows from
		     assumptions, and assumptions are adequate.  
		  \end{itemize}

            \item Designing out: outsourcing engineering work as a choice of design
         \end{itemize}

   \item Deployment
\end{itemize}

\Part{Architecture-driven information system engineering}
%Todo: map contents of ADW lectures by Erik.
\begin{itemize}
   \item The desire for alignment between business and IT. But not only
   business and IT. Also people, organization, etc. Different aspects to
   be aligned. 
   
   We shall use the following primary viewing framework, consisting of the following aspects:
   \begin{itemize}
      \item Business
      \item Information
      \item Application
      \item Infrastructure
   \end{itemize}
   They all need to be aligned.

   In addition, we shall add the following two dimensions:
   \begin{itemize}
      \item Quality: Vetruvius as a classification over ISO's quality properties.
      \item Scope: enterprise, business domains, information systems, work place 
   \end{itemize}

   \item The need for architecture. The need to constrain design space, and to
   communicate-about/motivate/rationalize/negotiate these constraints.  

   Relative to the needs for a family of systems or multiple incarnations of
   systems.

   \item Communicating about architectures
   
   Information needs of stakeholders, goals of development team, best means to
   achieve this, communication strategies, etc. 

   \item Requirements on architecture as a means. Given the needs leading to
   the use of architecture. What are the requirements to be put on this
   ``means''
   
   \item Other (but our own) definitions of architecture: IEEE, IAF, ArchiMate,
   XAF, ...

   Prescriptive versus descriptive.

   Our definition: Restriction of design space.

   \item Architecting versus engineering.

   \item The content of an architecture. Two kinds of content
         \begin{itemize}
	    \item Prescriptive; This is really where architecture is about.
	    \item Descriptive, supporting the prescriptive content.
            principles, rules, guidelines, reference designs, design rationale, etc.
	 \end{itemize}
   
   \item Revisit viewing frameworks: IAF, ArchiMate, E-Tom, Togaf, Tapscott, etc, etc

         Distinguish between engineering framework and architecture framework.

         Revisit our framework of choice. 

   \item Architecture prescription language: principles, guidelines, etc.

   \item Overview of architecture description languages: UML, ArchiMate, ...
   
   The semantics of prescription language can be expressed in terms of their
   limitation of the design space of a descriptive language.

   \item Architecture description language: ArchiMate (and relationship to
   ArchiMate-ish language used in modeling of organizations).

   Discuss specific notation per layer:
   \begin{itemize}
      \item Business
      \item Information
      \item Application
      \item Infrastructure
   \end{itemize}

   \item Architectures of the physical world versus architecture for the digital world.

   \item The role of the Architect.

   \item Architecture styles: service orientation, portal-thinking, ...

   \item Designing in \& designing out (the role of outsourcing, or not).
\end{itemize}


==> courses/architecture-driven-information-systems-engineering/tail.tex <==
\Header{Work forms}
\begin{enumerate}
   \item Lectures
   \item Tutorials
\end{enumerate}

\Header{Pre-requisites}
\begin{enumerate}
   \item Domain Modeling
   \item Work-systems Modeling 
   \item Storage and Retrieval
   \item Beweren \& Bewijzen
   \item Requirements Engineering
\end{enumerate}

\Header{Examination}
\begin{enumerate}
   \item Final exam
\end{enumerate}

\Header{Combinations}
\begin{enumerate}
   \item Digital architecture 
\end{enumerate}

\Header{Literature}
\begin{enumerate}
   \item Lecture notes
\end{enumerate}
Will be made available electronically.


==> courses/architecture-driven-work-systems-engineering/description.tex <==
\Course{Architecture-driven Work Systems Engineering}
\Version{30-10-05}

\Synopsis
This course comprises three parts. It starts (part 1) by revisiting the
modeling of work systems, were we provide an overview of the courses on
\emph{Domain Modeling} and \emph{Work-Systems Modeling} from the perspective of
work systems modeling. We then continue by considering work
systems engineering from an abstract point of view (part 2). As such, it ties
the courses of the previous courses in the \DaVinci\ series together. This
abstract view translates to taking a system theoretical perspective on
work systems, their engineering and the role of architecture in
bounding/guiding the engineering processes.

We then move on to the architecture level (part 3), by discussing both the
definition of architecture in an work systems engineering context, its
need, as well as its potential role as a means of negotiation and
communication.  Special attention will be paid to the mechanism of
\emph{architecture principles} as a mechanism to guide/bound the engineering
processes.  We also consider the process of architecting work systems,
in particular communication strategies and negotiation between different
stakeholders. An work system involves organisational, human and
technological issues, leading to a plethora of stakes and stakeholders. These
stakes need to be balanced during the development of an work system's
architecture.

\Goals
After this course, students are able to:
\begin{enumerate}
   \item argue about the different aspects of work system engineering
   and position the methods \& techniques as presented in the other courses in
   the \DaVinci\ series relative to these aspects,
   \item reason about organisations, work systems, and computerised
   work systems at an abstract (system theoretical) level,
   \item argue the need, and potential role, for architecture in the context of
   work systems engineering,
   \item discuss and relate different definitions of architecture,
   \item reason about different levels of abstraction at which an work 
   system, and its context, can be modelled/designed/architected, as well as
   identify situations for which these levels are relevant,
   \item reason about the selection of modelling techniques, for given goals and
   situations during work systems engineering, that are most apt to the
   situation at hand,
   \item develop, and reason about, communication and negotiation strategies 
   relevant to work systems engineering.
\end{enumerate}

\Topics
\begin{enumerate}
   \item Information systems modeling
   \item System theory
   \item Information systems engineering
   \item Architecture
   \item Viewpoints
   \item Architecture principles
   \item Stakeholders
   \item Communication \& negotiation
\end{enumerate}


==> courses/architecture-driven-work-systems-engineering/outline.tex <==
\Outline
\Version{28-07-05}

\Part{Introduction}
\begin{itemize}
   \item The digital era

   \item Enablers of the digital era

   \item The work systems area:

	 computerized information systems, information systems, organizational
	 systems, work systems, systems
	 
   \item Work systems engineering

         Quadrant: Define, Design, Construct, Deploy
   
         Approaches: Linear, evolutionary, etc.

   \item Challenges for work systems engineering in the digital era.

   \item Architecture-driven work system engineering
\end{itemize}

\Part{Model-driven Work Systems Engineering}
\begin{itemize}
   \item Enduring challenge for ISE: optimizing the desirability of a
   work systems behavior as perceived by the stakeholders.

   \item ISE as a communicative, model-driven, knowledge transformation process.
   
   Really: a second order Information System!!
   
   Stakeholders and their stakes, work needs of stakeholders, goals of
   development team, best means to achieve this, communication strategies, etc.
   This raise the question: which languages to use to express different aspects
   (to whom, for what reason) of the work system being developed? 

   \item Methodological perspective.

   Method of working: ways-of framework

   Key concepts: viewing frameworks, viewpoints, methods, techniques

   See: WSML.

   \item Viewing frameworks:
         \begin{itemize}
            \item Dimensions for viewpoints
         
	    \item Example viewing frameworks for (parts of) work systems: 4+1,
	    RM-ODP, E-Tom, ArchiMate, ...

	    \item Leading framework in this part: definition, design,
	    deployment.
         \end{itemize}
   
   \item Definition of work systems, and their engineering process.
    
	 High-level recap of the course \emph{definition of work
	 systems}.

	 Fundamental discussion of qualities. Qualities not only of the
	 product, but also of the process.

   \item Design of work systems, and their engineering processes
         \begin{itemize} 
	    \item High-level recap of design parts of \emph{(advanced) modeling
	    and design of work systems}.

            \item Design of product and process

	    \item Vitruvius perspectives on design of IS. See Daan's inaugural
	    speech.

            \item Tradeoff between resource use and qualities of product (oratie Mario)

            \item Design rationale: From \emph{what} + \emph{why} to \emph{how}.
            
	          A research methodological perspective: 
                  \begin{itemize}
                     \item Requirements are assumptions
                     \item Design is hypothesis
		     \item How do you test/validate/verify: design follows from
		     assumptions, and assumptions are adequate.  
		  \end{itemize}

            \item Designing out: outsourcing engineering work as a choice of design
         \end{itemize}

   \item Deployment
\end{itemize}

\Part{Architecture-driven work system engineering}
%Todo: map contents of ADW lectures by Erik.
\begin{itemize}
   \item The desire for alignment between business and IT. But not only
   business and IT. Also people, organization, etc. Different aspects to
   be aligned. 
   
   We shall use the following primary viewing framework, consisting of the following aspects:
   \begin{itemize}
      \item Business
      \item Information
      \item Application
      \item Infrastructure
   \end{itemize}
   They all need to be aligned.

   In addition, we shall add the following two dimensions:
   \begin{itemize}
      \item Quality: Vetruvius as a classification over ISO's quality properties.
      \item Scope: enterprise, business domains, work systems, work place 
   \end{itemize}

   \item The need for architecture. The need to constrain design space, and to
   communicate-about/motivate/rationalize/negotiate these constraints.  

   Relative to the needs for a family of systems or multiple incarnations of
   systems.

   \item Communicating about architectures
   
   Information needs of stakeholders, goals of development team, best means to
   achieve this, communication strategies, etc. 

   \item Requirements on architecture as a means. Given the needs leading to
   the use of architecture. What are the requirements to be put on this
   ``means''
   
   \item Other (but our own) definitions of architecture: IEEE, IAF, ArchiMate,
   XAF, ...

   Prescriptive versus descriptive.

   Our definition: Restriction of design space.

   \item Architecting versus engineering.

   \item The content of an architecture. Two kinds of content
         \begin{itemize}
	    \item Prescriptive; This is really where architecture is about.
	    \item Descriptive, supporting the prescriptive content.
            principles, rules, guidelines, reference designs, design rationale, etc.
	 \end{itemize}
   
   \item Revisit viewing frameworks: IAF, ArchiMate, E-Tom, Togaf, Tapscott, etc, etc

         Distinguish between engineering framework and architecture framework.

         Revisit our framework of choice. 

   \item Architecture prescription language: principles, guidelines, etc.

   \item Overview of architecture description languages: UML, ArchiMate, ...
   
   The semantics of prescription language can be expressed in terms of their
   limitation of the design space of a descriptive language.

   \item Architecture description language: ArchiMate (and relationship to
   ArchiMate-ish language used in modeling of organizations).

   Discuss specific notation per layer:
   \begin{itemize}
      \item Business
      \item Information
      \item Application
      \item Infrastructure
   \end{itemize}

   \item Architectures of the physical world versus architecture for the digital world.

   \item The role of the Architect.

   \item Architecture styles: service orientation, portal-thinking, ...

   \item Designing in \& designing out (the role of outsourcing, or not).
\end{itemize}


==> courses/architecture-driven-work-systems-engineering/tail.tex <==
\Header{Work forms}
\begin{enumerate}
   \item Lectures
   \item Tutorials
\end{enumerate}

\Header{Pre-requisites}
\begin{enumerate}
   \item Domain Modeling
   \item Work-systems Modeling 
   \item Storage and Retrieval
   \item Beweren \& Bewijzen
   \item Requirements Engineering
\end{enumerate}

\Header{Examination}
\begin{enumerate}
   \item Final exam
\end{enumerate}

\Header{Combinations}
\begin{enumerate}
   \item Digital architecture 
\end{enumerate}

\Header{Literature}
\begin{enumerate}
   \item Lecture notes
\end{enumerate}
Will be made available electronically.


==> courses/deployment-of-information-systems/description.tex <==
\Course{Deployment of Information Systems}

\Synopsis
This course focusses both on the deployment of a fully designed/constructed
information system in its usage context, as well as the processes and measures
needed to keep such a system in an operational state. The latter considerations
will also lead to additional insight into the design of information systems.
Maintenance of such systems should be designed ``in''.

In this course, attention will be paid to some public standards (ISPL,
ITIL, ASL) which are relevant to the deployment and ensuing maintenance
information systems. Specific attention will also be paid to so-called
service-level agreements (SLA's) with regards to the operational maintenance 
of systems, the risks that may threaten these service levels, and strategies
to manage these risks.

\Goals
After this course, students are able to:
\begin{enumerate}
  \item reason about the role of deployment in information systems engineering.
  \item identify, and discuss, the major elements in some relevant public
  standards for deployment and maintenance,
  \item apply the theories underlying these public standards to some practical
  cases,
  \item design and discuss organisational structures/processes for deployment,
  \item reason about service level agreements and their impact on both the
  using environment and the maintenance processes,
  \item assess potential risks to these service level agreements.
\end{enumerate}

\Topics
\begin{enumerate}
  \item Relevant public standards:
        \begin{description}
	  \item[ISPL --] Information Services Procurement Library.
	  \item[ITIL --] Information Technology Infrastructure Library.
	  \item[ASL --] Application Services Library.
	\end{description}
  \item Deployment
  \item Maintenance
  \item Service Level Agreements (SLA),
  \item Risk management
\end{enumerate}


==> courses/digital-architecture/description.tex <==
\Course{Digital Architecture}

\Synopsis
De kwaliteit van de informatievoorziening is voor moderne organisaties een
succesfactor van belang. In veel gevallen is die voorziening het resultaat van
ongeleide 'organische' groei. Vaak is dan tegelijk met de toename van het
aantal technische en informatorische voorzieningen het geheel uitgegroeid tot
een onontwarbare kluwen digitale onderdelen. 

De kosten zijn toegenomen en de inflexibiliteit eveneens terwijl het
reactievermogen van de organisatie juist groter moet worden en daardoor extra
eisen stelt aan de souplesse van de informatievoorziening. 

In dit vak wordt deze situatie nader geanalyseerd en ontleed, en worden
concepten ontwikkeld om de structurele veroudering en verstarring tegen te
gaan. Derhalve wordt veel aandacht besteed aan 'functies en constructies' van
de informatievoorziening en aan beheersing van de complexiteit. 

Architectuur en informatie-infrastructuur zijn daarbij belangrijke begrippen,
evenals architectuurprincipes. 

Note: Maybe we should also pay attention to outsourcing. Both IT services
(ISPL!) as well as entire business processes (BPO). By aligning the
\emph{Information Systems Architecture} course and the \emph{Enterprise
Information Architecture} course, there may be more room in the latter
course for oursourcing.

\Goals
\begin{enumerate}
   \item het concept architectuur en enkele van de definities die hieraan
   gegeven worden, met nadruk op de rol van architectuur als communicatie- en
   onderhandelingsmiddel. 
   \item de rol van digitale architectuur in ondernemingen en organisaties mbt
   het bereiken van een betere afstemming tussen de bedrijfsvoering en de ICT
   (business-ICT alignment). 
   \item adaptiviteitscriteria die organisaties in staat stellen om beter in te
   spelen op de immer veranderende, nauwelijks voorspelbare omgeving. 
   \item belangrijke raamwerken en patronen met betrekking tot architectuur,
   zoals service oriëntatie, etc. 
   \item in te schatten welke impact architectuurkeuzes hebben. 
   \item relevante wetenschappelijke/professionele literatuur op het gebied van
   architectuur te duiden en de relevantie ervan te bepalen voor een gegeven
   probleemsituatie. 
   \item de noodzaak te duiden van een goede afstemming tussen bedrijfsvoering
   en ICT. 
   \item te beredeneren welke adaptiviteitscriteria relevant zouden kunnen
   zijn. 
   \item een eerste inschatting te maken welke raamwerken en patronen met
   betrekking tot architectuur relevant zijn. 
\end{enumerate}

\Topics
\begin{enumerate}
   \item Digitale Wereld 
   \item Informatiearchitectuur 
   \item Architectuurprincipes 
\end{enumerate}


==> courses/domain-modeling/description.tex <==
\Course{Domain Modeling}
\Version{12-09-05}

\Synopsis
This course covers an important prerequisite in the information system
life-cycle where the intention is to obtain an (agreed) understanding of a given domain. In this course, students will be taught to demarcate a domain and identify its ontology, i.e. a specification of its conceptualization comprising the core concepts in the domain, their mutual relations and the laws (constraints) governing their behavior.
Students will get a deep understanding of conceptual modeling, and will be able to transform a model into a computational environment in general, and a relational database structure and SQL in particular. This will be related to the Unified Modeling Language UML.

\Goals
After this course the student
\begin{enumerate}
\item understands what a model is.
\item understands the ORM normalform for natural language sentences, and can transform a sentence into this normalform.
\item can systematically derive a conceptual model from a structured domain description.
\item understands how the conceptual language Lisa-D is derived, and can express conceptual operations in terms of this language.
\item has a base understanding of formal reasoning in Lisa-D.
\item can transform a conceptual model and its conceptual operations into a relational database structure and SQL.
\item understands how the action-oriented approach generalizes the fact-oriented approach.
\item has a basic understanding of UML, and knows how to apply conceptual modeling during UML.
\end{enumerate}

\Topics
The course is organized in 3 blocks:
\begin{enumerate}
\item Modeling
\begin{itemize}
\item Domain modeling is introduced as an activity that tries to describe how people communicate in some universe of discourse. The students learn how a controlled language approach helps to make an initial structuring.
\item Sentences from the controlled language are analyzed for concepts, leading to an overall description of concepts and their relations. This is called the conceptual schema, also referred to as a domain ontology.
\item The conceptual schema is seen as an information grammar. It is discussed how this grammar is the base for a conceptual domain language: Lisa-D.
\item Students learn how to formulate domain properties and conceptual information system operations in terms of Lisa-D. It is also discussed how Lisa-D can be used to formally prove properties of the underlying application domain.
\item As an information system creates a shadow world of the universe of discourse, special attention is paid to the required relation between the formal and informal world.
\end{itemize}
\item Transforming
\begin{itemize}
\item In this block the students will learn the principles of SQL as a general foundation to build information systems.
\item The students will learn syntax and get a clear impression of the semantics.
\item Students learn how the conceptual schema can be transformed into a relational model in SQL. They also learn how, in terms of this transformation,  the conceptual information system operations (Lisa-D) can be transformed into SQL-statements.
\item They will be trained in constructing SQL queries in non-trivial cases. The technique of working with refinements is a basic tool, that also gives a clue to reason about the correctness of a query.
\item The students get concrete hands on experience from an concrete SQL system.
\end{itemize}
\item Behavior
\begin{itemize}
\item In this block we first discuss the Unified Modeling Language UML, and show how conceptual modeling explains submodels of UML formally and also gives a concrete assist for the construction of these submodels.
\item In conceptual modeling, we have used a fact-oriented approach. In this block we will discuss how this can be generalized into an action-oriented approach.
\item Especially we will discuss the nature and construction of the Object-Life model.
\end{itemize}
\end{enumerate}

%\Outline


==> courses/domain-modeling/outline.tex <==
\Skip{
\Outline
\Version{17-07-05}

\Part{Domain modeling}
\begin{itemize}
   \item What is modeling?

   \item What is a domain?

     Main focus: (sub-)domains of the class ``work system'', such as
     organizations and information systems.

   \item Communication during modeling

   \item The process of modeling

   \item Modeling the communication (both syntax and semantics)

   \item The logbook approach 
 
     Basic paradigm: The logbook keeps a history of the domain. It is also
     the basis for a ``domain-modeling information-system'' which is able
     to answer queries about the domain. This makes the logbook behave like
     an information system for this domain.

   \item Type-instance distinction

     Why do we need the type level? Needed to discuss/express general
     properties and behavior. Makes it possible to implement generic
     routines when mapping to software. 

   \item Grammars
\end{itemize}

\Part{Basic modeling technique}
\begin{itemize}
   \item Data, information and reality
   \item Object-Role Modeling Normal Form (ORMNF)
   \item Transforming ORMNF into a schema fragment
   \item The formal model
\end{itemize}

\Part{Talking about models}
\begin{itemize}
   \item \emph{O}bject \emph{R}ole \emph{Ca}lculus (ORCa) = Fact Calculus + Lisa-D + Time + FORML

   \item ORCa as a constraint language $\Rightarrow$ Business rules!
\end{itemize}

\Part{Modeling large domains}
\begin{itemize}
   \item Schema decomposition
\end{itemize}

\Part{Advanced modeling concepts}
\begin{itemize}
   \item Objectification
   \item Basic (graphical) constraints: uniqueness, total role and extensional uniqueness

     Plus semantics in terms of ORCa or relational algebra (shouldn't we
     merge path expressions and relational algebra into one formalism?)

   \item Set types, multi-set types, sequence types, schema types.

   \item Advanced constraints

     Plus semantics in terms of ORCa or relational algebra (shouldn't we
     merge path expressions and relational algebra into one formalism?)

   \item Specialization and generalization
\end{itemize}

\Part{Semantics of a model and its evolution}
\begin{itemize}
   \item Identification of instances: weak and strong
\end{itemize}

\Part{Modeling of behavior}
\begin{itemize}
   \item Time axes
   \item Temporal dimension in ORCa
   \item Temporal/triggering constraints (graphical and ORCa)
\end{itemize}

\Part{Schema transformations}
\begin{itemize}
   \item Transformations between ORM models.
   \item Mapping to other languages: UML and SQL.
\end{itemize}
} 

==> courses/foundations-of-information-retrieval/description.tex <==
\Course{Foundations of Information Retrieval}

\Synopsis
IR (Een constructieve visie op Information Retrieval) behandelt de
achtergronden van Information Retrieval: (1) hoe zoeken mensen informatie, hoe
formaliseren we dat, (2) hoe beschrijven mensen wat ze bedoelen, hoe
formaliseren we 'betekenis', en (3) hoe brengen we (1) en (2) met elkaar in
verband? Een belangrijk toepassingsgebied is het Internet.

\Goals
De bedoeling van IR (Een constructieve visie op Information Retrieval) is dat
deelnemers na afloop:
\begin{enumerate}
   \item Bekend zijn met de basismodellen voor Information Retrieval.
   \item Kennis hebben van query talen, zowel syntactisch als semantisch.
   \item Elementaire kennis hebben van het indexeren van teksten
   \item Inzicht en vaardigheid in ontwerp en bouw van zoekmachines
   \item Bekend zijn met document-representatie methoden, hun achterliggende
   motivatie en begrenzingen. 
   \item Kennis hebben automatische documentclassicatie: de probleemstelling en
   algoritmen. 
   \item bekend zijn met de basisbegrippen en -technieken van datamining. 
   \item Vaardigheid bij het toepassen van tools op zoek naar begrijpelijke
   patronen en kennis. 
   \item Kennis van visualisatietechnieken voor kennisstructuren. 
   \item Vaardigheid in het toepassen hiervan bij de ontsluiting van een
   kennisbron. 
\end{enumerate}

\Topics
Na een algemene formulering van de probleemstelling worden de bekende retrieval
modellen besproken (zoals vector space model en boolean retrieval) en gekoppeld
aan een computationele (i.h.b. computationele) visie. Voor de evaluatie van een
retrieval systeem worden een aantal maten ingevoerd. 

Hierna worden query talen besproken, en manieren om de gebruiker te helpen bij
de formulering van de query door verrijkings- en feedback methoden. 

Kennisextractie uit teksten wordt inleidend besproken. Hierna wordt een keuze
gemaakt uit de volgende onderwerpen: multimedia IR, zoekmachines en digital
libraries.


==> courses/foundations-of-information-retrieval/outline.tex <==
\Outline
Het opslaan van grote hoeveelheden zwak gestructureerde informatie stelt extra
eisen aan de methoden om hieruit gericht informatie op te vragen. Voorbeelden
zijn bibliotheken en het internet. Op het internet wordt veel gebruik gemaakt
van zoekmachines. Deze machines proberen zoveel informatie te vergaren over wat
op het internet aangeboden wordt, en stellen gebruikers in staat hierover
vragen te stellen. Naast deze elementaire retrieval functie kunnen complexere
retrieval taken beschouwd worden. Bijvoorbeeld, het filteren van berichten die
via een nieuwsgroep verspreid worden. Of het bouwen van een systeem waarin
complexe vragen gesteld worden (question-answering systemen), zoals: wat is het
totaal aan studiepunten van vakken die over gegevensmodellering gaan? 

Omdat de toegankelijkheid van de informatie groot moet zijn, dient de vraagtaal
van een zoekmachine erg krachtig en eenvoudig bruikbaar te zijn. Die laatste
eis maakt het probleem extra lastig. Een mooi gemaakt retrieval systeem scoort
slecht wanneer het (brede) publiek er onvoldoende mee uit de voeten kan. De
interactie tussen de gebruiker van zo'n systeem vindt op 2 momenten plaats:
tijdens de probleemformulering en tijdens de presentatie van de gevonden
documenten. Daartussen is het systeem bezig de geformuleerde vraag te koppelen
aan documenten. Hoe beter de zoekmachine een beeld kan vormen over de inhoud
van documenten, hoe beter deze matching zal zijn. 


==> courses/foundations-of-information-systems/description.tex <==
\Course{Foundations of Information Systems}

\Synopsis
In this course, the fundamental techniques from previous parts of this series
are the topic of an in-depth study. This leads to a reflection of the
essentials of such techniques, and enables the student to reason about such
models, their properties and their qualities, and to make comparisons between
models.

The nature of this course is research-oriented, the students are challenged to
do research to advance the state-of-the-arts of both the craftsmanship and the
art of modelling.

Dit vak behandelt informatiemodellering, een essentieel onderdeel van
systeemanalyse. Er wordt ook gewerkt aan de modellering van websites. Centraal
staat de vraag hoe we op een nette manier de semantiek van informatie- modellen
kunnen vastleggen.

Deze cursus behandelt informatiemodellering, een essentieel onderdeel van
systeemanalyse ("Requirements Analysis"). Er wordt een modelleringstechniek
besproken, die voldoet aan de volgende eisen. De techniek heeft een formele
onderbouwing, is op een conceptueel nivo, heeft een ruime expressieve kracht,
is executeerbaar, leidt tot begrijpelijke en communiceerbare modellen, en is
geschikt voor het modelleren van gegevensintensieve domeinen. 
Communiceerbaarheid is een belangrijke eis, omdat conceptuele modellen een
cruciale rol spelen in de communicatie met domeinexperts. De
modelleringstechniek bevat naast de gebruikelijke gegevensmodellering ook
aspecten van Object Oriëntatie, bijvoorbeeld Object Life Cycle modellen. Er
wordt ook gewerkt aan de modellering van websites, waarbij elke student een
eigen website modelleert volgens de principes van datamodellering. Wat je gaat
leren: (1) Het belang van formele methoden kunnen beargumenteren. (2) De syntax
en semantiek van gegevensschema's zodanig begrijpen dat je complexe domeinen
kunt modelleren. 

\Goals
\begin{enumerate}
   \item De syntax en semantiek van informatiestructuren kennen. 
   \item De syntax en semantiek van veel voorkomende constrainttypen.
   Bovendien: tegenspraken in constraints bewijzen. 
   \item De formele definitie van identificeerbaarheid kennen en toepassen in
   concrete situaties en daarvan de theoretische consequenties overzien. 
   \item Het formuleren van theoretische uitspraken voor wat betreft
   complexiteit van verificatie en expressieve kracht van gegevensmodellen. 
   \item De syntax en semantiek van padexpressies kunnen begrijpen en toepassen 
\end{enumerate}

\Topics
\begin{enumerate}
   \item Foundations of information modelling techniques. Data models and
   process models. 
   \item Comparison of fact-oriented modelling and object-oriented modelling. 
   \item Abstraction mechanisms. 
   \item Semantics of complex integrity constraints. Static constraints versus
   dynamic constraints. 
   \item Meta data models of data models and process models. 
   \item Meta process models of data models and process models. 
   \item Artificial identification and real identification. 
   \item Validation of information models. 
   \item Verification and enforcement. 
   \item Path expressions through information structures. 
   \item Transformation of data models. Structure transformations. Guided
   transformations. Preprocessing and postprocessing. 
   \item Complexity analysis. 
   \item Transformation of database contents and integrity constraints. 
   \item Transformation of database operations (retrieval and updates). Proof
   schema for structural induction. 
   \item Correctness and completeness of transformations. 
   \item Repairment and penalization for incorrect transformations. 
   \item Equivalence of data models. 
   \item Distance between data models. Comparison of distance measures. 
   \item Modelling of web sites and semistructured data. 
   \item Object graphs, object coordination graphs, path definition and
   evaluation. 
   \item Representation language for data views. 
   \item Encoding of data views. Augmentations of basic encoding. 
   \item Database design and optimization. Hill climbing. Evolutionary
   algormithms. Genetic algorithms. 
   \item Solution spaces. Size, structure, and compactness of solution spaces. 
   \item Properties of solutaion space (e.g. local and global optima) versus
   properties of transformation algorithms (e.g. living and dead database
   structures). 
   \item Markov Chain analysis. 
   \item Relationship with ER, NIAM, UML, XML, OO, RDBMS, ORDBMS, SQL
\end{enumerate}


==> courses/information-retrieval/description.tex <==
\Course{Information Retrieval}
\Version{12-09-05}

\Synopsis
IR (A constructive approach to Information Retrieval) treats the backgrounds of Information Retrieval:
\begin{enumerate}
\item How do people search for information, and how can this be formalized?
\item How do people describe what they mean, and how can we formalize meaning?
\item How can these points be combined? 
\end{enumerate}
An important application area is the Internet.

\Goals
The goals of the course IR (A constructive approach to Information Retrieval) is that its participants
\begin{enumerate}
\item are familiar with the base models that are used for Information Retrieval.
\item have knowledge of query languages, both syntactically and semantically.
\item are familiar with information extraction from documents, inter-document relations and their appreciation.
\item have insight and proficiency in design and construction of search engines.
\item interaction techniques to support searchers in their quest for information.
\item have some experience with scientific literature in this field. 
\end{enumerate}

\Topics
The course consists of three main parts:
\begin{enumerate}
\item Fundamentals
  \begin{itemize}
  \item After a discussion on the problem areas of Information Retrieval,
  \item the evaluation methods for Information Retrieval are discussed.
  \item The Boolean model is discussed, together with techniques related with inverted list document representation.
  \item The vector model is the most used model. As a method for knowledge extraction, the singular value decomposition (main component analysis) is discussed.
  \item The probabilistic model applies Bayesian learning techniques to Information Retrieval.
  \item Some essentials to present the query results conclude the fundamental part. 
      The models are discussed both from a cognitive and a computational point of view.
  \end{itemize}
\item Information processing
  \begin{itemize}
  \item Query languages in relation with cognitive aspects of information searching.
  \item Autonomous query improvement techniques (global context analysis). Guided query improvement techniques (feedback).
  \item Pseudo relevance feedback (local context analysis).
  \item Clustering techniques for knowledge extraction 
  \end{itemize}
\item Document relations on the Web
  \begin{itemize}
  \item Web retrieval.
  \item Exploring the reference structure between documents (for example, page rank).
  \item Exploring document appreciations (collaborative techniques).
  \item Special topics contributed by the participants 
  \end{itemize}
\end{enumerate}

\Outline
Finding relevant documents no longer seems to be the major challenge of state-of-the-art search engines. Were recall and precision major concerns in the early days of their existence, trying to convey information rather than just data seems to be a major concern nowadays. Offering a long list of documents in order of their relevancy score is known to be a too simple interface.

In order to improve on this, solid knowledge of the information retrieval problem and its main techniques is imperative.

As there are still many questions about the essentials, a strong relation with ongoing research activities is indispensable.


\Skip{
Werkvormen

   1. The course is divided in three parts, each part is concluded with a test.
   2. Each week there are 4 contact hours, in which the new material is presented and exercised.
   3. The participants have to make a contribution to the course. Participants can choose between:
          * literature study
          * implementation
          * validation 

Vereiste voorkennis

Participant of IR (A constructive approach to Information Retrieval) should have the base qualifications as provided by the bachelor Informatica or Informatiekunde.
Tentaminering

The exam for IR consists of 3 exercises, corresponding with the three parts of the course. If a test has led to a result which is not smaller than 6, then the participant may choose to skip the corresponding exercise of the exam. In this case the mark for the test is the mark for that exercise. Would the participant choose to make the exam exercise, then the mark for the test is cancelled. This leads to a mark (e) for the exam. The students also get a mark (c) for their contribution to the course. During the course some homework exercises will be handed out. These lead to a bonus score (b). For each exercise a bonus of 1 point may be obtained. The bonus score is the average bonus for the exercises.

The result for the course IR is obtained by rounding:

    * 2*e/3 + c/3 

If this result is not smaller than 6, then the bonus is added (and maximized to 10).

Combinatiemogelijkheden

This course is a part of the Da Vinci series of courses.
Literatuur

Lecture notes will be made available via Blackboard.

The following books are advised:

    * Ricardo Baeza-Yates, Berthier Ribeiro-Neto, Modern Information Retrieval, Addison Wessley, ISBN 0 201 398 29X
    * Pierre Baldi, Paolo Frasconi, Padhraic Smyth, Modeling the Internet and the Web: Probabilistic Methods and Algorithms 
}% Skip 

==> courses/knowledge-based-information-systems/description.tex <==
\Course{Knowledge-based Information Systems}

\Synopsis
Dit vak heeft tot doel de cursist kennis te laten maken met de belangrijkste
onderwerpen uit de Kunstmatige Intelligentie: kennisrepresentatie, redeneren en
leren. Daarnaast wordt aandacht besteed aan de geschiedenis van kennissystemen,
de ontwikkeling van kennissystemen en de formele basis ervan. Het omgaan met
onzekerheid in kennissystemen is ook een onderwerp dat in een zekere mate van
detail bestudeerd zal worden. Tenslotte zullen cursisten enkele talen en tools
die gebruikt worden in de Kunstmatige Intelligentie leren kennen, en ook zelf
een kennissysteem hiermee ontwikkelen.
In dit vak zullen onderwerpen uit de computationele intelligentie, zoals
representaties bij automatisch leren (beslisbomen, classificatieregels, neurale
netwerken) aan de orde komen, naast onderwerpen uit de information retrieval
met betrekking tot kennisextractie uit concrete bronnen (text mining,
concepttralies, extentionele semantiek).

Daarnaast zal aandacht besteed worden aan probleemklasse-specifieke
redeneervormen, zoals case-based retrieval and reasoning, model-gebaseerd
redeneren, spatieel redeneren, en redeneren met ontwerpspecificaties.

Dit vak biedt een inleiding op de kunstmatige intelligentie,
in het bijzonder de onderwerpen probleemoplossers, kennisrepresentatie,
automatisch redeneren, kennisacquisitie en knowledge engineering.


\Goals
\begin{enumerate}
   \item Kennismaken met de belangrijkste onderwerpen in de kunstmatige
   intelligentie (AI), zoals probleemoplossen, toestandsruimte, heuristisch
   zoeken, kennisrepresentatie en automatisch redeneren, machinaal leren,
   intelligent agent, kennisacquisitie, knowledge engineering. 
   \item Inzicht opdoen in de toepassing van algoritmische, logische en
   wiskundige methoden in de kunstmatige intelligentie. 
   \item Ervaring opdoen met de ontwikkeling van een kennissysteem voor een
   concreet domein. 
   \item Ervaring opdoen in de ontwikkeling van AI-programma's. 
\end{enumerate}

\Topics
\begin{enumerate}
   \item Wat is kunstmatige intelligentie?
   \item Geschiedenis: GPS, MYCIN, DENDRAL, ATP.
   \item Probleemoplossen en zoeken in toestandsruimten:
   uitputtend zoeken, backtracking, heuristisch zoeken op basis van A*,
   hill climbing, tabu search, simulated annealing.
   \item Kennisrepresentatie en automatisch redeneren: produktieregels en
   redeneren, logica en resolutie, Herbrand universum en basis, object
   representatie in de AI, redeneren met onzekere kennis, produktieregels en
   onzekerheid, Bayesiaanse netwerken.
   \item Knowledge engineering: methodology van de ontwikkeling van
   kennissystemen, machinaal leren.
   \item AI programmeren in een daarvoor geschikte taal.
\end{enumerate}



==> courses/requirements-engineering/description.tex <==
\Course{Requirements Engineering}
\Version{18-07-05}

\Synopsis
Een inleiding in de kunst en wetenschap van "Requirements Engineering" (RE):
het boven water krijgen en uitspecificeren van wat opdrachtgevers en
gebruikers eisen en verwachten van een toekomstig softwaresysteem.

We bestuderen en oefenen de Use Case aanpak voor "Requirements Gathering", en
integreren in deze aanpak enige reeds bekende technieken (domeinmodellering,
logische specificatie van regels). Tevens is er aandacht voor enige
wetenschappelijke artikelen over RE.

Een belangrijk deelproces van systeemontwikkeling is het goed helder
krijgen van de behoeften. Dit is het ``requirements engineering'' proces.
Het belangrijkste doel van dit proces is er voor te zorgen dat een eventueel
te ontwikkelen systeem ook het goede systeem is. Centraal in dit proces
staat de vergaring, specificatie, validatie en de bewaking van de
systeemeisen.

\Goals
\begin{enumerate}
   \item De student is in staat requirements specificaties te onderscheiden van functionele onwerpspecificaties
   \item De student is in staat requirements specificaties beoordelen op hun kwaliteit
   \item De student is in staat zelf heldere en zorgvuldig verzamelde en gespecificeerde requirements op te leveren
	 gegeven voldoende goede en toegankelijke informatiebronnen (stakeholders, documenten)
   \item De student is in staat uit te leggen wat de plaats is van requirements documenten binnen verdere documentatie 
	 in organisaties en systeemontwikkelprojecten
   \item De student is in staat uit te leggen hoe processen voor requirements engineering te plaatsen zijn binnen
	 systeemontwikkelingsprocessen in het algemeen
   \item De student is in staat bepaalde technieken uit de domeinmodellering en bedrijfsprocesmodellering integreren in een RE traject
   \item De student is in staat vanuit systeemontwikkelingstheorie te reflecteren op het vakgebied requirements engineering en op het 
	 RE proces

\end{enumerate}

\Topics
\begin{enumerate}
   \item Wat zijn requirements? (functional en non-functional)
   \item Verzamelen van requirements
   \item Specificeren (nauwkeurig opschrijven) van requirements
   \item Fasering en planning in RE
   \item Use Cases
   \item Business rules
   \item Domeinmodelleren
   \item Terminologische definities
   \item Stakeholder Analysis
   \item Requirements engineering in systeemontwikkelingstheorie
   \item Requirements en Taal
   \item Praktijk van RE 
\end{enumerate}


==> courses/requirements-engineering/outline.tex <==
\Outline
\Version{18-07-05}

Currently based on the book: Uses-Cases -- Requirements in Context, by Kulam
and Guiney. The list below consist of issues treated in this latter book and
new issues. The new issues are marked with a (*). Note: we should probably look
at RE's discussion in Rational Unified Process and Volere. Also IEEE has
several thick documents on RE.

\Part{Requirements on work-systems}
\begin{itemize}
   \item Work-systems as a generalization of organizations and (computerized)
   informaiton systems.
   \item Defining work-systems as the formulation of requirements and their motivation.
   \item Why defining work-systems? Why requirements?
   \item Quality (*): Property + value-domain + value + evaluation
   method/approach/technique.
   \item Assessing quality: How to (SMART!) evaluate an artefact's value?
   \item Designing with quality: quality-driven design.
   \item Quality of work-systems (target-domain) (*): Functional/Non-functional
   and other classes. Black-box/white-box view on system.
   Run-time/development-time behavior of system
   \item Quality of work-system engineering processes (project-domain) (*)
   \item Requirements on work-systems and their engineering processes: desired
   qualities + motivation (= design rationale, from \emph{why} to \emph{what})
   + priority.
   \item Stakeholders: They pose the requirements
   \item Stakeholder requirements versus system requirements.
\end{itemize}

\Part{Requirements engineering}
\begin{itemize}
   \item Gathering
   \item Definition
   \item Specification
\end{itemize}
Is the above terminology in-line with Volere and/or Rational's Unified Process? 
Hans Burg's thesis also contains a discussion in the break down of the 

\Part{Challenges of requirements}
\begin{itemize}
   \item Finding out who the stakeholders are (*)
   \item Finding out what they want 
   \item Documenting their needs
   \item Avoiding premature design decisions
   \item Resolving conflicting requirements
   \item Eliminating redundancy
   \item Reducing volume of requirements
   \item Ensuring traceability
\end{itemize}
Where in all this is: 
\begin{itemize}
   \item Negotiation, understanding and commitment (*)
   \item Stakeholder requirements versus system requirements (*)
\end{itemize}

\Part{Interaction-cases}
\begin{itemize}
   \item Use-cases \'a la UML
   \item Interaction-cases: interaction cases between different work-systems,
   e.g.\ super-work-system versus sub-work-system. But also: new application
   and pre-existing (legacy!) application. Interaction-cases are not just
   usage-by-users cases (**)
   \item Modeling interaction-cases 
   \item Grounding interaction-cases: the relation to the domain model (*)
   \item Paths and Scenarios
   \item Interaction-cases and requirements
   \item Interaction-case driven approach to requirements engineering
\end{itemize}

\Part{Requirements on the engineering process}
\begin{itemize}
   \item Any theories here? 
   \item To some extend these requirements are the domain of the project
   manager. However, they do influence the depth/breadth of the requirements
   engineering activities and the ensuing development process. As such,
   defining the requirements on the engineering process should have premise to
   defining the requirements of the intended product. (***)
\end{itemize}

\Part{Requirements engineering processes}
Three iterations:
\begin{itemize}
   \item Facade iteration
   \item Filled iteration
   \item Focused iteration
\end{itemize}
Again, where in all this is: 
\begin{itemize}
   \item Negotiation, understanding and commitment (*)
   \item Stakeholder requirements versus system requirements (*)
\end{itemize}



==> courses/storage-and-retrieval/description.tex <==
\Course{Storage and Retrieval}
\Version{01-12-2005}

\Synopsis
For the design of a computerized information system, it is important to
consider the mapping of the conceptual structure, its processes and
its data, onto the underlying storage devices.
The course Domain Modeling has shown how a conceptual model is derived from the domain description (using controlled language).
From this model, a conceptual language is derived, as a base language to reason about the underlying domain.
Furthermore, it is shown how the conceptual model and language are transformed onto SQL.

In this course we start with the discussion of the most important hardware characteristics, and show how to build on the storage devices efficient and reliable file management systems.

Relational algebra is introduced as an intermediate between SQL and file management systems. The translation of SQL into relational algebra is discussed, and it is shown how relational algebra is used as a mechanism for query optimization.

We then proceed with the mapping of the relational table structure and its elementary operators onto the file management system. We discuss the important file structuring mechanisms like ISAM, B$^+$ tree and hashing.

We then discuss more advanced mechanism to retrieve information, that are based on the user point of view. We also relate this to structured files, especially in the context of XML.

Finally we focus on some special issues as transaction management.

\Goals
After this course the student
\begin{enumerate}
\item can describe the various storage techniques and can describe their performance for elementary access patterns.
\item has knowledge of the execution of SQL queries in terms of relational algebra and has an elementary understanding of query optimization.
\item has knowledge of the elementary principles of information retrieval.
\item has knowledge of structured documents and is aware of their representation in terms of XML.
\end{enumerate}

\Topics
The course is organized in 3 blocks:
\begin{enumerate}
\item Elementary organization storage media
  \begin{itemize}
  \item Properties and characteristics of storage media. In detail are discussed:
        hard disc, optical disc and tape storage media.
  \item Classic file management systems. The general allocation principles are discussed, and
        related to the FAT file system and the UNIX file system. Typical problems like
        defragmentation are treated.
  \item Memory management. The importance of memory management techniques are explained, the most
        important replacement techniques are acquired.
  \item The design of fault tolerant systems. Concepts like MTBF are introduced and related
        to probability theory. As an example the RAID technology is discussed in depth.
  \item Advanced file management systems. The requirements of modern file management are discussed
        and exemplified with the Windows file system NTFS.
  \end{itemize}
\item File organization techniques. 
  \begin{itemize}
  \item Relational Algebra.
        The relational data model is introduced in depth, and the relational algebra
        as the basic operators to manipulate relational tables.
        The translation of SQL into relational algebra is given, and the base techniques of
        query optimization are discussed, leading to the pushdown normalform.
  \item Records.
        Elementary data storage techniques are discussed, and the various strategies to organize
        data into records.
  \item List structure: the various variants of list structures and their representation in
        file structures.
  \item The ISAM file organization method.
  \item The B$^+$ tree. This is introduced as a recursive extension of ISAM.
  \item Hashing. Another way to efficiently organize data is the hashing technique. 
        The main attention is on the application of hashing in a dynamic environment, such that
        growth and shrinkage of the data set are smoothly handled.
  \end{itemize}
\item Retrieval and structured documents: the storage and retrieval of semi-structured data, and
  relation with Information Retrieval to search large volumes of data.
  \begin{itemize}
  \item Information Retrieval. The how and why of retrieval is discussed from the point of view
        of the searcher.
  \item XML. Modern techniques to organize storage and retrieval of semi-structured data.
        Typical subjects are: the object model, path expressions, retrieval algebra.
  \item Concurrency en Security. 
  \end{itemize}
\end{enumerate}
%\Skip{
%\begin{enumerate}
%   \item Storage devices and their parameters
%   \item Design issues (reliability, availability, mtbf, etc.)
%   \item Data organization as a file system (unix, fat, ntfs, winfs, longhorn)
%   \item Internal file organization techniques (record file, isam, hashing,
%   b-tree, text file, xml, efficiency)
%   \item Relational algebra as a calculation schema and base for query
%   optimization (transformation sql to relational algebra)
%   \item Why do we store information: essentials of information retrieval (search engine, sql)
%   \item elementaire gegevensopslag met behulp van fundamentele
%   opslagtechnieken (B-bomen, hashing), 
%   \item meerdere toegangen: het indexed-sequential bestand, 
%   \item de tabel en de relatie, de hierop gebaseerde relationele algebra en de
%   relatie met SQL databases, 
%   \item de geneste tabel en de relatie met Object-Oriented databases, 
%   \item XML gebaseerde opslag en de relatie met het Internet, 
%   \item opslag van ongestructureerde informatie en de relatie met Information
%   Retrieval en methoden om exploratief te zoeken in grote hoeveelheden
%   informatie, etc. 
%   \item recursieve uitbreidingen van de relationele algebra (Datalog) 
%\end{enumerate}
%}%Skip 


==> courses/work-systems-modeling/description.tex <==
\Course{Work-Systems Modeling}
\Version{18-06-05}

\Synopsis
Organizations can by found anywhere. A University is an organization, a sports
club is an organization, a bank is one, government departments are, etc.
Organizations are everywhere. In our modern western society, most organizations
use some information systems to support the activities of the organization.
Large parts of these information systems are likely to be computerized.

Organizations and (computerized) information systems are examples of so-called
\emph{work-systems}. For information system engineers it is relevant to be able
to model relevant aspects of the design of such systems. This may be the design
of a currently existing system or the design of the future
evolution/development of the current system. In this course we will discuss
several examples of work-systems from organizational, information systems,
biological and sociological domains.

\Goals
After this course, students are able to:
\begin{enumerate}
   \item given a case-description of an work-system (such as an
   organization):
   \begin{enumerate}
      \item produce models for different aspects of this system,
      \item understand and evaluate given models of that system,
   \end{enumerate}
   \item argue about, and prove, properties regarding the syntax \& semantics of the models,
   \item reason about the link between an work-system's strategy, and the
   services \& processes it uses to realize this strategy, 
   \item reason about the position of work-system modeling the context of
   information systems engineering. 
\end{enumerate}

\Topics
\begin{enumerate}
   \item Work-systems as a generalization of organizations and information systems
   \item Temporal ordering, actors, actions, actands.
   \item Activity modeling.
   \item Actor modeling.
   \item Actand modeling.
   \item Design patterns.
   \item Work-system strategy.
\end{enumerate}



==> courses/work-systems-modeling/outline.tex <==
\Outline
\Version{18-06-05}
\Part{Introduction}
\begin{itemize}
   \item Organizations, information systems and their history.

   \item Generalization to work-systems.

         Organizational systems, information systems and computerised information systems are
	 all examples of ``work systems'' (is-a). Furthemore, a CIS is part-of an IS and an IS
	 is part-of an OS.

   \item Why a fundamental view?

   \item Why a formal approach?
\end{itemize}

\Part{Modeling Foundations}
This part provides, to some extent, a repetition of domain modeling.  However,
this time around we can provide a more fundamental discussion of some of the
philosophical and linguistic foundations of modeling.

\SubPart{Work-Systems}
\begin{itemize}
   \item Exploration of `systems'.
   \item Observing systems (subjectivity; Peirce)
   \item Studying systems
   \item Knowledge, information and data.
   \item Classes of work systems: organization, information- \& knowledge
   intensive organizations, information \& knowledge systems, computerized
   information \& knowledge systems.
   \item Evolution of systems
\end{itemize}

\SubPart{Basic Object-Role Modeling}
This chapter provides a summary of domain modeling, embedded in the
formalization of the previous chapter.  
\begin{itemize}
   \item Natural language grounding of modeling
   \item The logbook heuristic
   \item Elementary facts
   \item From instances to types
\end{itemize}

\SubPart{Object-Role Calculus}
\begin{itemize}
   \item \emph{O}bject \emph{R}ole \emph{Ca}lculus (ORCa) = Fact Calculus +
   Lisa-D + Time + FORML
   \item Path expressions as a formal foundation
   \item ORCa expressions as verbalisations
   \item Graphical constraints
   \item Temporal constraints
\end{itemize}

\SubPart{Advanced Object-Role Modeling}
\begin{itemize}
   \item Subtyping: Specialization \& Generalization
   \item Decomposition
   \item Complex types
\end{itemize}

\SubPart{The Act of Modeling}
A reflection on the act of modeling
\begin{itemize}
   \item What to model? Intended audience/goals.
   \item The modeling challenge
   \item Ambition levels for modeling
   \item Meeting the challenge
\end{itemize}

\SubPart{Natural-language Foundations of Work-Systems Modeling}
\begin{itemize}
   \item Actions, actors, actands and predications

   \item LAP based heuristics for selection of the concept flavors: action,
   actor, actand and predication
   
   \item Temporal ordering (temporal constraints) of actions.
\end{itemize}

\Part{Modeling Work-Systems}
Now we switch to modeling languages dedicated to work-systems modeling. We
will, however, each time show how they can be regareded as `sugared' versions
of the ORM based models. The refined semantics of these `sugared' versions
will therefore also be expressed in terms of ORCa rather than predicate
calculus.

The notation will be based on the ArchiMate notation. However, it is more
important to have a notation that ties well to our theoretical approach and has
a similar look-and-feel across the spectrum. We should not just import a lot
of relevant notations, but rather `incorporate' them if needed. In addition,
mapping to appropriate other modeling languages like UML and the languages used
in SAP should be provided.

\SubPart{Activity Modeling}
\begin{itemize}
   \item Activity types (internal \& external view of composed actions)

   \item Interaction case (like UML's use case, but `using' has a biased
   co-notation. A work-system is not always some inanimate object one `uses'.).

   \item Syntax of YAWL$^+$ (YAWL with some ArchiMate-ish extensions pertaining
   to actors and actands, rather the other way around. ArchiMate notation
   extended with YAWL-like triggering symbols.).

   \item Work-flow patterns

   \item Formalization of syntax as specialization of ORM domain models.

   \item Formalization of process semantics based on ``petri-net'' like semantics.

   Preferably in ORCa.

   \item Formalization of process semantics using a statistical approach.

   In terms of probabilities.

   \item Mapping to UML activity diagrams, but also to SAP, etc.
\end{itemize}

\SubPart{Actor Modeling}
Modeling actors and their responsibilities. Activity modeling starts out from
an explicit notion of an interaction-case with a pre-defined flow of work. One
could also, however, focus on the responsibilities of actors. This is what we
will do in this chapter.

This chapter will be heavily based on the Organisational Dynamics course as it
is currently taught by NICI. It needs to be integrated with the structure of the
rest of this course. Also, can be use an ArchiMate-ish notation? At any rate a
notation with a similar look-and-feel should be used for activity, actor and
actand modeling.
\begin{itemize}
   \item Actor-Role modeling (ORM-ish interpretation of AGR-Modeling)

	 Note: we need to clarify the relation between agents/actors, roles,
	 role-types and actor-types. Also check the ``business concepts''
	 article on business-roles, etc.

	 Proposal: AGR.Agent = Actor, AGR.Group = Composed actor,
	 AGR.Role = ORM.Object Type, Involvement of AGR.Role in
	 AGR.Interaction/Transfer = ORM.Role Type, AGR.Interaction/Transfer = a
	 kind of ORM.Fact type.
 
   \item Modeling the behavior of actors

	 Role dynamics / transfer dynamics / Role interaction dynamics / Group
	 dynamics / Group interaction dynamics / Organization dynamics

   \item Specification of dynamic properties

         Informal / Semi-formal / Formal

         Relationship to ORCa versus path expression/rel. alg.?

   \item Inter level dynamics

   \item Dynamics of work-system realization (type - instance ??)

         Aren't these the semantics of the above discussed dynamic properties?

   \item Simulation of work-system behavior

         Scenario's? Cf. the CRC-card games in UML/RUP?

   \item Actor-meeting interaction protocol

	 How (if at all) does this relate to collaboration as in
	 ``collaboration engineering/CSCW'' and as in ``collaboration
	 diagrams'' from UML 
\end{itemize}
	 
\SubPart{Actand Modeling}
\begin{itemize}
   \item Not much to say about this.
   \item Just use ORM to describe the actands.
\end{itemize}

\SubPart{Service Modeling}
\begin{itemize}
   \item Abstracted view on activities
   \item Service states and transitions
   \item SLA's
   \item Mapping to UML
\end{itemize}

\SubPart{Work Rules Modeling}
``Business Rules'' generalized to work-systems.
\begin{itemize}
   \item Re-visit of constraints in a business rules context.
\end{itemize}

\Part{Analysis and Design of Work-Systems}

\SubPart{Analysing Classes of Work-Systems}
\begin{itemize}
   \item Biological systems
   \item Sociological systems
   \item Technological systems
   \item Organizational Systems
   \item Information Systems
   \item Computerised Information Systems
\end{itemize}

\SubPart{Paradigms for Work-Systems Design}
\begin{itemize}
   \item Coordination \& control
   \item Brain/Organism/Machine/...
   \item Matrix/network/...
   \item Mintzberg configurations
   \item Self organization
\end{itemize}

\SubPart{Strategy-driven Design of Work-Systems}
\begin{itemize}
  \item Goals/mission
  \item Strategy
  \item Structure follows strategy, or strategy follows structure?
  \item Design approach and types of design
  \item Design as refinement of requirements
  \item Models for deliberation and modification
  \item Strategic management
  \item Enables/disablers of change: 

        7-Ss framework; social, technical \& cultural issues
\end{itemize}



==> courses/work-systems-modeling/tail.tex <==
\Header{Work forms}
\begin{enumerate}
   \item Lectures
   \item Tutorials
\end{enumerate}

\Header{Pre-requisites}
\begin{enumerate}
   \item Domain Modeling
   \item Formeel denken
\end{enumerate}

\Header{Examination}
\begin{enumerate}
   \item Integrated examination
   \item Three sub-exams
\end{enumerate}

\Header{Combinations}
\begin{enumerate}
   \item Storage and Retrieval
\end{enumerate}

\Header{Literature}
\begin{enumerate}
   \item Lecture notes
\end{enumerate}
Will be made available electronically.


==> definitions/100-percent-principle/def.tex <==
The \DefinitionName{information-grammar}{ls} should describe 
\emph{precisely all} conceptual aspects.


==> definitions/100-percent-principle/lp.tex <==
100\% Principle%


==> definitions/100-percent-principle/ls.tex <==
100\% Principle%


==> definitions/100-percent-principle/up.tex <==
100\% Principle%


==> definitions/100-percent-principle/us.tex <==
100\% Principle%


==> definitions/WSML/def.tex <==
Abbreviation for \DefinitionName{work-system}{ls} 
\DefinitionName{modeling}{ls} library. A library of methodical
 \DefinitionName{knowledge}{ls} pertaining to the 
\DefinitionName{modeling}{ls} of \DefinitionName{work-system}{lp}.


==> definitions/WSML/lp.tex <==
WSMLs%


==> definitions/WSML/ls.tex <==
WSML%


==> definitions/WSML/up.tex <==
WSMLs%


==> definitions/WSML/us.tex <==
WSML%


==> definitions/abstraction/def.tex <==
Omitting unessential details.


==> definitions/abstraction/lp.tex <==
abstractions%


==> definitions/abstraction/ls.tex <==
abstraction%


==> definitions/abstraction/up.tex <==
Abstractions%


==> definitions/abstraction/us.tex <==
Abstraction%


==> definitions/action-oriented/def.tex <==
The action-oriented \DefinitionName{approach}{ls} interprets sentences 
as events occurring in the \DefinitionName{uod}{ls}. This 
\DefinitionName{approach}{ls} is when the operations on the 
\DefinitionName{data}{ls} are dominant. See also 
\DefinitionName{fact-oriented}{ls}.


==> definitions/action-oriented/lp.tex <==
action oriented%


==> definitions/action-oriented/ls.tex <==
action oriented%


==> definitions/action-oriented/up.tex <==
Action oriented%


==> definitions/action-oriented/us.tex <==
Action oriented%


==> definitions/active-system/def.tex <==
A special kind of \DefinitionName{system}{ls} that is conceived of as 
begin able to change parts of the \DefinitionName{universe}{ls}.


==> definitions/active-system/lp.tex <==
active systems%


==> definitions/active-system/ls.tex <==
active system%


==> definitions/active-system/up.tex <==
Active systems%


==> definitions/active-system/us.tex <==
Active system%


==> definitions/activity-participation/def.tex <==
A \DefinitionName{system-link}{ls} between a 
\DefinitionName{system-activity}{ls} and one of its 
\DefinitionName{actor}{ls}.


==> definitions/activity-participation/lp.tex <==
activity participations%


==> definitions/activity-participation/ls.tex <==
activity participation%


==> definitions/activity-participation/up.tex <==
Activity participations%


==> definitions/activity-participation/us.tex <==
Activity participation%


==> definitions/actor/def.tex <==
A \DefinitionName{system-element}{ls} that is conceived of as having 
some involvement in a \DefinitionName{system-activity}{ls}. This 
involvement is a special kind of \DefinitionName{system-link}{ls}, 
referred to as an \DefinitionName{activity-participation}{ls}.


==> definitions/actor/lp.tex <==
actors%


==> definitions/actor/ls.tex <==
actor%


==> definitions/actor/up.tex <==
Actors%


==> definitions/actor/us.tex <==
Actor%


==> definitions/agens/def.tex <==
The role in a sentence that most commonly is associated with the 
grammatical subject.


==> definitions/agens/lp.tex <==
agens%


==> definitions/agens/ls.tex <==
agens%


==> definitions/agens/up.tex <==
Agens%


==> definitions/agens/us.tex <==
Agens%


==> definitions/alignment/def.tex <==
A \DefinitionName{system}{ls} $S_1$ is aligned to a 
\DefinitionName{system}{ls} $S_2$ if, and only if, 
\DefinitionName{system}{ls} $S_1$ meets {\em all} 
\DefinitionName{requirement}{lp} posed by $S_2$ on $S_1$. This 
\DefinitionName{alignment}{ls} may be strived for at different levels 
of refinement of a \DefinitionName{system-design}{ls}.


==> definitions/alignment/lp.tex <==
alignment%


==> definitions/alignment/ls.tex <==
alignment%


==> definitions/alignment/up.tex <==
Alignment%


==> definitions/alignment/us.tex <==
Alignment%


==> definitions/application-domain/def.tex <==
That part of the world around is that is to be modelled in the context 
of the development of some application. See also 
\DefinitionName{uod}{ls}.


==> definitions/application-domain/lp.tex <==
application domains%


==> definitions/application-domain/ls.tex <==
application domains%


==> definitions/application-domain/up.tex <==
Application domains%


==> definitions/application-domain/us.tex <==
Application domain%


==> definitions/approach/def.tex <==
\Synonym{way-of-working}


==> definitions/approach/lp.tex <==
approaches%


==> definitions/approach/ls.tex <==
approach%


==> definitions/approach/up.tex <==
Approaches%


==> definitions/approach/us.tex <==
Approach%


==> definitions/architecting/lp.tex <==
architecting%


==> definitions/architecting/ls.tex <==
architecting%


==> definitions/architecting/up.tex <==
Architecting%


==> definitions/architecting/us.tex <==
Architecting%


==> definitions/architectural-description/def.tex <==
A \DefinitionName{system-description}{ls} documenting/describing an 
\DefinitionName{architecture}{ls}.


==> definitions/architectural-description/lp.tex <==
architectural descriptions%


==> definitions/architectural-description/ls.tex <==
architectural description%


==> definitions/architectural-description/up.tex <==
Architectural descriptions%


==> definitions/architectural-description/us.tex <==
Architectural description%


==> definitions/architecture-driven-information-system-engineering/def.tex <==
\DefinitionName{information-system-engineering}{us}, using 
\DefinitionName{architecture}{ls} as a means to
\begin{itemize}

\item guide \& control the \DefinitionName{design}{ls} and evolution of 
the \DefinitionName{information-system}{ls},
\item evaluate \& compare different 
\DefinitionName{information-system}{ls} alternatives,
\item negotiate the \DefinitionName{concern}{lp} of the 
\DefinitionName{information-system}{ls}'s 
\DefinitionName{stakeholder}{lp},
\end{itemize}
with the aim of optimising the \DefinitionName{alignment}{ls} of the 
resulting \DefinitionName{information-system}{ls} to its relevant, 
technological, organisation and human context 
(\DefinitionName{system}{lp}).


==> definitions/architecture-driven-information-system-engineering/lp.tex <==
architecture-driven information system engineering%


==> definitions/architecture-driven-information-system-engineering/ls.tex <==
architecture-driven information system engineering%


==> definitions/architecture-driven-information-system-engineering/up.tex <==
Architecture-driven information system engineering%


==> definitions/architecture-driven-information-system-engineering/us.tex <==
Architecture-driven information system engineering%


==> definitions/architecture-driven-system-engineering/def.tex <==
\UDN{system-engineering}, using \DN{architecture} as a means to
\begin{itemize}
   \item guide \& control the design and evolution of the \DN{system},
   \item evaluate \& compare different information system alternatives,
   \item negotiate the \PDN{concern} of the information system's \PDN{stakeholder},
\end{itemize}
with the aim of optimising the \DN{alignment} of the resulting
information system to its relevant, technological, organisation and human context (systems).



==> definitions/architecture-driven-system-engineering/lp.tex <==
architecture-driven-system-engineering%


==> definitions/architecture-driven-system-engineering/ls.tex <==
architecture-driven-system-engineering%


==> definitions/architecture-driven-system-engineering/up.tex <==
Architecture-driven-system-engineering%


==> definitions/architecture-driven-system-engineering/us.tex <==
Architecture-driven-system-engineering%


==> definitions/architecture-principle/def.tex <==
A \DefinitionName{design-principle}{ls} which is used to direct the 
design/architecting of an \DefinitionName{architecture}{ls}.


==> definitions/architecture-principle/lp.tex <==
architecture principles%


==> definitions/architecture-principle/ls.tex <==
architecture principle%


==> definitions/architecture-principle/up.tex <==
Architecture principles%


==> definitions/architecture-principle/us.tex <==
Architecture principle%


==> definitions/architecture/def.tex <==
A \DefinitionName{model}{ls} of which the 
\DefinitionName{system-description}{ls}, the so-called 
\DefinitionName{architectural-description}{ls}, is used during 
\DefinitionName{system-engineering}{ls} to:
\begin{itemize}

\item express the fundamental \DefinitionName{organization}{ls} of the 
\DefinitionName{system-domain}{ls} in terms of 
\DefinitionName{component}{lp}, their relationships to each other and 
to the \DefinitionName{environment}{ls} and
\item the principles guiding its evolution and 
\DefinitionName{design}{ls},
\end{itemize}
and which's explicit intend is to be used as a means:
\begin{itemize}

\item of \DefinitionName{communication}{ls} \& negotiation among 
\DefinitionName{stakeholder}{lp},
\item to evaluate and compare \DefinitionName{design}{ls} alternatives,
\item to plan, manage, and execute further 
\DefinitionName{system-development}{ls},
\item to verify the compliance of a \DefinitionName{system}{ls} 
implementation's.
\end{itemize}



==> definitions/architecture/lp.tex <==
architectures%


==> definitions/architecture/ls.tex <==
architecture%


==> definitions/architecture/up.tex <==
Architectures%


==> definitions/architecture/us.tex <==
Architecture%


==> definitions/aspect-system/def.tex <==
an aspect-system $S'$ of a \DefinitionName{system}{ls} $S$, is a 
\DefinitionName{sub-system}{ls}, where the set of 
\DefinitionName{model-link}{lp} in $S'$ is a proper subset of the set 
of the \DefinitionName{link}{lp} in $S$.


==> definitions/aspect-system/lp.tex <==
aspect systems%


==> definitions/aspect-system/ls.tex <==
aspect system%


==> definitions/aspect-system/up.tex <==
Aspect systems%


==> definitions/aspect-system/us.tex <==
Aspect system%


==> definitions/atomic-viewpoint/def.tex <==
A \DefinitionName{viewpoint}{ls} which is not decomposed into smaller 
\DefinitionName{viewpoint}{lp}. An
 \DefinitionName{atomic-viewpoint}{ls} is required to have a one-on-one 
correspondence to a
 \DefinitionName{way-of-modeling}{ls}/\DefinitionName{technique}{ls} 
that should be used to create \DefinitionName{model}{lp}
 conforming to this \DefinitionName{viewpoint}{ls}.


==> definitions/atomic-viewpoint/lp.tex <==
atomic viewpoints%


==> definitions/atomic-viewpoint/ls.tex <==
atomic viewpoint%


==> definitions/atomic-viewpoint/up.tex <==
Atomic viewpoints%


==> definitions/atomic-viewpoint/us.tex <==
Atomic viewpoint%


==> definitions/autonomous-system/def.tex <==
an \DefinitionName{open-active-system}{ls} (possibly also a 
\DefinitionName{responsive-system}{ls}, but not a 
\DefinitionName{reactive-system}{ls}) where at least one expression is 
an action. A human being and most (if not all) 
\DefinitionName{organization}{lp} can be regarded as 
\DefinitionName{autonomous-system}{lp}.


==> definitions/autonomous-system/lp.tex <==
autonomous systems%


==> definitions/autonomous-system/ls.tex <==
autonomous system%


==> definitions/autonomous-system/up.tex <==
Autonomous systems%


==> definitions/autonomous-system/us.tex <==
Autonomous system%


==> definitions/characterization-dimension/def.tex <==
A set of (possibly ordered) values by which an artefact may be 
characterized.


==> definitions/characterization-dimension/lp.tex <==
characterization dimensions%


==> definitions/characterization-dimension/ls.tex <==
characterization dimension%


==> definitions/characterization-dimension/up.tex <==
Characterization dimensions%


==> definitions/characterization-dimension/us.tex <==
Characterization dimension%


==> definitions/characterization-property/def.tex <==
A specific value from a \DefinitionName{characterization-dimension}{ls} 
that an artefact may
 exhibit. 


==> definitions/characterization-property/lp.tex <==
characterization properties%


==> definitions/characterization-property/ls.tex <==
characterization property%


==> definitions/characterization-property/up.tex <==
Characterization properties%


==> definitions/characterization-property/us.tex <==
Characterization property%


==> definitions/closed-world-assumption/def.tex <==
All facts not stored in an \DefinitionName{information-system}{ls} are 
assumed to be false. Not that this requires facts with 
\DefinitionName{complete-knowledge}{ls}.


==> definitions/closed-world-assumption/lp.tex <==
closed world assumptions%


==> definitions/closed-world-assumption/ls.tex <==
closed world assumption%


==> definitions/closed-world-assumption/up.tex <==
Closed world assumptions%


==> definitions/closed-world-assumption/us.tex <==
Closed world assumption%


==> definitions/communication/lp.tex <==
communications%


==> definitions/communication/ls.tex <==
communication%


==> definitions/communication/up.tex <==
Communications%


==> definitions/communication/us.tex <==
Communication%


==> definitions/complete-knowledge/def.tex <==
The value \emph{undefined} is not allowed.


==> definitions/complete-knowledge/lp.tex <==
complete knowledge%


==> definitions/complete-knowledge/ls.tex <==
complete knowledge%


==> definitions/complete-knowledge/up.tex <==
Complete knowledge%


==> definitions/complete-knowledge/us.tex <==
Complete knowledge%


==> definitions/component-system/def.tex <==
A component-system $S'$ of a \DefinitionName{system}{ls} $S$, is a 
\DefinitionName{sub-system}{ls}, where the set of 
\DefinitionName{model-concept}{lp} in $S'$ is a proper subset of the 
set of entities in $S$.


==> definitions/component-system/lp.tex <==
component systems%


==> definitions/component-system/ls.tex <==
component system%


==> definitions/component-system/up.tex <==
Component systems%


==> definitions/component-system/us.tex <==
Component system%


==> definitions/component/def.tex <==
\AbbreviationOf{component-system}


==> definitions/component/lp.tex <==
components%


==> definitions/component/ls.tex <==
component%


==> definitions/component/up.tex <==
Components%


==> definitions/component/us.tex <==
Component%


==> definitions/computerized-information-system/def.tex <==
A \DefinitionName{sub-system}{ls} of an 
\DefinitionName{information-system}{ls}, whereby all activities within 
that \DefinitionName{sub-system}{ls} are performed by one or several 
computer(s).


==> definitions/computerized-information-system/lp.tex <==
computerized information systems%


==> definitions/computerized-information-system/ls.tex <==
computerized information system%


==> definitions/computerized-information-system/up.tex <==
Computerized information systems%


==> definitions/computerized-information-system/us.tex <==
Computerized information system%


==> definitions/concept/def.tex <==
Any \DefinitionName{element}{ls} from a \DefinitionName{conception}{ls} 
that is not a \DefinitionName{link}{ls}.


==> definitions/concept/lp.tex <==
concepts%


==> definitions/concept/ls.tex <==
concept%


==> definitions/concept/up.tex <==
Concepts%


==> definitions/concept/us.tex <==
Concept%


==> definitions/conception-evolution/def.tex <==
The evolution of a \DefinitionName{conception}{ls}.


==> definitions/conception-evolution/lp.tex <==
conception evolutions%


==> definitions/conception-evolution/ls.tex <==
conception evolution%


==> definitions/conception-evolution/up.tex <==
Conception evolutions%


==> definitions/conception-evolution/us.tex <==
Conception evolution%


==> definitions/conception/def.tex <==
That what results, in the mind of a \DefinitionName{viewer}{ls}, when 
they interpret a \DefinitionName{perception}{ls} of a 
\DefinitionName{domain}{ls}.


==> definitions/conception/lp.tex <==
conceptions%


==> definitions/conception/ls.tex <==
conception%


==> definitions/conception/up.tex <==
Conceptions%


==> definitions/conception/us.tex <==
Conception%


==> definitions/conceptualization-principle/def.tex <==
The \DefinitionName{information-grammar}{ls} should not describe any 
does \emph{not} provide any realization (implementation) aspect.


==> definitions/conceptualization-principle/lp.tex <==
Conceptualization principle%


==> definitions/conceptualization-principle/ls.tex <==
conceptualization principle%


==> definitions/conceptualization-principle/up.tex <==
Conceptualization principle%


==> definitions/conceptualization-principle/us.tex <==
Conceptualization principle%


==> definitions/concern/def.tex <==
An \DefinitionName{interest}{ls} of a \DefinitionName{stakeholder}{ls}, 
resulting from the \DefinitionName{stakeholder-goal}{lp}, and the role 
played by some \DefinitionName{system}{ls}. This usually pertains to 
the \DefinitionName{system}{ls}'s development, its operation or any 
other aspects that are critical or otherwise important to one or more 
\DefinitionName{stakeholder}{lp}.


==> definitions/concern/lp.tex <==
concerns%


==> definitions/concern/ls.tex <==
concern%


==> definitions/concern/up.tex <==
Concerns%


==> definitions/concern/us.tex <==
Concern%


==> definitions/construction-process/def.tex <==
A process aiming to realize and test a \DefinitionName{system}{ls} that 
is regarded as a (possibly artificial) artifact that is not yet in 
operation.


==> definitions/construction-process/lp.tex <==
construction processes%


==> definitions/construction-process/ls.tex <==
construction process%


==> definitions/construction-process/up.tex <==
Construction processes%


==> definitions/construction-process/us.tex <==
Construction process%


==> definitions/construction/def.tex <==
\AbbreviationOf{construction-process}


==> definitions/construction/lp.tex <==
constructions%


==> definitions/construction/ls.tex <==
construction%


==> definitions/construction/up.tex <==
Constructions%


==> definitions/construction/us.tex <==
Construction%


==> definitions/controlled-language/def.tex <==
A \DefinitionName{controlled-language}{ls} is a form of language with 
special restrictions on grammar, style, and vocabulary usage, close to 
natural language, but with a formal base. The objective of a 
\DefinitionName{controlled-language}{ls} is to improve the consistency, 
readability, translatability, and retrievability of 
\DefinitionName{information}{ls}.


==> definitions/controlled-language/lp.tex <==
controlled languages%


==> definitions/controlled-language/ls.tex <==
controlled language%


==> definitions/controlled-language/up.tex <==
Controlled languages%


==> definitions/controlled-language/us.tex <==
Controlled language%


==> definitions/data/lp.tex <==
data%


==> definitions/data/ls.tex <==
data%


==> definitions/data/up.tex <==
Data%


==> definitions/data/us.tex <==
Data%


==> definitions/decomposer/def.tex <==
The \DefinitionName{link}{ls} between a composed 
\DefinitionName{concept}{ls} and one of its underlying 
\DefinitionName{concept}{lp}.


==> definitions/decomposer/lp.tex <==
decomposers%


==> definitions/decomposer/ls.tex <==
decomposer%


==> definitions/decomposer/up.tex <==
Decomposers%


==> definitions/decomposer/us.tex <==
Decomposer%


==> definitions/deep-sentence-structure/def.tex <==
Sentences with the same meaning may have distinct surface forms. These 
are derived from an unobservable common source, the so-called deep 
structure underlying both sentences.


==> definitions/deep-sentence-structure/lp.tex <==
deep sentence structures%


==> definitions/deep-sentence-structure/ls.tex <==
deep sentence structure%


==> definitions/deep-sentence-structure/up.tex <==
Deep sentence structures%


==> definitions/deep-sentence-structure/us.tex <==
Deep sentence structure%


==> definitions/definition-description/def.tex <==
The \DefinitionName{description}{ls} of a 
\DefinitionName{definition}{ls}.


==> definitions/definition-description/lp.tex <==
definition descriptions%


==> definitions/definition-description/ls.tex <==
definition description%


==> definitions/definition-description/up.tex <==
Definition descriptions%


==> definitions/definition-description/us.tex <==
Definition description%


==> definitions/definition-process/lp.tex <==
definition processes%


==> definitions/definition-process/ls.tex <==
definition process%


==> definitions/definition-process/up.tex <==
Definition processes%


==> definitions/definition-process/us.tex <==
Definition process%


==> definitions/definition/def.tex <==
The \DefinitionName{requirement}{lp} that should be met by a desired 
\DefinitionName{work-system}{ls} as well its 
\DefinitionName{system-description}{ls} including the 
\DefinitionName{description}{lp} of the \DefinitionName{system}{ls}'s 
\DefinitionName{definition}{ls}, \DefinitionName{design}{ls} as well as 
documentation for the operational \DefinitionName{system}{ls}. These 
\DefinitionName{requirement}{lp} will typically identify: \emph{what} 
it should do, \emph{how well} it should do this, and \emph{why} it 
should do so.


==> definitions/definition/lp.tex <==
definitions%


==> definitions/definition/ls.tex <==
definition%


==> definitions/definition/up.tex <==
Definitions%


==> definitions/definition/us.tex <==
Definition%


==> definitions/deployment-process/def.tex <==
A process aiming to make a \DefinitionName{system}{ls} operational, 
i.e.\ to implement the use of the \DefinitionName{system}{ls} by its 
prospective users.


==> definitions/deployment-process/lp.tex <==
deployment processes%


==> definitions/deployment-process/ls.tex <==
deployment process%


==> definitions/deployment-process/up.tex <==
Deployment processes%


==> definitions/deployment-process/us.tex <==
Deployment process%


==> definitions/deployment/def.tex <==
\AbbreviationOf{deployment}


==> definitions/deployment/lp.tex <==
deployments%


==> definitions/deployment/ls.tex <==
deployment%


==> definitions/deployment/up.tex <==
Deployments%


==> definitions/deployment/us.tex <==
Deployment%


==> definitions/description-process/def.tex <==
The combination of the \DefinitionName{definition-process}{ls} and 
\DefinitionName{design-process}{ls}.


==> definitions/description-process/lp.tex <==
description processes%


==> definitions/description-process/ls.tex <==
description process%


==> definitions/description-process/up.tex <==
Description processes%


==> definitions/description-process/us.tex <==
Description process%


==> definitions/description/def.tex <==
The result of a \DefinitionName{viewer}{ls} denoting a 
\DefinitionName{conception}{ls}, using some language to express 
themselves.


==> definitions/description/lp.tex <==
descriptions%


==> definitions/description/ls.tex <==
description%


==> definitions/description/up.tex <==
Descriptions%


==> definitions/description/us.tex <==
Description%


==> definitions/design-description/def.tex <==
The \DefinitionName{description}{ls} of a \DefinitionName{design}{ls}.


==> definitions/design-description/lp.tex <==
design descriptions%


==> definitions/design-description/ls.tex <==
design description%


==> definitions/design-description/up.tex <==
Design descriptions%


==> definitions/design-description/us.tex <==
Design description%


==> definitions/design-principle/def.tex <==
A \DefinitionName{system-description}{ls} language, which is intended 
to aid in the transition from \DefinitionName{requirement}{lp} to 
\DefinitionName{design}{ls}. Each principle is a predicate over the 
products of the \DefinitionName{design-process}{ls}, where a 
\DefinitionName{system}{ls} is no longer treated as a black-box. It 
thus provides direction to the ensuing 
\DefinitionName{design-process}{ls}.


==> definitions/design-principle/lp.tex <==
design principles%


==> definitions/design-principle/ls.tex <==
design principle%


==> definitions/design-principle/up.tex <==
Design principles%


==> definitions/design-principle/us.tex <==
Design principle%


==> definitions/design-process/lp.tex <==
design processes%


==> definitions/design-process/ls.tex <==
design process%


==> definitions/design-process/up.tex <==
Design processes%


==> definitions/design-process/us.tex <==
Design process%


==> definitions/design/def.tex <==
The identification and motivation of \emph{how} a 
\DefinitionName{work-system}{ls} will meet the 
\DefinitionName{requirement}{lp} set out in its 
\DefinitionName{definition}{ls}. The resulting 
\DefinitionName{design}{ls} may (depending on the 
\DefinitionName{design}{ls} \DefinitionName{goal}{lp}) range from 
high-level \DefinitionName{design}{lp} to the detailed level of 
programming statements or specific worker tasks.


==> definitions/design/lp.tex <==
designs%


==> definitions/design/ls.tex <==
design%


==> definitions/design/up.tex <==
Designs%


==> definitions/design/us.tex <==
Design%


==> definitions/domain-evolution/def.tex <==
The evolution of a \DefinitionName{domain}{ls} over time.


==> definitions/domain-evolution/lp.tex <==
domain evolutions%


==> definitions/domain-evolution/ls.tex <==
domain evolution%


==> definitions/domain-evolution/up.tex <==
Domain evolutions%


==> definitions/domain-evolution/us.tex <==
Domain evolution%


==> definitions/domain-expert/def.tex <==
A person that can reveal and assign meaning to statements about the 
\DefinitionName{uod}{ls}. The \DefinitionName{domain-expert}{ls} role 
is further divided into an \DefinitionName{informant}{ls} and a 
\DefinitionName{modeling-mediator}{ls}.


==> definitions/domain-expert/lp.tex <==
domain experts%


==> definitions/domain-expert/ls.tex <==
domain expert%


==> definitions/domain-expert/up.tex <==
Domain experts%


==> definitions/domain-expert/us.tex <==
Falsification%


==> definitions/domain-modeling/lp.tex <==
domain modeling%


==> definitions/domain-modeling/ls.tex <==
domain modeling%


==> definitions/domain-modeling/up.tex <==
Domain modeling%


==> definitions/domain-modeling/us.tex <==
Domain modeling%


==> definitions/domain/def.tex <==
Any `part' or `aspect' of the \DefinitionName{universe}{ls} a 
\DefinitionName{viewer}{ls} may have an \DefinitionName{interest}{ls} 
in.


==> definitions/domain/lp.tex <==
domains%


==> definitions/domain/ls.tex <==
domain%


==> definitions/domain/up.tex <==
Domains%


==> definitions/domain/us.tex <==
Domain%


==> definitions/dynamic-system/def.tex <==
A special kind of \DefinitionName{system}{ls} that is conceived of as 
undergoing change in the cause of time.


==> definitions/dynamic-system/lp.tex <==
dynamic systems%


==> definitions/dynamic-system/ls.tex <==
dynamic system%


==> definitions/dynamic-system/up.tex <==
Dynamic systems%


==> definitions/dynamic-system/us.tex <==
Dynamic system%


==> definitions/efficiency/def.tex <==
Is the relationship between the level of performance of the 
\DefinitionName{system}{ls} (or a \DefinitionName{sub-system}{ls}) and 
the amount of resources used, under stated conditions. 
\DefinitionName{efficiency}{us} may be related to time behaviour 
(response time, processing time, throughput rates) and to resource 
behaviour (amount of resources used and duration of such use).


==> definitions/efficiency/lp.tex <==
efficiency%


==> definitions/efficiency/ls.tex <==
efficiency%


==> definitions/efficiency/up.tex <==
Efficiency%


==> definitions/efficiency/us.tex <==
Efficiency%


==> definitions/element-evolution/def.tex <==
The evolution over time of an \DefinitionName{element}{ls} in the 
\DefinitionName{conception}{ls} of a \DefinitionName{viewer}{ls}.


==> definitions/element-evolution/lp.tex <==
element evolutions%


==> definitions/element-evolution/ls.tex <==
element evolution%


==> definitions/element-evolution/up.tex <==
Element evolutions%


==> definitions/element-evolution/us.tex <==
Element evolution%


==> definitions/element-version/def.tex <==
The version of an \DefinitionName{element-evolution}{ls} as it holds at 
some point in time. This version is an \DefinitionName{element}{ls} 
from a \DefinitionName{viewer}{ls}'s \DefinitionName{conception}{ls} of 
a \DefinitionName{universe}{ls}.


==> definitions/element-version/lp.tex <==
element versions%


==> definitions/element-version/ls.tex <==
element version%


==> definitions/element-version/up.tex <==
Element versions%


==> definitions/element-version/us.tex <==
Element version%


==> definitions/element/def.tex <==
The elementary parts of a \DefinitionName{viewer}{ls}'s 
\DefinitionName{conception}{ls}.


==> definitions/element/lp.tex <==
elements%


==> definitions/element/ls.tex <==
element%


==> definitions/element/up.tex <==
Elements%


==> definitions/element/us.tex <==
Element%


==> definitions/elementary-sentence/def.tex <==
Sentences that can not be split into smaller sentences without losing 
\DefinitionName{information}{ls}.


==> definitions/elementary-sentence/lp.tex <==
elementary sentences%


==> definitions/elementary-sentence/ls.tex <==
elementary sentence%


==> definitions/elementary-sentence/up.tex <==
Elementary sentences%


==> definitions/elementary-sentence/us.tex <==
Elementary sentence%


==> definitions/elicitation/def.tex <==
The activity in which the \DefinitionName{system-analyst}{ls} tries to 
obtain sample sentences form the \DefinitionName{domain-expert}{ls}.


==> definitions/elicitation/lp.tex <==
elicitation%


==> definitions/elicitation/ls.tex <==
elicitation%


==> definitions/elicitation/up.tex <==
Elicitation%


==> definitions/elicitation/us.tex <==
Elicitation%


==> definitions/engineering-time-requirement/def.tex <==
A \DefinitionName{product-requirement}{ls} on any of the products, 
pertaining to a \DefinitionName{system-engineering}{ls} process, other 
than the resulting \DefinitionName{system}{ls}. These 
\DefinitionName{requirement}{lp} usually refer to 
\DefinitionName{quality-attribute}{lp} such as: 
\DefinitionName{maintainability}{ls} and 
\DefinitionName{portability}{ls}.


==> definitions/engineering-time-requirement/lp.tex <==
engineering-time requirements%


==> definitions/engineering-time-requirement/ls.tex <==
engineering-time requirement%


==> definitions/engineering-time-requirement/up.tex <==
Engineering-time requirements%


==> definitions/engineering-time-requirement/us.tex <==
Engineering-time requirement%


==> definitions/environment-evolution/def.tex <==
The evolution of an \DefinitionName{environment}{ls} over time.


==> definitions/environment-evolution/lp.tex <==
environment evolutions%


==> definitions/environment-evolution/ls.tex <==
environment evolution%


==> definitions/environment-evolution/up.tex <==
Environment evolutions%


==> definitions/environment-evolution/us.tex <==
Environment evolution%


==> definitions/environment/def.tex <==
The \DefinitionName{environment}{ls} of a \DefinitionName{domain}{ls} 
is that part of a \DefinitionName{viewer}{ls}'s 
\DefinitionName{conception}{ls} of a \DefinitionName{universe}{ls}, 
which has a direct \DefinitionName{link}{ls} to the 
\DefinitionName{domain}{ls}.


==> definitions/environment/lp.tex <==
environments%


==> definitions/environment/ls.tex <==
environment%


==> definitions/environment/up.tex <==
Environments%


==> definitions/environment/us.tex <==
Environment%


==> definitions/evolutionary-approach/def.tex <==
A (part of a) development process is executed completely in several 
iterations, leading to several consecutive versions of the set of 
deliverables.


==> definitions/evolutionary-approach/lp.tex <==
evolutionary approaches%


==> definitions/evolutionary-approach/ls.tex <==
evolutionary approach%


==> definitions/evolutionary-approach/up.tex <==
Evolutionary approaches%


==> definitions/evolutionary-approach/us.tex <==
Evolutionary approach%


==> definitions/fact-oriented/def.tex <==
The fact-oriented \DefinitionName{approach}{ls} interprets sentences as 
facts about the \DefinitionName{uod}{ls}. This 
\DefinitionName{approach}{ls} is used data-intensive 
\DefinitionName{domain}{lp} when the structure of the 
\DefinitionName{data}{ls} is dominant. See also 
\DefinitionName{action-oriented}{ls}.


==> definitions/fact-oriented/lp.tex <==
fact oriented%


==> definitions/fact-oriented/ls.tex <==
fact oriented%


==> definitions/fact-oriented/up.tex <==
Fact oriented%


==> definitions/fact-oriented/us.tex <==
Fact oriented%


==> definitions/falsification/def.tex <==
A \DefinitionName{model}{ls} is assumed to be valid until contradicted 
by observation.


==> definitions/falsification/lp.tex <==
falsifications%


==> definitions/falsification/ls.tex <==
falsification%


==> definitions/falsification/up.tex <==
Falsifications%


==> definitions/falsification/us.tex <==
Falsification%


==> definitions/formal-communication/def.tex <==
\DefinitionName{communication}{us} that is based on an objective 
intermediate \DefinitionName{representation}{ls}, in which the 
\DefinitionName{information}{ls} transfer is independent of the actual 
interaction.


==> definitions/formal-communication/lp.tex <==
formal communications%


==> definitions/formal-communication/ls.tex <==
formal communication%


==> definitions/formal-communication/up.tex <==
Formal communications%


==> definitions/formal-communication/us.tex <==
Formal communication%


==> definitions/functional-requirement/def.tex <==
A \DefinitionName{requirement}{ls} which is based on the 
\DefinitionName{functionality}{ls} 
\DefinitionName{quality-attribute}{ls}.


==> definitions/functional-requirement/lp.tex <==
functional requirements%


==> definitions/functional-requirement/up.tex <==
Functional requirements%


==> definitions/functional-requirement/us.tex <==
Functional requirement%


==> definitions/functionality/def.tex <==
Bears on the existence of a set of functions and their specified 
properties. The functions are those that satisfy stated or implied 
needs. Sub-characteristics of \DefinitionName{functionality}{ls} are: 
suitability, accuracy, interoperability, compliance, security and 
traceability.


==> definitions/functionality/lp.tex <==
functionalities%


==> definitions/functionality/ls.tex <==
functionality%


==> definitions/functionality/up.tex <==
Functionalities%


==> definitions/functionality/us.tex <==
Functionality%


==> definitions/goal-seeking-process/def.tex <==
A process seeking a balance between what \emph{ought to be} the case 
and what \emph{can be} the case with respect to some pre-existing 
situation, taking into acount the context, resource limitations, etc. 
Achieving the balance is the \DefinitionName{goal}{ls} sought after.


==> definitions/goal-seeking-process/lp.tex <==
goal-seeking processes%


==> definitions/goal-seeking-process/ls.tex <==
goal-seeking process%


==> definitions/goal-seeking-process/up.tex <==
Goal-seeking processes%


==> definitions/goal-seeking-process/us.tex <==
Goal-seeking process%


==> definitions/goal/def.tex <==
\AbbreviationOf{stakeholder-goal}


==> definitions/goal/lp.tex <==
goals%


==> definitions/goal/ls.tex <==
goal%


==> definitions/goal/up.tex <==
Goals%


==> definitions/goal/us.tex <==
Goal%


==> definitions/human-actor/def.tex <==
An \DefinitionName{actor}{ls} which is a single human being, or 
essentially a set of human-beings, such as a team.


==> definitions/human-actor/lp.tex <==
human actors%


==> definitions/human-actor/ls.tex <==
human actor%


==> definitions/human-actor/up.tex <==
Human actors%


==> definitions/human-actor/us.tex <==
Human actors%


==> definitions/incremental-approach/def.tex <==
A (part of a) development process is executed on a 
\DefinitionName{sub-system}{ls} by \DefinitionName{sub-system}{ls} 
basis, using some well-defined division of a 
\DefinitionName{system}{ls} into sub-\DefinitionName{system}{lp}.


==> definitions/incremental-approach/lp.tex <==
incremental approaches%


==> definitions/incremental-approach/ls.tex <==
incremental approach%


==> definitions/incremental-approach/up.tex <==
Incremental approaches%


==> definitions/incremental-approach/us.tex <==
Incremental approach%


==> definitions/index-expression/def.tex <==
A simple structure for sentences, having some similarity with 
mathematical expressions. These expressions are used in the context of 
\DefinitionName{information}{us} Retrieval, as they provide a fair 
compromise between expressivity and feasibility. In the context of 
\DefinitionName{domain-modeling}{ls} they are a 
\DefinitionName{representation}{ls} for sentences structures in the 
contex of \DefinitionName{orm}{ls}.


==> definitions/index-expression/lp.tex <==
index expressions%


==> definitions/index-expression/ls.tex <==
index expression%


==> definitions/index-expression/up.tex <==
Index expressions%


==> definitions/index-expression/us.tex <==
Index expression%


==> definitions/informal-communication/def.tex <==
\DefinitionName{communication}{us} that is not based on an objective 
intermediate \DefinitionName{representation}{ls}, making the 
\DefinitionName{information}{ls} transfer independent of the actual 
interaction.


==> definitions/informal-communication/lp.tex <==
informal communications%


==> definitions/informal-communication/ls.tex <==
informal communication%


==> definitions/informal-communication/up.tex <==
Informal communications%


==> definitions/informal-communication/us.tex <==
Informal communication%


==> definitions/informant/def.tex <==
\Synonym{domain-expert}


==> definitions/informant/lp.tex <==
informants%


==> definitions/informant/ls.tex <==
informant%


==> definitions/informant/up.tex <==
Informants%


==> definitions/informant/us.tex <==
Informant%


==> definitions/information-architecture/def.tex <==
The \DefinitionName{architecture}{ls} of an 
\DefinitionName{information-system}{ls}. Note that an 
\DefinitionName{information-system}{ls} may range in scope from, e.g., 
a value-chain wide \DefinitionName{information-system}{ls} to a 
hand-held information-appliance.


==> definitions/information-architecture/lp.tex <==
information architectures%


==> definitions/information-architecture/ls.tex <==
information architecture%


==> definitions/information-architecture/up.tex <==
Information architectures%


==> definitions/information-architecture/us.tex <==
Information architecture%


==> definitions/information-base/def.tex <==
The set of facts stored in an \DefinitionName{information-system}{ls}. 
This set contains all base statements that are valid in the associated 
\DefinitionName{uod}{ls}. If the 
\DefinitionName{closed-world-assumption}{ls} holds, then all other base 
statements are deemed to be false.


==> definitions/information-base/lp.tex <==
information bases%


==> definitions/information-base/ls.tex <==
information base%


==> definitions/information-base/up.tex <==
Information bases%


==> definitions/information-base/us.tex <==
Information base%


==> definitions/information-grammar/def.tex <==
A \DefinitionName{model}{ls} of the underlying format of the 
\DefinitionName{message}{lp} and to grasp the essentials of their 
meaning. This \DefinitionName{model}{ls} is seen as grammar.


==> definitions/information-grammar/lp.tex <==
information grammars%


==> definitions/information-grammar/ls.tex <==
information grammar%


==> definitions/information-grammar/up.tex <==
Information grammars%


==> definitions/information-grammar/us.tex <==
Information grammar%


==> definitions/information-intensive-organization/def.tex <==
An \DefinitionName{organization}{ls} conceived of as an 
\DefinitionName{organizational-system}{ls}, where the 
\DefinitionName{information-system}{ls} \DefinitionName{sub-system}{ls} 
forms an essential part of the 
\DefinitionName{organizational-system}{ls}.


==> definitions/information-intensive-organization/lp.tex <==
information intensive organizations%


==> definitions/information-intensive-organization/ls.tex <==
information intensive organization%


==> definitions/information-intensive-organization/up.tex <==
Information intensive organizations%


==> definitions/information-intensive-organization/us.tex <==
Information intensive organization%


==> definitions/information-processor/def.tex <==
The active \DefinitionName{component}{ls} of an 
\DefinitionName{information-system}{ls}. It processes the incoming 
commands.


==> definitions/information-processor/lp.tex <==
information processors%


==> definitions/information-processor/ls.tex <==
information processor%


==> definitions/information-processor/up.tex <==
Information processors%


==> definitions/information-processor/us.tex <==
Information processor%


==> definitions/information-system-engineering/def.tex <==
A \DefinitionName{system-engineering}{ls} process pertaining to the 
creation or change of \DefinitionName{information-system}{lp}.


==> definitions/information-system-engineering/lp.tex <==
information system engineering%


==> definitions/information-system-engineering/ls.tex <==
information system engineering%


==> definitions/information-system-engineering/up.tex <==
Information system engineering%


==> definitions/information-system-engineering/us.tex <==
Information system engineering%


==> definitions/information-system/def.tex <==
A \DefinitionName{sub-system}{ls} of an 
\DefinitionName{organizational-system}{ls}, comprising the 
\DefinitionName{conception}{ls} of how the 
\DefinitionName{communication}{ls} and information-oriented aspects of 
an \DefinitionName{organization}{ls} are composed and how these 
operate, thus leading to a \DefinitionName{description}{ls} of the 
(explicit and/or implicit) commu\-nication-oriented and 
information-providing actions and arrangements existing within the 
\DefinitionName{organizational-system}{ls}.


==> definitions/information-system/lp.tex <==
information systems%


==> definitions/information-system/ls.tex <==
information system%


==> definitions/information-system/up.tex <==
Information systems%


==> definitions/information-system/us.tex <==
Information system%


==> definitions/information-technology/def.tex <==
To be defined.


==> definitions/information-technology/lp.tex <==
information technologys%


==> definitions/information-technology/ls.tex <==
information technology%


==> definitions/information-technology/up.tex <==
Information technologys%


==> definitions/information-technology/us.tex <==
Information technology%


==> definitions/information/lp.tex <==
information%


==> definitions/information/ls.tex <==
information%


==> definitions/information/up.tex <==
Information%


==> definitions/information/us.tex <==
Information%


==> definitions/installation-process/def.tex <==
A process aiming to make a \DefinitionName{system}{ls} operational, 
i.e.\ to implement the use of the \DefinitionName{system}{ls} by its 
prospective users.


==> definitions/installation-process/lp.tex <==
installation processes%


==> definitions/installation-process/ls.tex <==
installation process%


==> definitions/installation-process/up.tex <==
Installation processes%


==> definitions/installation-process/us.tex <==
Installation process%


==> definitions/interest/def.tex <==
The specific reason(s) why a \DefinitionName{viewer}{ls} observes a 
\DefinitionName{domain}{ls}. In the case of a 
\DefinitionName{system}{ls}, this this is usually a confluence of the 
\DefinitionName{systemic-property}{lp} of \DefinitionName{interest}{ls} 
to the \DefinitionName{system-viewer}{ls} and the aspects of the 
\DefinitionName{system}{ls} that are considered relevant (by the 
\DefinitionName{system-viewer}{ls} to these 
\DefinitionName{systemic-property}{lp}).


==> definitions/interest/lp.tex <==
interests%


==> definitions/interest/ls.tex <==
interest%


==> definitions/interest/up.tex <==
Interests%


==> definitions/interest/us.tex <==
Interest%


==> definitions/knowledge/lp.tex <==
knowledge%


==> definitions/knowledge/ls.tex <==
knowledge%


==> definitions/knowledge/up.tex <==
Knowledge%


==> definitions/knowledge/us.tex <==
Knowledge%


==> definitions/linear-approach/def.tex <==
Step by step execution of a (part of a) development process, where a 
consecutive step is not executed until the preceding step is finished.


==> definitions/linear-approach/lp.tex <==
linear approaches%


==> definitions/linear-approach/ls.tex <==
linear approach%


==> definitions/linear-approach/up.tex <==
Linear approaches%


==> definitions/linear-approach/us.tex <==
Linear approach%


==> definitions/link/def.tex <==
Any \DefinitionName{element}{ls} from a \DefinitionName{conception}{ls} 
that relates two \DefinitionName{concept}{lp}.


==> definitions/link/lp.tex <==
links%


==> definitions/link/ls.tex <==
link%


==> definitions/link/up.tex <==
Links%


==> definitions/link/us.tex <==
Link%


==> definitions/lisa-d/def.tex <==
Language for \DefinitionName{information}{us} Structure and Access 
\DefinitionName{description}{up}. \DefinitionName{lisa-d}{us} has also 
a symbolic interpretation. In George Bernard Shaw's 'Pygmalion', 
professor Higgins, a linguistics prof, transforms Eliza Doolittle into 
a lady, speaking her language very well, though a bit 'robotic'.


==> definitions/lisa-d/lp.tex <==
Lisa-D%


==> definitions/lisa-d/ls.tex <==
Lisa-D%


==> definitions/lisa-d/up.tex <==
Lisa-D%


==> definitions/lisa-d/us.tex <==
Lisa-D%


==> definitions/maintainability/def.tex <==
Bears on the effort needed to make specified modifications to the 
\DefinitionName{system}{ls} (or a \DefinitionName{sub-system}{ls}). 
Modification may include corrections, improvements or adaptation to 
changes in the \DefinitionName{environment}{ls}, the 
\DefinitionName{requirement}{lp} and the (higher levels of the) 
\DefinitionName{design}{ls}. Sub-characteristics of 
\DefinitionName{maintainability}{ls} are: analysability, changeability, 
stability, testability, manageability, re\DefinitionName{usability}{ls}.


==> definitions/maintainability/lp.tex <==
maintainabilities%


==> definitions/maintainability/ls.tex <==
maintainability%


==> definitions/maintainability/up.tex <==
Maintainabilities%


==> definitions/maintainability/us.tex <==
Maintainability%


==> definitions/maintenance/def.tex <==
An \DefinitionName{information-system}{ls} which is operational in its 
usage context, does not remain operational by itself. Both technical 
and non-technical \DefinitionName{element}{lp} of the 
\DefinitionName{system}{ls} need active 
\DefinitionName{maintenance}{ls} to keep the 
\DefinitionName{information-system}{ls} operational as is.


==> definitions/maintenance/lp.tex <==
maintenance%


==> definitions/maintenance/ls.tex <==
maintenance%


==> definitions/maintenance/up.tex <==
Maintenance%


==> definitions/maintenance/us.tex <==
Maintenance%


==> definitions/message/def.tex <==
\DefinitionName{data}{us} that is transmitted from one 
\DefinitionName{actor}{ls} (the sender) to another 
\DefinitionName{actor}{ls} (the receiver). A 
\DefinitionName{message}{ls} may actually be `routed' via several 
\DefinitionName{actor}{lp} before reaching its actual receiver. For 
example, when \DefinitionName{human-actor}{ls} exchange 
\DefinitionName{message}{lp}, they usually need to make use of some 
other \DefinitionName{actor}{ls} playing the role of a medium (for 
example, vibrations in the air, or an e-mail 
\DefinitionName{system}{ls}).


==> definitions/message/lp.tex <==
messages%


==> definitions/message/ls.tex <==
message%


==> definitions/message/up.tex <==
Messages%


==> definitions/message/us.tex <==
Message%


==> definitions/meta-model/def.tex <==
A \DefinitionName{conception}{ls} of a \DefinitionName{viewer}{ls}'s 
\DefinitionName{viewpoint}{ls} on the world.


==> definitions/meta-model/lp.tex <==
meta models%


==> definitions/meta-model/ls.tex <==
meta model%


==> definitions/meta-model/up.tex <==
Meta models%


==> definitions/meta-model/us.tex <==
Meta model%


==> definitions/method-fragment/def.tex <==
An identifiable part of methodical \DefinitionName{knowledge}{ls}.


==> definitions/method-fragment/lp.tex <==
method fragments%


==> definitions/method-fragment/ls.tex <==
method fragment%


==> definitions/method-fragment/up.tex <==
Method fragments%


==> definitions/method-fragment/us.tex <==
Method fragment%


==> definitions/method/def.tex <==
An integrated combination of a:
 \DefinitionName{way-of-thinking}{ls},
 \DefinitionName{way-of-controlling}{ls},
 \DefinitionName{way-of-working}{ls},
 \DefinitionName{way-of-modeling}{ls} (a 
\DefinitionName{technique}{ls}),
 and a \DefinitionName{way-of-supporting}{ls} aimed at obtaining 
results.
 


==> definitions/method/lp.tex <==
methods%


==> definitions/method/ls.tex <==
method%


==> definitions/method/up.tex <==
Methods%


==> definitions/method/us.tex <==
Method%


==> definitions/model-builder/def.tex <==
The person involved in the formal dialog with the 
\DefinitionName{modeling-mediator}{ls}, processing the semi-formal 
specifications provided by the \DefinitionName{modeling-mediator}{ls}. 
The combination of \DefinitionName{modeling-mediator}{ls} and 
\DefinitionName{model-builder}{ls} is also referred to as 
\DefinitionName{system-analyst}{ls}.


==> definitions/model-builder/lp.tex <==
model builders%


==> definitions/model-builder/ls.tex <==
model builder%


==> definitions/model-builder/up.tex <==
Model builders%


==> definitions/model-builder/us.tex <==
Model builder%


==> definitions/model-concept/def.tex <==
A \DefinitionName{concept}{ls} from a \DefinitionName{conception}{ls} 
which is a \DefinitionName{model}{ls}.


==> definitions/model-concept/lp.tex <==
model concepts%


==> definitions/model-concept/ls.tex <==
model concept%


==> definitions/model-concept/up.tex <==
Model concepts%


==> definitions/model-concept/us.tex <==
Model concept%


==> definitions/model-element/def.tex <==
An \DefinitionName{element}{ls} from a \DefinitionName{conception}{ls} 
which is a \DefinitionName{model}{ls}.


==> definitions/model-element/lp.tex <==
model elements%


==> definitions/model-element/ls.tex <==
model element%


==> definitions/model-element/up.tex <==
Model elements%


==> definitions/model-element/us.tex <==
Model element%


==> definitions/model-link/def.tex <==
A \DefinitionName{link}{ls} from a \DefinitionName{conception}{ls} 
which is a \DefinitionName{model}{ls}.


==> definitions/model-link/lp.tex <==
model links%


==> definitions/model-link/ls.tex <==
model link%


==> definitions/model-link/up.tex <==
Model links%


==> definitions/model-link/us.tex <==
Model link%


==> definitions/model-relation-type/def.tex <==
A type of well-defined relations between \DefinitionName{model}{lp}. An 
example would be a
 mapping algorithm between a conceptual \DefinitionName{model}{ls} and 
a relational database schema,
 the relation between the \DefinitionName{concept}{lp} of a business 
process \DefinitionName{model}{ls} and the concepts
 of a supporting work-flow, etc.


==> definitions/model-relation-type/lp.tex <==
model relation types%


==> definitions/model-relation-type/ls.tex <==
model relation type%


==> definitions/model-relation-type/up.tex <==
Model relation types%


==> definitions/model-relation-type/us.tex <==
Model relation type%


==> definitions/model/def.tex <==
A purposely abstracted \DefinitionName{domain}{ls} (possibly in 
conjunction with its \DefinitionName{environment}{ls}) of some `part' 
or `aspect' of the \DefinitionName{universe}{ls} a 
\DefinitionName{viewer}{ls} may have an \DefinitionName{interest}{ls} 
in. For practical reasons, a \DefinitionName{model}{ls} will typically 
be consistent and unambiguous with regards to some underlying 
semantical \DefinitionName{domain}{ls}, such as logic.


==> definitions/model/lp.tex <==
models%


==> definitions/model/ls.tex <==
model%


==> definitions/model/up.tex <==
Models%


==> definitions/model/us.tex <==
Model%


==> definitions/modeling-fragment/def.tex <==
A \DefinitionName{method-fragment}{ls} that is concerned with the 
actual \DefinitionName{modeling}{ls} of a
 \DefinitionName{domain}{ls}. Three classes of 
\DefinitionName{method-fragment}{lp} are identified:
 \DefinitionName{viewing-framework}{ls}, 
\DefinitionName{way-of-working}{ls}, \DefinitionName{viewpoint}{ls},
 \DefinitionName{model-relation-type}{ls}. Each 
\DefinitionName{method-fragment}{ls} must have a unique
 underlying \DefinitionName{way-of-thinking}{ls}.


==> definitions/modeling-fragment/lp.tex <==
modeling fragments%


==> definitions/modeling-fragment/ls.tex <==
modeling fragment%


==> definitions/modeling-fragment/up.tex <==
Modeling fragments%


==> definitions/modeling-fragment/us.tex <==
Modeling fragment%


==> definitions/modeling-mediator/def.tex <==
The person involved in the informal dialog with the 
\DefinitionName{domain-expert}{ls}, mediating between the 
\DefinitionName{domain-expert}{ls} and the 
\DefinitionName{model-builder}{ls}. The combination of 
\DefinitionName{modeling-mediator}{ls} and 
\DefinitionName{model-builder}{ls} is also referred to as 
\DefinitionName{system-analyst}{ls}.


==> definitions/modeling-mediator/lp.tex <==
modeling mediators%


==> definitions/modeling-mediator/ls.tex <==
modeling mediator%


==> definitions/modeling-mediator/up.tex <==
Modeling mediators%


==> definitions/modeling-mediator/us.tex <==
Modeling mediator%


==> definitions/modeling-technique/def.tex <==
The combination of a \DefinitionName{way-of-modeling}{ls} and a 
\DefinitionName{way-of-communicating}{ls}.


==> definitions/modeling-technique/lp.tex <==
modeling techniques%


==> definitions/modeling-technique/ls.tex <==
modeling technique%


==> definitions/modeling-technique/up.tex <==
Modeling techniques%


==> definitions/modeling-technique/us.tex <==
Modeling technique%


==> definitions/modeling/def.tex <==
The act of purposely abstracting a \DefinitionName{model}{ls} from 
(what is conceived to be) a part of the \DefinitionName{universe}{ls}.


==> definitions/modeling/lp.tex <==
modeling%


==> definitions/modeling/ls.tex <==
modeling%


==> definitions/modeling/up.tex <==
Modeling%


==> definitions/modeling/us.tex <==
Modeling%


==> definitions/new <==
#!/bin/bash
echo -n "lower case singular name: "
read LS

function Upper () {
  echo -n $1 | sed -e "s/^./&##/" | sed -e "s/##.*//" | tr [:lower:] [:upper:]
  echo $1 | sed -e "s/^.//"
}

KEY="`echo $LS | sed -e "s/ /-/g"`"
LP="`echo "$LS"s \
     | sed -e "s/cys/cy/"    \
     | sed -e "s/ings$/ing/" \
     | sed -e "s/chs$/ches/" \
     | sed -e "s/sss$/sses/" \
     | sed -e "s/tys$/ties/" \
     | cat`"
US="`Upper "$LS"`"
UP="`Upper "$LP"`"

echo "key                     : [$KEY]"
echo "lower case singular name: [$LS]"
echo "lower case plural   name: [$LP]"
echo "upper case singular name: [$US]"
echo "upper case plural   name: [$UP]"

mkdir $KEY
echo $LS% > $KEY/ls.tex
echo $LP% > $KEY/lp.tex
echo $US% > $KEY/us.tex
echo $UP% > $KEY/up.tex
vi $KEY/def.tex


==> definitions/niam/def.tex <==
aN \DefinitionName{information}{us} Analysis \DefinitionName{method}{us}


==> definitions/niam/lp.tex <==
NIAM%


==> definitions/niam/ls.tex <==
NIAM%


==> definitions/niam/up.tex <==
NIAM%


==> definitions/niam/us.tex <==
NIAM%


==> definitions/non-functional-requirement/def.tex <==
A \DefinitionName{requirement}{ls} which is not a 
\DefinitionName{functional-requirement}{ls}.


==> definitions/non-functional-requirement/lp.tex <==
non-functional requirements%


==> definitions/non-functional-requirement/ls.tex <==
non-functional requirement%


==> definitions/non-functional-requirement/up.tex <==
Non-functional requirements%


==> definitions/non-functional-requirement/us.tex <==
Non-functional requirement%


==> definitions/ockhams-razor/def.tex <==
The simplest explanation is usually the best.


==> definitions/ockhams-razor/lp.tex <==
Ockham's Razor%


==> definitions/ockhams-razor/ls.tex <==
Ockham's Razor%


==> definitions/ockhams-razor/up.tex <==
Ockham's Razor%


==> definitions/ockhams-razor/us.tex <==
Ockham's Razor%


==> definitions/ontology/def.tex <==
The subject of \DefinitionName{ontology}{ls} is the study of the 
categories of things that exist or may exist in some 
\DefinitionName{domain}{ls}. The product of such a study, called an 
\DefinitionName{ontology}{ls}, is a catalog of the types of things that 
are assumed to exist in a \DefinitionName{domain}{ls} of 
\DefinitionName{interest}{ls} $D$ from the 
\DefinitionName{perspective}{ls} of a person who uses a language $L$ 
for the purpose of talking about $D$. The types in the 
\DefinitionName{ontology}{ls} represent the predicates, word senses, or 
\DefinitionName{concept}{ls} and relation types of the language $L$ 
when used to discuss topics in the \DefinitionName{domain}{ls} $D$.


==> definitions/ontology/lp.tex <==
ontologies%


==> definitions/ontology/ls.tex <==
ontology%


==> definitions/ontology/up.tex <==
Ontologies%


==> definitions/ontology/us.tex <==
Ontology%


==> definitions/open-active-system/def.tex <==
A \DefinitionName{system}{ls} that is an 
\DefinitionName{open-system}{ls} as well as an 
\DefinitionName{active-system}{ls}.


==> definitions/open-active-system/lp.tex <==
open active systems%


==> definitions/open-active-system/ls.tex <==
open active system%


==> definitions/open-active-system/up.tex <==
Open active systems%


==> definitions/open-active-system/us.tex <==
Open active system%


==> definitions/open-system/def.tex <==
A special kind of \DefinitionName{dynamic-system}{ls} that is conceived 
as reacting to external triggers, i.e.\ there may be changes inside the 
\DefinitionName{system}{ls} due to external causes originating from the 
\DefinitionName{system}{ls}'s \DefinitionName{environment}{ls}.


==> definitions/open-system/lp.tex <==
open systems%


==> definitions/open-system/ls.tex <==
open system%


==> definitions/open-system/up.tex <==
Open systems%


==> definitions/open-system/us.tex <==
Open system%


==> definitions/organization/def.tex <==
A group of \DefinitionName{actor}{lp} with a purpose, who:
\begin{itemize}

\item interact with each other,
\item form a network of roles,
\item make use of (the services of) other \DefinitionName{actor}{lp}.
\end{itemize}
An \DefinitionName{organization}{ls} in itself is an 
\DefinitionName{actor}{ls} as well, and may as such participate in yet 
another \DefinitionName{organization}{lp}.


==> definitions/organization/lp.tex <==
organizations%


==> definitions/organization/ls.tex <==
organization%


==> definitions/organization/up.tex <==
Organizations%


==> definitions/organization/us.tex <==
Organization%


==> definitions/organizational-system/def.tex <==
A special kind of \DefinitionName{work-system}{ls}, being normally 
active and open, and comprising the \DefinitionName{conception}{ls} of 
how an \DefinitionName{organization}{ls} is composed and how it 
operates (i.e.\ performing specific actions in pursuit of 
organizational \DefinitionName{goal}{lp}, guided by organizational 
rules and informed by internal and external 
\DefinitionName{communication}{ls}), where its 
\DefinitionName{systemic-property}{ls} are that it responds to (certain 
kinds of) changes caused by the \DefinitionName{system}{ls} 
\DefinitionName{environment}{ls} and, itself, causes (certain kinds of) 
changes in the \DefinitionName{system}{ls} 
\DefinitionName{environment}{ls}.


==> definitions/organizational-system/lp.tex <==
organizational systems%


==> definitions/organizational-system/ls.tex <==
organizational system%


==> definitions/organizational-system/up.tex <==
Organizational systems%


==> definitions/organizational-system/us.tex <==
Organizational system%


==> definitions/orm/def.tex <==
Object-Role \DefinitionName{modeling}{us}


==> definitions/orm/lp.tex <==
ORM%


==> definitions/orm/ls.tex <==
ORM%


==> definitions/orm/up.tex <==
ORM%


==> definitions/orm/us.tex <==
ORM%


==> definitions/ornf/def.tex <==
Object Role Normalform, a \DefinitionName{controlled-language}{ls} 
developed in the context of object-role \DefinitionName{modeling}{ls}.


==> definitions/ornf/lp.tex <==
ORNF%


==> definitions/ornf/ls.tex <==
ORNF%


==> definitions/ornf/up.tex <==
ORNF%


==> definitions/ornf/us.tex <==
ORNF%


==> definitions/patiens/def.tex <==
The role in a sentence that most commonly is associated with the 
grammatical object.


==> definitions/patiens/lp.tex <==
patiens%


==> definitions/patiens/ls.tex <==
patiens%


==> definitions/patiens/up.tex <==
Patiens%


==> definitions/patiens/us.tex <==
Patiens%


==> definitions/perception/def.tex <==
That what results, in the mind of a \DefinitionName{viewer}{ls}, when 
they observe a \DefinitionName{domain}{ls} with their senses, and forms 
a specific pattern of visual, auditory or other sensations in their 
minds.


==> definitions/perception/lp.tex <==
perceptions%


==> definitions/perception/ls.tex <==
perception%


==> definitions/perception/up.tex <==
Perceptions%


==> definitions/perception/us.tex <==
Perception%


==> definitions/perspective/def.tex <==
A set of related \DefinitionName{interest}{lp} in terms of which 
\DefinitionName{viewer}{lp} may observe a \DefinitionName{domain}{ls}.


==> definitions/perspective/lp.tex <==
perspectives%


==> definitions/perspective/ls.tex <==
perspective%


==> definitions/perspective/up.tex <==
Perspectives%


==> definitions/perspective/us.tex <==
Perspective%


==> definitions/portability/def.tex <==
Is the ability of the \DefinitionName{system}{ls} (or one of its 
\DefinitionName{component}{lp}) to be transferred from one 
\DefinitionName{environment}{ls} to another. Sub-characteristics of 
\DefinitionName{portability}{ls} are: adaptability, installability, 
conformance, replaceability.


==> definitions/portability/lp.tex <==
portabilities%


==> definitions/portability/ls.tex <==
portability%


==> definitions/portability/up.tex <==
Portabilities%


==> definitions/portability/us.tex <==
Portability%


==> definitions/process-requirement/def.tex <==
A \DefinitionName{requirement}{ls} pertaining to the actual 
\DefinitionName{system-engineering}{ls} \emph{process}.


==> definitions/process-requirement/lp.tex <==
process requirements%


==> definitions/process-requirement/ls.tex <==
process requirement%


==> definitions/process-requirement/up.tex <==
Process requirements%


==> definitions/process-requirement/us.tex <==
Process requirement%


==> definitions/product-requirement/def.tex <==
A \DefinitionName{requirement}{ls} on any of the products, pertaining 
to a \DefinitionName{system}{ls} as it will eventually result from a 
\DefinitionName{system-engineering}{ls} process.


==> definitions/product-requirement/lp.tex <==
product requirements%


==> definitions/product-requirement/ls.tex <==
product requirement%


==> definitions/product-requirement/up.tex <==
Product requirements%


==> definitions/product-requirement/us.tex <==
Product requirement%


==> definitions/psm/def.tex <==
Predicator Set \DefinitionName{model}{us}


==> definitions/psm/lp.tex <==
PSM%


==> definitions/psm/ls.tex <==
PSM%


==> definitions/psm/up.tex <==
PSM%


==> definitions/psm/us.tex <==
PSM%


==> definitions/quality-attribute/def.tex <==
A specific class of \DefinitionName{quality-property}{lp}.


==> definitions/quality-attribute/lp.tex <==
quality attributes%


==> definitions/quality-attribute/up.tex <==
Quality attributes%


==> definitions/quality-attribute/us.tex <==
Quality attribute%


==> definitions/quality-property/def.tex <==
A \DefinitionName{systemic-property}{ls}, used to describe and asses 
the \DefinitionName{quality}{ls} of a \DefinitionName{system}{ls}.


==> definitions/quality-property/lp.tex <==
quality properties%


==> definitions/quality-property/ls.tex <==
quality property%


==> definitions/quality-property/up.tex <==
Quality properties%


==> definitions/quality-property/us.tex <==
Quality property%


==> definitions/quality/def.tex <==
Is the totality of \DefinitionName{systemic-property}{lp} of a 
\DefinitionName{system}{ls} that relate to its ability to satisfy 
stated and/or implied needs.


==> definitions/quality/lp.tex <==
qualities%


==> definitions/quality/ls.tex <==
quality%


==> definitions/quality/up.tex <==
Qualities%


==> definitions/quality/us.tex <==
Quality%


==> definitions/reactive-system/def.tex <==
An \DefinitionName{open-active-system}{ls} where each expression of the 
\DefinitionName{system}{ls} is a reaction, and where each impression 
immediately causes a reaction.


==> definitions/reactive-system/lp.tex <==
reactive systems%


==> definitions/reactive-system/ls.tex <==
reactive system%


==> definitions/reactive-system/up.tex <==
Reactive systems%


==> definitions/reactive-system/us.tex <==
Reactive system%


==> definitions/realization-process/lp.tex <==
realization processes%


==> definitions/realization-process/ls.tex <==
realization process%


==> definitions/realization-process/up.tex <==
Realization processes%


==> definitions/realization-process/us.tex <==
Realization process%


==> definitions/reliability/def.tex <==
Is the capability of the \DefinitionName{system}{ls} (or a 
\DefinitionName{sub-system}{ls}) to maintain its level of performance 
under stated conditions for a stated period of time. The mean time to 
failure metric is often used to assess \DefinitionName{reliability}{ls} 
of \DefinitionName{system}{lp}. The \DefinitionName{reliability}{ls} 
can be determined through defining the level of protection against 
failures and the necessary measures for recovery from failures. 
Sub-characteristics of \DefinitionName{reliability}{ls} are: maturity, 
fault tolerance, recoverability, availability and degradability.


==> definitions/reliability/lp.tex <==
reliabilities%


==> definitions/reliability/ls.tex <==
reliability%


==> definitions/reliability/up.tex <==
Reliabilities%


==> definitions/reliability/us.tex <==
Reliability%


==> definitions/representation/def.tex <==
The result of a \DefinitionName{viewer}{ls} denoting a 
\DefinitionName{conception}{ls}, using some language and medium to 
express themselves.


==> definitions/representation/lp.tex <==
representations%


==> definitions/representation/ls.tex <==
representation%


==> definitions/representation/up.tex <==
Representations%


==> definitions/representation/us.tex <==
Representation%


==> definitions/requirement/def.tex <==
an essential \DefinitionName{quality-property}{ls} that a 
\DefinitionName{system}{ls} or its 
\DefinitionName{system-description}{ls} has to satisfy.


==> definitions/requirement/lp.tex <==
requirements%


==> definitions/requirement/ls.tex <==
requirement%


==> definitions/requirement/up.tex <==
Requirements%


==> definitions/requirement/us.tex <==
Requirement%


==> definitions/responsive-system/def.tex <==
An \DefinitionName{open-active-system}{ls} (possibly also a 
\DefinitionName{reactive-system}{ls}) where it holds for at least one 
expression that a certain impression or a temporal pattern of 
impressions is a necessary, but not a sufficient dynamic condition for 
its occurrence. The receipt of an order is a necessary impression to a 
``sales \DefinitionName{system}{ls}'', for the expression ``delivery of 
the ordered goods", but it is not a sufficient condition.


==> definitions/responsive-system/lp.tex <==
responsive systems%


==> definitions/responsive-system/ls.tex <==
responsive system%


==> definitions/responsive-system/up.tex <==
Responsive systems%


==> definitions/responsive-system/us.tex <==
Responsive system%


==> definitions/ridl/def.tex <==
Reference and IDea Language


==> definitions/ridl/lp.tex <==
RIDL%


==> definitions/ridl/ls.tex <==
RIDL%


==> definitions/ridl/up.tex <==
RIDL%


==> definitions/ridl/us.tex <==
RIDL%


==> definitions/run-time-requirement/def.tex <==
A \DefinitionName{product-requirement}{ls} on a 
\DefinitionName{system}{ls} as it will eventually result from a 
\DefinitionName{system-engineering}{ls} process. These 
\DefinitionName{requirement}{lp} usually refer to 
\DefinitionName{quality-attribute}{lp} such as: 
\DefinitionName{functionality}{ls}, \DefinitionName{usability}{ls}, 
\DefinitionName{efficiency}{ls} and \DefinitionName{reliability}{ls}. 
Note that these \DefinitionName{requirement}{lp} are observable as 
\DefinitionName{systemic-property}{lp} of the 
\DefinitionName{system}{ls} resulting from the development process.


==> definitions/run-time-requirement/lp.tex <==
run-time requirements%


==> definitions/run-time-requirement/ls.tex <==
run-time requirement%


==> definitions/run-time-requirement/up.tex <==
Run-time requirements%


==> definitions/run-time-requirement/us.tex <==
Run-time requirement%


==> definitions/shadow-world/def.tex <==
A (usually formal) world that keeps track of the wheeling and reeling 
in the \DefinitionName{uod}{ls}.


==> definitions/shadow-world/lp.tex <==
shadow worlds%


==> definitions/shadow-world/ls.tex <==
shadow world%


==> definitions/shadow-world/up.tex <==
Shadow worlds%


==> definitions/shadow-world/us.tex <==
Shadow world%


==> definitions/simulation/def.tex <==
The imitative \DefinitionName{representation}{ls} of the functioning of 
one \DefinitionName{system}{ls} by means of the functioning of another.


==> definitions/simulation/lp.tex <==
simulations%


==> definitions/simulation/ls.tex <==
simulation%


==> definitions/simulation/up.tex <==
Simulations%


==> definitions/simulation/us.tex <==
Simulation%


==> definitions/sql/def.tex <==
Structured Query Language


==> definitions/sql/lp.tex <==
SQL%


==> definitions/sql/ls.tex <==
SQL%


==> definitions/sql/up.tex <==
SQL%


==> definitions/sql/us.tex <==
SQL%


==> definitions/stakeholder-concern/def.tex <==
An \DefinitionName{interest}{ls} of a \DefinitionName{stakeholder}{ls}, 
resulting from the \DefinitionName{stakeholder}{ls}'s 
\DefinitionName{goal}{ls}, and the role played by some 
\DefinitionName{system}{ls}. This usually pertains to the 
\DefinitionName{system}{ls}'s engineering, its operation or any other 
aspects that are critical or otherwise important to one or more 
\DefinitionName{stakeholder}{lp}.


==> definitions/stakeholder-concern/lp.tex <==
stakeholder concerns%


==> definitions/stakeholder-concern/ls.tex <==
stakeholder concern%


==> definitions/stakeholder-concern/up.tex <==
Stakeholder concerns%


==> definitions/stakeholder-concern/us.tex <==
Stakeholder concern%


==> definitions/stakeholder-goal/def.tex <==
The end toward which effort is directed by a 
\DefinitionName{stakeholder}{ls}, in which the 
\DefinitionName{system}{ls} (of which the 
\DefinitionName{stakeholder}{ls} is indeed a 
\DefinitionName{stakeholder}{ls}) plays a role. This may pertain to 
strategic, tactical or operational end. The role of the 
\DefinitionName{system}{ls} may range from passive to active. For 
example, a financial controller's \DefinitionName{goal}{ls} with 
regards to a future/changed \DefinitionName{system}{ls} may be to 
control \DefinitionName{system-engineering}{ls} costs, while the 
\DefinitionName{goal}{ls} of users of the \DefinitionName{system}{ls} 
may be to get their job done more efficiently.


==> definitions/stakeholder-goal/lp.tex <==
stakeholder goals%


==> definitions/stakeholder-goal/ls.tex <==
stakeholder goal%


==> definitions/stakeholder-goal/up.tex <==
Stakeholder goals%


==> definitions/stakeholder-goal/us.tex <==
Stakeholder goal%


==> definitions/stakeholder-requirement/def.tex <==
A \DefinitionName{requirement}{ls} posed on a future/changed 
\DefinitionName{system}{ls} by a specific 
\DefinitionName{stakeholder}{ls}. These 
\DefinitionName{requirement}{lp} should essentially be refinements of 
the \DefinitionName{stakeholder-concern}{lp}.


==> definitions/stakeholder-requirement/lp.tex <==
stakeholder requirements%


==> definitions/stakeholder-requirement/ls.tex <==
stakeholder requirement%


==> definitions/stakeholder-requirement/up.tex <==
Stakeholder requirements%


==> definitions/stakeholder-requirement/us.tex <==
Stakeholder requirement%


==> definitions/stakeholder-requirements-description/def.tex <==
A \DefinitionName{system-description}{ls} of the 
\DefinitionName{stakeholder-requirement}{lp} on a future/changed 
\DefinitionName{system}{ls} $S$, which covers:
\begin{itemize}

\item the \DefinitionName{requirement}{lp} which will be imposed by the 
\DefinitionName{environment}{ls} on \DefinitionName{system}{ls} $S$ and
\item the \DefinitionName{requirement}{lp} on other 
\DefinitionName{system}{lp} in the \DefinitionName{environment}{ls} of 
\DefinitionName{system}{ls} $S$ which \DefinitionName{system}{ls} $S$ 
may/must use for its own purposes. For example: the properties of a 
given infrastructure that must/may be used, `legacy' 
\DefinitionName{system}{lp} with which $S$ needs to interface, etc.
\end{itemize}
The gap between these sets of \DefinitionName{requirement}{lp}, is what 
needs to be `designed in' by the \DefinitionName{design-process}{ls}.


==> definitions/stakeholder-requirements-description/lp.tex <==
stakeholder requirements descriptions%


==> definitions/stakeholder-requirements-description/ls.tex <==
stakeholder requirements description%


==> definitions/stakeholder-requirements-description/up.tex <==
Stakeholder requirements descriptions%


==> definitions/stakeholder-requirements-description/us.tex <==
Stakeholder requirements description%


==> definitions/stakeholder/def.tex <==
A party (a \DefinitionName{system-viewer}{ls}) with a specific 
\DefinitionName{interest}{ls} pertaining to a 
\DefinitionName{system}{ls}'s development, its operation or any other 
aspects that are critical or otherwise important. Examples are: Users, 
operators, owners, architects, engineers, testers, project managers, 
business management, ...


==> definitions/stakeholder/lp.tex <==
stakeholders%


==> definitions/stakeholder/ls.tex <==
stakeholder%


==> definitions/stakeholder/up.tex <==
Stakeholders%


==> definitions/stakeholder/us.tex <==
Stakeholder%


==> definitions/standard-name/def.tex <==
An agreed standard denotation for objects and things.


==> definitions/standard-name/lp.tex <==
standard names%


==> definitions/standard-name/ls.tex <==
standard name%


==> definitions/standard-name/up.tex <==
Standard names%


==> definitions/standard-name/us.tex <==
standard names%


==> definitions/strong-identification/def.tex <==
A sufficient condition to be able to uniquely identify objects and 
things, stating each object has a \DefinitionName{standard-name}{ls} 
derived from the associated object type.


==> definitions/strong-identification/lp.tex <==
strong identification%


==> definitions/strong-identification/ls.tex <==
strong identification%


==> definitions/strong-identification/up.tex <==
Strong identification%


==> definitions/strong-identification/us.tex <==
Strong identification%


==> definitions/sub-system/def.tex <==
A \DefinitionName{sub-system}{ls} $S'$ of a \DefinitionName{system}{ls} 
$S$, is a \DefinitionName{system}{ls} where the set of 
\DefinitionName{element}{lp} in $S'$ is a subset of the 
\DefinitionName{element}{lp} in $S$.


==> definitions/sub-system/lp.tex <==
sub-systems%


==> definitions/sub-system/ls.tex <==
sub-system%


==> definitions/sub-system/up.tex <==
Sub-systems%


==> definitions/sub-system/us.tex <==
Sub-system%


==> definitions/system-activity/def.tex <==
A \DefinitionName{system-concept}{ls} that is conceived of as changing 
parts of the \DefinitionName{universe}{ls}.


==> definitions/system-activity/lp.tex <==
system activities%


==> definitions/system-activity/ls.tex <==
system activity%


==> definitions/system-activity/up.tex <==
System activities%


==> definitions/system-activity/us.tex <==
System activity%


==> definitions/system-analyst/def.tex <==
A person constructing a \DefinitionName{model}{ls} of a 
\DefinitionName{uod}{ls} from a semi-formal specification. Also 
referred as \DefinitionName{model-builder}{ls}.


==> definitions/system-analyst/lp.tex <==
system analysts%


==> definitions/system-analyst/ls.tex <==
system analyst%


==> definitions/system-analyst/up.tex <==
System analysts%


==> definitions/system-analyst/us.tex <==
System analyst%


==> definitions/system-builder/def.tex <==
A person constructing a \DefinitionName{model}{ls} of a 
\DefinitionName{uod}{ls} from a semi-formal specification. Also 
referred to as \DefinitionName{system-analyst}{ls}.


==> definitions/system-builder/lp.tex <==
system builders%


==> definitions/system-builder/ls.tex <==
system builder%


==> definitions/system-builder/up.tex <==
System builder%


==> definitions/system-builder/us.tex <==
System builder%


==> definitions/system-concept/def.tex <==
Any \DefinitionName{element}{ls} from a \DefinitionName{system}{ls} 
that is a \DefinitionName{concept}{ls}.


==> definitions/system-concept/lp.tex <==
system concepts%


==> definitions/system-concept/ls.tex <==
system concept%


==> definitions/system-concept/up.tex <==
System concepts%


==> definitions/system-concept/us.tex <==
System concept%


==> definitions/system-description/def.tex <==
The \DefinitionName{description}{ls} of a \DefinitionName{system}{ls}.


==> definitions/system-description/lp.tex <==
system descriptions%


==> definitions/system-description/ls.tex <==
system description%


==> definitions/system-description/up.tex <==
System descriptions%


==> definitions/system-description/us.tex <==
System description%


==> definitions/system-design/def.tex <==
To do


==> definitions/system-design/lp.tex <==
system designs%


==> definitions/system-design/ls.tex <==
system design%


==> definitions/system-design/up.tex <==
System designs%


==> definitions/system-design/us.tex <==
System design%


==> definitions/system-development-community/def.tex <==
A group of objects, such as \DefinitionName{actor}{lp} and 
\DefinitionName{representation}{lp}, which are involved in the 
development of a \DefinitionName{system}{ls}.


==> definitions/system-development-community/lp.tex <==
system development communities%


==> definitions/system-development-community/ls.tex <==
system development community%


==> definitions/system-development-community/up.tex <==
System development communities%


==> definitions/system-development-community/us.tex <==
System development community%


==> definitions/system-development/def.tex <==
To be done


==> definitions/system-development/lp.tex <==
system developments%


==> definitions/system-development/ls.tex <==
system development%


==> definitions/system-development/up.tex <==
System developments%


==> definitions/system-development/us.tex <==
System development%


==> definitions/system-domain/def.tex <==
A \DefinitionName{domain}{ls} that is conceived to be a 
\DefinitionName{system}{ls}, by some \DefinitionName{viewer}{ls}, by 
the distinction from its \DefinitionName{environment}{ls}, by its 
coherence, and because of its \DefinitionName{systemic-property}{ls}.


==> definitions/system-domain/lp.tex <==
system domains%


==> definitions/system-domain/ls.tex <==
system domain%


==> definitions/system-domain/up.tex <==
System domains%


==> definitions/system-domain/us.tex <==
System domain%


==> definitions/system-element/def.tex <==
Any \DefinitionName{element}{ls} from a \DefinitionName{system}{ls}.


==> definitions/system-element/lp.tex <==
system elements%


==> definitions/system-element/ls.tex <==
system element%


==> definitions/system-element/up.tex <==
System elements%


==> definitions/system-element/us.tex <==
System element%


==> definitions/system-engineering-community/def.tex <==
A group of objects, such as \DefinitionName{actor}{lp} and 
\DefinitionName{representation}{lp}, which are involved in a 
\DefinitionName{system-engineering}{ls} process.


==> definitions/system-engineering-community/lp.tex <==
system engineering communities%


==> definitions/system-engineering-community/ls.tex <==
system engineering community%


==> definitions/system-engineering-community/up.tex <==
System engineering communities%


==> definitions/system-engineering-community/us.tex <==
System engineering community%


==> definitions/system-engineering/def.tex <==
A process aimed at producing a changed \DefinitionName{system}{ls}, 
involving the execution of four sub-processes: 
\DO{definition-process}{definition}, \DO{design-process}{design}, 
\DO{construction-process}{construction} and 
\DO{deployment-process}{deployment}. Processes that may be executed 
sequentially, incrementally, interleaved, or in parallel.


==> definitions/system-engineering/lp.tex <==
system engineering%


==> definitions/system-engineering/ls.tex <==
system engineering%


==> definitions/system-engineering/up.tex <==
System engineering%


==> definitions/system-engineering/us.tex <==
System engineering%


==> definitions/system-evolution/def.tex <==
The evolution, over time, of a \DefinitionName{system}{ls}.


==> definitions/system-evolution/lp.tex <==
system evolutions%


==> definitions/system-evolution/ls.tex <==
system evolution%


==> definitions/system-evolution/up.tex <==
System evolutions%


==> definitions/system-evolution/us.tex <==
System evolution%


==> definitions/system-exposition/def.tex <==
a \DefinitionName{description}{ls} of all the 
\DefinitionName{element}{lp} of the \DefinitionName{system-domain}{ls} 
where each \DefinitionName{element}{ls} is specified by all its 
relevant aspects and all the roles it plays, being of importance for 
the \DefinitionName{interest}{ls} of the \DefinitionName{viewer}{ls}. 
(The \DefinitionName{system-viewer}{ls} may conceive one and the same 
thing in the \DefinitionName{system-domain}{ls} to play more than one 
role in the \DefinitionName{system}{ls}.)


==> definitions/system-exposition/lp.tex <==
system expositions%


==> definitions/system-exposition/ls.tex <==
system exposition%


==> definitions/system-exposition/up.tex <==
System expositions%


==> definitions/system-exposition/us.tex <==
System exposition%


==> definitions/system-link/def.tex <==
Any \DefinitionName{element}{ls} from a \DefinitionName{system}{ls} 
that is a \DefinitionName{link}{ls}.


==> definitions/system-link/lp.tex <==
system links%


==> definitions/system-link/ls.tex <==
system link%


==> definitions/system-link/up.tex <==
System links%


==> definitions/system-link/us.tex <==
System link%


==> definitions/system-mission/def.tex <==
A role, to the benefit of \DefinitionName{stakeholder-goal}{lp}, for 
which the \DefinitionName{system}{ls} is intended.


==> definitions/system-mission/lp.tex <==
system missions%


==> definitions/system-mission/ls.tex <==
system mission%


==> definitions/system-mission/up.tex <==
System missions%


==> definitions/system-mission/us.tex <==
System mission%


==> definitions/system-model/def.tex <==
A \DefinitionName{model}{ls} of a \DefinitionName{system}{ls}.


==> definitions/system-model/lp.tex <==
system models%


==> definitions/system-model/ls.tex <==
system model%


==> definitions/system-model/up.tex <==
System models%


==> definitions/system-model/us.tex <==
System model%


==> definitions/system-requirement/def.tex <==
A \DefinitionName{requirement}{ls} on a future/changed 
\DefinitionName{system}{ls}. These \DefinitionName{requirement}{lp} are 
usually an negotiated integration of 
\DefinitionName{stakeholder-requirement}{lp} and should essentially be 
refinements of the \DefinitionName{system-mission}{ls}.


==> definitions/system-requirement/lp.tex <==
system requirements%


==> definitions/system-requirement/ls.tex <==
system requirement%


==> definitions/system-requirement/up.tex <==
System requirements%


==> definitions/system-requirement/us.tex <==
System requirement%


==> definitions/system-requirements-description/def.tex <==
A \DefinitionName{system-description}{ls} of the 
\DefinitionName{system-requirement}{lp} on a future/changed 
\DefinitionName{system}{ls} $S$, which covers:
\begin{itemize}

\item the \DefinitionName{requirement}{lp} which will be imposed by the 
\DefinitionName{environment}{ls} on \DefinitionName{system}{ls} $S$ and
\item the \DefinitionName{requirement}{lp} on other 
\DefinitionName{system}{lp} in the \DefinitionName{environment}{ls} of 
\DefinitionName{system}{ls} $S$ which \DefinitionName{system}{ls} $S$ 
may/must use for its own purposes. For example: the properties of a 
given infrastructure that must/may be used, `legacy' 
\DefinitionName{system}{lp} with which $S$ needs to interface, etc.
\end{itemize}
The gap between these sets of \DefinitionName{requirement}{lp}, is what 
needs to be `designed in' by the \DefinitionName{design-process}{ls}.


==> definitions/system-requirements-description/lp.tex <==
system requirements descriptions%


==> definitions/system-requirements-description/ls.tex <==
system requirements description%


==> definitions/system-requirements-description/up.tex <==
System requirements descriptions%


==> definitions/system-requirements-description/us.tex <==
System requirements description%


==> definitions/system-type/def.tex <==
A type that determines the potential kinds of 
\DefinitionName{systemic-property}{lp}, \DefinitionName{element}{lp} of 
the \DefinitionName{system-domain}{ls} and roles of the 
\DefinitionName{element}{lp} in achieving the 
\DefinitionName{systemic-property}{lp}.


==> definitions/system-type/lp.tex <==
system types%


==> definitions/system-type/ls.tex <==
system type%


==> definitions/system-type/up.tex <==
System types%


==> definitions/system-type/us.tex <==
System type%


==> definitions/system-view/def.tex <==
A \DefinitionName{model}{ls} of a \DefinitionName{system-domain}{ls} 
from the \DefinitionName{perspective}{ls} of a related set of 
\DefinitionName{interest}{lp} of a \DefinitionName{system-viewer}{ls}.


==> definitions/system-view/lp.tex <==
system views%


==> definitions/system-view/ls.tex <==
system view%


==> definitions/system-view/up.tex <==
System views%


==> definitions/system-view/us.tex <==
System view%


==> definitions/system-viewer/def.tex <==
A \DefinitionName{viewer}{ls} of a \DefinitionName{system-domain}{ls}.


==> definitions/system-viewer/lp.tex <==
system viewers%


==> definitions/system-viewer/ls.tex <==
system viewer%


==> definitions/system-viewer/up.tex <==
System viewers%


==> definitions/system-viewer/us.tex <==
System viewer%


==> definitions/system-viewpoint/def.tex <==
A specification of the conventions for constructing and using 
\DefinitionName{system-view}{lp}. This involves: a 
\DefinitionName{way-of-thinking}{ls}, a 
\DefinitionName{way-of-modeling}{ls}, a 
\DefinitionName{way-of-communicating}{ls}, a 
\DefinitionName{way-of-working}{ls}, a 
\DefinitionName{way-of-supporting}{ls} and a 
\DefinitionName{way-of-using}{ls}


==> definitions/system-viewpoint/lp.tex <==
system-viewpoints%


==> definitions/system-viewpoint/ls.tex <==
system-viewpoint%


==> definitions/system-viewpoint/up.tex <==
System-viewpoints%


==> definitions/system-viewpoint/us.tex <==
System-viewpoint%


==> definitions/system/def.tex <==
A special \DefinitionName{model}{ls} of a 
\DefinitionName{system-domain}{ls}, whereby all the things contained in 
that \DefinitionName{model}{ls} are transitively coherent, i.e.\ all of 
them are directly or indirectly related to each other and form a 
coherent whole. A \DefinitionName{system}{ls} is conceived as having 
assigned to it, as a whole, a specific characterisation (a non-empty 
set of \DefinitionName{systemic-property}{lp}) which, in general, 
cannot be attributed exclusively to any of its 
\DefinitionName{component}{lp}.


==> definitions/system/lp.tex <==
systems%


==> definitions/system/ls.tex <==
system%


==> definitions/system/up.tex <==
Systems%


==> definitions/system/us.tex <==
System%


==> definitions/systemic-property/lp.tex <==
systemic properties%


==> definitions/systemic-property/ls.tex <==
systemic property%


==> definitions/systemic-property/up.tex <==
Systemic properties%


==> definitions/systemic-property/us.tex <==
Systemic property%


==> definitions/technique-relation/def.tex <==
A well-defined relation between the sets of \DefinitionName{model}{lp} 
that may be represented in a \DefinitionName{technique}{ls}. An example 
would be a
 mapping algorithm between a conceptual \DefinitionName{model}{ls} and 
a relational database schema,
 the relation between the \DefinitionName{concept}{lp} of a business 
process \DefinitionName{model}{ls} and the concepts
 of a supporting work-flow, etc.


==> definitions/technique-relation/lp.tex <==
technique relations%


==> definitions/technique-relation/ls.tex <==
technique relation%


==> definitions/technique-relation/up.tex <==
Technique relations%


==> definitions/technique-relation/us.tex <==
Technique relation%


==> definitions/technique/def.tex <==
\Synonym{way-of-modeling}


==> definitions/technique/lp.tex <==
techniques%


==> definitions/technique/ls.tex <==
technique%


==> definitions/technique/up.tex <==
Techniques%


==> definitions/technique/us.tex <==
Technique%


==> definitions/telephone-heuristic/def.tex <==
\DefinitionName{communication}{us} form where the way to carry over 
\DefinitionName{information}{ls} is by written text.


==> definitions/telephone-heuristic/lp.tex <==
telephone heuristics%


==> definitions/telephone-heuristic/ls.tex <==
telephone heuristic%


==> definitions/telephone-heuristic/up.tex <==
Telephone heuristics%


==> definitions/telephone-heuristic/us.tex <==
Telephone heuristic%


==> definitions/turing-test/def.tex <==
An test to see if an human can make the distinction between the program 
in question and a human respondent.


==> definitions/turing-test/lp.tex <==
Turing tests%


==> definitions/turing-test/ls.tex <==
Turing test%


==> definitions/turing-test/up.tex <==
Turing tests%


==> definitions/turing-test/us.tex <==
Turing test%


==> definitions/uml/def.tex <==
Unified \DefinitionName{modeling}{us} Language


==> definitions/uml/lp.tex <==
UML%


==> definitions/uml/ls.tex <==
UML%


==> definitions/uml/up.tex <==
UML%


==> definitions/uml/us.tex <==
UML%


==> definitions/universe/def.tex <==
The `world' under consideration.


==> definitions/universe/lp.tex <==
universes%


==> definitions/universe/ls.tex <==
universe%


==> definitions/universe/up.tex <==
Universes%


==> definitions/universe/us.tex <==
Universe%


==> definitions/uod/def.tex <==
That part of the world around is that is to be modelled. See also 
\DefinitionName{application-domain}{ls}.


==> definitions/uod/lp.tex <==
universes of discourse%


==> definitions/uod/ls.tex <==
universe of discourse%


==> definitions/uod/up.tex <==
Universes of discourse%


==> definitions/uod/us.tex <==
Universe of discourse%


==> definitions/usability/def.tex <==
Bears on the effort needed for the use of the 
\DefinitionName{system}{ls} (or one of its 
\DefinitionName{sub-system}{lp}) by the \DefinitionName{actor}{lp} in 
the \DefinitionName{environment}{ls} of the 
\DefinitionName{system}{ls}. Sub-characteristics of 
\DefinitionName{usability}{ls} are: understandability, learnability, 
operability, explicitness, customisability, attractivity, clarity, 
helpfulness and user-friendliness.


==> definitions/usability/lp.tex <==
usabilities%


==> definitions/usability/ls.tex <==
usability%


==> definitions/usability/up.tex <==
Usabilities%


==> definitions/usability/us.tex <==
Usability%


==> definitions/view/def.tex <==
A \DefinitionName{model}{ls} of a \DefinitionName{domain}{ls} from the 
\DefinitionName{perspective}{ls} of a related set of 
\DefinitionName{interest}{lp} of a \DefinitionName{viewer}{ls}.


==> definitions/view/lp.tex <==
views%


==> definitions/view/ls.tex <==
view%


==> definitions/view/up.tex <==
Views%


==> definitions/view/us.tex <==
View%


==> definitions/viewer/def.tex <==
An \DefinitionName{actor}{ls} perceiving and conceiving (part of) a 
\DefinitionName{domain}{ls}.


==> definitions/viewer/lp.tex <==
viewers%


==> definitions/viewer/ls.tex <==
viewer%


==> definitions/viewer/up.tex <==
Viewers%


==> definitions/viewer/us.tex <==
Viewer%


==> definitions/viewing-cell/def.tex <==
A \DefinitionName{viewing-framework}{ls} that is not decomposed into a 
(covering) set of
 smaller \DefinitionName{viewing-framework}{lp}.


==> definitions/viewing-cell/lp.tex <==
viewing cells%


==> definitions/viewing-cell/ls.tex <==
viewing cell%


==> definitions/viewing-cell/up.tex <==
Viewing cells%


==> definitions/viewing-cell/us.tex <==
Viewing cell%


==> definitions/viewing-framework/def.tex <==
A kind of \DefinitionName{modeling-fragment}{ls}, which identifies a 
set of related
 \DefinitionName{perspective}{lp} from which to 
\DefinitionName{view}{ls} a \DefinitionName{system}{ls}. A 
\DefinitionName{viewing-framework}{ls} may be
 composed of yet other \DefinitionName{viewing-framework}{lp}.


==> definitions/viewing-framework/lp.tex <==
viewing frameworks%


==> definitions/viewing-framework/ls.tex <==
viewing framework%


==> definitions/viewing-framework/up.tex <==
Viewing frameworks%


==> definitions/viewing-framework/us.tex <==
Viewing framework%


==> definitions/viewpoint/def.tex <==
A kind of \DefinitionName{modeling-fragment}{ls}, which specifies the 
conventions for constructing and using \DefinitionName{model}{lp} which 
address the \DefinitionName{viewing-cell}{lp} contained in a specific 
\DefinitionName{viewing-framework}{ls}. A 
\DefinitionName{viewpoint}{ls} comprises at least a 
\DefinitionName{viewing-framework}{ls} and a 
\DefinitionName{way-of-modeling}{ls}, and possibly a 
\DefinitionName{way-of-working}{ls}.


==> definitions/viewpoint/lp.tex <==
viewpoints%


==> definitions/viewpoint/ls.tex <==
viewpoint%


==> definitions/viewpoint/up.tex <==
Viewpoints%


==> definitions/viewpoint/us.tex <==
Viewpoint%


==> definitions/way-of-communicating/def.tex <==
describes how the abstract \DefinitionName{concept}{lp} from the 
\DefinitionName{way-of-modeling}{ls} are communicated to human beings, 
for example in terms of a textual or a graphical notation. The 
\DefinitionName{way-of-communicating}{ls} essentially forms the bridge 
between the \DefinitionName{way-of-modeling}{ls} and the 
\DefinitionName{way-of-working}{ls}, it matches the abstract 
\DefinitionName{concept}{lp} of the 
\DefinitionName{way-of-modeling}{ls} to the pragmatic needs of the 
\DefinitionName{way-of-working}{ls}. Note that it may very well be the 
case that different \DefinitionName{modeling-technique}{lp} are based 
on the same \DefinitionName{way-of-modeling}{ls}, yet use different 
notations.


==> definitions/way-of-communicating/lp.tex <==
way of communicating%


==> definitions/way-of-communicating/ls.tex <==
way of communicating%


==> definitions/way-of-communicating/up.tex <==
Way of communicating%


==> definitions/way-of-communicating/us.tex <==
Way of communicating%


==> definitions/way-of-conceiving/def.tex <==
A set of \DefinitionName{modeling}{ls} \DefinitionName{concept}{lp} by 
which \DefinitionName{viewer}{lp} are to observe 
\DefinitionName{domain}{lp}.
 This usually takes the form of a \DefinitionName{meta-model}{ls}.


==> definitions/way-of-conceiving/lp.tex <==
way of conceiving%


==> definitions/way-of-conceiving/ls.tex <==
way of conceiving%


==> definitions/way-of-conceiving/up.tex <==
Way of conceiving%


==> definitions/way-of-conceiving/us.tex <==
Way of conceiving%


==> definitions/way-of-controlling/def.tex <==
The managerial aspects of \DefinitionName{system-development}{ls}. It 
includes such aspects as human resource management, 
\DefinitionName{quality}{ls} and progress control, and evaluation of 
plans, i.e.\ overall project management and governance (see 
\cite{1984-Kensing-MethodEvaluation, 1988-Sol-InfSystDev}).


==> definitions/way-of-controlling/lp.tex <==
way of controlling%


==> definitions/way-of-controlling/ls.tex <==
way of controlling%


==> definitions/way-of-controlling/up.tex <==
Way of controlling%


==> definitions/way-of-controlling/us.tex <==
Way of controlling%


==> definitions/way-of-describing/def.tex <==
The medium and `notations' used to represent the 
\DefinitionName{concept}{lp} as identified in
 a \DefinitionName{way-of-conceiving}{ls}.


==> definitions/way-of-describing/lp.tex <==
way of describing%


==> definitions/way-of-describing/ls.tex <==
way of describing%


==> definitions/way-of-describing/us.tex <==
Way of describing%


==> definitions/way-of-modeling/def.tex <==
The \DefinitionName{concept}{lp} and the notation of the language that 
may be used to denote, analyze, visualize and/or animate 
\DefinitionName{description}{lp}. A 
\DefinitionName{way-of-modeling}{ls} comprises a 
\DefinitionName{way-of-conceiving}{ls} and a 
\DefinitionName{way-of-describing}{ls}.


==> definitions/way-of-modeling/lp.tex <==
way of modeling%


==> definitions/way-of-modeling/ls.tex <==
way of modeling%


==> definitions/way-of-modeling/up.tex <==
Way of modeling%


==> definitions/way-of-modeling/us.tex <==
Way of modeling%


==> definitions/way-of-supporting/def.tex <==
The support to \DefinitionName{system-development}{ls} that is offered 
by (possibly automated) tools. In general, a 
\DefinitionName{way-of-supporting}{ls} is supplied in the form of some 
computerized tool (see for instance \cite{1989-McClure-CASE}).


==> definitions/way-of-supporting/lp.tex <==
way of supporting%


==> definitions/way-of-supporting/ls.tex <==
way of supporting%


==> definitions/way-of-supporting/up.tex <==
Way of supporting%


==> definitions/way-of-supporting/us.tex <==
Way of supporting%


==> definitions/way-of-thinking/def.tex <==
Articulates the assumptions on the kinds of problem 
\DefinitionName{domain}{lp}, solutions and modelers. This notion is 
also referred to as \emph{die Weltanschauung} 
\cite{1983-Sol-MethodConsideration, 1985-WoodHarper-Multiview}, 
\emph{underlying perspective} \cite{1981-Mathiassen-SystemDevelopment} 
or \emph{philosophy} \cite{1995-Avison-ISDevMeth}.


==> definitions/way-of-thinking/lp.tex <==
way of thinking%


==> definitions/way-of-thinking/ls.tex <==
way of thinking%


==> definitions/way-of-thinking/up.tex <==
Way of thinking%


==> definitions/way-of-thinking/us.tex <==
Way of thinking%


==> definitions/way-of-using/def.tex <==
Identification of heuristics that:
\begin{itemize}

\item define situations, classes of \DefinitionName{viewer}{lp} and 
\DefinitionName{interest}{lp}, for which a given 
\DefinitionName{viewpoint}{ls} is most suitable,
\item provide guidance in tuning a given \DefinitionName{viewpoint}{ls} 
to specific situations, classes of \DefinitionName{viewer}{lp} and 
their \DefinitionName{interest}{lp} at hand. For example, in terms of 
the set of modelling \DefinitionName{concept}{lp} to be used, effective 
notations, visualisations, etc.
\end{itemize}



==> definitions/way-of-using/lp.tex <==
way of using%


==> definitions/way-of-using/ls.tex <==
way of using%


==> definitions/way-of-using/up.tex <==
Way of using%


==> definitions/way-of-using/us.tex <==
Way of using%


==> definitions/way-of-working/def.tex <==
A structuring of (parts of) the way in which a 
\DefinitionName{system}{ls} is developed. It defines the possible 
tasks, including sub-tasks, and ordering of tasks, to be performed as 
part of the development process. It furthermore provides guidelines and 
suggestions (heuristics) on how these tasks should be performed.


==> definitions/way-of-working/lp.tex <==
way of working%


==> definitions/way-of-working/ls.tex <==
way of working%


==> definitions/way-of-working/up.tex <==
Way of working%


==> definitions/way-of-working/us.tex <==
Way of working%


==> definitions/weak-identification/def.tex <==
A sufficient condition to be able to uniquely identify objects and 
things, stating that no two objects or things have the same properties.


==> definitions/weak-identification/lp.tex <==
weak identification%


==> definitions/weak-identification/ls.tex <==
weak identification%


==> definitions/weak-identification/up.tex <==
Weak identification%


==> definitions/weak-identification/us.tex <==
Weak identification%


==> definitions/work-system-engineering/100-percent-principle/def.tex <==
The \DN{information-grammar} should describe \emph{precisely all} conceptual aspects. 

==> definitions/work-system-engineering/100-percent-principle/lp.tex <==
100\% Principle% 

==> definitions/work-system-engineering/100-percent-principle/ls.tex <==
100\% Principle% 

==> definitions/work-system-engineering/100-percent-principle/up.tex <==
100\% Principle% 

==> definitions/work-system-engineering/100-percent-principle/us.tex <==
100\% Principle% 

==> definitions/work-system-engineering/WSML/def.tex <==
Abbreviation for work system modeling library. A library of methodical
knowledge pertaining to the \DN{modeling} of \PDN{work-system}.


==> definitions/work-system-engineering/WSML/lp.tex <==
WSMLs%


==> definitions/work-system-engineering/WSML/ls.tex <==
WSML%


==> definitions/work-system-engineering/WSML/up.tex <==
WSMLs%


==> definitions/work-system-engineering/WSML/us.tex <==
WSML%


==> definitions/work-system-engineering/abstraction/def.tex <==
Omitting unessential details.


==> definitions/work-system-engineering/abstraction/lp.tex <==
abstractions% 

==> definitions/work-system-engineering/abstraction/ls.tex <==
abstraction% 

==> definitions/work-system-engineering/abstraction/up.tex <==
Abstractions% 

==> definitions/work-system-engineering/abstraction/us.tex <==
Abstraction% 

==> definitions/work-system-engineering/action-oriented/def.tex <==
The action-oriented approach interprets sentences as events occurring in the \DN{uod}. This approach is when the operations on the data are dominant.
See also \DN{fact-oriented}. 

==> definitions/work-system-engineering/action-oriented/lp.tex <==
action oriented% 

==> definitions/work-system-engineering/action-oriented/ls.tex <==
action oriented% 

==> definitions/work-system-engineering/action-oriented/up.tex <==
Action oriented% 

==> definitions/work-system-engineering/action-oriented/us.tex <==
Action oriented% 

==> definitions/work-system-engineering/active-system/def.tex <==
A special kind of \DN{system} that is conceived of as begin able to change
parts of the \DN{universe}.


==> definitions/work-system-engineering/active-system/lp.tex <==
active systems%


==> definitions/work-system-engineering/active-system/ls.tex <==
active system%


==> definitions/work-system-engineering/active-system/up.tex <==
Active systems%


==> definitions/work-system-engineering/active-system/us.tex <==
Active system%


==> definitions/work-system-engineering/activity-participation/def.tex <==
A \DN{system-link} between a \DN{system-activity} and one of its
\DN{actor}.


==> definitions/work-system-engineering/activity-participation/lp.tex <==
activity participations%


==> definitions/work-system-engineering/activity-participation/ls.tex <==
activity participation%


==> definitions/work-system-engineering/activity-participation/up.tex <==
Activity participations%


==> definitions/work-system-engineering/activity-participation/us.tex <==
Activity participation%


==> definitions/work-system-engineering/actor/def.tex <==
A \DN{system-element} that is conceived of as having some involvement in a
\DN{system-activity}. This involvement is a special kind of
\DN{system-link}, referred to as an \DN{activity-participation}.


==> definitions/work-system-engineering/actor/lp.tex <==
actors%


==> definitions/work-system-engineering/actor/ls.tex <==
actor%


==> definitions/work-system-engineering/actor/up.tex <==
Actors%


==> definitions/work-system-engineering/actor/us.tex <==
Actor%


==> definitions/work-system-engineering/agens/def.tex <==
The role in a sentence that most commonly is associated with the grammatical subject. 

==> definitions/work-system-engineering/agens/lp.tex <==
agens% 

==> definitions/work-system-engineering/agens/ls.tex <==
agens% 

==> definitions/work-system-engineering/agens/up.tex <==
Agens% 

==> definitions/work-system-engineering/agens/us.tex <==
Agens% 

==> definitions/work-system-engineering/alignment/def.tex <==
A \DN{system} $S_1$ is aligned to a system $S_2$ if, and only if, system $S_1$ meets {\em all} \PDN{requirement} posed by $S_2$ on $S_1$.

This alignment may be strived for at different levels of refinement of a system design.


==> definitions/work-system-engineering/alignment/lp.tex <==
alignment%


==> definitions/work-system-engineering/alignment/ls.tex <==
alignment%


==> definitions/work-system-engineering/alignment/up.tex <==
Alignment%


==> definitions/work-system-engineering/alignment/us.tex <==
Alignment%


==> definitions/work-system-engineering/application-domain/def.tex <==
That part of the world around is that is to be modelled in the context of the development of some application. See also \DN{uod}. 

==> definitions/work-system-engineering/application-domain/lp.tex <==
application domains% 

==> definitions/work-system-engineering/application-domain/ls.tex <==
application domains% 

==> definitions/work-system-engineering/application-domain/up.tex <==
Application domains% 

==> definitions/work-system-engineering/application-domain/us.tex <==
Application domain% 

==> definitions/work-system-engineering/approach/def.tex <==
\Synonym{way-of-working}


==> definitions/work-system-engineering/approach/lp.tex <==
approaches%


==> definitions/work-system-engineering/approach/ls.tex <==
approach%


==> definitions/work-system-engineering/approach/up.tex <==
Approaches%


==> definitions/work-system-engineering/approach/us.tex <==
Approach%


==> definitions/work-system-engineering/architecting/def.tex <==
The processes which tie \DN{definition}, \DN{design} and \DN{deployment} and
to the explicit and implicit needs, desires and requirements
of the usage context. Issues such as: business/IT alignment, stakeholders,
limiting design freedom, negotiation between stakeholders, enterprise
architectures, stakeholder communication, and outsourcing, typify these
processes. 


==> definitions/work-system-engineering/architecting/lp.tex <==
architecting%


==> definitions/work-system-engineering/architecting/ls.tex <==
architecting%


==> definitions/work-system-engineering/architecting/up.tex <==
Architecting%


==> definitions/work-system-engineering/architecting/us.tex <==
Architecting%


==> definitions/work-system-engineering/architectural-description/def.tex <==
A \DN{system-description} documenting/describing an \DN{architecture}.


==> definitions/work-system-engineering/architectural-description/lp.tex <==
architectural descriptions%


==> definitions/work-system-engineering/architectural-description/ls.tex <==
architectural description%


==> definitions/work-system-engineering/architectural-description/up.tex <==
Architectural descriptions%


==> definitions/work-system-engineering/architectural-description/us.tex <==
Architectural description%


==> definitions/work-system-engineering/architecture-driven-information-system-engineering/def.tex <==
\UDN{information-system-engineering}, using \DN{architecture} as a means to
\begin{itemize}
   \item guide \& control the design and evolution of the \DN{information-system},
   \item evaluate \& compare different information system alternatives, 
   \item negotiate the \PDN{concern} of the information system's \PDN{stakeholder},
\end{itemize}
with the aim of optimising the \DN{alignment} of the resulting
information system to its relevant, technological, organisation and human context (systems).


==> definitions/work-system-engineering/architecture-driven-information-system-engineering/lp.tex <==
architecture-driven information system engineering%


==> definitions/work-system-engineering/architecture-driven-information-system-engineering/ls.tex <==
architecture-driven information system engineering%


==> definitions/work-system-engineering/architecture-driven-information-system-engineering/up.tex <==
Architecture-driven information system engineering%


==> definitions/work-system-engineering/architecture-driven-information-system-engineering/us.tex <==
Architecture-driven information system engineering%


==> definitions/work-system-engineering/architecture-principle/def.tex <==
A \DN{design-principle} which is used to direct the design/architecting of
an \DN{architecture}.


==> definitions/work-system-engineering/architecture-principle/lp.tex <==
architecture principles%


==> definitions/work-system-engineering/architecture-principle/ls.tex <==
architecture principle%


==> definitions/work-system-engineering/architecture-principle/up.tex <==
Architecture principles%


==> definitions/work-system-engineering/architecture-principle/us.tex <==
Architecture principle%


==> definitions/work-system-engineering/architecture/def.tex <==
A \DN{model} of which the \DN{system-description}, the so-called
\DN{architectural-description}, is used during \DN{system-engineering} to:
    \begin{itemize}
      \item express the fundamental organization of the \DN{system-domain} in 
    terms of \PDN{component}, their relationships to each other and 
    to the \DN{environment} and 
      \item the principles guiding its evolution and design,
    \end{itemize}
    and which's explicit intend is to be used as a means:
    \begin{itemize}
      \item of communication \& negotiation among stakeholders,
      \item to evaluate and compare design alternatives,
      \item to plan, manage, and execute further system development,
      \item to verify the compliance of a system implementation's.
    \end{itemize}
  


==> definitions/work-system-engineering/architecture/lp.tex <==
architectures%


==> definitions/work-system-engineering/architecture/ls.tex <==
architecture%


==> definitions/work-system-engineering/architecture/up.tex <==
Architectures%


==> definitions/work-system-engineering/architecture/us.tex <==
Architecture%


==> definitions/work-system-engineering/aspect-system/def.tex <==
an aspect-system $S'$ of a \DN{system} $S$, is a \DN{sub-system}, where the set
of \PDN{model-link} in $S'$ is a proper subset of the set of the
\PDN{link} in $S$.


==> definitions/work-system-engineering/aspect-system/lp.tex <==
aspect systems%


==> definitions/work-system-engineering/aspect-system/ls.tex <==
aspect system%


==> definitions/work-system-engineering/aspect-system/up.tex <==
Aspect systems%


==> definitions/work-system-engineering/aspect-system/us.tex <==
Aspect system%


==> definitions/work-system-engineering/atomic-viewpoint/def.tex <==
A \DN{viewpoint} which is not decomposed into smaller \PDN{viewpoint}. An
\DN{atomic-viewpoint} is required to have a one-on-one correspondence to a
\DN{way-of-modeling}/\DN{technique} that should be used to create \PDN{model}
conforming to this \DN{viewpoint}.


==> definitions/work-system-engineering/atomic-viewpoint/lp.tex <==
atomic viewpoints%


==> definitions/work-system-engineering/atomic-viewpoint/ls.tex <==
atomic viewpoint%


==> definitions/work-system-engineering/atomic-viewpoint/up.tex <==
Atomic viewpoints%


==> definitions/work-system-engineering/atomic-viewpoint/us.tex <==
Atomic viewpoint%


==> definitions/work-system-engineering/autonomous-system/def.tex <==
an \DN{open-active-system} (possibly also a \DN{responsive-system}, but not a
\DN{reactive-system}) where at least one expression is an action.  A human
being and most (if not all) \PDN{organization} can be regarded as 
\PDN{autonomous-system}.



==> definitions/work-system-engineering/autonomous-system/lp.tex <==
autonomous systems%


==> definitions/work-system-engineering/autonomous-system/ls.tex <==
autonomous system%


==> definitions/work-system-engineering/autonomous-system/up.tex <==
Autonomous systems%


==> definitions/work-system-engineering/autonomous-system/us.tex <==
Autonomous system%


==> definitions/work-system-engineering/characterization-dimension/def.tex <==
A set of (possibly ordered) values by which an artefact may be characterized.


==> definitions/work-system-engineering/characterization-dimension/lp.tex <==
characterization dimensions%


==> definitions/work-system-engineering/characterization-dimension/ls.tex <==
characterization dimension%


==> definitions/work-system-engineering/characterization-dimension/up.tex <==
Characterization dimensions%


==> definitions/work-system-engineering/characterization-dimension/us.tex <==
Characterization dimension%


==> definitions/work-system-engineering/characterization-property/def.tex <==
A specific value from a \DN{characterization-dimension} that an artefact may
exhibit. 


==> definitions/work-system-engineering/characterization-property/lp.tex <==
characterization properties%


==> definitions/work-system-engineering/characterization-property/ls.tex <==
characterization property%


==> definitions/work-system-engineering/characterization-property/up.tex <==
Characterization properties%


==> definitions/work-system-engineering/characterization-property/us.tex <==
Characterization property%


==> definitions/work-system-engineering/closed-world-assumption/def.tex <==
All facts not stored in an \DN{information-system} are assumed to be false.
Not that this requires facts with \DN{complete-knowledge}. 

==> definitions/work-system-engineering/closed-world-assumption/lp.tex <==
closed world assumptions% 

==> definitions/work-system-engineering/closed-world-assumption/ls.tex <==
closed world assumption% 

==> definitions/work-system-engineering/closed-world-assumption/up.tex <==
Closed world assumptions% 

==> definitions/work-system-engineering/closed-world-assumption/us.tex <==
Closed world assumption% 

==> definitions/work-system-engineering/communication/def.tex <==
An exchange of \PDN{message}, i.e.\ a sequence of mutual and alternating
message transfers between at least two \PDN{human-actor}, called communication
partners, whereby these \PDN{message} represent some \DN{knowledge} and are
expressed in languages understood by all communication partners, and whereby
some amount of \DN{knowledge} about the domain of communication and about the
action context and the goal of the communication is made present in all
communication partners.



==> definitions/work-system-engineering/communication/lp.tex <==
communications%


==> definitions/work-system-engineering/communication/ls.tex <==
communication%


==> definitions/work-system-engineering/communication/up.tex <==
Communications%


==> definitions/work-system-engineering/communication/us.tex <==
Communication%


==> definitions/work-system-engineering/complete-knowledge/def.tex <==
The value \emph{undefined} is not allowed.


==> definitions/work-system-engineering/complete-knowledge/lp.tex <==
complete knowledge% 

==> definitions/work-system-engineering/complete-knowledge/ls.tex <==
complete knowledge% 

==> definitions/work-system-engineering/complete-knowledge/up.tex <==
Complete knowledge% 

==> definitions/work-system-engineering/complete-knowledge/us.tex <==
Complete knowledge% 

==> definitions/work-system-engineering/component-system/def.tex <==
A component-system $S'$ of a \DN{system} $S$, is a \DN{sub-system},  where the
set of \PDN{model-concept} in $S'$ is a proper subset of the set of entities in
$S$.


==> definitions/work-system-engineering/component-system/lp.tex <==
component systems%


==> definitions/work-system-engineering/component-system/ls.tex <==
component system%


==> definitions/work-system-engineering/component-system/up.tex <==
Component systems%


==> definitions/work-system-engineering/component-system/us.tex <==
Component system%


==> definitions/work-system-engineering/component/def.tex <==
\AbbreviationOf{component-system}



==> definitions/work-system-engineering/component/lp.tex <==
components%


==> definitions/work-system-engineering/component/ls.tex <==
component%


==> definitions/work-system-engineering/component/up.tex <==
Components%


==> definitions/work-system-engineering/component/us.tex <==
Component%


==> definitions/work-system-engineering/computerized-information-system/def.tex <==
A \DN{sub-system} of an \DN{information-system}, whereby all activities within
that sub-system are performed by one or several computer(s).	


==> definitions/work-system-engineering/computerized-information-system/lp.tex <==
computerized information systems%


==> definitions/work-system-engineering/computerized-information-system/ls.tex <==
computerized information system%


==> definitions/work-system-engineering/computerized-information-system/up.tex <==
Computerized information systems%


==> definitions/work-system-engineering/computerized-information-system/us.tex <==
Computerized information system%


==> definitions/work-system-engineering/concept/def.tex <==
Any \DN{element} from a \DN{conception} that is not a \DN{link}.


==> definitions/work-system-engineering/concept/lp.tex <==
concepts%


==> definitions/work-system-engineering/concept/ls.tex <==
concept%


==> definitions/work-system-engineering/concept/up.tex <==
Concepts%


==> definitions/work-system-engineering/concept/us.tex <==
Concept%


==> definitions/work-system-engineering/conception-evolution/def.tex <==
The evolution of a \DN{conception}.


==> definitions/work-system-engineering/conception-evolution/lp.tex <==
conception evolutions%


==> definitions/work-system-engineering/conception-evolution/ls.tex <==
conception evolution%


==> definitions/work-system-engineering/conception-evolution/up.tex <==
Conception evolutions%


==> definitions/work-system-engineering/conception-evolution/us.tex <==
Conception evolution%


==> definitions/work-system-engineering/conception/def.tex <==
That what results, in the mind of a \DN{viewer}, when they interpret a
\DN{perception} of a \DN{domain}.


==> definitions/work-system-engineering/conception/lp.tex <==
conceptions%


==> definitions/work-system-engineering/conception/ls.tex <==
conception%


==> definitions/work-system-engineering/conception/up.tex <==
Conceptions%


==> definitions/work-system-engineering/conception/us.tex <==
Conception%


==> definitions/work-system-engineering/conceptualization-principle/def.tex <==
The \DN{information-grammar} should not describe any does \emph{not} provide any realization (implementation) aspect. 

==> definitions/work-system-engineering/conceptualization-principle/lp.tex <==
Conceptualization principle% 

==> definitions/work-system-engineering/conceptualization-principle/ls.tex <==
conceptualization principle% 

==> definitions/work-system-engineering/conceptualization-principle/up.tex <==
Conceptualization principle% 

==> definitions/work-system-engineering/def.tex <==
A process aimed at adapting a \DefinitionName{work-system}{ls} to 
(possibly implicit and informal) needs, using limited means. These 
processes involving the execution of four sub-processes: 
\DefinitionName{definition-process}{ls}, 
\DefinitionName{design-process}{ls}, 
\DefinitionName{construction-process}{ls} and 
\DefinitionName{deployment-process}{ls}. Processes that may be executed 
sequentially, incrementally, interleaved, or in parallel.


==> definitions/work-system-engineering/lp.tex <==
work system engineering%


==> definitions/work-system-engineering/ls.tex <==
work system engineering%


==> definitions/work-system-engineering/up.tex <==
Work system engineering%


==> definitions/work-system-engineering/us.tex <==
Work system engineering%


==> definitions/work-system/def.tex <==
An \DefinitionName{open-active-system}{ls} in which 
\DefinitionName{actor}{lp} perform processes using
 \DefinitionName{information}{ls}, technologies, and other resources to 
produce products and/or
 services for internal or external \DefinitionName{actor}{lp}. 


==> definitions/work-system/lp.tex <==
work systems%


==> definitions/work-system/ls.tex <==
work system%


==> definitions/work-system/up.tex <==
Work systems%


==> definitions/work-system/us.tex <==
Work system%


==> images/jpgtoall <==
#!/bin/bash
function Convert () {
   FILE="`echo $1 | sed -e "s/.jpg$//"`"

   if [ -e $FILE.jpg ]; then
      echo Conversions for \"$FILE\":

      echo -n "  "
      jpegtopnm $FILE.jpg             2> /dev/null \
      | pnmtops -noturn -nosetpage 2> /dev/null > $FILE.eps
      echo "$FILE.jpg --> $FILE.eps"

      echo -n "  "
      echo "$FILE.jpg --> $FILE.pdf"
      epstopdf $FILE.eps

      echo
   else
      echo Can not find: $FILE.jpg
   fi
}

if [ "$1" == "" ]; then
   for f in *.jpg; do 
       Convert $f
   done
else
   Convert $1
fi


==> series/back.tex <==
\makeatletter
\ifodd\c@page
\else
   \mbox{~~~}
   \newpage
\fi
\makeatother

\pagestyle{empty}
\stepcounter{page}

\begin{titlepage}
   \setcounter{page}{20001}

   \vspace{3cm}

   {\Large The \DaVinci\ Lecture Notes Series:}

   \begin{quote}
      The \DaVinci\ series of lecture notes is concerned with \emph{The Art \&
      Craft of Information Systems Engineering}. On the one hand, this series
      of lecture notes takes a fundamental view (\emph{craft}) on the field
      information systems engineering. At the same time, it does so with an
      open eye to practical experiences (the \emph{art}) gained from
      information system engineering in industry.
   \end{quote}

   \vspace{1cm}

   {\Large Main contributors:}
   \def\Person#1#2{
     \begin{tabular}[b]{c}
        \ImageBox{2.5cm}{#1}\\
	{\small #2}
     \end{tabular}
   }
   \begin{center}
      \begin{tabular}{cc}
         \Person{patrick}{P. (Patrick) van Bommel} &
         \Person{stijn}{S.J.B.A. (Stijn) Hoppenbrouwers} 
	 \\~~\\
	 \Person{ger}{G.F.M. (Ger) Paulussen}
	 \\~~\\
	 \Person{erik}{H.A. (Erik) Proper} &
         \Person{theo}{Th.P. (Theo) van der Weide} 
      \end{tabular}
   \end{center}
\end{titlepage}


==> series/front.tex <==
\pagestyle{empty}

\begin{titlepage}
   \begin{center}
      \mbox{~~}

      \vspace{2cm}

      {\Huge \Title}

      \vspace{1cm}
      
      {\LARGE \Author}

      {\large \TheVersion}

      \vspace{2cm} 

      \centerline{\ImageBox{8cm}{vitruvius}}

      \vspace{1cm}

      {\large \DaVinciSub}

      \vspace{1cm}
   \end{center}
\end{titlepage}

\begin{titlepage}
   \setcounter{page}{3}
   \begin{center}
      \mbox{~~}

      \vspace{2cm}

      {\Huge \Title}

      \vspace{1cm}

      {\LARGE \Author}
   \end{center}
\end{titlepage}

\mbox{~~}
\vfill
\Colophon
\newpage

\pagestyle{headings}
\tableofcontents


==> symbols/AspectSystem/def.tex <==
For \DN{viewer} $v$ viewing \DN{universe} $U$, \DN{system} $S'$ is a \DN{aspect-system} of $S$


==> symbols/AspectSystem/sym.tex <==
\AspectSystem{U}{v}{S'}{S} ~\EQ 
  \SubSystem{U}{v}{S'}{S} \mbox{~~and~~} (S' \intersect \Links) \subset S


==> symbols/ComponentSystem/def.tex <==
For \DN{viewer} $v$ viewing \DN{universe} $U$, \DN{system} $S'$ is a \DN{component-system} of $S$


==> symbols/ComponentSystem/sym.tex <==
\ComponentSystem{U}{v}{S'}{S} ~\EQ 
  \SubSystem{U}{v}{S'}{S} \mbox{~~and~~} (S' \intersect \Concepts) \subset S


==> symbols/Conceives/def.tex <==
The fact that a viewer $v$ harbours a conception of \DN{domain} $D$ and
\DN{environment} $E$ for universe $U$ can be expressed as: 
$\Conception{U}{v}{E}{D}$.



==> symbols/Conceives/sym.tex <==
\Conception{\_}{\_}{\_}{\_} \subseteq 
      \Universes \times \Viewers \times \Powerset(\Elements) \times \Powerset(\Elements)


==> symbols/Conception/def.tex <==
A relationship expressing which \DN{conception} is held by which \DN{viewer}. 
The fact that a \DN{viewer} $v$ harbours a \DN{conception} 
$C$ for \DN{universe} $U$ is expressed as $\Conception{U}{v}{C}$.



==> symbols/Conception/sym.tex <==
\Conception{\_}{\_}{\_} \subseteq \Universes \times \Viewers \times \Powerset(\Elements)


==> symbols/ConceptionEvolutions/def.tex <==
The set of \PDN{conception-evolution}.


==> symbols/ConceptionEvolutions/sym.tex <==
\CEvolutions \EQ \Powerset(\EEvolutions)


==> symbols/Concepts/def.tex <==
The set of \PDN{element} of a \DN{conception} that are \PDN{concept}.


==> symbols/Concepts/sym.tex <==
\Concepts \subseteq \Elements


==> symbols/ConceptsSubset/def.tex <==
A subset of the set of \PDN{concept}.


==> symbols/ConceptsSubset/sym.tex <==
\ConceptsSub{X} \EQ X \intersect \Concepts


==> symbols/DecomposedInto/def.tex <==
A derived relationship providing the decomposition of a composed \DN{concept}
in some \DN{viewer}'s \DN{conception}. If $\DecomposedInto{x}{C}{y}$,
the \DN{concept} $x$ in \DN{conception} $C$ is decomposed into (possibly amongst
others) \DN{concept} $y$.


==> symbols/DecomposedInto/sym.tex <==
\DecomposedInto{\_}{\_}{\_} \subseteq 
   \Concepts \times \Powerset(\Elements) \times \Concepts


==> symbols/DecomposedIntoEq/def.tex <==
A derived relationship providing the decomposition of a composed \DN{concept}
in some \DN{viewer}'s \DN{conception}. If $\DecomposedIntoEq{x}{C}{y}$,
the \DN{concept} $x$ in \DN{conception} $C$ is decomposed into (possibly amongst
others) \DN{concept} $y$, or $x$ and $y$ are equal.


==> symbols/DecomposedIntoEq/sym.tex <==
\DecomposedIntoEq{x}{C}{y} \EQ x = y \lor \DecomposedInto{x}{C}{y}


==> symbols/Decomposers/def.tex <==
Decomposer \PDN{link}.


==> symbols/Decomposers/sym.tex <==
\Decomposers \subseteq \Links


==> symbols/Decomposition/def.tex <==
Decomposition of a composed \DN{concept} in a \PDN{viewers} \DN{conception}.


==> symbols/Decomposition/sym.tex <==
\Decomposition{x}{C}{y}


==> symbols/DomainConception/def.tex <==
A relationship expressing which \DN{conception} of a \DN{domain} is held by
which \DN{viewer}. The fact that a \DN{viewer} $v$ harbours a \DN{conception}
$D$ of a \DN{domain} in \DN{universe} $U$ is expressed as
$\DomainConception{U}{v}{C}$.



==> symbols/DomainConception/sym.tex <==
\DomainConception{\_}{\_}{\_} \subseteq \Universes \times \Viewers \times \Powerset(\Elements)


==> symbols/DomainInEnvironment/def.tex <==
A relationship expressing which \DN{conception} of a \DN{domain} and
\DN{environment} is held by which \DN{viewer} with a particular \DN{interest}.
The fact that a \DN{viewer} $v$ harbours a \DN{conception} $C$ of domain $D$
with environment $E$ an for \DN{universe} $U$ is expressed as
$\DomainInEnvironment{U}{v}{C}{D}{E}$.



==> symbols/DomainInEnvironment/sym.tex <==
\DomainInEnvironment{\_}{\_}{\_}{\_}{\_} \subseteq 
  \Universes \times \Viewers \times 
  \Powerset(\Elements) \times \Powerset(\Elements) \times \Powerset(\Elements)


==> symbols/ElementEvolutions/def.tex <==
The set of \PDN{element-evolution}.


==> symbols/ElementEvolutions/sym.tex <==
\EEvolutions \EQ \TimePoints \PartFunc \Elements


==> symbols/Elements/def.tex <==
The set of \PDN{element} that may be part of a \DN{conception}.


==> symbols/Elements/sym.tex <==
\Elements


==> symbols/Entities/def.tex <==
The set of \PDN{element} of a \DN{conception} that are \PDN{entity}.


==> symbols/Entities/sym.tex <==
\Entities \subseteq \Elements


==> symbols/EntitiesSubset/def.tex <==
A subset of the set of \PDN{entity}.


==> symbols/EntitiesSubset/sym.tex <==
\EntitiesSub{X} \EQ X \intersect \Entities


==> symbols/From/def.tex <==
The source \DN{concept} of a \DN{link}.


==> symbols/From/sym.tex <==
\From: \Links \Func \Concepts


==> symbols/Involved/def.tex <==
The set comprising the source and destination \PDN{element} of a \DN{link} in a
\DN{conception}.


==> symbols/Involved/sym.tex <==
\Involved(r) \EQ \setje{\From(r),\To(r)}


==> symbols/Label/def.tex <==
Hallo


==> symbols/Label/sym.tex <==
H \subseteq J


==> symbols/Later/def.tex <==
A complete and total order over points in time.


==> symbols/Later/sym.tex <==
\Later \subseteq \TimePoints \times \TimePoints


==> symbols/LinkedTo/def.tex <==
A (derived) relationship denoting the fact that there exists a \DN{link} from
one \DN{concept} to another.


==> symbols/LinkedTo/sym.tex <==
e \LinkedTo_C f \EQ \Ex{l \in \LinksSub{C}}{\From(l) = e \land \To(l) = f}


==> symbols/Links/def.tex <==
The set of \PDN{element} of a \DN{conception} that are \PDN{link} between \PDN{concept}.


==> symbols/Links/sym.tex <==
\Links \subseteq \Elements


==> symbols/LinksSubset/def.tex <==
A subset of the set of \PDN{link}.


==> symbols/LinksSubset/sym.tex <==
\LinksSub{X} \EQ X \intersect \Links


==> symbols/ModelConception/def.tex <==
A relationship expressing which \DN{model} is held by
which \DN{viewer}. The fact that a \DN{viewer} $v$ harbours a
\DN{model} $M$ of part of \DN{universe} $U$ is expressed as
$\ModelConception{U}{v}{M}$.



==> symbols/ModelConception/sym.tex <==
\ModelConception{U}{v}{M} \EQ \Ex{C,E}{\ModelInEnvironment{U}{v}{C}{E}{M}}


==> symbols/ModelInEnvironment/def.tex <==
A relationship expressing which \DN{model} and \DN{environment} or some part
of the \DN{universe} are held by which \DN{viewer}.  The fact that a
\DN{viewer} $v$ with a \DN{conception} $C$ harbours a \DN{model} $M$ with
\DN{environment} $E$ for a part of \DN{universe} $U$ is expressed as
$\ModelInEnvironment{U}{v}{C}{M}{E}$.



==> symbols/ModelInEnvironment/sym.tex <==
\ModelInEnvironment{\_}{\_}{\_}{\_}{\_} \subseteq 
  \Universes \times \Viewers \times 
  \Powerset(\Elements) \times \Powerset(\Elements) \times \Powerset(\Elements)


==> symbols/Next/def.tex <==
The next point in time. As $\Later$ is a complete and total order, there is
always a unique next point in time. This allows us to write $\Next t$.


==> symbols/Next/sym.tex <==
t_1 \Next t_2 \EQ t_1 \Later t_2 \land \lnot\Ex{s}{t_1 \Later s \Later t_2}


==> symbols/Relationships/def.tex <==
The set of \PDN{element} of a \DN{conception} that are \PDN{relationship} between \PDN{entity}.


==> symbols/Relationships/sym.tex <==
\Relationships \subseteq \Elements


==> symbols/RelationshipsSubset/def.tex <==
A subset of the set of \DN{relationship}.


==> symbols/RelationshipsSubset/sym.tex <==
\RelationshipsSub{X} \EQ X \intersect \Relationships 


==> symbols/SubSystem/def.tex <==
For \DN{viewer} $v$ viewing \DN{universe} $U$, \DN{system} $S'$ is a \DN{sub-system} of $S$


==> symbols/SubSystem/sym.tex <==
\SubSystem{U}{v}{S'}{S} ~\EQ 
  \SystemConception{U}{v}{S}, \mbox{~~}
  \SystemConception{U}{v}{S'} \mbox{~and~}
  S' \subset S 


==> symbols/SystemConception/def.tex <==
A relationship expressing which \DN{system} is viewed by
which \DN{viewer}. The fact that a \DN{viewer} $v$ views
system $S$ in \DN{universe} $U$ is expressed as
$\SystemConception{U}{v}{S}$.



==> symbols/SystemConception/sym.tex <==
\SystemConception{U}{v}{S} \EQ \Ex{C,E}{\SystemInEnvironment{U}{v}{C}{E}{S}}


==> symbols/SystemInEnvironment/def.tex <==
A relationship expressing which \DN{system} and \DN{environment} are viewed
in the \DN{universe} by a \DN{viewer}.  The fact that a \DN{viewer} $v$
with \DN{conception} $C$ views \DN{system} $M$ with \DN{environment} $E$ for a
part of \DN{universe} $U$ is expressed as
$\SystemInEnvironment{U}{v}{C}{S}{E}$.



==> symbols/SystemInEnvironment/sym.tex <==
\SystemInEnvironment{\_}{\_}{\_}{\_}{\_} \subseteq 
  \Universes \times \Viewers \times 
  \Powerset(\Elements) \times \Powerset(\Elements) \times \Powerset(\Elements)


==> symbols/TimePoints/def.tex <==
Points of time.


==> symbols/TimePoints/sym.tex <==
\TimePoints


==> symbols/To/def.tex <==
The destination \DN{concept} of a \DN{link}.


==> symbols/To/sym.tex <==
\To: \Links \Func \Concepts


==> symbols/Universes/def.tex <==
The set of \PDN{universe}.


==> symbols/Universes/sym.tex <==
\Universes


==> symbols/Viewers/def.tex <==
The set of \PDN{viewer}.


==> symbols/Viewers/sym.tex <==
\Viewers


==> symbols/new <==
#!/bin/bash
echo -n "Symbol key: "
read DN

mkdir $DN
echo "\\$DN" > $DN/sym.tex

gvim $DN/def.tex $DN/sym.tex


==> wsm01.tex <==
%
% Roadmap:
% - Use "as is" in 05/06
% - Evolve firther in 06/07:
%   - Streamline initial sections
%   - Elaborate fundamental-approach and formal-approach sections.

\Chapter{Introduction}{introduction}
\Version{17-01-06}

The focus of these lecture notes is on modeling of different aspects of
\PDN{work-system}. In doing so, we will build on top of the general modeling
foundations laid in the \emph{Domain Modeling} course. 
%% Neem een cite op naar het DM dictaat

In this chapter, we provide a brief exploration of the concept of
\PDN{work-system}. The understanding of this concept as provided in this chapter
will serve as a starting point. In the next chapters, this concept will be put in
a more fundamental context. We will do so by discussing the concept of
\DN{work-system}, from the bottom up. We will start
with a fundamental discussion of the
underlying ontology of \PDN{system}, \DN{modeling} and \PDN{work-system} from
which we will approach these phenomenon. We will then proceed
by discussing specific modeling techniques
for the modeling of an \DN{work-system}'s formal structures as well as their
potential evolution over time. In the last part, we will consider the design of
\PDN{work-system} from the perspective of their strategies.

Note: Not all parts of these lecture notes will be used in the ``Modelleren van
Organisaties'' course.

\Section{Organizations}{organizations}
\UPDN{organization} are an ubiquitous phenomenon in our modern day society.
Most of our lives are spent in the context of \PDN{organization}. We are born
in \emph{hospitals}, we receive an education from \emph{schools} and
\emph{universities}. Later on we work for \emph{factories}, \emph{enterprises},
etc. In our spare-time, we visit \emph{restaurants}, \emph{sportclubs}, etc.
These are all examples of \PDN{organization}.  Our modern-day lives are
surrounded by a plethora of \PDN{organization}.

However, the ubiquity of \PDN{organization} is not something new. Also in the
past \PDN{organization} have always been dominantly present. In line with our
working definition, \PDN{organization} can be regarded as a more or less stable
network of social relationships. In doing so, the concept of \PDN{organization}
can be said to be as old as humanity itself.

At first glance, the concept of organization comes natural to us.
\UPDN{organization} can be found anywhere. A University is an
\DN{organization}, a sports club is an \DN{organization}, a bank is one,
government departments are, etc. \UPDN{organization} are everywhere. In
general, an \DN{organization} could be an enterprise, an institution, a
company, a factory, etc., or it could be a functional, geographic or
organizational part thereof, typically a department or a specific kind of the
business. The concept of \DN{organization}, however, is not limited to such
``formal'' and ``explicit'' \PDN{organization}. Ad-hoc groupings of people,
such as a group of friends regularly having a beer after office hours in order
to relax after a day of work, may also classify as (ad-hoc) \PDN{organization}.
In this textbook, we will use the following definition of \DN{organization}:
\begin{Definitions}
   \DefinitionItem{organization}
\end{Definitions}
Note the term \emph{purposely}. An \DN{organization} is formed by a group of
\PDN{actor}. They will typically do so in order to achieve some shared/private
goals.

\Section{Information systems}{information-systems}
% Meer uit "van Aken" halen
In our modern western society, most \PDN{organization} use some form of
\PDN{information-system} to support the activities of the \DN{organization}.
With ``\DN{information-system}'' we (informally) refer to information
processing activities that may be performed by computerized as well as
non-computerized actors. Without these \PDN{information-system}, most
\PDN{organization} would no longer be able to exist. Even more, some
\PDN{organization} are actually large \PDN{information-system} themselves. For
example, banks, insurance companies, taxation offices, are really `just' very
large \PDN{information-system} comprising human, physical (money, bankcards,
etc.) and computerized actors.

The concept of \DN{information-system} can roughly be defined as that aspect of
an \DN{organization} that provides, uses and distributes information. An
\DN{information-system} \emph{may} contain computerized sub-systems to automate
certain elements. Some \DN{information-system} may not even be computerized at
all. A filing cabinet used to store and retrieve several dossiers is, in
essence, an \DN{information-system}. The kind of \PDN{information-system} we
are interested in, however, are indeed presumed to have some computerized core
parts.

What we may perceive to be an \DN{information-system}, may vary highly in terms
of their scope. Some examples would be:
\begin{itemize}
   \item Personal information appliances, such as electronic agenda's,
   telephone registries in mobile phones, etc.
   \item Specific information processing applications.
   \item Enterprise wide information processing.
   \item Value-chain wide information processing.
\end{itemize}
Some concrete examples are:
\begin{itemize}
   \item An insurance-policy administration is an information system
   \item A bank is (primarily) an information system
   \item Clients are actors in that information system
   \item The taxation department is an information system
   \item The PDA you use as an agenda
   \item The phone number collection in your mobile phone
\end{itemize}
In practice, the concept of ``\emph{\DN{information-system}}'' is used quite
differently by different groups of people.  It seems (see e.g.\
\cite{1998-Lindgreen-FRISCO}) to be interpreted in at least three different
ways:
\begin{itemize}
  \item As a technical system, implemented with computer and telecommunications
  technology.
  \item As a social system, such as an \DN{organization}, in connection with
  its information processing needs.
  \item As a conceptual system (i.e.\ an abstraction of either of the above).
\end{itemize}

\section{Work-systems}
In the field of information systems, this has also lead to a
generalisation of the notion of organization and information systems to
\emph{\PDN{work-system}}, focusing on the essential common properties such as
actors, resources, etc.  In~\cite{1999-Alter-WorkSystems,
2002-Alter-WorkSystems} Alter defines a work system as:
\begin{quote} \it
   A work system is a system in which human participants and/or machines
   perform business processes using information, technologies, and other
   resources to produce products and/or services for internal or external
   customers.
\end{quote}
Typical business organizations contain work systems that procure materials from
suppliers, produce products, deliver products to customers, find customers,
create financial reports, hire employees, coordinate work across departments,
and perform many other functions. 

We will actually generalize the definition of work-system even further to:
\begin{Definitions}
   \DefinitionItem{work-system}
\end{Definitions}
where we have purposely generalized ``human participants and/or machines''
as used in Alter's definition of work systems to the notion of actors in order
to abstract from the fact wether these actors are of a biological, mechanical,
chemical, electronical, or whichever, means. Actors are presumed to perform
\emph{activities} (work!) in order to achieve some \emph{purpose}. We have furthermore 
replaced any explicit reference to business like terminology as work-systems is
intended to be a more general notion that just organisations, enterprises, etc.

As discussed in~\cite{1999-Alter-WorkSystems, 2002-Alter-WorkSystems}, the
work-system concept can be used as a common denominator for many types of
systems. Enterprises, value chains, organizations, operational information
systems, projects, supply chains, and ecommerce web sites can all be viewed as
special cases of work systems. Organisations are work systems. An information
system is a work system whose work practices are devoted to processing
information. A project is a work system designed to produce a product and then
go out of existence. A supply chain is an interorganizational work system
devoted to procuring materials and other inputs required to produce a firm's
products. An ecommerce web set can be viewed as a work system in which a buyer
uses a seller's web site to obtain product information and perform purchase
transactions. The relationship between work systems in general and the special
cases implies that the same basic concepts apply to all of the special cases,
which also have their own specialized vocabulary. In turn, this implies that
much of the body of knowledge for the current information systems discipline
can be organized around a work system core.

Specific information systems exist to support (other) work systems. Many
different degrees of overlap are possible between an information system and a
work system that it supports. For example, an information system might provide
information for a non-overlapping work system, as happens when a commercial
marketing survey provides information to a firm's marketing managers In other
cases, an information system may be an integral part of a work system, as
happens in highly automated manufacturing and in ecommerce web sites. In these
situations, participants in the work system are also participants in the
information system, the work system cannot operate properly without the
information system, and the information system has little significance outside
of the work system.

\section{A fundamental view on work-systems modeling}
%
% Bas: Onderstaande stuk uitbreiden met meer tekst?
%
Modeling is at the very heart of the field of information systems engineering
as well as organizational engineering. Any course on the modeling of
\PDN{work-system} should therefore also provide a
fundamental understanding of modeling, in particular the modeling of
\PDN{work-system}. As we will see in the next chapter, when two people model
the same \DN{domain}, they are likely to produce quite different models.
Even when they use the same information (informants, documents, etc.) to
produce the models, the models are still likely to differ considerably. This
also means that if two people communicate about the same \DN{work-system},
they are likely to do so with different models of this \DN{work-system} in
mind. \emph{Why do these differences occur} \emph{What are the origins of these
different models?} \emph{What happens when people produce models?} Questions
that beg for a fundamental answer. These lecture notes try to provide some of
the answers.

\section{Formal approach}
In developing our understanding of modeling \PDN{organization}, we will discuss
several modeling languages for different aspects of \PDN{organization}. When
discussing these modeling languages, we will also discuss their syntax and
semantics from a formal (mathematical) perspective.
In~\cite{1990-Hofstede-PredModForm, 1992-Hofstede-DataMod, 1998-Hofstede-HowTo}
three major reasons for a formal approach to the syntax and semantics of
modeling techniques are given. 
%%% Below, we will briefly review these reasons.

Even though in literature it has often been emphasized that modeling languages
should have a rigorous formal basis (see e.g.~\cite{1989-Cohen-FormMeth,
1991-Tse-ReqSpecLang, 1988-Spivey-Z, 1986-Jones-VDM, 1989-Horenbeek-AlgSpec},
somehow this need for formality has not been generally acknowledged in the
field of information systems engineering and organization engineering.  This
has contributed greatly to the appearance of the
%%% Zie Dietz ivm organization engineering.
``\emph{Methodology Jungle}'', a term introduced
in~\cite{1995-Avison-ISDevMeth}. In \cite{1986-Bubenko-Methodology} it is
estimated that during the past years, hundreds if not thousands of information
system development methods have been introduced.  Most organizations and
research groups have defined their own methods.  The techniques advocated in
these methods usually do not have a formal foundation.  In some cases their
syntax is defined, but attention is hardly ever paid to their formal semantics.
The discussion of numerous examples, mostly with the use of pictures, is a
popular style for the ``definition'' of new concepts and their behavior. This
has led to \emph{fuzzy} and \emph{artificial} concepts in
information systems development methods (see also \cite{1986-Bubenko-Methodology}).

%%%%%%%%%%% Zie CAiSE artikel!!
%% Die "zie below" van boven nog uncommentent.

% The formalization provided in chapter 2 may seem overdoing it. However, it
% provides a good first exercise in the use of a formal approach to theorising.

%The attitude towards formalization
%in the field of information systems is changing however.
%In several papers the need for formal foundations
%in this field has been addressed
%(see e.g.~\cite{Article:89:Sernadas:NIAM},
%\cite{Finkelstein:FormFrame},
%\cite{Hohenstein:CADDY},
%\cite{Article:89:Tse:DFD},
%\cite{Report:89:Falkenberg:ProcSem},
%\cite{Report:90:Hofstede:PredModForm}).
%In~\cite{Hagelstein:Industry} it is noted
%that without a formal approach it is difficult
%to avoid deficiencies such as inconsistency,
%lack of structure, overspecification, incompleteness,
%ambiguity, and redundancy.
%These problems are caused by the fact that
%informal notations can be ambiguous and
%do not allow for sophisticated (automated) support
%and formal reasoning.
%Each of these problems will be addressed 
%and illustrated in the following sections in the
%con of information modeling.
%\subsubsection{Ambiguity}
%As stated before, many techniques have been
%introduced by discussing examples only.
%If that occurs,
%different interpretations
%will easily arise in cases not covered by these examples.
%Worse, situations that are not covered by any
%example are hardly ever recognized.
%The intention behind examples is to give hands on
%experience, in order to try to convey the general idea.
%This may however be difficult
%and sometimes even impossible.
%As an example, consider \keyword{NIAM}
%as presented in~\cite{Book:90:Nijssen:NIAM}.
%
%\PostFigure{NIAMComUni}{8.8}
%	   {Uniqueness constraint over objectification}
%	   {NIAM:ComUni}
%In figure~\ref{NIAM:ComUni} a simple NIAM schema,
%taken from \cite{Book:90:Nijssen:NIAM}, is shown.
%In this figure, a uniqueness constraint
%is expressed over a so-called
%objectified fact type ({\em Enrollment\/}).
%Obviously the schema of figure~\ref{NIAM:ComUni} is a
%well-formed schema according to NIAM.
%The meaning of the schema requires knowledge of the meaning
%of the uniqueness constraint.
%The semantics of this constraint
% explained in \cite{Book:90:Nijssen:NIAM}
%by stating that it
%expresses a key on the ternary relation that is the result
%of \Keyword{flattening} objectified fact type {\em Enrollment\/}.
%This key is shown in figure~\ref{NIAM:ComUniFlat}
%and implies that for {\em Person\/} the combination
%of {\em Subject\/} and {\em Position\/} is unique.
% 
%\PostFigure{NIAM-ComUniFlat}{8.8}
%           {Semantics of uniqueness constraint}
%           {NIAM:ComUniFlat}
%This example does not seem difficult to understand,
%but does certainly not convey the general idea.
%The relation between the fact types in figure~\ref{NIAM:ComUni}
%on the one
%hand and the fact type in figure~\ref{NIAM:ComUniFlat}
%on the other hand is not clear.
%As stated before,
%this relation is to be found by flattening
%the \keyword{objectified}[fact objectification] fact type {\em Enrollment\/}.
%Flattening is not an operation which
%is easily explained intuitively.
%
%Furthermore the reader might get the impression,
%that the schemata of figures~\ref{NIAM:ComUni}
%and \ref{NIAM:ComUniFlat} are
%equivalent (which they are {\em not\/},
%as contrary to figure~\ref{NIAM:ComUniFlat},
%in figure~\ref{NIAM:ComUni} a {\em Position\/}
%is not required for each recorded combination
%of a {\em Person\/} and a {\em Subject\/}),
%which would allow for switching freely between both alternatives,
%depending on the taste of an information analyst.
%Schema equivalence is not more than obliquely referred to
%in~\cite{Book:90:Nijssen:NIAM},
%although the reader might have some intuition.
%Even then, however, the example does not suffice
%to clarify the situation.
%What e.g.,
%is the meaning of the uniqueness constraints in figures~\ref{NIAM:ComUniEx1}
%and~\ref{NIAM:ComUniEx2}?
%\PostFigure{NIAM-ComUniEx1}{8.8}
%           {Complex uniqueness constraint}
%           {NIAM:ComUniEx1}
%\PostFigure{NIAM-ComUniEx2}{8.25}
%           {Another complex uniqueness constraint}
%           {NIAM:ComUniEx2}
%
%Particular interpretation problems are caused by techniques
%based on natural language, as e.g.\ \Keyword{structured English}
%(\cite{DeMarco78}),
%since natural language is notoriously ambiguous.
%
%Seemingly identical notions can have entirely different semantics,
%thus increasing the possibility of interpretation problems.
%In the field of artificial intelligence
%the \keyword{IS-A link},
%employed in many knowledge representation systems, serves as a typical example.
%Nearly every type of \keyword{semantic network} assigns a different
%(often only intuitive) meaning to this type of link
%(\cite{Brachman:ISAlinks}).
%
%The consequences of different interpretations among persons,
%or persons and machines, can be disastrous.
%Interpretation problems will certainly
%cause the resulting system to malfunction.
%% lead to a system which does
%% not function the way users (or even analysts or designers)
%% require it to function.
%% is between man and machine (``the computer does not work''
%% or ``the computer makes a mistake'').
%\subsubsection{Automated support}
%A \keyword{}[automated support]
%second reason for the need of formalization is
%that a formal model provides a good clue for implementation.
%The better the formalism, the easier the implementation.
%In fact, an implementation can be seen as yet another,
%but enormously more detailed formal description,
%usually in an imperative programming language.
%
%Not only the implementation benefits from a formal description.
%It also provides scope for much more sophisticated
%and extended support to information analysts.
%Due to the lack of formality of the
%underlying concepts of the supported techniques,
%state-of-the-art \keyword{CASE tools}[CASE tool] are not able to perform
%sophisticated \keyword{verification} checks,
%nor give warnings on suspect constructs.
%Again, let us consider \keyword{NIAM} as an example.
%
%\PostFigure{NIAM-ComplSchema}{7.26}
%           {Inconsistent NIAM schema}
%           {NIAM:ComplSchema}
%Consider the NIAM schemata of figures~\ref{NIAM:ComplSchema}
%and \ref{NIAM:ComplSchema1}.
%Current CASE tools supporting NIAM (e.g.\ SDW, ProNIAM, RIDL*)
%do not detect the inconsistencies in these schemata, which are:
%\PostFigure{NIAM-ComplSchema1}{7.26}
%           {A suspect NIAM schema}
%           {NIAM:ComplSchema1}
%\begin{enumerate}
%\item
%  In figure~\ref{NIAM:ComplSchema},
%  the subset constraint states that a {\em Person\/}
%  managing a certain {\em Project\/} should
%  also be a coworker of that Project.
%  The exclusion constraint in figure~\ref{NIAM:ComplSchema} expresses that
%  a {\em Person\/} is never both a manager and a coworker.
%  Clearly,
%  the only populations of this schema that satisfy
%  both requirements are those populations with no
%  managers.
%\item
%  The subset constraint of figure~\ref{NIAM:ComplSchema1} states
%  that a {\em Company\/} that produces a certain {\em Product\/}
%  also promotes that {\em Product\/}.
%  The uniqueness constraint on the upper fact type
%  states that a {\em Company\/} may produce several {\em Products\/},
%  and that a {\em Product\/} may be produced by several {\em Companies\/}.
%  The uniqueness constraint on the lower fact type
%  states that a {\em Company\/} may promote at most
%  one {\em Product\/}.
%  The only populations that satisfy these three constraints,
%  are those populations where each {\em Company\/}
%  produces at most one {\em Product\/}.
%% The total role constraint
%% (represented by the black dot on object type {\em Company\/})
%% states that every {\em Company\/} produces a {\em Product\/}.
%% If both constraints are correct,
%% then a total role constraint stating that every
%% {\em Company\/} promotes a {\em Product\/}
%% is obviously missing.
%\end{enumerate}
%In both cases we have well-formed schemata,
%i.e.\ schemata that fulfill the syntactical rules of NIAM.
%If CASE tools are to detect such inconsistencies,
%they need to be aware of the semantic definition
%of NIAM schemata in general (and in this case,
%of constraints in particular).
%
%Checking whether a model has certain properties,
%using the rules of a technique,
%is called \Keyword{verification}.
%If these properties are formally
%expressed and computable,
%it is possible to perform verification automatically.
%Checking whether a model is well-formed according
%to a certain technique,
%is an example of verification.
%Often however, verification not only deals with well-formedness,
%but also deals with more
%complicated checks (as e.g.\ required in schema~\ref{NIAM:ComplSchema}),
%usually referred to as \keyword{static semantic checks}[static semantic check].
%% verwijzen naar CAiSE verhaal van Terry ??
%
%Another important issue regarding automated
%support is \Keyword{validation},
%the question whether a well-formed model \Cal{D}
%meets its intended requirements in the Universe of Discourse.
%In contrast with verification,
%this cannot be checked by a computer,
%as the Universe of Discourse is only available in
%a highly informal format.
%Therefore, in order to validate \Cal{D}
%a formal description \Cal{F} of the Universe of Discourse
%is needed
%as well as a proof of the equivalence of \Cal{D} and \Cal{F}.
%That leaves the problem of validating \Cal{F}, etc.
%Validation however, can be {\em supported\/} by tools.
%By executing a specification,
%a domain expert can improve
%his (or her) understanding of the meaning of that specification.
%By offering a domain expert the
%possibility to specify a population
%of a certain data model,
%which (s)he considers to be correct,
%it can be checked whether that population
%satisfies the constraints in that data model,
%and therefore,
%whether these constraints
%meet their intended meaning.
%Only formal techniques have these features.
%
%An extended form of validation is testing on \Keyword{plausibility}.
%Certain constructs are accepted during verification,
%yet are most probably incorrect.
%In some cases these implausibilities can be detected automatically.
%The implausibility of the schema of figure~\ref{NIAM:ComplSchema1} is an example.
%Another example is a data flow diagram that contains a process
%that produces information out of nothing
%(i.e.\ a process without input flows),
%or a process that only consumes information
%(i.e.\ a process without output flows).
%Another example would be a program fragment
%\[ \ProgL{i := 1; S; i := 2} \]
%where program fragment \ProgL{S} does
%not contain an application of variable \ProgL{i},
%directly or indirectly.
%In this case, the assignment \ProgL{i := 1} is superfluous.
%It is not plausible that the programmer writes useless statements,
%so a warning should be given.
%\subsubsection{Properties}
%\label{NeedFormalism}
%
%A third reason for
%formalization is that a formal definition makes
%it possible to formulate and prove properties.
%For example, one could look at the expressive power of
%a technique and compare it with the expressive power
%of other techniques.
%A conclusion could be,
%that a certain technique allows a much more
%precise specification than another technique
%and that this other technique
%provides insufficient possibilities
%to exclude invalid situations.
%
%Furthermore, models specified
%according to the same technique
%can be compared and (dis)proved \keyword{equivalent}[equivalence].
%This is important in order to abstract from the peculiarities
%of an information analyst.
%The introduction of a set of transformation rules,
%transforming models into equivalent models,
%offers the opportunity to describe normal forms for
%well-formed models.
%A normal form is a base for comparing different models,
%probably originating from different information analysts
%trying to model the same Universe of Discourse.
%
%Also, properties of specific well-formed models
%according to some technique can be
%formulated and proved.
%An example of a property of a data model is
%structural identifiability, i.e.\ the question
%whether every entity type is identifiable.
%For process models it is interesting
%to determine whether they are free of
%deadlock or starvation.
%
%From the above it is clear that properties
%can be proved both for models in a technique
%and for a technique itself.
%\subsection{Conceptual level}
%% Hier ook noemen dat b.v. het relationele model
%% niet conceptueel is ?
%An important principle that is included in the definition
%of information modeling is the \Keyword{Conceptualization Principle}
%(\cite{Report:82:ISO:Concepts}).
%This principle states that \keyword{conceptual models}[conceptual model] should deal
%only and exclusively with aspects of the Universe of Discourse.
%Any aspects irrelevant to that meaning should be avoided.
%Examples of these \keyword{conceptually}[conceptual level]
%irrelevant aspects are e.g.\ (see~\cite{Report:82:ISO:Concepts})
%aspects of (external or internal) data representation,
%physical data organization and access as
%well as all aspects of particular external
%user representation such as message formats and data structures.
%
%The Conceptualization Principle is important because
%in the early phases of systems development no
%implementation decisions should have to be made.
%Such decisions easily become outdated and impede
%successful implementation.
%Furthermore, they tend to lead to models that
%are difficult to comprehend and to communicate.
%
%\PostFigure{ERmany}{10}
%           {Transformation of many-to-many relations}
%           {ERnonconceptual}
%In some \keyword{ER} variants,
%many-to-many relations are not allowed,
%% Bachman !! Bekijk ook Semantisch data model van Ter Bekke
%but need to be replaced by one-to-many relations.
%This process,
%graphically depicted in figure~\ref{ERnonconceptual},
%is explained by the fact that it facilitates
%the subsequent transformation of the ER schemata
%to \keyword{CODASYL} network structures.
%As such, this restriction
%is a clear example of a violation of the Conceptualization
%Principle.
%% Many-to-many relations are also not allowed
%% in the Semantic Data Model of~\cite{PhdThesis:91:Bekke}.
%
%The \keyword{Relational Model} (\cite{Article:70:Codd:RM})
%also violates the Conceptualization
%Principle as this technique is based on the notion
%of tables. 
%Tables are a particular kind of data structure,
%and therefore not on a conceptual level.
%
%%% Examples of complex application domains
%%% are, beside \keyword{meta-modeling},
%%% \keyword{hypermedia} and \keyword{CAD/CAM}.
%%% Modeling documents in the field of hypermedia or
%%% products in the field of CAD/CAM with contemporary
%%% data modeling techniques typically leads to overspecification.
%% van verificatieberekeningen
%% Voorbeeld: JSD action diagrams, hierin zit geen parallelliteit.
%% Op meta-niveau krijg je een aardig voorbeeld met een sequence type
%% maak een meta model in ER en laat het positie-probleem zien
%% is dat dan een conceptueel of een expressiviteitsprobleem ?
%\subsection{Expressive power}
%\label{ExprPower}
%The \Keyword{100 Percent Principle} (\cite{Report:82:ISO:Concepts})
%states that a conceptual model (or information model) should describe
%all relevant static and dynamic aspects of the Universe of Discourse.
%An information modeling technique should therefore be capable of modeling
%the data and process perspective of an application domain adequately.
%This implies that an information modeling technique
%should have sufficient \Keyword{expressive power}.
%
%\PostFigure{Jackson-Example}{9}
%           {An example of a JSD entity structure diagram}
%           {Jackson:Example}
%As an illustration of the notion of expressive power,
%consider the \keyword{JSD entity structure diagrams}[JSD?entity structure diagrams].
%In these diagrams, the central notion is {\em action\/}.
%An action can be an ordered sequence of other actions,
%it can be a choice between actions, an iteration of another
%action (zero or more times) or it can be an atomic action.
%As an example of an entity structure diagram consider figure~\ref{Jackson:Example}
%taken from \cite{Jackson83}.
%In this action diagram the actions {\em invest\/},
%{\em pay-in\/}, {\em withdraw\/} and {\em terminate\/}
%are atomic.
%The action {\em movement\/} represents a choice between the actions
%{\em pay-in\/} and {\em withdraw\/}.
%The action {\em customer body\/}
%consists of a number of {\em movements\/}. 
%Finally, the action {\em customer\/} first performs
%the action {\em invest\/}, then {\em customer body\/}
%and then {\em terminate\/}.
%% 
%% \PostFigure{Jackson-Overspec}{8}
%% 	   {Overspecification in JSD entity structure diagrams}
%% 	   {{Jackson:OverSpec}
%% Now suppose that we have an action {\em prepare document\/}
%% which consist of two (atomic) actions: {\em get address\/}
%% and {\em get document\/}.
%% The order in which these
%% actions have to be executed is irrelevant.
%% Modeling this situation with JSD entity structure diagrams would lead
%% to overspecification as the order in which the
%% atomic actions {\em get address\/} and {\em get document\/}
%% would have to be explicitly specified.
%% This would lead
%% to one of the diagrams depicted in figure~\ref{Jackson:OverSpec}.
%%
%
%Clearly, JSD entity structure diagrams correspond to \keyword{regular expressions},
%which have a very limited expressive power.
%A simple domain in which an action $c$ consists of first
%performing an action $a$ a number of times and then an action $b$
%the {\em same\/} number of times,
%cannot be modeled in JSD entity structure diagrams.
%The reason is that the language $\Set{a^nb^n}{n \in \N}$ is not
%regular (see e.g.~\cite{Book:81:Papadimitriou:ComputationalTheory}).
%Regular expressions are less powerful than
%\keyword{context-free grammars} which on their turn are less powerful
%than \keyword{Turing machines}[Turing machine].
%The \Keyword{Church-Turing Thesis} states that every computable
%function can be computed on a Turing machine (or alternatively:
%is recursive).
%
%\PostFigure{Yourdon-DFDExprPow}{5.5}
%	   {Process with input and output flows}
%	   {Yourdon:DFDExprPow}
%As another example consider the Yourdon
%data flow \keyword{diagram}[DFD]
%of figure~\ref{Yourdon:DFDExprPow}.
%Process {\em Report Production\/} has flows {\em order information\/}
%and {\em product information\/} as input and
%flows {\em monthly report\/} and {\em management report\/} as output.
%From this diagram it cannot be derived whether both {\em order
%information\/} and {\em product information\/} are necessary to
%produce a {\em monthly report\/} or a {\em management report\/}.
%This is caused by the fact that in data flow diagrams,
%it is not possible
%to express the precise input-output relations.
%To this end, the technique lacks expressive power.
%
%\PostFigure{ERproject}{8}
%	   {A simple ER diagram}
%	   {ER:Project}
%An example in the context of data modeling would be
%the situation of projects having coworkers and managers.
%In \keyword{ER} this could be modeled as in figure~\ref{ER:Project}.
%The constraint stating that a person cannot manage a project
%of which (s)he is a coworker, cannot be expressed in ER.
%Therefore, such constraints are
%usually expressed in natural language.
%
%Lack of expressive power might result in violations of
%the \keyword{Conceptualization Principle}.
%Choices that are not relevant
%with respect to the Universe of Discourse
%then might have to be made,
%leading to \Keyword{overspecification},
%or even worse, the Universe of Discourse might have to be adapted.
%As an illustration consider the \keyword{Relational Model}.
%As \cite{Kim:ECOOP} notes, the Relational Model
%cannot represent
%complex nested entities (e.g.\ compound documents).
%When an analyst attempts to represent such
%entities in a relational schema, 
%(s)he has to flatten them.
%Usually, several alternative ways of flattening are possible,
%therefore, an analyst has to choose.
%% Is dat werkelijk waar ????????
%This choice, however, is not relevant from a conceptual
%point of view and leads to overspecification.
%\subsection{Executable}
%Validating requirements as early as possible
%might prevent errors in later stages of systems development.
%As stated before,
%the later an error is detected the more it will
%cost to correct it.
%To make \keyword{validation} possible in the early phases of system
%development it is
%important that a specification can be executed.
%This enhances the understanding of
%the meaning of a specification and its implications considerably.
%Therefore, it is to be preferred that
%an information modeling technique
%yields \keyword{executable}[executability] models.
%Note that in order to be executable, a technique should
%be formal.
%A formal technique on the other hand, is not necessarily executable.
%\subsection{Comprehensible}
%Since one of the important roles of conceptual models
%is to reach a common understanding of the Universe
%of Discourse,
%not only between information analysts,
%but especially between domain experts and information analysts,
%it is vital that a conceptual model is {\em comprehensible\/}.
%While the previous requirement stated that an information model
%should be interpretable by a machine, this requirement
%states that it should be interpretable by human beings.
%In \cite{Report:90:Engels:ConcMod} it is stressed
%that languages for conceptual modeling should
%be {\em easy to use\/} and {\em easy to learn\/}.
%
%One way of achieving \keyword{comprehensibility} is by offering structuring
%mechanisms.
%In this way a specification remains surveyable.
%An often used structuring mechanism is decomposition.
%In Yourdon \Keyword{state transition diagrams} for example,
%a state in a state transition diagram may be decomposed into
%another state transition diagram.
%
%Often, comprehensibility is achieved by the use
%of graphical notations.
%Harel (\cite{Article:88:Harel:VisualForm}) emphasizes the
%importance of {\em visual\/} formalisms:
%\begin{quote} \em
%Visual, because they are to be generated, comprehended
%and communicated by humans,
%and formal, because they are to be manipulated,
%maintained, and analyzed by computers.
%\end{quote}
%In~\cite{Tse:ReqSpecLang} several reasons are given
%why a graphical representation is more comprehensible
%than its textual counterpart:
%\begin{enumerate}
%\item Graphics is in two dimensions,
%      while text is in one dimension.
%      The former gives an additional degree
%      of freedom in presentation.
%\item Graphics is more useful in showing the hierarchical
%      structure of complex systems and more natural in
%      describing parallelism.
%\item A person reading graphics can do so selectively,
%      depending on the level of details required.
%      If he reads text, he has to do so linearly.
%\item There is a limit to the number of concepts which
%      can be reasonably held in the short-term memory of
%      the human mind (\cite{Miller:CogCap}).
%      A person reading graphics can start off
%      generally and go down to detail
%      after some degree of familiarisation.
%      If one is reading text,
%      then one has to start off with detail and abstract
%      the skeleton concepts afterwards.
%\end{enumerate}
%Of course, it is not always possible, or desirable,
%to fully represent a specification graphically.
%In~\cite{Article:89:Creasy:ENIAM} extensions to NIAM
%are proposed that allow for the graphical specification
%of complex constraints.
%These extensions tend however to clutter
%the diagrams and make them hard to read.
%
%Finally, specifications should be in a style close
%to intuition.
%Specifications resembling natural language for example are
%close to the human intuition.
%An important presumption is then that
%the formal semantics is close to the
%intuitive semantics.

\QuestionsInChapter

%\begin{RecommendedReading}
%   \ReadingItem{1962-Austin-Word} Daarom!
%\end{RecommendedReading}

%\begin{OptionalReading}
%   \ReadingItem{2004-VeldhuijzenVanZanten-Rational} Eventueel
%\end{OptionalReading}

\ChapterBib


==> wsm02.tex <==
% The focus of WSM is on analysis of the design/structure of work-systems.
% Definition of (work) systems follows in RE. The context of ISE will be given
% in ADISE.

\Chapter{Work Systems}{work-systems}
\Version{30-01-06}

\Comment{Beter vooruitlopen op ons doel. Laat vast een ORM voorbeeld zien en
ontleed die in elementen, etc.}

\Xander{In} this chapter, we discuss our fundamental view on \PDN{work-system},
\PDN{organization} and \PDN{information-system}. We will provide a definition
of terms, which is based on a system theoretic~\cite{2001-Bertalanffy-GST}
foundation. 

\Comment{Discuss the idea that we are using DM approach to understanding OASs,
and ultimately IIO and/or IS. Repeat this (or move) discussion to next chapter.}

\section{Exploring systems}
Even though the notion of \DN{system} is, in an IT context, often equated to
`software \DN{system}', the original sense of the word is much broader. The
notion of \DN{system}\footnote{The term `\UDN{system}' is derived from the
Greek phrase `Syn histanai' ($\sigma\upsilon\nu$
$\acute{\i}\sigma\tau\eta\nu\alpha\iota$): `to put together'.} is also not
uniquely defined in the literature, but typically, it can be found explained
as: ``\emph{A collection of interrelated parts characterized by a boundary with
respect to its environment}''~\cite{1983-Iivari-Systemeering} or just as:
``\emph{A set of objects with a set of
\PDN{link}}''~\cite{1971-Langefors-InformationSystemsTheory}.  In general,
humans refer to all sorts of things as `\PDN{system}'.  The broadness of our
understanding of the concept of `\DN{system}' comes, for example, to the fore
in the definition as found in \cite{2003-Webster-Dictionary}:
\begin{quote}
   A regularly interacting or interdependent group of items forming a unified
   whole, as:
   \begin{enumerate}
      \item a group of interacting bodies under the influence of related forces,
      \item an assemblage of substances that is in or tends to equilibrium,
      \item a group of body organs that together perform one or more vital
      functions,
      \item the body considered as a functional unit,
      \item a group of related natural objects or forces,
      \item a group of devices or artificial objects or an organization forming
      a network especially for distributing something or serving a common
      purpose,
      \item a major division of rocks usually larger than a series and
      including all formed during a period or era, 
      \item a form of social, economic, or political organization or practice.
   \end{enumerate}
\end{quote}
The IEEE Recommended Practice for Architectural Description of
Software-Intensive Systems~\cite{1999-IEEE-Architecture} provides a
functionality-oriented perspective on systems:
\begin{quote}
   A collection of \PDN{component} organized to accomplish a specific function
   or a set of functions.
\end{quote}

In practice, most people intuitively agree on such simple definitions of
\PDN{system}. Apparently these definitions are broad enough to cover the
meaning of usual linguistic constructs where `\DN{system}' is used. But
\DN{system} is a much more difficult concept.  If we look at what in practice
are considered \PDN{system}, and if we really think about it, it becomes
obvious that some very important aspects of the \DN{system} concepts are
missing in the traditional definitions.  In \cite{1998-Lindgreen-FRISCO} some
examples are given of what we would, and would not, observe to be \PDN{system}
in our daily life: 
\begin{example} 
   One can regard an \DN{organization} or a bicycle as \PDN{system}. Also a
   Hitchcock film recorded on a video cassette, which is inserted in a video
   cassette player, which again is connected to a TV-set, could easily be
   interpreted as a \DN{system}. Nothing is unusual with such \DN{system}
   views, and they are well covered by the definitions. But if you buy some
   eggs from a farmer and use two of them for breakfast, then the \DN{domain}
   of obviously interrelated phenomena: You, the farmer, the farmers hen that
   laid the eggs, the frying pan you used to prepare the eggs, and the two eggs
   now in your stomach (and thereby in some transformed form a part of
   yourself) -- this \DN{domain} might probably not be regarded as a
   \DN{system}, because it might be difficult to see a purpose for that. But it
   fits the definitions.
   
   Or consider a single raindrop in an April shower: It consists of a vast
   number of water molecules, kept together by surface tension and constantly
   moving around among each other in a complicated manner controlled by a set
   of (thermo-) dynamic forces. Again according to the simple definitions
   above, the drop qualifies as a \DN{system}. But that is strange, because
   when you on your way back from the farmer, happen to get soaked in the
   shower, you might feel it is caused by raindrops -- not by \PDN{system}.
 
   On the other hand, a meteorologist studying possible weather situations that
   could cause rain, may see a purpose in regarding a raindrop as a \DN{system}
   in interaction with the surrounding atmosphere, but in most other situations
   a raindrop is just a raindrop.
\end{example}
However, when looking at what is regarded as a \DN{system} in practice, it
becomes apparent that some very important aspects of the \DN{system} concept
are missing from the traditional definitions.

In~\cite{1999-Ropohl-SocioTech} it is argued that, strictly speaking, there
exist three different interpretations of \PDN{system}:
\begin{description}
   \DefItem[Structural] The structural interpretation is known best.  According
   to this interpretation, a \DN{system} includes a set of \PDN{element} and a
   set of \PDN{link} between these \PDN{element}.  This interpretation complies
   with the ancient definition of the \emph{holon} by Aristotle. 

   \DefItem[Functional] The functional interpretation views a \DN{system} as an
   entity, sometimes called black box, which transforms inputs into outputs.
   Depending on specific internal states; the kind of transformation is called
   a function (in the descriptive meaning of the word). 

   %% Viewing a \DN{system} as a service providing entity!!

   \DefItem[Hierarchical] The structural interpretation turns into the
   hierarchical interpretation, if (some of) the constituting \PDN{element} are
   regarded as subsystems. Concluding by analogy, the original \DN{system} may
   be considered as a subsystem of a more extensive supersystem.
\end{description}

% Kun je die laatste niet beter weglaten? Is die wel nodig??

% En in beide gevallen bestaat een systeem uit elements. De ene keer van de
% binnenkant, en de andere keer van de buitenkant.

%%%%% Moeten we geen brug slaan tussen domain en situatie a la Barwise/Devlin
%en Wisse????

\section{Observing systems}
The aim of this section is to more precisely define the concept of \DN{system},
also giving more foundation to our earlier definitions of \DN{work-system},
\DN{organizational-system}, and \DN{information-system}.

\subsection{Subjectivity}
% Gebruik onderwijs/universiteit als voorbeeld voor "wat is het systeem".
% Subjectiviteit: ook de context van de viewer als reden voor subjectiviteit
% meenemen.

When two people discuss a \DN{system}, do they really mean the same
\DN{system}?  One serious cause for confusion in our professional domain is,
that people, usually, think about a \DN{system} as something that can be
objectively determined, for example by a specification of its parts and their
relationships, as the above quoted definitions may indicate. But even then, the
problem remains. Are both people indeed discussing the same \DN{system}?

As an example take the simple domain of a car and its driver in the traffic of
a city.  One person may see it as a useful transport \DN{system} in action,
which is able to move large objects from one location to another in a
convenient way.  The driver alone cannot, nor can the car, but in combination
they can.  However, a policeman on his job will regard the same domain
differently -- as a controllable \DN{system} which behavior can be directed by
road regulations, traffic lights, arm signals and by certain traffic rules.
Again, an environmental activist would probably regard the car as a dangerous
polluting system, which is a potential cause of injury or death to persons in
the traffic.

Here we have three views of the same domain, but with quite different sets of
properties. All three persons could in fact be the same viewer of the same
system, e.g.\ a transport conscious public servant caring about the conditions
for people in the city, who just conceives different properties by regarding
the same \DN{system} from different points of view.

Let us elaborate this car example a little further in order to illustrate the
difficulties we face when we regard something as a \DN{system}.  Consider for
example the question about which parts and which activities are involved in the
possible system view:  Are the driver and the car two interacting
\PDN{sub-system} -- one with the property of being able to observe the traffic
and to control the car, and the other with the property of being able to
transform chemical energy into movement in a controlled manner.  Or is the car
to be regarded as a single \DN{system} with the driver, motor, gear, and
steering devices as \PDN{sub-system} each with their own properties? Is the
motor the active part and the chassis a passive component, or is it the other
way around -- the car as a device transporting among other things the motor.
Quite another view -- but still one from the same domain -- could be to regard
the car as a moving cage of Faraday protecting the driver from certain kinds of
dangerous electrical fields.  There are many possible \DN{system} views, and
still the domain is extremely simple compared with the organizational domains
usually considered as \PDN{system}.

If we regard a business enterprise, an institution or any other kind of
organization as a \DN{system} -- an organizational \DN{system} -- we have a
domain which is much more complicated than a car and driver.  Furthermore, the
number of possible views of an organization is most often enormous.

Key to understanding the \DN{system} concept, and ultimately \PDN{organization}
is therefore to realize that a \DN{system} is a subjective phenomenon.  In
other words, it is not an absolute or objective thing. \UPDN{system} are not a
priori given.  As Checkland~\cite{1981-Checkland-SystemThinking} expresses it,
there must be a describer/observer who conceives or thinks about a part of the
world as a \DN{system}.  In other words, it is important, that there is a
\emph{\DN{viewer}} who can see a purpose in regarding some `\emph{set of
\PDN{element}}' as a \DN{system}.  

\UPDN{viewer} may also be regarded at an aggregated level.  For example, a
\emph{single} business manager, observing an \DN{organization}, is indeed a
viewer, but the \emph{collective} business management can be seen as a
\DN{viewer} of the \DN{organization} as well.

The purpose in regarding some \emph{set of \PDN{element}} as a
\DN{system} should be expressed in terms of at least one meaningful \PDN{link}
between the \emph{set of \PDN{element}} and its \emph{\DN{environment}}.
Such a \DN{link} is called a \emph{\DN{systemic-property}}.  It is a property
the \DN{viewer} associates with the \emph{set of \PDN{element}} they experience
as a \DN{system}. One \DN{viewer} may regard the \emph{set of \PDN{element}} as
a \DN{system} having one set of \PDN{systemic-property}, while another
\DN{viewer} may see other \PDN{systemic-property} concerning the same set of
\PDN{element}. 

Most often, the \PDN{systemic-property} of a \DN{system} cannot be attributed
exclusively to any of its constituent \PDN{component}. For example, none of the
constituent parts of a train has the exclusive `train property'. A separate
carriage is not a train. A locomotive on its own is (from the perspective of a
passenger) also not a train.  Together, however, the parts do have the `train
property'.  In other words, the whole is more than just the collection of its
parts.  The farmer-you-frying-pan-eggs-hen situation as discussed in the above
example, is a situation which may not constitute a `whole' with any sensible
\DN{systemic-property}.  In which case we will not consider it to be a
\DN{system}. In the case of the train, we have an interesting situation if the
train consists of two connected train-sets. In this case, each of the
individual train-sets still has the `train property'.

In order for us to gain a fundamental understanding of \PDN{system}, and
ultimately the kind of systems we refer to as \PDN{organization}, we first need
to introduce some core concepts, most of which are based on the ones found in
\cite{1998-Lindgreen-FRISCO}.

\subsection{Observing the universe}
Let us start by considering what happens if some \DN{viewer} observes `the
\DN{universe}'.  It is our assumption, based on the work of C.S.\
Peirce~\cite{1969-Peirce-Collection1, 1969-Peirce-Collection2,
1969-Peirce-Collection3, 1969-Peirce-Collection4}, that \emph{\PDN{viewer}}
perceive a \emph{\DN{universe}}, leading to a \emph{\DN{perception}} of this
\DN{universe} and then produce a \emph{\DN{conception}} of that part they deem
relevant.  Peirce argues that both the \DN{perception} and \DN{conception} of a
\DN{viewer} are strongly influenced by their \DN{interest} in the observed
\DN{universe}. This leads to the following (necessarily cyclic, yet
irreflexive) set of definitions:
\begin{Definitions}
   \DefinitionItem{universe}
   \DefinitionItem{viewer}
   \DefinitionItem{perception}
   \DefinitionItem{conception}
\end{Definitions}
In general, people tend to think of the universe as consisting of
\PDN{element}.  In~\cite{1998-Lindgreen-FRISCO} this approach is indeed taken.
In our view, presuming that the \DN{universe} consists of a set of
\PDN{element} constitutes a subjective choice, which essentially depends on the
\DN{viewer} observing the \DN{universe}. Nevertheless, taking this assumption
has proven to be a sensible assumption, in particular in the context of
\PDN{system}.  However, we do \emph{not} presume the \emph{\DN{universe}}
itself to consist of elements, but \emph{rather} the \emph{\DN{conception}} of
a \DN{universe}.  This makes the identification of \PDN{element} relative to a
\DN{viewer}.  

The \PDN{conception} harbored by a \DN{viewer} are impossible to communicate
and discuss with other \PDN{viewer} unless they are articulated somehow.  In
other words, a \DN{conception} needs to be \emph{described} somehow in terms of
a \DN{description}:\footnote{In \cite{1998-Lindgreen-FRISCO} the term
\emph{representation} is used rather than the term \emph{\DN{description}} as
it is used here.  We have chosen to favor the term \emph{\DN{description}}, as
it is the term of choice of \cite{1999-IEEE-Architecture}.}
\begin{Definitions}
   \DefinitionItem{description}
\end{Definitions}

The resulting situation is illustrated in \SmartRef{description}.
\Image{13cm}{
  A viewer, having a conception of the universe, and describing this in terms
  of a description.
}{description} 
\UPDN{description} may be:
\begin{itemize}
  \item Formal or informal
  \item Complete or incomplete
  \item More refined/less refined
%  \item See also the "Architecture Documentation" stuff from SEI
\end{itemize}
A system description may have a formal semantics, in mathematical terms, and will
also have an intensional (pragmatics!) semantics. Formal semantics is needed
when approaching design. The latter is likely to be of more use when
communicating with different stakeholders.

The underlying relationships between \DN{viewer}, \DN{universe},
\DN{conception} and \DN{description} can be expressed in terms of the so-called
FRISCO tetrahedron \cite{1998-Lindgreen-FRISCO}, as depicted in
\SmartRef{tetrahedron}\footnote{The original FRISCO tetrahedron uses
`\DN{domain}' where we use `\DN{universe}'. This difference is due to the
above, more refined, discussion on the subjectivity of viewing the
\DN{universe} as a set of \PDN{element}.}.
\Image{8cm}{The (revised) FRISCO tetrahedron.}{tetrahedron}

\subsection{Conceptions}
To express the above discussions more formally, let
\SymbolDefinition{Universes}\footnote{The reader is advised that
appendix~\ref{ch:Math} provides an overview of the mathematical
notations/conventions used in this textbook.} be the set of \PDN{universe} that
may be observed, and let \SymbolDefinition{Viewers}\footnote{One should
actually regard this set as the set of \emph{states} a \DN{viewer} may have. A
\DN{viewer} may for example have, in differing states, different \PDN{interest}
with which they conceive the \DN{universe}. The elements from $\Viewers$ should
really be regarded as the states of these \PDN{viewer}.} be the set of all
possible \PDN{viewer}.  Let furthermore, \SymbolDefinition{Elements} be the set
of \PDN{element} that may be part of \PDN{conception}.  These basic sets should
be disjoint: 
\begin{Axiom}{S}
  $\Viewers$, $\Universes$ and $\Elements$ are mutually disjoint.
\end{Axiom}
Let \SymbolDefinition{Conception} be the \PDN{link} expressing which
\DN{conception} is held by which \DN{viewer}. The fact that a \DN{viewer} $v
\in \Viewers$ harbors a \DN{conception} $C \subseteq \Powerset(\Elements)$ for
\DN{universe} $U \in \Universes$ can be expressed as $\Conception{U}{v}{C}$.
This situation is depicted more graphically in \SmartRef{painting1}. A viewer,
when observing a domain, draws a picture of the observed universe (their
\DN{conception}). In painting this picture of the world, they will use certain
`constructs'. At the moment the only constructs we presume to exist are
\emph{\PDN{element}}.  Note: the fact that \PDN{viewer} can change their
\DN{conception} over time is ignored for the moment.
\Image{6cm}{Painting a picture of the universe}{painting1}

% We take a pragmatic approach to the `ontology' of a viewer. We will only
% make distinctions in the kinds of things they see if we have a need to do so.

\subsubsection{Domains and their environments}
A \DN{viewer} may zoom in on a particular part of the \DN{universe} they
observe, or to state it more precisely, they may zoom in on a particular part
of their conception of the universe. 
\begin{Definitions}
  \DefinitionItem{domain}
\end{Definitions}
When reasoning about \PDN{system}, which we will regard as a particular class
of \PDN{domain}, it is commonplace to also identify their
\PDN{environment}~\cite{2001-Bertalanffy-GST}.  Even more, the very definition
of a \DN{system} depends on our ability to distinguish it from its
\DN{environment}. This is illustrated in \SmartRef{painting2}.
\Image{6cm}{Identifying a domain and its environment}{painting2}

To be able to define the \DN{environment} of a \DN{domain} in general and a
\DN{system} in particular, however, we must first be able to define the direct
\DN{environment} of a \DN{domain}. Formally, a \DN{domain} $D$ can be regarded
as a subset of a \DN{conception} $C$, in other words a sub-\DN{conception} $D
\subseteq C$. If $\Conception{U}{v}{C}$ and $D \subset C$ is some \DN{domain}
within $C$, then the \DN{environment} of $D$ will not generally be $C \SetMinus
D$ as a whole, but rather a subset $E \subseteq C \SetMinus D$. For $E$ to be a
sensible \DN{environment} of \DN{domain} $D$, the \PDN{element} in $E$ must
have some \PDN{link} to the \PDN{element} in $D$. In order to more precisely
define the notion of \DN{environment}, we should therefore first refine our
notion of \PDN{element} of a \PDN{conception}.  There are really two types of
\PDN{element}: \PDN{concept} and \PDN{link} connecting the \PDN{concept}.  We
will define these notions as follows:
\begin{Definitions}
   \DefinitionItem{element}
   \DefinitionItem{concept}
   \DefinitionItem{link}
\end{Definitions}
The distinction between a \DN{link} and an \DN{concept} for the \PDN{element}
of a given \DN{conception}, may not always be that clear, as the distinction is
rather \emph{subjective}.  It all depends, to no surprise, on the \DN{viewer}
of a \DN{domain}.

Let \SymbolDefinition{Concepts} be the set of \PDN{concept} and let
\SymbolDefinition{Links} be the set of \PDN{link}.  These sets should form a
partition of $\Elements$:
\begin{Axiom}{S}
   $\Concepts \intersect \Links = \emptyset$ ~and~ $\Elements = \Concepts \union \Links$.
\end{Axiom}
In terms of \SmartRef{painting2}, our viewer can now select from two classes of
\PDN{element}: \PDN{concept} and \PDN{link}. This is depicted in
\SmartRef{painting3}. In the next chapter, we will provide an even more refined
view on the classes of \PDN{element} we identify.  
\Image{6cm}{Painting a more refined picture of the observed domain}{painting3}

If $X \subseteq \Elements$, then we will use the following abbreviations:
\[ \SymbolDefinition{ConceptsSubset} \mbox{~and~} \SymbolDefinition{LinksSubset} \]
\UPDN{link} run between \PDN{concept}. We furthermore presume functions
\SymbolDefinition{From} and \SymbolDefinition{To} to exist, providing the
source and destination of these \PDN{link} respectively. As an abbreviation we
will use:
\[ \SymbolDefinition{Involved} \]
to select the \PDN{concept} involved in a \DN{link}, and:
\[ \SymbolDefinition{LinkedTo} \]
to represent the fact that a concept $e$ is connected to concept $f$. 

A \DN{conception} $C$ is considered to be closed iff: 
\[ \Al{r \in \LinksSub{C}}{\Involved(r) \subseteq C} \] 
\UPDN{conception} of \PDN{viewer} should indeed be closed:
\begin{Axiom}{S}\Label{closed-conception}
   If $\Conception{U}{v}{C}$, then $C$ is closed.
\end{Axiom}

\SmartRef{ontology1} provides a model, our ontology, of the classes of elements
which a conception may consist of and their mutual relationships. The notation
we have used there is the ORM (Object-Role
Modeling)~\cite{2001-Halpin-ORM}\footnote{We have used the extension introduced
in~\cite{1995-Halpin-ORMPoly} to signify that \SF{Concept} and \SF{Link}
are really self-defining subtypes, i.e.\ not requiring a dedicated subtype
defining rule.} notation, which is the same notation as used in the
\emph{Domain Modeling} course.  
\Image{8cm}{The ontology of a viewer's conception}{ontology1}

%%% Na een Visio migratie deze eventueel anders tekenen!!

A conception $C$ which is closed under $\Links$ can essentially be regarded as
a graph:
\[ \tuple{\ConceptsSub{C},\LinksSub{C},\From,\To} \]  
A conception $C$ is called connected iff the associated graph is connected. A
conception is required to be a connected graph:
\begin{Axiom}{S}\Label{connected-conception}
   If $\Conception{U}{v}{C}$, then $C$ is connected.
\end{Axiom}
Note: if a conception would not be a connected graph, it would be a conception
of multiple universes.

We generalise $\From$ and $\To$ to sets of \PDN{link} as follows:
\begin{eqn}
   \From(L) \EQ \Set{\From(l)}{l \in L}\\
   \To(L)   \EQ \Set{  \To(l)}{l \in L}
\end{eqn}

We are now in a position to properly define the \DN{environment} of a \DN{domain}:
\begin{Definitions}
   \DefinitionItem{environment}
\end{Definitions}

%
% Eigenlijk pijlen gebruiken in de voorbeelden van
% concepties!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
% In plaats van lijnen.
%

Formally, we view a \DN{domain} $D$ and an \DN{environment} $E$ as being a
subset of a \DN{conception} $C$, in other words a sub-\DN{conception} $D, E
\subseteq C$. Let \SymbolDefinition{DomainInEnvironment} now be the relation
expressing which \DN{domain} and \DN{environment} a \DN{viewer} conceives. The
fact that a \DN{viewer} $v$ harbors a \DN{conception} of \DN{domain} $D$ and
\DN{environment} $E$ for \DN{universe} $U$ can be expressed as
$\DomainInEnvironment{U}{v}{C}{E}{D}$. This \DN{link} should limit itself to
the \PDN{conception} held by \DN{viewer} $v$: 
\begin{Axiom}{S}
   If $\DomainInEnvironment{U}{v}{C}{E}{D}$, then $\Conception{U}{v}{C}$ and
   $E, D \subseteq C$.
\end{Axiom}
A \DN{domain} and its \DN{environment} should not overlap:
\begin{Axiom}{S}\Label{non-overlapping-domain-environment}
   If $\DomainInEnvironment{U}{v}{C}{E}{D}$, then $E \intersect D = \emptyset$.
\end{Axiom}
The \DN{domain} and \DN{environment} should be closed:
\begin{Axiom}{S}\Label{closed-domain}
   If $\DomainInEnvironment{U}{v}{C}{E}{D}$, then $D$ is closed.
\end{Axiom}
\begin{Axiom}{S}\Label{closed-domain-environment}
   If $\DomainInEnvironment{U}{v}{C}{E}{D}$, then $E \union D$ is closed.
\end{Axiom}
A \DN{domain} should be connected:
\begin{Axiom}{S}
   If $\DomainInEnvironment{U}{v}{C}{E}{D}$, then $D$ is connected.
\end{Axiom}
The combination of a \DN{domain} and its \DN{environment} is connected as well:
\begin{Axiom}{S}\Label{connected-domain-and-environment}
   If $\DomainInEnvironment{U}{v}{C}{E}{D}$, then $D \union E$ is connected.
\end{Axiom}
Note that an environment does not have to be connected!

\UPDN{concept} in the \DN{environment} are related somehow to \PDN{concept} in
the \DN{domain}:
\begin{lemma}\Label{related-environment}
   Let $\DomainInEnvironment{U}{v}{C}{E}{D}$ with a non-empty environment $E$.
   If $P$ is a \emph{maximum}\footnote{In other words, there is no $P'$ such
   that $P \subset P' \subseteq E$ while $P'$ is still connected.} subset of
   $E$ such that it is connected, then:
   \[ \Ex{e \in \ConceptsSub{P}, r \in \LinksSub{E}, d \in \ConceptsSub{D}}{
         \setje{e,d} = \Involved(r) } 
   \] 
\end{lemma}
\ReaderProof

The authors of \cite{1998-Lindgreen-FRISCO} also define the notions of
\DN{domain} and \DN{environment}. However, they do not take the subjectivity
with regards to viewing the \DN{universe} as a set of \PDN{element}  into
consideration.  As a result, they define \DN{domain} and \DN{environment} as
being parts of the \emph{universe} as opposed to being parts of a viewer's
conception of the universe. 

In the remainder of this book, we will use the phrase: \emph{a \DN{viewer} $v$
observing a \DN{domain} (of \DN{interest}) $D$ (with \DN{environment} $E$)} as
an abbreviation for: \emph{a \DN{viewer} $v$ having a \DN{conception} of the
\DN{universe}, zooming in on \DN{domain} $D$ (with \DN{environment} $E$)}.

\subsubsection{Decomposition of conceptions}
When a \DN{viewer} conceives a \DN{domain}, we presume there to be an
\DN{concept} in their \DN{conception} representing the \emph{whole} of the
\DN{domain} as well as one representing the \emph{whole} of the environment.
The same applies to the \DN{universe}.  In other words, the \PDN{concept} in
the \DN{domain} and the \DN{environment} can be regarded as decompositions of
entities representing the whole of the \DN{domain} and \DN{environment}, while
these latter \PDN{concept} are decompositions of another \DN{concept}
representing the \DN{universe} as a whole. This is illustrated in
figure~\ref{decomposition1}.
\Image{4cm}{Decomposition of the universe}{decomposition1}

This `decomposition game' can be played repeatedly. When viewing a
\DN{domain} a \DN{viewer} may decide to zoom in further into a specific part of
this \DN{domain}. For example, when observing an insurance claim-handling
process, involving amongst other things an evaluation of the claim, one may
decide to zoom in closer into the actual evaluation process. This has been
illustrated in figure~\ref{decomposition2}.
\Image{4cm}{Decomposition of a part of a domain}{decomposition2}

The fact that one \DN{concept} is in the `decomposition' of another
\DN{concept} really means that there is a \DN{link} between them in the
\DN{viewer}'s \DN{conception}. This has been illustrated in
figure~\ref{decomposition3}. This really implies we need to identify a specific
class of \PDN{link} called \PDN{decomposer}. Let us therefore presume we have a
set: \SymbolDefinition{Decomposers} of \PDN{link}.
\Image{4cm}{Decomposer relationships}{decomposition3}

To more easily reason about decompositions within a conception, we will
introduce the derived relationship $\SymbolDefinition{DecomposedInto}$. If
$\DecomposedInto{x}{C}{y}$, the \DN{concept} $x$ in \DN{conception} $C$ is
decomposed into (possibly amongst others) \DN{concept} $y$. This relationship
is defined (precisely) by the two following (recursive) derivation rules:
\[ \begin{array}{llll}
  1: & \Ex{d \in \DecomposersSub{C}}{x = \From(d) \land y = \To(d)} 
     & \vdash & \DecomposedInto{x}{C}{y} \Eol
  2: & \DecomposedInto{x}{C}{y} \land \DecomposedInto{y}{C}{z}
     & \vdash & \DecomposedInto{x}{C}{z}
\end{array} \]
The decompositions should be acyclic:
\begin{Axiom}{S}\Label{acyclic-decompositions}
   $\DecomposedInto{x}{C}{y} \implies x \neq y$
\end{Axiom}
As an abbreviation we introduce: \SymbolDefinition{DecomposedIntoEq}.

To enforce the fact that a \DN{viewer}'s \DN{conception} of a \DN{universe}
consists of one `top' \DN{concept} representing the \DN{universe} as a whole,
we require:
\begin{Axiom}{S}\Label{conception-has-top}
   If $\Conception{U}{v}{C}$, then: 
   $\ExAl{u \in \ConceptsSub{C}}{x \in \ConceptsSub{C}}{\DecomposedIntoEq{u}{C}{x}}$
\end{Axiom}
Even more, the $u \in C$ is unique:
\begin{corollary}\Label{unique-top}
   If $\Conception{U}{v}{C}$, then: 
   $\EuAl{u \in \ConceptsSub{C}}{x \in \ConceptsSub{C}}{\DecomposedIntoEq{u}{C}{x}}$
\end{corollary}
\ReaderProof
Similarly, for \PDN{domain} and \PDN{environment} we have:
\begin{Axiom}{S}\Label{domain-has-top}
   If $\DomainInEnvironment{U}{v}{C}{E}{D}$, then: 
   $\ExAl{d \in D}{x \in \ConceptsSub{D}}{\DecomposedIntoEq{d}{D}{x}}$
\end{Axiom}
\begin{Axiom}{S}\Label{environment-has-top}
   If $\DomainInEnvironment{U}{v}{C}{E}{D}$, then: 
   $\ExAl{e \in E}{x \in \ConceptsSub{E}}{\DecomposedIntoEq{e}{E}{x}}$
\end{Axiom}
\SmartRef{unique-top} applies to each of these as well. So for $C$, $D$ and $E$
there are unique tops in the hierarchies.  This unique \emph{top} \PDN{element}
will be referred to as $\Top(C)$, $\Top(D)$ and $\Top(E)$ respectively. For
these tops, we should have:
\begin{Axiom}{S}
   If $\DomainInEnvironment{U}{v}{C}{E}{D}$, then: 
   $\Eu{d \in \DecomposersSub{C}}{\Top(C) = \From(d) \land \Top(E) = \To(d)}$ 
\end{Axiom}
\begin{Axiom}{S}
   If $\DomainInEnvironment{U}{v}{C}{E}{D}$, then: 
   $\Eu{d \in \DecomposersSub{C}}{\Top(C) = \From(d) \land \Top(D) = \To(d)}$ 
\end{Axiom}
\begin{Axiom}{S}
   If $\DomainInEnvironment{U}{v}{C}{E}{D}$, then: 
   $\Eu{r \in \LinksSub{C} \SetMinus \DecomposersSub{C}}{\Top(D) = \From(d) \land \Top(E) = \To(d)}$ 
\end{Axiom}
These three axioms require the top part of a conception to have the structure
as depicted in \SmartRef{decomposition3}.

% Voor 2006: x,y \in decomposition, and x -[r]-> y dan zit r als rel ook in de decomposition. Iets mee doen.

By adding the set of \PDN{decomposer}, we have now enriched our ontology to the
situation as depicted in figure~\ref{ontology2}. Note that the asterisk (*)
attached to the \mbox{\sffamily \small is decomposed into} relationship
signifies this to be a derived relationship. 
\Image{8cm}{Ontology refined with decomposers}{ontology2}

\subsection{Model}
In the context of \PDN{organization}, we are not interested in all types of
\PDN{conception}. Our interest is limited to those \PDN{conception}, that may
be referred to as a \emph{\DN{model}}:
\begin{Definitions}
  \DefinitionItem{model}
\end{Definitions}
As a \DN{model} is a \DN{conception}, it also consists of \PDN{element}, which
can be specialized further into \PDN{concept} and \PDN{link}:
\begin{Definitions}
  \DefinitionItem{model-element}
  \DefinitionItem{model-concept}
  \DefinitionItem{model-link}
\end{Definitions}
We are now also in a position to define more precisely what we mean by
\emph{\DN{modeling}}:
\begin{Definitions}
  \DefinitionItem{modeling}
\end{Definitions}
For practical reasons, we will understand the act of \emph{\DN{modeling}} to
also include the activities involved in the \emph{\DN{description}} of the
\DN{model} by means of some language and medium. 

To represent the fact that some \DN{viewer} produces a \DN{model} in an
\DN{environment} when they observe some part of the \DN{universe}, we introduce
the relation:
\[ \SymbolDefinition{ModelInEnvironment} \]
Formally, the fact that a \DN{viewer} $v$ views the \DN{universe} $U$ and in
doing so has a conception $C$ including a \DN{model} $M$ with environment $E$
is represented by: $\ModelInEnvironment{U}{v}{C}{E}{M}$. Every \DN{model} is a
\DN{conception}. We should therefore have:
\begin{Axiom}{S}\Label{model-as-domain}
   If $\ModelInEnvironment{U}{v}{C}{E}{M}$, then
   $\DomainInEnvironment{U}{v}{C}{E}{M}$.
\end{Axiom}
\begin{corollary}
   If $\DomainInEnvironment{U}{v}{C}{E}{M}$, then 
   $\Conception{U}{v}{C}$.
\end{corollary}
\ReaderProof
Note that not all \PDN{conception} of a \DN{domain} produce \PDN{model}. So the
reverse of the above axiom does \emph{not} hold!  As an abbreviation we also
introduce: 
\[ \SymbolDefinition{ModelConception} \]

\subsection{System}
Using the above general definitions, we can, in line
with~\cite{1998-Lindgreen-FRISCO}, more precisely define the way we view
\PDN{system}:
\begin{Definitions}
  \DefinitionItem{system-domain}
  \DefinitionItem{systemic-property}
  \DefinitionItem{system-viewer}
  \DefinitionItem{system}
  \DefinitionItem{system-description}
\end{Definitions}
The \PDN{element}, \PDN{concept} and \PDN{link} concepts can be further
specialized to \PDN{system}:
\begin{Definitions}
  \DefinitionItem{system-element}
  \DefinitionItem{system-concept}
  \DefinitionItem{system-link}
\end{Definitions}
As identified in \cite{1998-Lindgreen-FRISCO}, there is a potential objection
against our subjectivity-based definition of \DN{system}.  In daily life, it is
quite sensible to talk about ``designing, constructing and implementing a
\DN{system}'' or ``to interact with a \DN{system}''.  The use of the terms
`\DN{system}' gives associations to this term as denoting something that can be
interacted with in a rather concrete way and not just as a \DN{conception}.
These associations, however, do not lead to any inconsistencies.  These example
phrases are simply convenient abbreviations for more elaborate expressions. For
instance, ``to interact with a \DN{system}'' really means:
\begin{quote} \it
   to interact with phenomena in the \DN{system-domain} that is conceived as a
   \DN{system} (because of its \PDN{systemic-property}).
\end{quote}
To ``design, construct and implement'' a \DN{system} really means:
\begin{quote} \it
   to bring together and structure phenomena in a particular part of the world
   (which then becomes the \DN{system-domain}) with the purpose of constructing
   them such that they together have certain \PDN{systemic-property}.
\end{quote}

To represent the fact that some \DN{viewer} `sees' a \DN{system} in an
\DN{environment} when they observe some part of the \DN{universe}, we introduce
the relation:
\[ \SymbolDefinition{SystemInEnvironment} \]
Formally, the fact that a \DN{viewer} $v$ views the \DN{universe} $U$ and in
doing so has a conception $C$ including a \DN{system} $S$ with environment $E$
is represented by: $\SystemInEnvironment{U}{v}{C}{E}{S}$. Every \DN{system} is
a \DN{model}. We should therefore have:
\begin{Axiom}{S}\Label{system-as-model}
   If $\SystemInEnvironment{U}{v}{C}{E}{M}$, then
   $E \neq \emptyset$ and $\ModelInEnvironment{U}{v}{C}{E}{M}$.
\end{Axiom}
Note that not all \PDN{conception} of a \DN{domain} produce \PDN{model}. So the
reverse of the above axiom does \emph{not} hold! As an abbreviation we also
introduce:
\[ \SymbolDefinition{SystemConception} \]

In our informal exploration of the concept of \DN{system}, we already discussed
that there are three major ways of viewing
\PDN{system}~\cite{1999-Ropohl-SocioTech}: \emph{structural}, \emph{functional}
and \emph{hierarchical} (as a specific class of structural). A major difference
between a structural and a functional perspective is the distinction between
the white-box and black-box approach when regarding \PDN{system}. In other
words, is one looking \emph{inside} the \DN{system} (white-box) or is one only
looking at the \emph{outside} of the \DN{system}. This does seem to raise the
question whether, when viewing a \DN{system} as a black-box, one can still
argue that the \DN{system} consists of \PDN{element}? The answer to this
question is a resounding \emph{yes}. When a \DN{viewer}, for some reason, views
a \DN{domain} as a \DN{system}, and does so using a black-box approach, that
what they conceive of as being a \DN{system} is still a \DN{conception}
consisting of \PDN{element}.  The difference between a white-box and a
black-box approach when viewing a \DN{system}, however, is in the \PDN{concept}
and \PDN{link} one will see. When taking a black-box approach, one will only
see the external behavior of the \DN{system}, while when taking the white-box
approach one will see the internal structure/behavior of the \DN{system} as
well.

\section{Studying systems}
In order to really to understand the concept system it is necessary to be aware
of a number of important aspects:
\begin{itemize}
   \item that the system domain always comprises several elements,
   \item that all elements are related to each other such that it constitutes a
   transitively coherent whole,
   \item that the whole is conceived to have at least one systemic property,
   \item that it is only relevant to incorporate a thing as an element of the
   particular system domain if in the system view it somehow contributes to the
   systemic property,
   \item that when viewing a thing as an element of a system domain then only
   those aspects of the thing that directly or indirectly contributes to the
   systemic properties are relevant for the system view.
\end{itemize}

\subsection{Sub-systems}
To gain a better understanding of complex \PDN{system} it has proven to be
useful to identify smaller-scale \PDN{system} within a larger \DN{system},
leading to \DN{sub-system}. A detailed discussion on dealing with complexity by
\PDN{system} in general, and the role played by hierarchical decomposition, may
be found in e.g.\ \cite{1962-Simon-ComplexArch}. In this textbook, for example,
\PDN{information-system} will be positioned as \PDN{sub-system} of
\PDN{organizational-system}. 

However, when it comes to the point of being less intuitive and more explicit
about the concept, there is little consensus about what really characterizes a
\DN{sub-system} -- or rather what should characterize it, if the concept is to
be a useful one. The influence from the absoluteness of the `classical'
\DN{system} concept together with some apparent preference to associate the
understanding of \DN{sub-system} with the subset concept seem to be the main
cause of the confusion.

The `old', simple interpretation of the concept \DN{system} as being just `a
set of interrelated parts', made it rather obvious to think of \DN{sub-system}
as:  A subset of the parts together with an appropriate subset of their mutual
relationships. However, with the introduction of the notion that in order for
something to be a \DN{system}, it must have at least one
\DN{systemic-property}, the matters became more difficult:  Should the
definition of \DN{sub-system} then also involve the specification of a subset
of the \PDN{systemic-property}?  Intuitively this notion could be reasonable,
and it may even work in some cases, but the problem is that this is not always
so.  Consider, for example, a well-functioning mechanical watch. It can be
conceived to have the \DN{systemic-property} that under certain conditions it
`shows the time'.  A possible \DN{sub-system} of such a watch is the energy
supplying device for the clockwork consisting of the spring, the winding knob,
the exchange and click mechanism for tightening the spring, and a part of the
frame to support these mechanical parts.  The only sensible
\DN{systemic-property} of such a \DN{sub-system} is that it serves as a storage
of mechanical energy.  But then we have a serious problem with the subset
notion applied on the \DN{systemic-property}, because being an energy storage
is in no way a subset of the \DN{systemic-property} of showing the time.

The problem of defining a sensible \DN{sub-system} concept by means of subset
relationships becomes even more difficult with the notion of a \DN{system} as a
subjective issue. Apart from the \PDN{systemic-property} not being absolute,
but rather depending of the \DN{viewer}, one element in the \DN{system-domain}
may now also potentially be viewed as several different \PDN{component} in the
\DN{system}.  Consider, for example, an \DN{organization} that is viewed as an
and a person from that \DN{organization}:  Here the person may appear as an
\DN{actor} of the type \SF{salesman} that is the agent of various sales
activities.  But independent hereof, the same person may also be conceived as
having the type \SF{employee} relevant in connection with calculations of
salaries and the planning of sales campaigns.  The person may even be regarded
as being of type \SF{transportable object} in the context of an activity
\SF{transport by car during sales trips}.  This causes the following question:
Should a possible subset relationship applied in attempts to define a
\DN{sub-system} concept then refer to the \DN{domain} alone, or to the
\DN{system} alone, or to both?  It is certainly difficult to find logical or
pragmatic arguments that universally justify any of these choices.  (For
further aspects of the problems encountered when one is aiming at defining
\DN{sub-system} by means of subsets, see the more comprehensive discussion
in~\cite{1998-Lindgreen-FRISCO}.)

It is necessary to consider the \DN{sub-system} concept differently -- in fact,
in a way that very well is in accordance with the way people intuitively apply
it in practice.  The `solution' is to realize that when viewing something as a
\DN{system} then only one \DN{system} should be considered at a time.  Applied
here, either one must consider that which is regarded as the \DN{system} or
that which is regarded as the \DN{sub-system}. The advantage of this
\DN{sub-system} interpretation is exactly what appears to be the main positive
feature of the intuitively applied concept:  Depending on which level of detail
as regard potential \PDN{component} you want to consider, you can use the
concept to encapsulate unnecessary details on a chosen level of abstraction.
Applied to \PDN{organization} one obvious way to consider the relationship
between an \DN{organization} and a \DN{sub-system} of it, is to conceive the
\DN{sub-system} equivalent with what an \DN{actor} in the \DN{organization}
does (or a part of that). Typically a whole department (a possible \DN{system}
candidate in itself) may be considered a single \DN{actor} in the
\DN{organization}, and (part of) what is done in that department in respect to
other departments (i.e.\ possible \PDN{systemic-property} of the ``department
\DN{system}'') may be conceived as a single action at the organizational-level.
A data-processing \DN{system} may be conceived as a single (artificial)
\DN{actor} carrying out data-processing actions in the \DN{organization}, even
if we know that it, in fact, is composed of a lot of \PDN{component}.
% See discussion in e.g.\ In't Veld

A \DN{sub-system} may, in line with \cite{1998-Lindgreen-FRISCO}, defined as:
\begin{Definitions}
  \DefinitionItem{sub-system} 

  Formally, this can be expressed as: 
  \[ \SymbolDefinition{SubSystem} \]
\end{Definitions}
\begin{corollary}\Label{sub-sys-top}
   If $\SubSystem{U}{v}{S'}{S}$, then: 
   $\ExAl{s \in S'}{x \in \ConceptsSub{S'}}{\DecomposedIntoEq{s}{S'}{x}}$
\end{corollary}
\ReaderProof

Two common dimensions along which to define \PDN{sub-system} are:
\DN{component-system} and \DN{aspect-system}.
\begin{Definitions}
  \DefinitionItem{component-system}

  Formally: \[ \SymbolDefinition{ComponentSystem}\]

  \DefinitionItem{aspect-system} 
  
  Formally: \[ \SymbolDefinition{AspectSystem}\]
\end{Definitions}
Note that some authors, for example \cite{1992-In'tVeld-SystemenProcessen,
1998-Bemelmans-BISA}, use the term \DN{sub-system} to refer to the above
defined concept of \DN{component-system}. However, we prefer to use the term
\DN{sub-system} as defined above (following the definition
in~\cite{1998-Lindgreen-FRISCO}), as it allows us to view it as a
generalization of the concepts \DN{component-system} and \DN{aspect-system}.

Different \PDN{viewer} may disagree on the fact whether some \DN{sub-system} is
an \DN{aspect-system} or a \DN{component-system} (or a combination thereof).
This can be traced back to the subjectivity involved in distinguishing between
\PDN{link} and \PDN{concept}.  Whenever there is a `clear' analogy to physical
structures, it will be easier to identify the difference.  Consider a
freight-train as an example \DN{system}.  Typical \PDN{component-system} of
such a \DN{system} are: the locomotive, the engine-driver, several types of
box-cars, etc.  An \DN{aspect-system} of a freight-train would be the hydraulic
braking \DN{system} of the train as a whole.

A \DN{sub-system} is indeed a \DN{system}. As such, a \DN{sub-system} $S'$ of a
\DN{system} $S$ will also have its own \PDN{systemic-property}.  However, these
properties are most likely no subset of the \PDN{systemic-property} of $S$.
For example, the engine-driver's \PDN{systemic-property} are by no-means a
clear subset of the \PDN{systemic-property} of a freight-train.

\subsection{Describing systems}
When a \DN{system} developer in a \DN{system} viewing or \DN{modeling} process
gradually realizes what (currently) `is the system', i.e.\ becomes conscious
of all relevant aspects of the involved \PDN{element} and of each of the
\DN{systemic-property}, it is very useful to be aware of the type of
\DN{system} in question and to produce a \DN{system-exposition} in accordance
with the \DN{system-type}.
\begin{Definitions}
   \DefinitionItem{system-type}
   \DefinitionItem{system-exposition}
\end{Definitions}
A \DN{system-type} can be regarded as a viewing template to be used by a
\DN{system} developer, analyst or modeler in order to decide which kinds of
things (and thereby which aspects of the things) to consider relevant in
realizing what actually `is the \DN{system}'.  A \DN{system} type comprises: 
\begin{itemize}
   \item Properties determining `the nature' of the systemic properties, for
   example for open active systems that the \DN{system} is seen as something
   that changes things in the domain of the environment and that the
   environment is seen as changing things in the \DN{system} domain.  This set
   of properties may be called the \emph{\DN{system} characteristic}.
   \item Properties determining the kinds of things which are relevant to
   incorporate in the exposition of the \DN{system} domain, and for each kind
   the kinds of roles they may play in respect to the potential kinds of
   systemic properties.  Examples of such kinds of things are for dynamic
   systems: states, transitions and transition occurrences, and for open active
   systems (among other things): actions, subjects, agents, transitions in the
   domain of the environment caused by actions in the system, etc.  This set of
   properties may be called the \emph{exposition characteristic}.
\end{itemize}
A more detailed elaboration of concepts related with the \DN{system} viewing
process can be found in~\cite{1998-Lindgreen-FRISCO}. A semi-formal description
of it based on an example is presented
in~\cite{1992-Lindgreen-SemanticStructures}.

% Will this still be here? Should apply to MvO and ADISE!!
%Morgan's organizational metaphors~\cite{1998-Morgan-OrganisationParadigms} as
%discussed in \SmartRef{metaphors} are examples of \PDN{system-type} that may be
%relevant when viewing \PDN{organization}. 

In conceiving a \DN{domain} as an \DN{organization}, several classes of
\PDN{element} may be relevant to include in a \DN{system-exposition} of that
domain. As part of the domain it may also be relevant to incorporate a number
of concepts generally relevant in an organizational context, for example public
services, laws or other kinds of constraints imposed by society, or aspects of
the particular professional field of the organization.  However, for an
\DN{organization} it is generally relevant to consider the following kinds of
things as candidates to (at least) be included in a \DN{system-exposition}:
\begin{Definitions}
   \DefItem[Actors] human actors as well as artificial actors and all kinds of
   symbiotic compositions of these two kinds.
   \DefItem[Actions] (together with the associated goals) such that a (not
   exclusive) distinction is made between those influenced by impressions from
   the environment and those either directly constituting expressions of the
   \DN{system} or only contributing to (or in some cases even explicitly
   counteracting) the expressions. Actions that are irrelevant for the
   expression of the \DN{system} should be ignored in the exposition.
   \DefItem[Co-actions] i.e.\ co-ordinated actions performed by several actors
   together.
   \DefItem[Knowledge] that is necessary for the actors to know the relevant
   pre-states of their actions and the respective goals.  A goal may be
   situation dependent.
   \DefItem[Triggers] involving internal and/or external dynamic criteria for
   the initiation of actions (temporal, impressive and actor- or action-caused
   transitions).
   \DefItem[Communication] between actors to ensure that they have the
   information necessary to perform their actions.
   \DefItem[Representation] of the information/knowledge relevant to the
   organization's activities, in order to enable the preservation or
   communication of it.  That includes all relevant aspects of the use of data
   technology and/or data-technical \DN{sub-system}s to accomplish the
   preservation or communication.
\end{Definitions}
In practice, aspects of organizational culture, social norms, empation (i.e.\
knowledge that cannot be properly represented), resources in general (energy,
skills, intellect, etc.), ecology, economy, etc., may be added to this list.

%\textbf{The System Development Process}\\
%The subjective nature of systems is probably the main cause of the serious
%problems recognised in practice in systems development (`systemeering').
%Conceiving something as a system may appear as relatively simple for a single
%person as long as the system will be kept only in his mind.  However, it is
%absolutely not a trivial task for the system viewer to be explicit about it,
%such that other persons can understand it.  And exactly that is the core of
%the problem, because the process of  `developing a system' nearly always
%involves the expertise of several - often many - persons who may have quite
%different organisational and professional background and who not necessarily
%will be fully aware of all the concepts relevant in systemeering.  Thereby the
%practical problem of establishing inter-subjectivity among the involved
%persons about the system may easily become quite overwhelming.\\
%The main reason is that for a very long period each of the involved persons
%will have their own personal view of what the system in question is, and these
%views may be different.  But adding to the problem is that people are not
%always aware of the need of a long and intense communication period as a part
%of the project.  Most often without reflecting about any uncertainty, each
%person will simply assume that the system they collectively aim at is exactly
%the one covered by the person's own view.\\
%Even if everybody is conscious of the diversity of system views, in the
%systemeering process they must still collectively overcome three kinds of
%uncertainties:
%\begin{itemize}
%	\item What are the elements of the system domain?
%	\item What are the systemic properties?
%	\item In which way do the elements contribute to the systemic properties?
%\end{itemize}
%The combined area of uncertainties about all these things from all the
%individual system views may be called the systemeering domain.
%In order to co-ordinate their efforts such that everybody finally works in the
%same direction - on the same system - each of the system viewers must express
%themselves unambiguously about their own individual system, and each one must
%try to understand the other viewers' systems.  Furthermore, as the mutual
%understanding of the different systems (hopefully) grows, they must aim at and
%finally agree on a synthesis - a single common view - the system.\\
%In the long and enduring communication process that is necessary to achieve
%this goal, the only means of the involved partners is mutually to produce,
%distribute, read and understand (partial) system representations expressed in
%some commonly accepted and usually system-type-dependent system language.
%Regardless of whether the representations are expressed orally, on paper or on
%a screen by means of some CASE-tool, and independent of whether it is
%expressed as text or by graphical means - being explicit about the systems by
%means of system representations is the only way the involved system viewers
%can unite their views.
%\begin{itemize}
%	\item A system representation is a representation produced by a system
%	viewer about certain aspects of a system.
%	\item A system language is a professional language designed to enable
%	the representation of a certain type of system.
%\end{itemize}
%To succeed in the exchange of system views and thereby ending with a single
%inter-subjectively shared system requires knowledge on two abstraction levels
%and the corresponding linguistic means for expressing it: \begin{itemize}
%	\item System-type-specific knowledge
%	\item Systemeering-domain-specific knowledge
%\end{itemize}
%The knowledge specific for the system type comprises insight with all the
%kinds of things and corresponding concepts which are relevant to consider for
%all potential instances of that system type, and an according terminology
%necessary to express oneself properly about the assumed system.  This kind of
%knowledge is a part of the qualifications required for professional systems.
%It serves as a kind of template for the systemeering work, and it constitutes
%the basis for the professional language that is used by systems.\\ The
%knowledge specific for the systemeering domain is knowledge of the concepts
%and kinds of things and of the (local) professional terminology that is
%relevant, respectively used in the particular systemeering domain (and more
%specifically in the system domains).  This knowledge is obtained through the
%systemeering process, by observing the system domains and by communicating
%with people who are active there and/or supposed to know of them.

\subsection{Classes of systems}
A \DN{work-system}, a \DN{organization}, as well as an \PDN{information-system}
belong to a \DN{system} type that primarily is characterized as being open and
active (where the latter implies also that it is dynamic). We can define these
specific types of \PDN{system} as:
\begin{Definitions}
   \DefinitionItem{active-system}
   \DefinitionItem{dynamic-system}
   \DefinitionItem{open-system}
\end{Definitions}
Note that a \DN{system} may be active and yet be non-dynamic.  For example, the
mere presence of a dummy speeding camera, i.e.\ one that is not able to capture
speeding vehicles on film, may lead drivers to drive more slowly.  The dummy
speeding camera may thus be seen as an \DO{active-system}{active}, yet
non-dynamic, system.

Note that the \DN{sub-system} of an \DN{open-active-system} does not have to be
an \DN{open-active-system}.  In other words, even though our main interest lies
with \DN{open-active-system}, we may quite well need to consider non-open or
non-active \PDN{sub-system} of these \PDN{system}.

For \PDN{open-active-system} -- therefore for \PDN{organization} too -- it is
relevant to consider the following. The behavior of an \DN{open-active-system}
is generally reflected as:
\begin{description}
   \DefItem[Internal function] \UPDN{conception} of changes in the \DN{system}
   domain caused by processes in the domain itself.
   \DefItem[External function] Here the following two kinds are distinguished:
      \begin{description}
	 \DefItem[Impression] \UPDN{conception} of changes in the \DN{system}
	 as caused by the \DN{environment}.
	 \DefItem[Expression] \UPDN{conception} of changes in the
	 \DN{environment} as caused by the \DN{system}.
      \end{description}
\end{description}
The very fact that something is regarded as a \DN{system} often serve the
purpose of hiding the internal function and focus on the external function.
(Like the phrase ``a black-box \DN{system}'').  The internal function of an
\DN{open-active-system} is referred to as ``the function \emph{in} the
\DN{system}'', while the external function is ``the function \emph{of} the
\DN{system}''. The latter is equivalent with the \DN{systemic-property} of an
\DN{open-active-system}.

One can classify \PDN{open-active-system} in several ways according to their
behavior (for details see~\cite{1971-Ackoff-SystemConcepts}).  Here we shall
only distinguish between three kinds of \DN{open-active-system} based on the
following distinctions.  A reaction of an \DN{open-active-system} is an
expression that is seen as unconditionally caused by an impression.  An action
of an \DN{open-active-system} is an expression that is seen as being completely
independent on any kind of impression. Thereby we can define the three
additional types of \PDN{open-active-system}:
\begin{Definitions}
   \DefinitionItem{reactive-system}
   \DefinitionItem{responsive-system}
   \DefinitionItem{autonomous-system}
\end{Definitions}

As mentioned before, in~\cite{1999-Alter-WorkSystems, 2002-Alter-WorkSystems}
Alter defines a work system as:
\begin{quote} \it
   A work system is a system in which human participants and/or machines
   perform business processes using information, technologies, and other
   resources to produce products and/or services for internal or external
   customers.
\end{quote}
where \emph{information systems} are to be regarded as special classes of work
systems. We will therefore operate under the assumption that we have the
following hierarchy of systems: 
\begin{enumerate}
   \item Systems in general.
   \item Open active systems: Subclass of systems
   \item Work systems: Subclass of open active systems.
   \item Organizational systems: Subclass of work systems.
   \item Information systems: Subclass of work systems and a sub-system of
   organisational systems.
   \item Computerised information systems: Subclass of work systems and a
   sub-system of information systems.
\end{enumerate}
Based on~\cite{1998-Lindgreen-FRISCO} and \cite{1999-Alter-WorkSystems}, we can
provide the following stacked set of definitions:
\begin{Definitions}
   \DefinitionItem{work-system}
   \DefinitionItem{organizational-system}
   \DefinitionItem{computerized-information-system}
   \DefinitionItem{information-system}
\end{Definitions}

\section{Dealing with evolution of conceptions}
Before concluding this chapter, there is one final issue to deal with. An
\DN{organizational-system} is an \OAS. This specifically means that it is a
\DN{system} which changes over time. Thus far we have taken the assumption that
the \DN{conception} of a \DN{viewer} is a static notion. If we write
$\Conception{U}{v}{C}$ it really means that \DN{viewer} $v$ has \emph{at some
point in time} the \DN{conception} $C$ when observing (a part of) \DN{universe}
$U$. However, in the course of time this \DN{conception} will evolve, which
raises the question: \emph{How to deal with evolution of \PDN{conception}?}.

% Bas: Examples!!!!

\Image{6cm}{Modeling evolution by snapshots}{snapshots}
Several strategies exist to deal with
evolution~\cite{1994-Proper-EvolvConcModels}. One strategy to deal with this
evolution is to take snapshots, like photographs, of a \DN{viewer}'s
\PDN{conception}. This leads to the situation depicted in
figure~\ref{snapshots}. This approach, however, does have as drawback that one
cannot `trace' the evolution of a specific \DN{element} in a \DN{viewer}'s
\DN{conception}. The approach we take, therefore, is illustrated in
figure~\ref{evolution1}. 
\Image{6cm}{Modeling evolution by functions in time}{evolution1}

Based on the approach taken in~\cite{1994-Proper-EvolvConcModels}, the
evolution of the \PDN{element} in a \DN{viewer}'s \DN{conception} is treated as
a set of (partial\footnote{For a discussion on the difference between total and
partial functions, see appendix~\ref{ch:Math}.}) functions over time. At each
point in time, a specific \DN{element} (a version) may be associated to such a
function. This means (as also illustrated in figure~\ref{evolution2}), the
situation depicted in figure~\ref{snapshots} can still be derived. When we know
the entire evolution of a nation, we can also provide a detailed descriptions
of the state-of-affairs as it holds at any arbitrary point in time.
\Image{6cm}{Deriving snapshots}{evolution2}

In order to introduce the notion of evolution formally, we first need to define
a time axes. We presume all viewers to agree that the time axes (at least)
consists of:
\begin{itemize}
   \item A set of points in time \SymbolDefinition{TimePoints}.
   \item A complete and total order \SymbolDefinition{Later}.
\end{itemize}
We also define: $t_1 \LaterEq t_2 \EQ t_1 \Later t_2 \lor t_1 = t_2$.

Since we have a complete order on the points in time, we can define the
relation $\Next \subseteq \TimePoints \times \TimePoints$ with intended
intuition: if $t_1 \Next t_2$, then $t_2$ is the next point in time immediately
after $t_1$. Formally, this relation is defined as:
\[ \SymbolDefinition{Next} \]
As, $\Later$ provides a \emph{complete} and \emph{total} order, for a given
$t_1$ there is always at most one $t_2$ such that $t_1 \Next t_2$:
\begin{corollary}\Label{single-next}
   $t_1 \Next t_2 \land t_1 \Next t_3 \implies t_2 = t_3$
\end{corollary}
\ReaderProof
As a result, we can actually view $\Next$ as a function: $\Next: \TimePoints
\Func \TimePoints$ and write $\Next t$ as an abbreviation for: the unique $t'$
such that $t \Next t'$.

The evolution over time of an \DN{element} from a \DN{conception}, can now
indeed be modelled formally as a function: 
   $h: \TimePoints \PartFunc \Elements$. 
By means of $h(t)$ we obtain the ``version'' of the \DN{element}'s evolution as
described by $h$ at point of time $t$, while $h(\Next t)$ would yield the
version at the next point in time. These functions, which represent an
\DN{element}'s evolution, will be referred to as
\emph{\PDN{element-evolution}}. This also requires us to think of the
\PDN{element} in $\Elements$ as the possible \emph{versions} an
\DN{element-evolution} may take on. Whenever we need to emphasize this, we
shall therefore use the term \emph{\DN{element-version}}.  

\UPDN{element-evolution} are \emph{partial} functions, which means that they
are not required to be defined for all points in time. In other words, at some
point in time an \DN{element-evolution} may not have an \DN{element-version}
associated, which really means that the \DN{element-evolution} does not exist
yet at that point in time (it has not been born yet), or that it has ceased to
exist (it died). In other words, \PDN{element-evolution} are allowed to be
re-born. We could, for example, have a situation where: $h$ is an
\DN{element-evolution}, $t_1 \Later t_2 \Later t_3$ are points in time, while:
$\DefinedAt{h}{t_t} \land \lnot \DefinedAt{h}{t_2} \land
\DefinedAt{h}{t_3}$\footnote{Please refer to appendix~\ref{ch:Math} for an
explanation of the notion used.}.

The set of all \PDN{element-evolution} is defined as:
\SymbolDefinition{ElementEvolutions}, in other words the set of partial
functions from the time axes to the possible \PDN{element-version}. The
evolution of an entire \DN{conception} can then be represented formally as a
set of \PDN{element-evolution}. In other words:
\SymbolDefinition{ConceptionEvolutions}. To formally express the fact that $H
\in \CEvolutions$ is a \DN{conception} of \DN{viewer} $v$ for \DN{universe}
$U$, we will write $\Conception{U}{v}{H}$.

\Image{6cm}{An element evolution migrating from the environment to the domain}{element-migration}
If $H \in \CEvolutions$, then we will use as abbreviation: $H(t) \EQ
\Set{h(t)}{h \in H}$, yielding the entire ``state'' of $H$ at time $t$. If $H$
is a \DN{conception} of some \DN{viewer}, then each of the states should be a
valid \DN{conception}:
\begin{Axiom}{S}
   If $\Conception{U}{v}{H}$, then: $\Al{t \in \TimePoints}{\Conception{U}{v}{H(t)}}$. 
\end{Axiom}
%% Doe iets met de signatures!! Wellicht gewoon twee signatures opnemen voor deze symbolen.
Similarly, to $\Conception{\_}{\_}{\_}$ we want to extend
$\DomainInEnvironment{\_}{\_}{\_}{\_}{\_}$,
$\ModelInEnvironment{\_}{\_}{\_}{\_}{\_}$ and
$\SystemInEnvironment{\_}{\_}{\_}{\_}{\_}$ to deal with evolution as well. We
might, for example, view $\DomainInEnvironment{U}{v}{H_C}{H_E}{H_D}$ to means:
\DN{viewer} $v$ has a \DN{conception-evolution} $H_C$,
\DN{environment-evolution} $H_E$ and \DN{domain-evolution} $H_D$ of
\DN{universe} $U$, where $H_D, H_E \subseteq H_C$. The difficulty with this is
that an \DN{element-evolution} might start out as being in the
\DN{environment}, but might evolve \emph{into} the \DN{domain}, or vice versa.
This is illustrated in \SmartRef{element-migration}. To properly deal with such
evolution, we will need to regard $H_E$ and $H_D$ as a classification of the
\PDN{element-evolution} from $H_C$ at each point in time. In other words as
functions: 
\[ H_E, H_D: \TimePoints \Func \Powerset(H_C) \]
yielding the set of \PDN{conception-evolution} from $H_C$ that are part of the
\DN{environment}/\DN{domain} respectively at a given point in time. This means
that $H_E(t), H_D(t) \subseteq H_C$ are sets of \PDN{element-evolution}, while
$H_E(t)(t)$ and $H_D(t)(t)$ yield the actual \DN{environment} and \DN{domain}
as it holds at $t$. For this we have:
\begin{corollary}\Label{bound-environment-domain}
   If $\DomainInEnvironment{U}{v}{H_C}{H_E}{H_D}$, then:
   $\Al{t \in \TimePoints}{H_E(t)(t) \subseteq H_C(t)}$ and 
   $\Al{t \in \TimePoints}{H_D(t)(t) \subseteq H_C(t)}$.
\end{corollary}
\ReaderProof
Note: the same would hold for $\ModelInEnvironment{U}{v}{H_C}{H_E}{H_D}$ and
$\SystemInEnvironment{U}{v}{H_C}{H_E}{H_D}$. In each case, the states of the
evolutions should be valid \PDN{conception}/\PDN{environment}/\PDN{domain} as
well:
%
% More text!!!!!!!
%
\begin{Axiom}{S}\Label{correct-snapshots}
   If $\DomainInEnvironment{U}{v}{H_C}{H_E}{H_D}$, 
   then $\Al{t \in \TimePoints}{\DomainInEnvironment{U}{v}{H_C(t)}{H_E(t)(t)}{H_D(t)(t)}}$
\end{Axiom}
\begin{Axiom}{S}
   If $\ModelInEnvironment{U}{v}{H_C}{H_E}{H_D}$, 
   then $\Al{t \in \TimePoints}{\ModelInEnvironment{U}{v}{H_C(t)}{H_E(t)(t)}{H_D(t)(t)}}$
\end{Axiom}
\begin{Axiom}{S}
   If $\SystemInEnvironment{U}{v}{H_C}{H_E}{H_D}$, 
   then $\Al{t \in \TimePoints}{\SystemInEnvironment{U}{v}{H_C(t)}{H_E(t)(t)}{H_D(t)(t)}}$
\end{Axiom}
Adding evolution of \PDN{conception} to our ontology from
figure~\ref{ontology2}, leads to the refinement of our ontology to the
situation as depicted in figure~\ref{ontology3}. 
\Image{13cm}{Ontology with evolution added}{ontology3}
% 
% A problem with this diagram is the notation! Students don't know the notation
% yet!
%

Mainly due to \SmartPageRef{non-overlapping-domain-environment}, we have:
\begin{corollary}\Label{non-overlapping-evolution}
   If $\DomainInEnvironment{U}{v}{H_C}{H_E}{H_D}$, then:
   $\Al{t \in \TimePoints}{H_E(t)(t) \intersect H_D(t)(t) = \emptyset}$
\end{corollary}
\ReaderProof
Even more specifically, we have:
\begin{lemma}\Label{non-overlapping-evolutionsets}
   If $\DomainInEnvironment{U}{v}{H_C}{H_E}{H_D}$, then:
   $\Al{t \in \TimePoints}{H_E(t) \intersect H_D(t) = \emptyset}$
\end{lemma}
\ReaderProof

\section{Conclusion}
In this chapter we have taken a highly fundamental and formal outlook on
information systems, organizations and work systems, and the way they are
modeled, including their decompositions and evolutions.

\QuestionsInChapter

\ChapterBib


==> wsm03.tex <==
\Chapter{Basic Object-Role Modeling}{object-role-modeling}
\Version{30-01-06}

\Comment{In this chapter we talk about sub-domains (situations). We should
really (in the previous chapter probably) look at Wisse, Devlin and Barwise how
they talk about situations. The subjectivity of modeling related to specific
situations should be made more concrete and fundamental.}

\Comment{In a future next chapter we should then zoom in on the Language
Action Perspective, which should really provide more methodological support for
the actual modeling. This will be inspired by Reijswoud \& Dietz' DEMO
approach.}

\Comment{This should incorporate more from ORMPoly and also the InfoSupply
articles}

The previous chapter did (see \SmartRef{description}) refer to the fact that
\PDN{viewer} are able to provide a \DN{description} of the \DN{conception}.
However, we did not really follow up on this. This chapter, however, will
indeed take these \PDN{description} as a starting point. In this chapter, we
will essentially provide a brief summary of the modeling approach from
\emph{Domain Modeling}. In~\SmartRef{advanced-object-role-modeling}, we will
enrich this modeling approach with constructs that allow us to model work
systems. 

\section{Natural language grounding of modeling}
It is not an uncommon approach to base modeling on natural language analysis:
\begin{itemize}
  \item ORM~\cite{2001-Halpin-ORM},
  \item NIAM~\cite{1990-Wintraecken-NIAM, 1989-Nijssen-NIAM},
  \item UML use cases~\cite{1999-Booch-UML},
  \item DEMO~\cite{1999-Reijswoud-DEMO},
  \item KISS~\cite{1994-Kristen-KISS} and
  \item OOSA~\cite{1992-Embley-OOSA}.
\end{itemize}

When people work together, they are bound to use some language. The language
skills of the human race evolved hand-in-hand with the levels of organization
of our activities. From organization of hunting parties by our pre-historic
ancestors, to the organization of factories and businesses in the present.
Without the use of language, it would not have worked. As a result, most (if
not all) organizations we see around us are social constructs that are the
result of communication between actors, mostly \emph{human} actors.

This makes it all the more natural to base our modeling endeavors on the
language we use most to talk about organizations, i.e.\ natural language.

\section{The logbook heuristic}
\Comment{Check Terry's book on the telephone heuristic. Or is it more Nijssen's
book? Also take more aboard from PaulF's and ErikP's PhDs. Bas: Waarom per telefoon?}

Natural language based modeling approaches such as ORM employ different
variations of the so-called telephone heuristic. This heuristic presumes some
viewer to observe a domain (including its \emph{evolution}), and use a
`telephone' to convey their observations to some other person (or computer).
This is depicted in \SmartRef{telephone-heuristic}. The left hand viewer tells
the right hand viewer `what they see'.
\Image{\textwidth}{The telephone heuristic}{telephone-heuristic}

In this chapter we are interested in having a ``transcript'' of the telephone
conversation from \SmartRef{telephone-heuristic}. More specifically, we want to
maintain a \emph{logbook} of this telephone conversation, leading to the
situation as depicted in \SmartRef{logbook-telephone}.
\Image{\textwidth}{Logging the telephone conversation}{logbook-telephone}

Even more, we could actually replace the second person from
\SmartRef{telephone-heuristic}, leaving only the original viewer and the
logbook to maintain the transcript. This leads to the \emph{logbook heuristic}
as depicted in \SmartRef{logbook-heuristic}.
\Image{\textwidth}{The logbook heuristic}{logbook-heuristic}

Note that the logbook is regarded as having a \emph{\DN{conception}} based on
an \emph{ontology} as well. As a starting point, we will presume this ontology
to consist at least of the situation as depicted in \SmartPageRef{ontology3}.

Let $\lambda$ be a logbook, logging the transcript as produced by a viewer
leads to a situation where the logbook has its own conception of the observed
universe (by way of the viewer). In the case of a viewer observing a
\DN{system}, we will denote this as:
$\SystemInEnvironment{U}{\lambda}{H_C}{H_E}{H_S}$.

All of the \AxiomClass{S} axioms apply to the conception held by logbook
$\lambda$.

In the remainder of this text book, we will further refine the ontology as
presented in \SmartPageRef{ontology3}

\section{Verbalizing conceptions}
We presume the transcriptions that are entered into the logbook to refer to
events `in the life' of specific \PDN{element-evolution}. These events refer to
changes in the state of the elements, and are presumed to be reported in terms
of \emph{facts} about the elements.  An example would be:
\begin{quote} \sffamily \scriptsize
   \begin{tabular}{ll}
      Person \#001 was born                                                         & 22-05-1967\\
      Person \#001 received name Erik Proper                                        & 23-05-1967\\
      Person \#001 lives at address: Koperwiekstraat 6, Rheden, The Netherlands, EU & 23-05-1967\\
      Person \#001 lives at address: 3/26 Rylatt Street, Brisbane, Australia        & 28-06-1994\\
      Person \#002 lives at address: Koperwiekstraat 6, Rheden, The Netherlands, EU & 29-06-1994\\
      Person \#001 works for employer: University of Queensland                     & 28-06-1994\\
      Person \#003 works for employer: University of Queensland                     & 22-04-1995\\
   \end{tabular}
\end{quote}
\Comment{This should be refined more based on PaulF's and ErikP's PhDs. By the
way, the facts report on events that take place. One of the things that might
take place is the dead of the evolution.}

When considering this transcript, it is easy to spot that it really deals with
more than one element evolution. The following element evolutions \emph{might}
be discerned:
\begin{quote} \sffamily \scriptsize
   persons: \#001; \#002; \#003\\
   name Erik Proper\\
   addresses: Koperwiekstraat 6, Rheden, The Netherlands, EU; 3/26 Rylatt Street, Brisbane, Australia\\
   employer: University of Queensland\\
   ownership of the name Erik Proper by person \#001\\
   living of person \#001 at some address\\
   living of person \#002 at some address\\
   habitation of address Koperwiekstraat 6, Rheden, The Netherlands by some person\\
   habitation of address 3/26 Rylatt Street, Brisbane, Australia  by some person\\
   coworkership of person \#001 for some employer\\
   coworkership of person \#002 for some employer\\
   employment offered by University of Queensland to a group of people
\end{quote}
In the above example, an important trade-off already comes to the surface. What
should be selected as element evolutions:\\
\mbox{\sffamily \scriptsize ~~~coworkership of person \#001 for some employer}\\
and/or\\
\mbox{\sffamily \scriptsize ~~~employment offered by University of Queensland to a group of people}\\
What is it that evolves? Either? Both? Ultimately, this is a subjective matter.
To be able to better understand the underlying trade-off, we will now first
focus on the transcription of a specific snapshot of a conception.

\Comment{The logbook gives us an account of \emph{actions} which occur in the
world. These actions may occur to non-active things. These latter are the
predications.}

\section{Elementary facts}
Similarly to \emph{Domain Modeling}, we require the facts in the transcripts to
be \emph{elementary}, in other words, no logical connectors like \emph{and} and
\emph{or}, and most likely no \emph{not}s either.

Consider, the following domain:
\begin{quote} \sffamily \scriptsize
  A person with name Erik is writing a letter to his loved one, at the desk in
  a romantically lit 
  room, on a mid-summer's day, using a pencil, while the cat is watching.
\end{quote}
We can rephrase this as the set of elementary facts:
\begin{quote} \sffamily \scriptsize
  A person is writing a letter\\
  This person has the name Erik\\
  This letter has a romantic nature\\
  This letter has intended recipient Erik's loved one\\
  The writing of this letter by Erik, occurs on a mid-summer's day\\ 
  The writing of this letter by Erik, is done using a pencil\\
  The writing of this letter by Erik, is done while the cat is watching\\
  The writing of this letter by Erik, is taking place at a desk\\
  This desk is located in a room\\
  This room is romantically lit
\end{quote}
Within these elementary facts, several \emph{players} can be discerned, such
as: \SF{person Erik}, \SF{letter}, etc.  Such players can be any `object', be
it human, physical, social, fictive, etc.  The players are regarded as playing
a \emph{role} in the facts.  In the above example, we can isolate the players
and facts as follows:
\begin{quote} \sffamily \scriptsize
  [A person] is writing [a letter]\\{}
  [This person] has [the name Erik]\\{}
  [This letter] has a [romantic nature]\\{}
  [This letter] has intended recipient [Erik's loved one]\\{}
  [The writing of this letter by Erik], occurs on a [mid-summer's day]\\{} 
  [The writing of this letter by Erik], is done using [a pencil]\\{}
  [The writing of this letter by Erik], is done while [the cat] is watching\\{}
  [The writing of this letter by Erik], is taking place at [a desk]\\{}
  [This desk] is located in [a room]\\{}
  [This room] is lit in [a romantic] way
\end{quote}
The roles played by the players can be made more explicit as follows:
\begin{quote} \sffamily \scriptsize
  [A person (writer)] is writing [a letter (written)]\\{}
  [This desk (positioned object)] is located in [a room (location)]\\{}
\end{quote}
The roles involved in a fact are linked to the \emph{players} of these roles
and to the \emph{facts} in which these roles take part by means of the
relationships:
\[ \Player, \Fact \subseteq \LinkedTo \]
respectively, with intuition:
\[ \begin{array}{lll}
   r \Player x &=& \mbox{role $r$ is played by $x$}\\
   r \Fact x   &=& \mbox{role $r$ is involved in fact $x$}
\end{array} \]
The set of roles is defined as:
\[ \Roles \EQ \Set{r}{\Ex{x}{r \Player x \lor r \Fact x}} \]
The $\Player$ and $\Fact$ relationships are exclusive:
\begin{Axiom}{S}
   $\Player \intersect \Fact = \emptyset$
\end{Axiom}
Even more, they behave as total functions from roles to concepts:
\begin{Axiom}{S}
   $\Player, \Fact \in \Roles \Func \Concepts$
\end{Axiom}
This allows us to write $\Player(r)$ and $\Fact(r)$. We generalize these
functions to sets of roles as follows:
\begin{eqn}
   \Player(R) \EQ \Set{\Player(r)}{r \in R}\\
   \Fact(R)   \EQ \Set{\Fact(r)  }{r \in R}
\end{eqn}
With this we can define the set of facts and players as:
\begin{eqn}
   \Facts   \EQ \Fact(\Roles)\\
   \Players \EQ \Player(\Roles)
\end{eqn}
The set of objects is defined as:
\[ \Objects \EQ \Facts \union \Players \]
Objects and roles are disjunct classes of concepts:
\begin{Axiom}{S}
   $\Roles \intersect \Objects = \emptyset$
\end{Axiom}
The set of roles involved in a fact is defined as:
\[ \RolesOf(f) \EQ \Set{r}{\Fact(r) = f} \]

Facts are to be regarded as complex objects. In other words, the roles and
players involved in a fact are part of its decomposition:
\begin{Axiom}{S}
   $\Al{r \in \RolesOf(f)}{r \DecompositionOf f}$
\end{Axiom}
\begin{Axiom}{S}
   $r \in \Roles \land r \DecompositionOf f \implies \Player(r) \DecompositionOf f$
\end{Axiom}

At this moment, we have actually refined our ontology from
\SmartPageRef{ontology3} to the situation as depicted in \SmartRef{ontology4}
(where we have omitted the aspects pertaining to the evolution of conceptions
for reasons of compactness).
\Image{14cm}{Our ontology refined with facts and participants}{ontology4}

\Comment{The formal bits given below should really move to chapter 2 next
year.}
Our formal considerations take place in the context of some logbook $\lambda$.
In other words, we have: $\SystemInEnvironment{U}{\lambda}{H_C}{H_E}{H_S}$.
Given a $H_C$, the set of elements of the conception at some point in time $t$
is given by: $H_C(t)$. For any subset $X \subseteq \Elements$ of elements we
introduce the abbreviation:
\begin{eqn}
   X_t \EQ X \intersect H_C(t)
\end{eqn}
A conception version should be closed with regards to the roles included in it:
\begin{Axiom}{S}\Label{closed-for-roles}
   $r \in \Roles_t \iff \Fact(r)   \in \Facts_t$ and 
   $r \in \Roles_t \iff \Player(r) \in \Players_t$ 
\end{Axiom}
As a direct consequence we have:
\begin{corollary}\Label{closed-version}
  $\Facts_t = \Fact(\Roles_t)$ and 
  $\Players_t = \Player(\Roles_t)$.
\end{corollary}
\ReaderProof

\section{From instances to types}
Consider the elementary sentences:
\begin{quote} \sffamily \scriptsize
   Person "Erik" is examined by Doctor "Jones"\\
   Person "Wil" is examined by Doctor "Smith"\\
   Person "Marc" is examined by Doctor "Jones"\\
\end{quote}
As we have learned in \emph{Domain Modeling}, we can generalize these sentences
to the ``type'' level:
\begin{quote} \sffamily \scriptsize
   A Person is examined by a Doctor
\end{quote}
with sample population:
\begin{quote} \sffamily \scriptsize
   \begin{tabular}{|l|l|}
       \hline
       Person & Doctor\\
       \hline
       \hline
       Erik   & Jones\\
       Wil    & Smith\\
       Marc   & Jones\\
       \hline
   \end{tabular}
\end{quote}

Formally, we introduce typing as a special kind of decomposition $\HasType
\subseteq \DecompositionOf$.  The set of instances ($\Instances$) and the set
of types ($\Types$) can be defined as:
\begin{eqn}
   \Types     \EQ \Set{y}{\Ex{x}{x \HasType y}}\\
   \Instances \EQ \Set{x}{\Ex{y}{x \HasType y}} 
\end{eqn}
Types and instances form a partition of the set of concepts:
\begin{Axiom}{S}
   $\Types \intersect \Instances = \emptyset$ and
   $\Types \union \Instances = \Concepts$.
\end{Axiom}
All instances have some type:
\begin{corollary}\Label{total-typing}
   $\AlEx{x \in \Instances}{y \in \Types}{x \HasType y}$
\end{corollary}
\ReaderProof
Note that the reverse does not hold. In other words, we do not generally have:
\[ \AlEx{y \in \Types}{x \in \Instances}{x \HasType y} \]
Some types may have an empty population.

We actually require \SmartRef{total-typing} to hold at each point in time:
\begin{Axiom}{S} 
   Let $t \in \TimePoints$, then:
   $\AlEx{x \in \Instances}{y \in \Types}{x \HasType_t y}$
\end{Axiom}

Sets such as $\Facts$, $\Players$, etc, contain both types and instances. To be
able to refer to the types and instances respectively, we introduce:
\[ \begin{array}{rcl}
   \TP{X} \EQ X \intersect \Types 
   &\mbox{and}&
   \IN{X} \EQ X \intersect \Instances
\end{array} \]
for any set $X \subseteq \Elements$ of elements. As a direct consequence we
have:
\begin{corollary}\Label{type-specialization}
   $\begin{array}{rclcrcl}
      \TP{\Players} &\Eq& \Player(\TP{\Roles}) && \IN{\Players} &\Eq& \Player(\IN{\Roles})\\
      \TP{\Facts}   &\Eq& \Fact(\TP{\Roles})   && \IN{\Facts}   &\Eq& \Fact(\IN{\Roles})\\
   \end{array}$
\end{corollary}
\ReaderProof

As abbreviations we will also use:
\begin{eqn}
   \TypesOf_t(x)      \EQ \Set{y}{x \HasType_t y}\\
   \TypesOf_t(X)      \EQ \Union_{x \in X} \TypesOf_t(x)\\
   \Pop_t(y)          \EQ \Set{x}{x \HasType_t y}\\
   \Pop_t(Y)          \EQ \Union_{y \in Y} \Pop_t(y)
\end{eqn}
The \emph{extra temporal} versions are defined as:
\begin{eqn}
   x \HasType y   \EQ \Ex{t \in \TimePoints}{x \HasType_t y}\\
   \TypesOf(x)    \EQ \Union_{t \in \TimePoints} \TypesOf_t(x)\\
   \TypesOf(X)    \EQ \Union_{t \in \TimePoints} \TypesOf_t(X)\\
   \Pop(y)        \EQ \Union_{t \in \TimePoints} \Pop_t(y)\\
   \Pop(Y)        \EQ \Union_{t \in \TimePoints} \Pop_t(Y)
\end{eqn}

Typing should adhere to the classification in our ontology. In other words:
\begin{Axiom}{S}
   For all $X \in \setje{\Facts, \Roles, \Players}$ we have:
   \[ x \HasType y \implies (x \in X \iff y \in X) \]
\end{Axiom}
The $\Fact$ and $\Player$ functions should never cross the type/instance level:
\begin{Axiom}{S}\Label{no-fact-cross}
   $\Al{r \in \Roles}{r \in \Types \iff \Fact(r) \in \Types}$
\end{Axiom}
\begin{Axiom}{S}\Label{no-player-cross}
   $\Al{r \in \Roles}{r \in \Types \iff \Player(r) \in \Types}$
\end{Axiom}
All non-typing forms of decomposition should also not cross the type/instance level:
\begin{Axiom}{S}
   If $x \DecompositionOf y$, then: 
   \[ x \HasType y \lor x,y \in \Types \lor x,y \in \Instances \]
\end{Axiom}

Players involved in role instances should behave as stipulated at the type level:
\begin{Axiom}{S}\Label{player-role-follow-type}
   If $r \in \TP{\Roles}$, then:
   $\Player(\Pop(r)) \subseteq \Pop(\Player(r))$
\end{Axiom}
The same applies to facts:
\begin{Axiom}{S}\Label{fact-role-follow-type}
   If $r \in \TP{\Roles}$, then:
   $\Fact(\Pop(r)) \subseteq \Pop(\Fact(r))$
\end{Axiom}
Even more, as all role types of a fact type should be populated, the reverse
should hold as well:
\begin{Axiom}{S}\Label{fact-type-dictate-role}
   If $r \in \TP{\Roles}$, then:
   $\Fact(\Pop(r)) \supseteq \Pop(\Fact(r))$
\end{Axiom}
%
% Check time dimension on these ones!!
%
As an immediate result we have:
% (at each point in time) 
\begin{corollary}\Label{total-roles-of-facts}
   If $f \in \TP{\Facts}$, then:
   \[ \Pop(f) = \Fact(\Pop(\RolesOf(f))) \]
\end{corollary}
\ReaderProof
We can express this at the type level as:
\begin{corollary}\Label{total-roles-of-facts-typing}
   Let $f \in \IN{\Facts}$, then:
   \[ \TypesOf(\RolesOf(f)) = \RolesOf(\TypesOf(f)) \] 
\end{corollary}

\SmartRef{fact-type-dictate-role} does not have a pendent for players. In other
words, we do not generally have:
\[ \Player(\Pop(r)) \supseteq \Pop(\Player(r)) \]
as this would require all instances of a player type to be involved in
\emph{all} roles in which the type is involved. However, we do have a weaker
version as we will see in \SmartRef{subtyping}.

Facts should behave as a function from role types to instances:
\begin{Axiom}{S}
  Let $r \in \TP{\Roles}$ and $s_1, s_2 \in \Pop(r)$, then:
  \[ \Fact(s_1) = \Fact(s_2) \implies s_1 = s_2 \]
\end{Axiom}
This axiom allows us, for any fact instance $f \in \IN{\Facts}$, to define the
\emph{partial} function $\Vec{f}: \TP{\Roles} \PartFunc \IN{\Objects}$ as:
\[ \Vec{f} \EQ \Set{\tuple{r,\Player(s)}}{s \in \Pop(r) \land \Fact(s) = f} \]

If $f$ is some fact and $R \subseteq \RolesOf(\TypesOf(f))$, then we define the \emph{total}
function $\Vec{f}[R]: R \Func \IN{\Objects}$ as:
\[ \Vec{f}[R] \EQ \Set{\tuple{r,\smash{\Vec{f}}(r)}}{r \in R} \]

The ontology resulting after this refinement is depicted in \SmartRef{ontology5}.
\Image{14cm}{Our ontology refined with typing}{ontology5}

\Comment{In the formal discussion we should also visit the notion of generative
models. An ORM model is a partial model in the sense that it needs a population
model to make it complete. The semantics of an ORM model is the set of allowed
populations. A similar situation can be observed with process models, where the
semantics is the set of possible traces (i.e.\ populations of the process
model)}

\Comment{We need to extend this with subtyping, etc, etc. See ORMPoly and
CDMKernel. Stay in line with DM as much as possible.  Note: what is missing
(deliberately) is the axiom requiring the populations of different to be
disjoint unless they are type related. But since we don't discuss the latter,
we'll skip this for now.}

\Section{Subtyping}{subtyping}
Sub-typing is an important feature of object-role modeling.
\SmartRef{specialization-hierarchy} shows an example of subtyping in terms of a
specialization hierarchy.
\Image{10cm}{Example of a specialization hierarchy}{specialization-hierarchy}

\Comment{Discuss the animal example in detail. It is a great way of discussing
generalisation and specialisation \emph{processes}.}

In general, sub-typing involves the identification of a sub-set of the
population of some super-type. For example, in the situation depicted in
\SmartRef{specialization-hierarchy} \emph{flesh eater} is a specific sub-set of
\emph{animals}. In different versions of ORM, different rules apply to
sub-typing~\cite{1993-Hofstede-PSM,1995-Halpin-ORMPoly,2001-Halpin-ORM}. In
this textbook we present a rather generic interpretation. 
%%% Make this more explicit in the future

Formally, sub-typing is captured as a relationship $\Sub \subseteq \LinkedTo$
with intuition: if $x \Sub y$, then type $x$ is considered to be a subtype of
$y$. We will also refer to $x$ as the \emph{sub-type} and $y$ as the
\emph{super-type}. Sub-typing is a relationship over object types:
\begin{Axiom}{S}
   $\Sub \subseteq \TP{\Objects} \times \TP{\Objects}$
\end{Axiom}
The sub-typing relationship should be transitive and acyclic:
\begin{Axiom}{S}
  $x \Sub y \Sub z \implies x \Sub z$
\end{Axiom}
\begin{Axiom}{S}
  $\lnot x \Sub x$
\end{Axiom}
The semantics of sub-typing in terms of populations is that the population of a
specialized type should be a subset of the population of the supertype:
\begin{Axiom}{S}
  $x \Sub y \implies \Pop(x) \subseteq \Pop(y)$
\end{Axiom}
We will also use as an abbreviation:
  $x \SubEq y \EQ x \Sub y \lor x = y$.

%
% Ontology uitbreide!!
%

The population of a subtype can be restrained further. In ORM, this is commonly
done using a so-called sub-type defining rule. Using the language introduced in
the next chapter, \SmartRef{defining-subtypes} will return to the issue of
precisely defining the population of a subtype.

As promised, we would introduce a weaker pendant of
\SmartRef{fact-type-dictate-role} for players. First, the set of roles types
which are played by an object type as: 
\[ \Plays(p) \EQ \Set{r}{p \SubEq \Player(r)} \]
This is actually the set of role-types that may be played by the instances of
$x$, which we enforce by:
\begin{Axiom}{S}\Label{active-player-population}
   If $p \in \TP{\Players}$, then:
   \[ \Pop(p) \subseteq \Player(\Pop(\Plays(p))) \]
\end{Axiom}
In other words, instances of a player type \emph{must} be active in one of the
associated roles. With \SmartRef{player-role-follow-type} we have:
\begin{corollary}\Label{total-roles-of-players}
   If $p \in \TP{\Players}$, then:
   \[ \Pop(p) = \Player(\Pop(\Plays(p))) \]
\end{corollary}
\ReaderProof

\section{Overlap of populations}
When considering the ORM schema as depicted in
\SmartRef{multi-root-specialization}, one would expect the populations of
\SF{Vehicle} and \SF{Distance} to be disjoint, while the populations of
\SF{Vehicle} and \SF{Product} are expected to overlap. Thus far, we have not
introduced any formal mechanism to enforce this type of behavior other that the
inclusion of populations for sub-types. To properly formalize this, we first
define the family (as it is `alive' at some point in time) of an object type
based on the sub-typing hierarchy as follows: 
\[ \Family_t(x) \EQ \Set{y \in \TP{\Objects}_t}{y \Sub x \lor y = x} \]
Two object types are deemed \emph{type related} iff their families overlap:
\[ x \TypeRel_t y \EQ \Family(x) \intersect \Family(y) \neq \emptyset \]
If the population of object types overlaps, then they mus be type related:
\begin{Axiom}{S}
  $\Pop_t(x) \intersect \Pop_t(y) \neq \emptyset \implies x \TypeRel_t y$
\end{Axiom}
Note that the converse does not necessarily hold.
\Image{\textwidth}{Example of a multi-rooted specialization hierarchy}{multi-root-specialization}

\QuestionsInChapter

\ChapterBib


==> wsm04.tex <==
\Chapter{Object-Role Calculus}{object-role-calculus}
\Version{10-10-05}

\section{Introduction}
This chapter is concerned with a language to express rules over domains that
are modeled by means of an ORM model. An ORM model is typically produced in a
natural-language driven process. As a side-product, the fact types in an ORM
model receive verbalizations that closely match natural language. In a rule
language we would like to be able to re-use these verbalizations to arrive at
rules that also closely resemble natural language. This resemblance will allow
different stakeholders to understand (and validate) the rules.

% Why do we need a rule language in the first place?

In this chapter, we therefore propose a fact-based approach to the formulation
of rules, and reasoning with these rules, which is based entirely on concepts
that are familiar to a domain expert, as modeled through ORM. In doing so, we will
built on conceptual rule languages such as Lisa-D~\cite{1993-Hofstede-LISA-D},
RIDL~\cite{1982-Meersman-RIDL} and ConQuer~\cite{1994-Proper-ConQuer,
1996-Halpin-ConQuer}. These languages allow for the specification of rules in a
semi-natural language format that can be more easily understood by domain
experts than languages such as predicate calculus, Z~\cite{1988-Spivey-Z} or
OCL~\cite{2003-Warmer-OCL}.

The language we introduce in this chapter will be referred to as the
\emph{object role calculus} (ORC), a name which clearly signifies its relation
to \emph{object role modeling} and the fact that it is a language in which one
cannot only express rules but also reason/calculate with these rules
analogously to \emph{predicate calculus}. 

Note: In the current version of this chapter, we do not yet include reasoning.

The ORC is built up in four layers:
\begin{description}
   \item[Computational layer --] Instances from the population of an ORM model
   will occur in the result of a rule with a certain frequency. This frequency
   may be binary: \emph{Does a specific instance occur: yes/no?}, but it may
   also be natural number: \emph{How many times does a specific instance
   occur?} Even more, one may associate uncertainties to these frequencies.

   \item[Logic layer --] The ORC is built on top of a multi-valued logic (using
   the underlying computational layer), where the computational domain is used
   as (one of) the underlying domains.  Theoretically, this could be any kind
   of logic, but for practical purposes we will use traditional predicate
   calculus with some minor temporal extensions. This could be replaced by more
   advanced modal logics.

   \item[Path-expression layer --] In its most basic form, rules formulated in
   ORC correspond to paths of fact-types strung together using connectors. At
   this layer we are concerned with the construction of these paths. Path
   expressions form the bones of ORC rules, while the logic layer provides the
   atoms from the these bones are constructed.

   \item[Information-descriptor layer --] Path expressions still not utilize
   the rich verbalizations that are typical for ORM models. In the last layer
   we finally add skin to the bare bones in terms of natural looking
   expressions that can be understood by a wide(r) audience.
\end{description}

\section{Computational domain}
Let $\Frequencies$ be a set of quantities. In a concrete case this could be
boolean, natural numbers, probabilities, etc. These frequencies are best
thought of as stating the frequency at which an element may occur in a set of
results.

We need six operations to combine quantities:
\[ \lor, \land, \oplus, \otimes, \ominus:  
       \Frequencies \times \Frequencies \Func \Frequencies \]
and two constants:
\[ \One, \Zero \in \Frequencies \]
These operations have the following intended meaning:
\begin{itemize}
   \item $a \lor b$ is the resulting frequency when counting elements occuring
   $a$ times \emph{or} $b$ times.
   \item $a \land b$ is the resulting frequency when counting elements occuring
   $a$ times \emph{and} $b$ times.  
   \item $a \oplus b$ is the resulting frequency of when adding an element
   occuring $a$ times to an element occuring $b$ times.
   \item $a \otimes b$ is the resulting frequency of a cartesian combination of
   an element occuring $a$ times and $b$ times.
   \item $a \ominus b$ is the resulting frequency when doing a set exclusion on
   an element occuring $a$ times and $b$ times.
\end{itemize}
The $\lor$, $\land$, $\oplus$ and $\otimes$ operations should be cummutative
and associative.  Let $\Theta$ be one of these operations, then:
\begin{eqn}
   a \MT{\Theta} b                 &=& b \MT{\Theta} a\\
   a \MT{\Theta} (b \MT{\Theta} c) &=& (a \MT{\Theta} b) \MT{\Theta} c
\end{eqn}
The $\One$ and $\Zero$ constants should behave as neutral elements:
\[ \begin{array}{c}
   a \otimes \Zero = \Zero\\
   a \land \Zero = \Zero\\
   a \lor \Zero = a\\
   a \oplus \Zero = a\\
   a \otimes \One  = a\\
   a \land \One  = a\\
\end{array} \]

If $X$ is some set, then $\Count{X} = \bigoplus_{x \in X} \One$.

This leaves us with the task of defining these operations and constants for
specific computational domains.

For normal logic we would have:
\begin{eqn}
   \Frequencies_{\B} \EQ \B\\
   a \lor      b \EQ \SF{Max}(a, b)\\
   a \land     b \EQ \SF{Min}(a, b)\\
   a \oplus    b \EQ \SF{Max}(a, b)\\
   a \otimes   b \EQ \SF{Min}(a, b)\\
   a \ominus b \EQ \SF{Max}(a - b, 0)\\
   \One          \EQ 1\\
   \Zero         \EQ 0
\end{eqn}
Note that in this case, $\oplus$ and $\otimes$ have the samen semantics as
$\lor$ and $\land$ respectively.

For multi-sets we have:
\begin{eqn}
   \Frequencies_{\N} \EQ \N\\
   a \lor      b \EQ \SF{Max}(a, b)\\
   a \land     b \EQ \SF{Min}(a, b)\\
   a \oplus    b \EQ a + b\\
   a \otimes   b \EQ a \times b\\
   a \ominus b \EQ \SF{Max}(a - b, 0)\\
   \One          \EQ 1\\
   \Zero         \EQ 0
\end{eqn}

We might define generalized frequency sets as:
\begin{eqn}
   \Frequencies_{\Z} \EQ \Z\\
   a \lor      b \EQ \SF{Max}(a, b)\\
   a \land     b \EQ \SF{Min}(a, b)\\
   a \oplus    b \EQ a + b\\
   a \otimes   b \EQ a \times b\\
   a \ominus b \EQ a - b\\
   \One          \EQ 1\\
   \Zero         \EQ 0
\end{eqn}
Let $\Frequencies^d_F$ be one of the three above computational domains for
frequencies, then we can define a probabilistic distribution version over
$\Frequencies$ as follows: 
\begin{eqn}
   \Frequencies^{\!d}_F \EQ \Frequencies_F \Func [0..1]\\
   a \MT{\Theta} b \EQ \LambdaFun{n}{1 - ( \Pi_{i,j \in \N: i \MT{\Theta} j = n} (1 - a(i) \times b(j)))}\\
\end{eqn}
where $\Theta$ is any of $\lor$, $\land$, $\oplus$, $\otimes$ and $\ominus$.

\section{Logic layer}
If $\phi$ is a well-formed formula, we will use $\VSem{\phi}$ to express the
valuation of $\phi$, where we will also write:
\[ \Pop \models_t^v \phi \mbox{~~iff~~} v = \VSem{\phi} \]

Given an ORM model with role type $r \in \TP{\Roles}$, object types $o \in
\TP{\Objects}$, instances $i, j \in \IN{\Objects}$ and population $\Pop$, we
have the following atomic constructions:
\begin{eqn}
  \VSem{o(i)}   \EQ \Count{\Set{x \in \Pop_t(o)}{x = i}}\\
  \VSem{r(i,j)} \EQ \Count{\Set{x \in \Pop_t(r)}{i = \Player(x) \land j = \Fact(x)}}
\end{eqn}
If $\Theta$ is one of the operators $\lor$, $\land$, $\oplus$, $\otimes$ and
$\ominus$, then we have:
\begin{eqn}
  \VSem{\phi \MT{\Theta} \psi} \EQ \VSem{\phi} \MT{\Theta} \VSem{\psi}\\
  \VSem{\lnot \phi}            \EQ \One \ominus \VSem{\phi}\\
  \VSem{\Al{x}{\phi}}          \EQ \Land_c \VSem{\phi\tuple{x/c}}\\
  \VSem{\Ex{x}{\phi}}          \EQ \Lor_c  \VSem{\phi\tuple{x/v}}
\end{eqn}
Using the traditional logic operators, path expressions would only be able to deal
with specific points in time only.  Since we take the evolution of a domain
(conception) into account we need rules that refer to time as well.  We
therefore also introduce the following constructions into the logical layer:
\begin{eqn}
   \VSem{\always \phi} \EQ \Land_{s \in \TimePoints} \Vsem{\phi}(\Pop,s)\\
   \VSem{\next \phi}   \EQ \Vsem{\phi}(\Pop,\Next t)
\end{eqn}
In addition we introduce the following abreviations:
\begin{eqn}
   \sometime X   \EQ \lnot \always \lnot X \\
   X \precedes Y \EQ \always ((X \land \next Y) \implies (\next \lnot X \land \lnot Y))
\end{eqn}
%%%% See PhD Terry!!!

\section{Path expression layer}
Path expressions are essentially paths through an ORM model. As a path has a
head and a tail, path expressions can be regarded as binary predicates in a
logic, where the head and tail are the first two parameters. However, we will not
only maintain heads and tails, but also the frequencies in which a path from head
to tail is available.  This leads to the view that a path expression
is a ternary predicate. Even more, to enable us to express such rules as: 
\begin{quote} \it
   People who work for a department must be involved in a project conducted by
   that department, where the project is managed by another person.
\end{quote}
we need to be able to introduce additional variables. So, in general, path
expressions need to have an arity of $n+3$. 

The semantics of path expressions is defined by means of a set of re-write
rules, in the style of denotational semantics~\cite{1977-Stoy-DenSem}. If $P$
is a path expression, each rule will aim to rewrite $P$ in terms of logic
expressions, breaking down $P$ into its constituent elements. Formally we will
write $x \PSem{P} y$ at the left hand side of each of these rewrite rules.
The $x$ and $y$ are variables representing the head and tail of a path
expression, while $t$ is a sequence representing the actual path of instances
from $x$ to $y$ combination. In addition to $x$ and $y$, the path expression
$P$ can contain other variables.  These will be drawn from a special set
$\omega$. Let, in the remainder of this chapter, $x, y, z$ be variables that
are not in $\omega$.

\subsection{Atomic path expressions}
At this point we can describe the meaning of elementary path expressions as
follows.  Let $o$ be an object type and $r$ a role type, then $o$ and $r$
are (atomic) path expressions with semantics:
\begin{eqn}
  x \PSem{o} y \EQ o(x) \land x = y\\
  x \PSem{r} y \EQ r(x,y)
\end{eqn}
If $c$ is a constant and $v \in \omega$ is some variable, then we also have:
\begin{eqn}
  x \PSem{c} y \EQ c = x \land x = y\\
  x \PSem{v} y \EQ v = x \land x = y
\end{eqn}
As special atomic path expressions we introduce:
\begin{eqn}
  x \PSem{\One}  y \EQ x = y\\
  x \PSem{\Zero} y \EQ \Zero\\
  x \PSem{\Full} y \EQ {\it true}
\end{eqn}
As an example, consider the ORM model depicted in \SmartRef{join}.
\Image{7cm}{Basic ORM model}{join}

In this case we would have for $x \PSem{p} y$, $x \PSem{q} x$ and 
$x \PSem{B} y$:
\[ 
  \def\Show#1#2{#1 & \tuple{#1,#2} & \One\\}
  \begin{array}[t]{|c|c|c|}
     \hline
     x & y & \mbox{frequency}\\
     \hline
     \Show{1}{A}
     \Show{2}{B}
     \Show{3}{A}
     \Show{1}{C}
  \end{array}
  \mbox{~~}
  \def\Show#1#2{\tuple{#1,#2} & #1 & \One\\}
  \begin{array}[t]{|c|c|c|}
     \hline
     x & y & \mbox{frequency}\\
     \hline
     \Show{1}{A}
     \Show{2}{B}
     \Show{3}{A}
     \Show{1}{C}
  \end{array}
  \mbox{~~}
  \def\Show#1{#1 & #1 & \One\\}
  \begin{array}[t]{|c|c|c|}
     \hline
     x & y & \mbox{frequency}\\
     \hline
     \Show{A}
     \Show{B}
     \Show{C}
  \end{array}
\]

\subsection{Composing paths}
If $P$ and $Q$ are path expressions, then we can concatenate path expressions
as follows:
\begin{eqn}
  x \PSem{P \Conc Q} y \EQ \Ex{z}{x \PSem{P} z \otimes z \PSem{P} y}
\end{eqn}
We immediately have:
\begin{corollary}
   $P \Conc \One = P$ and $P \Conc \Zero = \Zero$.
\end{corollary}
For the manipulation of heads and tails we introduce:
\begin{eqn}
  x \PSem{\Reverse{P}} y \EQ y \PSem{P} x\\
  x \PSem{\Head P} y     \EQ x = y \land \Ex{z}{x \PSem{P} z}\\
  x \PSem{\Tail P} y     \EQ x = y \land \Ex{z}{z \PSem{P} y}
\end{eqn}
where we use as an abbreviation: $x \PSem{P} y \EQ \Ex{a}{x \PSem{P} y}$.

As an example, in the case of \SmartRef{join} we would have for 
   $x \PSem{p \Conc \Reverse{q}} y$,
   $x \PSem{p \Conc \Reverse{q} \Conc r \Conc \Reverse{s}} y$ and
   $x \PSem{p \Conc \Reverse{q} \Conc v \Conc r \Conc \Reverse{s}} y$ (where $v$ is a variable):
\[
  \def\Show#1#2{#1 & #2 & \One\\}
  \begin{array}[t]{|c|c|c|}
     \hline
     x & y & \mbox{frequency}\\
     \hline
     \Show{1}{A}
     \Show{2}{B}
     \Show{3}{A}
     \Show{1}{C}
  \end{array}
  \mbox{~~}
  \def\Show#1#2#3{#1 & #2 & #3\\}
  \begin{array}[t]{|c|c|c|}
     \hline
     x & y & \mbox{frequency}\\
     \hline
     \Show{1}{l}{2}
     \Show{2}{k}{1}
     \Show{3}{l}{1}
     \Show{1}{k}{1}
  \end{array}
\]
A special construction operator for path expression is the \emph{confluence}
operator. This operator is essential in formalizing graphical uniqueness
constraints. Let $P_1$, \ldots $P_n$ be path expressions, then:
\begin{eqn}
  x \PSem{\Confluence{P_1, \ldots, P_n}} y \EQ 
     \Ex{x_1,\ldots,x_n}{
        x_1 \PSem{P_1} y \land \ldots \land x_n \PSem{P_n} y \land
        x = \tuple{x_1,\ldots,x_n} 
     }
\end{eqn}
By combining this operator with $\Full$, we can also construct cartesian
products:
\begin{eqn}
  P_1 \times \ldots \times P_n \EQ
  \Confluence{P_1 \Conc \Full, \ldots, P_n \Conc \Full}
\end{eqn}

In addition to path composition operators, we also have the following ways of
combining path expressions.  If $\Theta$ is one of the operators $\lor$,
$\land$, $\oplus$, $\otimes$ and $\ominus$, then we have:
\begin{eqn}
  x \PSem{P \MT{\Theta} Q} y \EQ x \PSem{P} y \MT{\Theta} x \PSem{P} y\\
  x \PSem{\lnot P} y      \EQ \lnot (x \PSem{P} y)
\end{eqn}
Note that these logical connectives `reset' the paths between heads and tails
of instances. Implication and equality of path expressions can be defined as:
\begin{eqn}
  P \implies Q \EQ \lnot P \lor Q\\
  P \iff Q     \EQ (P \implies Q) \land (Q \implies P)
\end{eqn}
For practical purposes, however, we would like to use logical connectives
that allow us to combine the heads of paths. For example, in an expressions such
as:
\begin{quote} \it
   Person working for department `IRIS', who also owns a car.
\end{quote}
In this case we would like to require:
\begin{quote} 
  $\Ex{y}{x \PSem{\SF{Person working for Department `IRIS'}} y} \land
   \Ex{y}{x \PSem{\SF{Person owning a Car}} y}$
\end{quote}
To be able to expres rules like these, we also introduce the following
abbreviations:
\begin{eqn}
  P \hand     Q \EQ \Head P \land    \Head Q\\
  P \hor      Q \EQ \Head P \lor     \Head Q\\
  P \hplus    Q \EQ \Head P \oplus   \Head Q\\
  P \hminus   Q \EQ \Head P \ominus  \Head Q\\
  P \himplies Q \EQ \Head P \implies \Head Q\\
  P \hiff     Q \EQ \Head P \iff     \Head Q\\
\end{eqn}

\subsection{Evolution and path expressions}
To allow for path expressions to refer to evolution of the population,
we introduce:
\begin{eqn}
  x \PSem{\sometime P} y   \EQ \sometime (x \PSem{P} y)\\
  x \PSem{\always   P} y   \EQ \always   (x \PSem{P} y)\\
  x \PSem{P \precedes Q} y \EQ (x \PSem{P} y) \precedes (x \PSem{Q} y)
\end{eqn}

\subsection{Path expressions as logic}
If $P$ is a path expression, then we have the following logic expressions:
\begin{eqn}
   \ANY{P} \EQ \Ex{x,y}{x \PSem{P} y}\\
   \ALL{P} \EQ \Al{x,y}{x \PSem{P} y}
\end{eqn}

\section{Graphical constraints}
In this section we briefly visit some of the graphical constraints that are
used in ORM models.

\subsection{Mandatory roles}
If $o$ is an object type and $r_1$, \ldots, $r_n$ are roles types such that
$\Al{1 \leq i \leq n}{o \SubEq \Player(r_i)}$, then:
\begin{eqn}
   \Total(o:\setje{r_1,\ldots,r_n}) \EQ \always \ALL{o \himplies (r_1 \hor \ldots \hor r_n)}
\end{eqn}
We may even further generalize this to mandatory combination over cartesian
products of object types. Let $o_1$, \ldots, $o_m$ be object types and
$r_{1,1}, \ldots, r_{n,1}, \ldots, \ldots, r_{1,m}, \ldots, r_{n,m}$ are
role types such that:
$\All{1 \leq i,j \leq m}\Al{1 \leq k \leq n}{
  o_i \SubEq \Player(r_{k,i}) \land \Fact(r_{k,i}) = \Fact)r_{k,j}
}$, then:
\[ \begin{array}{l}
   \Total(\tuple{o_1,\ldots,o_m}:
     \setje{
        \tuple{r_{1,1},\ldots,r_{1,m}}, 
        \ldots,
        \tuple{r_{n,1},\ldots,r_{n,m}}
     }
   ) \EQ \Eol \Tab
   \always \ALL{(o_1 \times \ldots \times o_m) 
                \himplies 
		(\Confluence{r_{1,1},\ldots,r_{1,m}} 
		 \hor \ldots \hor 
		 \Confluence{r_{n,1},\ldots,r_{n,m}})
	   }
\end{array} \]

\subsection{Uniqueness}
Given a set of role types, we may be able to automatically determine a derived
fact type that joins all fact types involved in these role types. The algorithm
to compute the actual derivation is referred to as the \emph{uniquest}
algorithm~\cite{1990-Weide-Uniquest}. It was designed, initially, to provide
the semantics of graphical uniquess constraints as depicted in
\SmartRef{constraints}. In the case of roles \SF{r} and \SF{s}, the result would be:
$\Confluence{\SF{r},\SF{s}}$,
while in the case of roles \SF{q} and \SF{s} the result would be:
$\Confluence{\SF{q} \Conc \SF{r}, \SF{s}}$.
Note that not all combinations of role types lead to join paths.
In~\cite{1990-Weide-Uniquest} this is discussed in more detail.
\Image{6cm}{Example uniqueness constraints}{constraints}

Let $\JoinPath(R)$ be the function determining a join path for some sequence of
roles types $R$, while $o$ is the central object type, using the uniques
algorithm. If $\JoinPath(R)$ is defined for some sequence $R$ of role types,
then the uniqueness of the roles types in $R$ is defined as:
\begin{eqn}
   \Unique(R) \EQ 
   \always \ALL{\JoinPath(R) \Conc \Reverse{\JoinPath(R)} \implies \One}
\end{eqn}

\subsection{Subsets}
The $\JoinPath$ function cannot only be used to define uniqueness constraints,
but also to define subset constraints. If $R_1$ and $R_2$ are two sequences of role
types with the same length (i.e.\ $\Card{R_1} = \Card{R_2}$) such that the players
are type related: $\Al{1 \leq i \leq \Card{R_1}}{R_1[i] \TypeRel R_2[i]}$, then a
subset constraint from $R_1$ to $R_2$ is defined as:
\begin{eqn}
   \SubSet(R_1,R_2) \EQ \always \ALL{\JoinPath(R_1) \himplies \JoinPath(R_2)}
\end{eqn}
As an example, consider the model depicted in \SmartRef{subsets}. In this case
we would have: 
\[ \always \ALL{\Confluence{r,s} \himplies \Confluence{p,q}} \]
\Image{6cm}{Example subset constraint}{subsets}

\subsection{Temporal ordering}
\Comment{We should add more methodological support. Split verbalizations into
predications/actions/ordering}

\Comment{This section should be move to the advanced ORM chapter.}

Now consider the following verbalizations (at the type level):
\begin{quote} \sffamily \scriptsize
   A Person fills in a Form\\
   A Person is examined by a Doctor\\
   A Doctor produces a Diagnose\\
   A Doctor writes a Prescription
\end{quote}
This leads to the situation as depicted in \SmartRef{doctor-visit1}.
\Image{8cm}{Basic model of a visit to a Doctor}{doctor-visit1}

Thus far we have not discussed properties pertaining to temporal ordering.
Suppose now that in this domain:
\begin{quote} \sffamily \scriptsize
   Before a Person can be examined by a Doctor, they should have filled in a Form.\\
   Before a Doctor produces a Diagnose, a Person should have been Examined.\\
   Before a Doctor writes a Prescription, a Person should have been Diagnosed.
\end{quote}
This is, however, is still an incomplete picture. The production of a diagnose
and the writing of a prescription should all pertain to the same person. Even
more, as a person may visit a doctor twice for two different reasons, the
diagnose and prescription really pertain to one specific doctor visit. This
leads to the situation as depicted in \SmartRef{doctor-visit2}.
\Image{12cm}{Model of a visit to a Doctor with explicit entity}{doctor-visit2}

But also consider the situation as depicted in \SmartRef{doctor-visit3}. What
is the semantic difference? 
\Image{12cm}{Model of a visit to a Doctor with alternative semantics}{doctor-visit3}

\Image{7cm}{Compact model of a visit to a Doctor}{doctor-visit4}
As a graphical abbreviation, we will use the notation as depicted in
\SmartRef{doctor-visit4} and \SmartRef{doctor-visit5} respectively.
\Image{7cm}{Compact model of a visit to a Doctor with alternative semantics}{doctor-visit5}

\Comment{Formally, we should really view state-sequence types as composed
types. In other words, types with an underlying decomposition using
decomposers. Also check Udo Lipeck and Guenter Saake's work on temporal
Sonstraints.}

Formally, temporal dependency constraints can be defined as follows:
\[ \precedes(R_1,R_2) \EQ \always \ALL{\JoinPath(R_1) \precedes \JoinPath(R_2)} \]

\Comment{It is only obvious that we should also introduce and/or split/join constructions.}

\section{Information-descriptor layer}
%Textual or with graphical support

\subsection{Naming of types}
To each object type, a name is associated: 
   $\ONm: \TP{\Objects} \Func \Names$.  
To each role type, we can actually associated two names, a normal
role name, and a so-called reverse role name: 
   $\RNm: \TP{\Roles} \Func \Names$ and 
   $\RRNm: \TP{\Roles} \Func \Names$.

In terms of \SmartRef{join}, we might have:
\[ \begin{array}{lll}
  \ONm(A) = \SF{Person}     & \RNm(p) = \SF{is a coworker in} & \RRNm(p) = \SF{has coworker}\\
  \ONm(B) = \SF{Department} & \RNm(q) = \SF{is employer in}   & \RRNm(q) = \SF{has employer}\\
  \ONm(F) = \SF{Department coworkership}
\end{array} \]

When verbalizing facts, one will typically use verbalizations such as:
\[ \SF{Person working for Department} \]
The \SF{working for} phrase is not the name of a role type, but really
referring to the combination of two role types. For example, in the case
of \SmartRef{join}, this might be $p \Conc \Reverse{q}$. Using the
function:
   $\CNm: \TP{\Roles} \times \TP{\Roles} \Func \Names$
we associate a name to such role pairs. For example:
   $\CNm(p,q) = \SF{working for}$.

\subsection{Basic information descriptors}
Information descriptors can now be defined by providing their mapping to path
expressions. Let $o$ be an object type with $\ONm(o) = n$, then we have the
following atomic information descriptors:
\begin{eqn}
   \DSem{n} \EQ o
\end{eqn}
Also the role names lead to atomic information descriptors.  Let $p$ a role
type with $\RNm(p) = n$ and $\RRNm(p) = m$, then:
\begin{eqn}
   \DSem{n} \EQ p\\
   \DSem{m} \EQ \Reverse{p}
\end{eqn}
The names for role pairs lead to the following information descriptors. Let
$p$ and $q$ be role types such that $\CNm(p,q) = n$, then:
\begin{eqn}
   \DSem{n} \EQ p \Conc \Reverse{q}
\end{eqn}

If $v$ is a variable and $c$ a constant, we also have:
\begin{eqn}
   \DSem{v} \EQ v\\
   \DSem{c} \EQ c
\end{eqn}

\subsection{Complex information descriptors}
If $X$ and $Y$ are information descriptors, then so is the combination:
\begin{eqn}
   \DSem{X~~Y} \EQ \DSem{X} \Conc \DSem{Y}
\end{eqn}
With this concatenation operator, we for example have:
\[ \begin{array}{l}
   \DSem{\SF{Person working\_for Department}} = \Eol
   \DSem{\SF{Person}} \Conc \DSem{\SF{working for}} \Conc \DSem{\SF{Department}} =\Eol
   A \Conc p \Conc \Reverse{q} \Conc B
\end{array} \]

If $X_1$, \ldots, $X_n$ are information descriptors, then the confluence
operator is introduced at the information descriptor level as follows:
\begin{eqn}
   \DSem{\SFMT{THE~COMBINATION~OF} ( X_1, \ldots, X_n )} \EQ
      \Confluence{\DSem{X_1}, \ldots, \DSem{X_n}}
\end{eqn}
The head oriented logical connectives $\hand$, $\hor$, $\himplies$, $\hiff$ and
$\hminus$ lead to the following information descriptors:
\begin{eqn}
   \DSem{X \SFMT{AND~ALSO} Y}            \EQ \DSem{X} \hand     \DSem{Y}\\
   \DSem{X \SFMT{MUST~ALSO~BE} Y}        \EQ \DSem{X} \himplies \DSem{Y}\\
   \DSem{\SFMT{IF} X \SFMT{THEN~ALSO} Y} \EQ \DSem{X} \himplies \DSem{Y}\\
   \DSem{X \SFMT{IF~AND~ONLY IF} Y}      \EQ \DSem{X} \hiff     \DSem{Y}\\
   \DSem{X \SFMT{OR~IS} Y}               \EQ \DSem{X} \hor      \DSem{Y}\\
   \DSem{X \SFMT{COMBINED~WITH} Y}       \EQ \DSem{X} \hplus    \DSem{Y}\\
   \DSem{X \SFMT{BUT~NOT} Y}             \EQ \DSem{X} \hminus   \DSem{Y}
\end{eqn}
For the temporal operators we have:
\begin{eqn}
   \DSem{\SFMT{ALWAYS} X}     \EQ \always \DSem{X}\\
   \DSem{\SFMT{SOMETIME} X}   \EQ \sometime \DSem{X}\\
   \DSem{X \SFMT{PRECEDES} Y} \EQ \DSem{X} \precedes \DSem{Y}
\end{eqn}

\subsection{Domain rules}
Using information descriptors we can also define rules/predicates
pertaining to the domain modeled by an ORM model. If $X$ is an 
information descriptor, then we have the following atomic rules:
\begin{eqn}
   \RSem{\SFMT{ANY} X}  \EQ \ANY{\DSem{X}}\\
   \RSem{\SFMT{SOME} X} \EQ \ANY{\DSem{X}}\\
   \RSem{\SFMT{ALL} X}  \EQ \ALL{\DSem{X}}
\end{eqn}
Logical connectives are introduced as:
\begin{eqn}
   \RSem{R \SFMT{AND} S}     \EQ \RSem{R} \land \RSem{S}\\
   \RSem{R \SFMT{OR} S}      \EQ \RSem{R} \lor \RSem{S}\\
   \RSem{R \SFMT{IMPLIES} S} \EQ \RSem{R} \implies \RSem{S}\\
   \RSem{R \SFMT{IFF} S}     \EQ \RSem{R} \iff \RSem{S}\\
   \RSem{\SFMT{NOT} R}       \EQ \lnot \RSem{R}
\end{eqn}
As an abbreviation we also use:
\begin{eqn}
  \SFMT{NO} X \EQ \SFMT{NOT~SOME} X
\end{eqn}
For the temporal operators we have:
\begin{eqn}
   \RSem{\SFMT{ALWAYS} R}     \EQ \always \RSem{R}\\
   \RSem{\SFMT{SOMETIME} R}   \EQ \sometime \RSem{R}\\
   \RSem{R \SFMT{PRECEDES} S} \EQ \RSem{R} \precedes \RSem{S}
\end{eqn}


%\section{Reasoning with ORC}

%Express semantics of actions (transactions!) in terms of ORL. Pre-/Post-condition style.

%\QuestionsInChapter

\ChapterBib



==> wsm05.tex <==
\Chapter{Advanced Object-Role Modeling}{advanced-object-role-modeling}
\Version{13-05-05}

This chapter is mainly based on the work reported in~\cite{1993-Hofstede-PSM,
1995-Brouwer-ORMKernel, 1995-Halpin-ORMPoly, 1996-Proper-CDMKernel}.

\Section{Subtyping}{defining-subtypes}
Sub-typing is an important feature of fact-based modeling.
\SmartPageRef{specialization-hierarchy} showed an example of subtyping in terms
of a specialization hierarchy.

%\Image{10cm}{Example of a specialization hierarchy}{specialization-hierarchy}
\Comment{Discuss the animal example in detail. It is a great way of discussing
generalisation and specialisation \emph{processes}.}

The population of a subtype can be restrained further. Rules can be specified
that specify the `maximum' and `minimum' population of a sub-type. Normally, if
$x \Sub y$ then the population of $x$ is bounded by
\[ \emptyset \subseteq \Pop(x) \subseteq \Pop(y) \] 
Graphically, this leads to the situation i) as depicted in
\SmartRef{restricted-subtyping}. 
\Image{0.7\textwidth}{Restricting subtyping}{restricted-subtyping}

The population of a subtyping can be restricted further by requiring it to be a
sub/superset of some set of instances specified by a (subtype constraining)
rule. Situations ii), iii) and iv) of \SmartRef{subtyping} depict this
graphically. In situation ii), the population of $\SF{X}$ should at least
consist of those match rule $R$. In general, this can be defined as follows:
\[ \Subset(x,R) \EQ \always \All{\DSem{R} \himplies x} \]
Note: for $R$ to be a sensible rule, we should at least have for any $y$ such
that $x \Sub y$:
\[ \Pop \models_t \always \All{\DSem{R} \himplies y} \]
otherwise $\Subset(x,R)$ would lead to an inconsistent set of constraints on
the population.
 
While the situation from ii) provides a minimum population for $\SF{X}$, the
situation depicted in iii) does the reverse by demanding a maximimum
population. The population of \SF{X} is limited to those instances of
$\SF{X}$'s \emph{supertypes} that match rule $S$.
\[ \Superset(x,S) \EQ \always \All{x \himplies \DSem{S}} \]
The situation provided in iv) combines the maximum and minimum population.
Situation v) represents a very special case. In this case, the rule $R$
actually fully determines the population of the subtype, since:
\[ \DSem{R} \himplies x \himplies \DSem{R} \]
in other words:
\[ \DSem{R} \hiff x \] 
As a graphical abbreviation we will use the notation provided in situation vi),
which corresponds to the traditional notion of \emph{specialization} from
ORM~\cite{2001-Halpin-ORM}.

%\Image{\textwidth}{Example of a multi-rooted specialization hierarchy}{multi-root-specialization}
A further interesting case of specialization is depicted in
\SmartPageRef{multi-root-specialization}. It illustrates how specialization
hierarchies can have multiple roots. This example also introduces two important
classes of constraints: exclusiveness and totality of specializations.  If
$x_1$, \ldots, $x_n$ are types, then we can define:
\[ \Exclusive(x_1, \ldots, x_n) \EQ 
   \always \All{
      (x_1 \land (x_2 \lor \ldots \lor x_n)     \implies 0) 
      \land \ldots \land 
      (x_n \land (x_1 \lor \ldots \lor x_{n-1}) \implies 0)
   }
\]
If $x_1$, \ldots, $x_n$ are types with a common supertype $s$ 
  (such that $x_1 \Sub s \land \ldots \land x_n \Sub s$) 
then we can define:
\[ \Total(s:x_1, \ldots x_n) \EQ s \hiff x_1 \lor \ldots x_n \]
To express the semantics of totality in general we first need to identify all
common supertypes of a set of types:
\[ \CommonSuper(T) \EQ \Set{y}{\Al{x \in T}{x \Sub y}} \]
If $T$ is a set of types such that 
   $\CommonSuper(T) \EQ \setje{y_1, \ldots, y_m}$,
with $n > 0$, then we can define:
\[ \Total(T) \EQ \Total(y_1:T) \land \ldots \land \Total(y_n:T) \]
Based on~\cite{1993-Hofstede-PSM} a graphical abbreviation can be used for this
kind of sub-typing. This is depicted in \SmartRef{generalization}. The
right-hand side provides an abbreviation for the situation depicted in the
left-hand side.
\Image{0.8\textwidth}{Generalization}{generalization}

\section{Overlap of populations}
When considering the ORM schema as depicted in
\SmartRef{multi-root-specialization}, one would expect the populations of
\SF{Vehicle} and \SF{Distance} to be disjoint, while the populations of
\SF{Vehicle} and \SF{Product} are expected to overlap. Thus far, we have not
introduced any formal mechanism to enforce this type of behavior other that the
inclusion of populations for sub-types. To properly formalize this, we first
define the family (as it is `alive' at some point in time) of an object type
based on the sub-typing hierarchy as follows:
\[ \Family_t(x) \EQ \Set{y \in \TP{\Objects}_t}{y \Sub x \lor y = x} \]
Two object types are deemed \emph{type related} iff their families overlap:
\[ x \TypeRel_t y \EQ \Family(x) \intersect \Family(y) = \emptyset \]
If the population of object types overlaps, then they must be type related:
\begin{Axiom}{S}
  $\Pop_t(x) \intersect \Pop_t(y) \neq \emptyset \implies x \TypeRel_t y$
\end{Axiom}
Note that the converse does not necessarily hold.
  
\section{Abstraction}
To introduce abstraction (\emph{schema decomposition}), we start with an
example domain taken from~\cite{1996-Proper-CDMKernel}.

For our example domain, we consider a bank. \SmartRef{bank} shows the top level
abstraction of the banking domain. This schema displays five types: \SF{Bank},
\SF{Client}, \SF{Service}, \SF{enjoy}, \SF{of}. The \SF{Bank} type is an
abstracted type and forms the top abstraction of the entire banking
application. This is also the reason why the \SF{enjoy} and \SF{of}
relationship types, together with the remaining object types playing a role in
these relationship types, are drawn inside the \SF{Bank} type. Both \SF{Client}
and \SF{Service} types are abstractions themselves, although their underlying
structure is not shown at the moment. When stepping down to a lower level of
abstraction, the \EM{void} in these types will be filled with more detail.

\ScaledImage{0.5}{The top diagram of the Bank domain}{bank}
The \SF{Client} and \SF{Service} type are involved in a relationship type
called \SF{enjoys}. This is a many to many relationship where each client must
at least enjoy one service and each service offering must be enjoyed by some
person. The two black dots indicate that a client of the bank must indeed enjoy
some service, and conversely each service must be used by some client. The
arrow tipped bar spanning the two roles of the \SF{enjoys} relationship type
indicates that it is a many to many relationship. Similarly, the \SF{of}
relationship type models the fact that a bank has many clients, and clients can
be client of many banks. The \SF{(name)} suffix to \SF{Bank} indicates that a
bank is identified by a name. Basically, the use of the \SF{(name)} suffix is a
graphical abbreviation of the schema fragment depicted in \SmartRef{bank-full}.
The broken ellipse of \SF{BankName} type indicate that it is a {\em value
type}; i.e.\ its instances are directly denotable (strings, numbers, audio,
video, html).

\ScaledImage{0.5}{Fully detailed top diagram}{bank-full}
As a first refinement step we can now take a closer look at what a client is.
The details of the \SF{Client} type are shown in \SmartRef{bank-client}. There
we can see that each client is identified by a \SF{Client Nr}, as indicated by
the \SF{(nr)} suffix to \SF{Client}. Each client provides the bank with a
unique address as indicated by the arrow tipped bar spanning the role of the
\SF{lives at} relationship type that is attached to \SF{Client}. This address
is mandatory for each client. This "mandatoryness" is indicated by the black
dot. \SF{Address} is a normal object type without any other types clustered to
it. Therefore, it is drawn in the traditional ORM way using a solid ellipse.
The \SF{(description)} suffix to \SF{Address} within the solid ellipse
indicates that an address is identified by a description. This corresponds to
the same underlying graphical abbreviation.

Clients must all provide at least one name, but they may have aliases. This
leads to the arrow tipped bar spanning both roles of the \SF{has} fact type,
and the black dot on the client side. For authorization of transactions ordered
by telephone or fax, the bank and the client agree upon a unique password. The
combination of a password and address must uniquely identify a client
(indicated in the diagram by the encircled \SF{U}). Finally, clients may have a
number of phone numbers at which they can be reached.

With respect to the abstractions, we can now say that the relationship types
\SF{has identifying}, \SF{lives at}, \SF{reachable at}, \SF{has} (together with
the types playing a role in these relationship types) are clustered to
\SF{Client}. For each abstracted type, like \SF{Client}, such a clustering of
types (from a lower level of abstraction) is provided. This could be an
emptyset.
\ScaledImage{0.5}{Refinement of the client type}{bank-client}

In this example we refer to relationship types used in the bank example by
means of the text associated with these relationship types, such as \SF{has
identifying}. This text is a so-called \emph{mix fix predicate} verbalization.
These mix fix predicate verbalizations do not have to be unique. The
verbalization \SF{has} typically occurs numerous times in an average conceptual
schema. For example: \SF{Client has Client Name} and \SF{Client has Password}.
To uniquely identify relationship types (and types in general), each type
receives a unique name. For instance \SF{Client Naming} and \SF{Issued
Passwords} for the two earlier given examples.

The next refinement of the bank domain provides us with more details about the
service types available from the bank. This is depicted in
\SmartRef{bank-service}. The \SF{Service} type is a generalization of three
basic types: \SF{Credit Card Account}, \SF{Access Account}, and \SF{Term
Deposit Account}. The \SF{Access Account}s and \SF{Credit Card Account}s are
first combined into a so-called \SF{Statement Account}. It should be noted that
during a top-down modeling process, a type like \SF{Credit Card Account} will
start out as a `normal' entity type like \SF{Address}. However, as soon as
other types are clustered to such an entity type, they become abstracted types.

The double lining around the \SF{Access Account} type indicates that this type
occurs in multiple clusterings. A CASE Tool supporting this kind of graphical
representation, could have a feature in which clicking on such a double lining
results in a list of (abstracted) types in whose clustering this type occurs.
\ScaledImage{0.5}{Refinement of the service type}{bank-service}

As stated before, a statement account is a generalization of an access account
and a credit card account. The intuition behind a statement account is that for
such an account regular statements are sent to the clients and that a
transaction record is kept. These details of the statement account are shown in
\SmartRef{statement-account}. For each statement account, a number of
statements can be issued. A statement lists a number of transactions This is
captured by the \SF{lists} fact type. This fact type is, however, derivable
from the (to be introduced) issue date of a statement and the dates at which
the transactions took place. This derivability is indicated by the asterisk.
\ScaledImage{0.5}{Refinement of statement account}{statement-account}

One of the key features of the fact based modeling is inheritance of properties
between types in specializations. Instances (populations) are inherited in the
direction of the arrows. For example, each credit card account is a statement
account. Other properties, like clustered types, are inherited downwards.
Typically, properties at the type level are inherited downward, while
properties on the instance level are inherited upwards. The types clustered to
\SF{Statement Account} are therefore formally also part of the clusterings of
\SF{Credit Card Account} and \SF{Access Account}. Nevertheless, to avoid
cluttered diagrams, we have chosen not to show this inheritance explicitly in
the diagrams. Therefore, the details of the \SF{Credit Card} type do not show
the details of \SF{Statement Account}. The details of the \SF{Credit Card Type}
are provided in \SmartRef{credit-card}. For each credit card the bank stores
its kind, the spending limit, as well as the access account to which the credit
card is linked. The suffix "\SF{: Statement Account}" to "\SF{Credit Card
Account (nr)}" hints at the inheritance of the clustered types to \SF{Statement
Account}. In a CASE Tool supporting our technique, one could implement the
facility that clicking on the \SF{Statement Account} suffix leads to the
inclusion of the clustered types introduced by \SF{Statement Account}. Note
that both \SF{Access Account} and \SF{Money Amount} have double lining,
indicating that they occur in multiple clusters.
\ScaledImage{0.5}{Refinement of the credit card type}{credit-card}

For \SF{Access Account}, the details are shown in \SmartRef{access-account}.
All extra information actually shown there is the identification of an access
account; an \SF{Access Account Nr} as indicated by the \SF{(nr)} suffix.
Similar to the \SF{Credit Card Account}, all types clustered to \SF{Statement
Account} are also clustered to \SF{Access Account}, but we do not display this
graphically.
\ScaledImage{0.5}{Refinement of an access account}{access-account}

\SmartRef{bank-statement} shows the details of a \SF{statement}. Each
\SF{Statement} is issued on a unique date. This date, together with the
\SF{Statement Account} for which the \SF{Statement} was issued, identifies each
\SF{Statement}. Note that we decided to draw some contextual information of the
\SF{Statement} type to show how this type is identified. The \SF{for ... was
issued ...} and \SF{Statement Account} types are not part of the clustering of
\SF{Statement}. The balance as listed on a \SF{Statement} is, for obvious
reasons, derivable from the \SF{Transaction}s that have taken place on this
account.
\ScaledImage{0.5}{Refinement of a statement}{bank-statement}

The refined view on a transaction is shown in \SmartRef{bank-transaction}. A
\SF{Transaction} is identified by the combination of the account it is for and
a unique (for that account) transaction number. Note that contrary to a
\SF{Statement}, all components needed for the identification of
\SF{Transaction}s are part of the clustering. Each \SF{Transaction} involves a
certain money amount, occurs on a date, and is either a debit or credit
transaction (depicted by \SF{TR Kind}). Furthermore, for each \SF{Transaction},
some (unique) description may be provided. This example also shows that we must
allow for {\em mutually recursive} abstractions, as the \SF{Transaction} and
\SF{Statement Account} refinements refer to each other.
\ScaledImage{0.5}{Refinement of a transaction}{bank-transaction}

Term deposits form a world on their own. This is elaborated in
\SmartRef{term-deposit-account}. On each \SF{Term Deposit Account}, a client
can have a series of term deposits. Each time a \SF{Term Deposit} matures, this
term deposit can be rolled-over leading to a new \SF{Term Deposit} on the
current \SF{Term Deposit Account}. A special kind of \SF{Term Deposit} is the
\SF{Long Term Deposit}, which is a subtype of \SF{Term Deposit}. As each
subtype inherits all properties from its supertype, the \SF{Long Term Deposit}
type is an abstracted type as well. For these \SF{Long Term Deposit}s we store
whether the deposit is to be automatically rolled-over into a new deposit (the
short \SF{Term Deposit}s are of this kind by default). In the refinement of a
\SF{Long Term Deposit}, we shall also see what the so-called subtype defining
rule for these \SF{Long Term Deposits} is. Upon maturation, the invested amount
including the interest accrued is transferred to a pre-nominated \SF{Access
Account}. Finally, the interest rate given on the deposit is derived from a
table listing the \SF{Period}s for which amounts can be invested. The details
of the \SF{Period} type are given below.
\ScaledImage{0.5}{Refinement of a term deposit account}{term-deposit-account}

\ScaledImage{0.5}{Refinement of a term deposit}{term-deposit-refined}
A \SF{Term Deposit} itself is a clustering of the start and ending dates of the
deposits and the money amount invested. This is depicted in
\SmartRef{term-deposit-refined}. A \SF{Long Term Deposit} is a term deposit
with a duration of more than 60 days. In \SmartRef{long-term-deposit} the
details of a long term deposit are shown, including the subtype defining rule.
The \SF{Long Term Deposit} type inherits all clustered types from \SF{Term
Deposit}, while not adding anything to this. Finally, the complete definition
of the interest periods are given in \SmartRef{deposit-periods}.
\ScaledImage{0.5}{Refinement of a long term deposit}{long-term-deposit}

\ScaledImage{0.5}{Refinement of periods}{deposit-periods}
This completes the schema of the example domain. When modeling a domain like
this, the modeler has the choice of using as many layers of abstraction as the
modeler sees fit. We only provide a mechanism to introduce these abstractions
and are (initially) not so much concerned with the `sensibility' of abstraction
steps. One may, for example, argue that the example given in this section has
been split up into too many abstraction levels.

\WidthImage{\textwidth}{Complete diagram of the Bank domain}{full-bank-domain}
Sometimes, an analyst may want to see the entire schema. This is quite easy to
do by uniting all clusterings into one large schema. From the above discussed
schema fragments, one can derive the complete ORM schema as depicted in
\SmartRef{full-bank-domain} by uniting all clusters. This is, however, still
not the `lowest' level at which an ORM diagram can be displayed, since we have
used the standard abbreviations for simple identifications and the short
notation for objectifications. Objectification is a concept we have not yet
discussed in this paper. 

\Skip{
In general, when object type $x$ is a compositely identified object
type, i.e.\ more than one value type is used to identify its instances,
and all relationship types used to identify instances of $x$ are clustered to
$x$, then we can use the graphical abbreviation.
Examples of compositely identified object types are: \SF{Transaction}, 
\SF{Period}, \SF{Statement}, and \SF{Term Deposit}.
The only object types which have all relationship types needed for their 
identification clustered to themselves are \SF{Period} and \SF{Transaction}.
That is why in those cases we can use the graphical abbreviation as used
in \SmartRef{full-bank-domain}.
}

Also when looking at a design procedure for ORM schemas as presented in
\cite{1994-Halpin-ORM} the decision to model a \SF{Transaction}, say, as an
objectification or a flat entity type is based on considerations of
abstraction. When, for the modeling of the relationship types \SF{was for},
\SF{has}, \SF{took place on}, and \SF{is of} it is preferred to regard a
transaction as an abstraction from its underlying relationships to a statement
account and transaction number, then the objectified view is preferred to the
flat entity view. This directly corresponds to the decision whether these
underlying relationships should be clustered to the \SF{Transaction} object
type or not. Later we shall see that \emph{set types}, \emph{sequence types}
and \emph{schema typing} can be treated in a similar way. In
\cite{1994-Hofstede-EU,1994-Hofstede-EU-Identity} it is shown that \emph{set
types}, \emph{sequence types} and some other composed types are not fundamental
when introducing a special class of constraints which correspond to the set
theoretic notion of {\em axiom of extensionality}. This then allows us to
regard set typing, sequence typing and schema typing as forms of abstraction.

The schema depicted in \SmartRef{full-bank-domain} has the same {\em formal
semantics} as the combination of all previous schema fragments. However, the
{\em conceptual semantics} is different as the abstraction levels (the third
dimension) are now missing. Schema abstraction is purely a syntactical issue,
and thus carries no formal semantics. From the point of view of a modeler (and
a participant of the universe of discourse), the abstractions do have a
conceptual meaning. The abstractions represent certain choices of importance
within the universe of discourse.

An (E)ER view can easily be derived as well by uniting all clusterings except
for the lowest ones, but interpreting these as attributes. The (E)ER view on
this domain is given in \SmartRef{bank-domain-er}. The version we used there is
based on the one discussed in \cite{1992-Batini-ConceptualDBDesign}. Differing
extended ER versions use different notations for this concept
\cite{1985-Elmasri-ERSetModel,1994-Elmasri-DBFundamentals,1990-Engels-ConcMod}.
The names for attributes in this diagram are simply based on the verbalizations
given in the ORM schema. For most ER modelers, the concept of using elaborate
verbalizations is new. One could allow for the specification of specific
attribute names to, for example, abbreviate \SF{with minimum deposit of
MoneyAmount (\$)+} to \SF{MinDeposit}. In this article we do not discuss naming
conventions in detail but rather focus on the underlying conceptual issues. In
\cite{1995-Brouwer-ORMKernel} we have provided a more detailed study of the
relationship between different ER versions and ORM. A detailed case study is
also presented there, in which the different concepts underlying these modeling
techniques are related, together with a mapping of the (graphical) concepts
between the two classes of data modeling techniques.
\Image{\textwidth}{Complete ER diagram of the Bank domain}{bank-domain-er}

\Skip{
Of course for the (E)ER case one can also take objectifications into
consideration and treat them as a graphical abbreviation
In the example domain, however, they have all disappeared.
When there would be a compositely identified object type occurring on
an abstraction level higher than one, then this would have lead to an
objectification in the (E)ER representation.
In the remainder we shall also see fragments of an OMT
(\cite{Book:91:Rumbaugh:OO}) view on this same domain. 
An OMT view does not become very interesting until we have introduced some
notion of operations on the types of the schema.
Without operations, an OMT diagram can simply be seen as another 
(E)ER dialect.

Some modeling techniques, for example OMT and 
some Extended ER versions (e.g.\ \cite{Book:94:Elmasri:DBFundamentals}) 
support forms of aggregation. 
Although one has to be careful with the notion of {\em aggregation}, as 
different authors define this concept differently, most of the definitions
known to us are simply forms of abstraction similarly to objectification.
As an example consider \SRef{\Aggregation}.
The left hand side diagram is an OMT representation of the schema on
the right hand side.
\EpsfFig[\Aggregation]{OMT aggregation as abstraction mechanism}

One might now successfully argue that by combining all existing
abstraction mechanisms into one single unifying abstraction concept we lose
expressiveness with respect to the conceptual semantics.
When a modeler decides to model something as an aggregation, as opposed
to an objectification, then this decision is of conceptual relevance.
Therefore, we shall introduce in the CDM Kernel the possibility to distinguish
between different flavors of abstraction.
The ones we have seen so far are: objectification, grouping (set types, 
sequence types, etc), aggregation, and abstraction in general.
In the CDM Kernel, we shall not prescribe a fixed set of abstraction
flavors. 
This is left as a configuration option for a concrete application of
the CDM Kernel.

Finally, when entering a model into the CDM Kernel using a normal `flat' 
conceptual modeling view, like traditional ORM or (E)ER, the `third 
dimension' can be added (reverse engineered) to such a flat model by 
means of existing algorithms.
Examples of such algorithms can be found in 
\cite{Article:83:Vermeir:Abstraction,% 
Article:85:Shoval:DBDesign,%
Article:86:Feldman:Abstraction,% 
Article:93:Campbell:ExternalMapping,%
Article:94:Campbell:AbstractionORM,%
Article:94:Campbell:Abstraction,%
Article:94:Shoval:BRM-OO}.
The key difference between each of these algorithms lies in the extent to
which they try to incorporate semantic information that is hidden
in the constraints and verbalizations provided with the schema.
Currently, work is underway with the authors of 
\cite{Article:94:Campbell:Abstraction} in formalizing their approach
more in line with the CDM Kernel presented in this article.
}

\section{Set types}
In set theory we use $\Powerset(X)$ to denote the set consisting of all subsets of $X$ (see for instance~\cite{1979-Levy-SetTheory}). When modeling complex domains, we sometimes have the need to model set types being types whose instances can be regarded as being sets of other instances. This notion is the same as the notion of grouping introduced in the  IFO data model~\cite{1987-Abiteboul-IFO}).  An illustrative example, taken from~\cite{1994-Hofstede-EU}, is shown in \SmartRef{convoy}. A \SF{Convoy} is taken to consist of a set of \SF{Ship}s, where this set of ships really \emph{identifies} the convoy. In other words, if two convoys contain the same set of ships, they really are the same convoy. This is actually similar to the existentiality axiom from set theory:
\[ \Al{i}{i \in X \iff i \in Y} \implies X = Y \] 
In \SmartRef{convoy} the existential uniqueness is expressed by the circle with the two horizontal bars. If there would be only one bar, this would be normal uniqueness of the associated role. The extra (slightly shorter) bar signifies this to be an \emph{existential} uniqueness constraint.
\ScaledImage{0.75}{Convoy of ships}{convoy}

Formally, we introduce existential uniqueness by first identifying the variety an instance of a fact type may have with regards to a set of roles. Let $f \in \TP{\Facts}$ be a fact type and $R \subseteq \RolesOf(f)$ be a set of roles involved in this fact type. The variety of instances $i \in \Pop(f)$ with regard to their roles $R$ is defined as:
\[ \Variety(i,f,R) \EQ \Set{j[R]}{j \in \Pop(f) \land j[\;\Complement{R}\;] = i[\;\Complement{R}\;]} \] 
For a set of roles $R$ of some fact type $f$, we can now express the existantial uniqueness constraint as:
\[ \ExtUnique(f:R) \EQ 
   \Al{i,j \in \Pop(f)}{\Al{e}{e \in \Variety(i,f,R) \iff e \in \Variety(j,f,R)} \implies
   j[\;\Complement{R}\;] = i[\;\Complement{R}\;]} 
\] 
where $\Complement{R} = \RolesOf(f) \SetMinus R$. Note the correspondance to existantiality from set theory. A more compact form (which we are allowed to use due to the existantiality axiom from set theory) would be:
\[ \ExtUnique(f:R) \EQ \Al{i,j \in \Pop(f)}{\Variety(i,f,R) = \Variety(j,f,R) \implies 
   j[\;\Complement{R}\;] = i[\;\Complement{R}\;]} 
\] 

Using the abstraction mechanism from the previous section, we are able to more introduce a number of shorthand notations for set types. These are depicted in \SmartRef{convoy-decomp}.
\ScaledImage{0.75}{Shorthand notations for convoys of ships}{convoy-decomp}

\section{Multi-set types}
A variation of sets is a multi-set. In a multiset, elements can occur multiple times. Using the existantial uniqueness constraints, a multi-set can be modeled as depicted in \SmartRef{train-composition}. In the depicted domain, a train composition class is defined as a multi-set of types of carriages. 
\ScaledImage{0.75}{Train composition classes}{train-composition}

Using the abstraction mechanism, we are again able to more introduce a number of shorthand notations for multi-set types. These are depicted in \SmartRef{train-composition-decomp}.
\ScaledImage{0.75}{Shorthand notations for train composition classes}{train-composition-decomp}

\section{Sequence types}
A specific train consists of a sequence of carriages. To model this compactly, we introduce the notion of a sequence type. This leads to the situation as depicted in \SmartRef{train-sequence}.
\ScaledImage{0.75}{Train as a sequence of carriages}{train-sequence}

Using the abstraction mechanism, we are again able to more introduce a number of shorthand notations for sequence types. These are depicted in \SmartRef{train-sequence-decomp}.
\ScaledImage{0.75}{Shorthand notations for trains as sequences of carriages}{train-sequence-decomp}

\section{Schema types}
In some situations we need types whose instances are really entire populations of other (smaller) schemas. An example of such a situation is shown in \SmartRef{activity-graphs}.
\ScaledImage{0.75}{Activity graphs usign a schema type}{activity-graphs}

Using the abstraction mechanism, we are again able to more introduce a number of shorthand notations for schema types. These are depicted in \SmartRef{schema-type-decomp}.
\Image{\textwidth}{Shorthand notations for schema types}{schema-type-decomp}

\Comment{We should also add the grammar box!!}

\QuestionsInChapter

\ChapterBib


==> wsm06.tex <==
\Chapter{The Act of Modelling}{act-of-modeling}
\Version{13-04-05}

In this chapter, which is based on the work reported in~\cite{2004-Proper-ORMforDM, 2004-Hoppenbrouwers-LinguisticComplexity}, we turn to the question \emph{how to model a domain}; a question to which there is no simple, one-size-fits-all answer.

\section{What to model?}
\begin{itemize}
   \item Modeling goal
   \item Intended audience
   \item Viewpoint
\end{itemize}
% Don't discuss viewpoints here yet! Focus on the challenge. The other parts should be moved to MDSE as it allows us to put modelling in an SE context. Announce this in this chapter!!

\section{The modeling challenge}
\subsection{Goal-bounded and communication-driven}
Some modeling approaches, such as NIAM~\cite{1989-Nijssen-NIAM} and ORM~\cite{2001-Halpin-ORM}, suggest or prescribe a detailed procedure. Practice shows, however, that experienced modelers frequently deviate from such procedures \cite{1993-Verhoef-ModellingSupport}:
\begin{quote}
  In most cases, [the information engineers] stated that they preferred to pay attention to a specific part of the problem domain, usually to fill clear lacunae in their insights in the problem domain.  Their momentary needs strongly influenced the order in which the several modelling techniques were used. Modelling techniques were used as a means to increase insights or to communicate insights, be it in the problem domain itself or in a specific solution domain.
\end{quote}
Yet deviating from a modeling procedure should be done with some caution. While a pre-defined modeling procedure should never become ``an excuse to stop thinking'', situational specificity should not become an excuse for taking an ad-hoc approach to the modeling effort. A more stable anchor is needed upon which modelers can base themselves when making decisions during the modeling process. We believe that domain modeling requires a goal-bounded and communication-driven approach. With goal-bounded we hint at the fact that when modeling a domain, a modeler is confronted with a plethora of modeling decisions. These decisions range from the modeling approach used, the intended use of the results, to decisions pertaining to the model itself.  For example:
\begin{itemize}
  \item What parts of the domain should be considered relevant?
  \item What is the desired level of detail and formality?
  \item To what level should all stakeholders agree upon the model?
  \item Should the model be a representation of an actual situation (\emph{system analysis}) or of a desired situation (\emph{design})?
  \item Should the model be a representation of \emph{what} a system should do, or should it be a representation of \emph{how} a system should do this?
% Die laatste vergt overigens ook
% de constructie van een nieuwe relevante sociale structuur (en ....
% gaat daar niet juist ook veel mis bij IT systemen .......).
  \item Should a certain phenomenon in the domain be modeled as a relationship, or is it an object on its own?
\end{itemize}
Having an explicit, and articulated, understanding of the modeling goals provides modelers with guidance in making the right decisions with regards to the above mentioned issues.  Modeling goals, therefore, essentially provide the \emph{means} to \emph{bound} modeling space.

In most situations where a domain needs to be modeled, the modeler cannot merely passively observe the domain. Modelers will need to interact with representatives from the domain. These representatives then become \emph{informers} (who are likely to also have a stake with regards to the system being developed). Therefore, modelers will need to communicate intensively with the informers in order to refine the model. What is more, numerous domain models that are produced during system development will need to be accepted and agreed upon --validated-- by the informers (being stakeholders of the future system). The claim has often been voiced that in modeling practice, `the process is just as important as the end result', suggesting that a correct end-result is not always a guarantee for success. A domain model should ideally be a product of a \emph{shared understanding of a domain's stakeholders}. It requires a `buy-in' by all stakeholders involved. A domain model that is correct from a theoretical or technical point of view but does not have the required support from the key stakeholders is arguably worse than a domain model with some flaws that does have such support.

A modeling process can thus be seen as a communication-driven process \cite{2003-Frederiks-InformationModeling,2003-VeldhuijzenVanZanten-Rational}. The principles of natural language driven modeling approaches \cite{1989-Nijssen-NIAM,1992-Embley-OOSA,1994-Kristen-KISS,2001-Halpin-ORM} can be used as a basis for shaping the communication process between informer and modeler.

\subsection{Aspects of a method}
When considering a modeling approach or method, several aspects thereof can be discerned \cite{1989-Seligmann-Framework,1990-Wijers-Modelling}. An important distinction to be made is that between a product oriented perspective and a process oriented perspective. In terms of the framework presented in \cite{1989-Seligmann-Framework,1990-Wijers-Modelling} these are referred to as the \emph{way of modeling} and \emph{way of working}, respectively:
\begin{description}
  \DefItem[Way of modeling] The way of modelling provides an abstract description of the underlying modelling concepts together with their interrelationships and properties. It structures the models which can be used in the information system development, i.e.\ it provides an abstract language in which to express the models.
  \DefItem[Way of working] The way of working structures the way in which an information system is developed. It defines the possible tasks, including sub-tasks and ordering of tasks, to be performed as part of the development process. It furthermore provides guidelines and suggestions (heuristics) on how these tasks should be performed.
\end{description}
In the case of domain modeling, the \emph{way of working} represents the process followed when modeling a domain. In the following sections, we will mainly elaborate on this aspect. The \emph{way of modeling} used for domain modeling is likely to be prescribed by a diagramming technique such as ORM diagrams~\cite{2001-Halpin-ORM}, ER diagrams~\cite{1976-Chen-ER} or UML class diagrams~\cite{1999-Booch-UML}.

\subsection{The process of modeling}
In general, the goals underlying (business) domain modeling are~\cite{2004-Bleeker-ConceptManagement}-
\begin{enumerate}
  \item articulate clear and concise meanings of business domain concepts and
  \item achieve a shared understanding of the concepts among relevant stakeholders.
\end{enumerate}
Based on the results reported in~\cite{2003-Hoppenbrouwers-FreezingLanguage}, we consider domain modeling in the context of system development to chiefly concern three streams of (mutually influencing) activities-
\begin{description}
  \DefItem[Scoping environments of discourse] The aim of this stream of activities is to scope the environments of discourse that are relevant to the system being developed, and determine the set of actors associated to each of these environments.
  \DefItem[Concept specification] For each of the identified environments of discourse, the relevant business domain concepts should be specified in terms of their:
  \begin{itemize}
    \item meaning
    \item relationships to other concepts (and the constraints governing these relationships)
    \item possible names used to refer to them
  \end{itemize}
  \DefItem[Concept integration] The concepts as identified and defined in the different environments of discourse may well clash. As a part of this, homonyms and synonyms are likely to hold between different terminologies. The aim of this stream of activities is to determine how to deal with this, and act upon it. %In section~\ref{pluriformity} we will elaborate on this.
\end{description}
Since these streams of activities can be expected to influence each other, it is not likely that they can be executed in a strict linear order.

In general, the processes that aim to arrive at a set of concepts together with their meaning and names, are referred to as \emph{conceptualization processes}~\cite{2003-Hoppenbrouwers-FreezingLanguage}. When, as in the context of software development, conceptualization is performed deliberately, as a specific task and with a specific goal in mind, it is referred to as an \emph{explicit conceptualization process}. The above mentioned stream of activities called concept specification is such an explicit conceptualization process. In~\cite{2003-Hoppenbrouwers-FreezingLanguage,2004-Bleeker-ConceptManagement} a reference model for conceptualization processes is provided. This reference model distinguishes five streams of activities or \emph{phases}:
\begin{description}
   \DefItem[Assess domain and acquire raw material] Domain modeling always begins with a brief scan or assessment of the domain to get a feeling for scope, diversity and complexity of the domain, as well as to identify the relevant stakeholders for the domain (usually but not necessarily a subset of the project stakeholders).
   In addition, the activity aims to bring together input documents of all sorts that provide a basic understanding of the environment of discourse that is relevant to the environment of discourse under consideration.
   \DefItem[Scope the concept set] In this phase, formal decisions are to be made regarding the concepts that somehow play a role in the environment of discourse and how these concepts interrelate.\footnote{In an earlier version of this framework, this was referred to as \emph{scoping the universe of discourse}.}
   \DefItem[Select relevant concepts] The goal of this phase is to focus on those concepts in the environment of discourse that bear some relevance to the system to be developed. These are the concepts that should be defined and named formally in the next step.
   \DefItem[Name and define concepts] All of the concepts selected in the previous phase should be named and defined. Defining the concepts may also include the identification of rules/laws/constraints governing instances of the defined concepts.
   \DefItem[Quality checks] Final quality checks on the validity, consistency and completeness of the set of defined concepts.
\end{description}
These streams should essentially be regarded as sub-streams of the concept specification stream.

\section{Ambition levels for modeling}
We have made a distinction between four levels of ambition at which a modeler may approach the task of modeling a domain. These levels can also be regarded as the order in which a novice modeler may learn the art of domain modeling:
\begin{description}
  \DefItem[Singular] This level of ambition corresponds to the modeling approaches as described in e.g.\ NIAM~\cite{1989-Nijssen-NIAM} and ORM~\cite{2001-Halpin-ORM}. It involves the modeling of a \emph{single} environment of discourse based on complete input; usually in terms of a \emph{complete} verbalization of (\emph{only}) the relevant parts of the domain.
  \DefItem[Elusive] At this level of ambition, modelers need to cope with the unavoidable iterative nature of the modeling process. As a modeling and/or system development process proceeds, the insight into the domain may increase along the way. This replaces the idealized notion of completeness of input with one of incremental input. The increments in the model are not related to a changing domain, but rather to improved ways of conceptualizing it.
  \DefItem[Pluriform] At this next level of ambition, we recognize the fact that when developing a realistic system, we do not simply deal with one single unified environment of discourse (and related terminologies and concepts), but rather with a number of interrelated environments of discourse \cite{2004-Proper-ConceptEvolution}.
  \DefItem[Evolving] The final ambition level recognizes the fact that domains themselves are not stable; they evolve over time \cite{2004-Proper-ConceptEvolution}.  As a result, what may have started out as a correct model of a domain, may become obsolete due to changes in the domain. New concepts may be introduced, or existing ones may cease to be used. However, subtle changes may occur as well, such as minor changes in the meaning of concepts, or the forms used to represent them.
\end{description}
In the next section, we will discuss domain modeling at the \emph{singular}, \emph{elusive} and \emph{pluriform} levels of ambition. The \emph{evolving} level is omitted for now.

%%%%%% , as it is applies generally, i.e.\ is not typically language-related.

% Which ones shall we discuss in detail in this article? Stijn says-
% elusiveness is linked to completeness- refinement of concepts,
% adding of concepts; linked to increasing insight in domain. This
% is linguistically relevant. Pluriformity is directly linked to my
% thesis, i.e. clearly also linguistically relevant. Evolution is
% related to pluriformity, but entaisl time to be included as a
% factor. This is linguistically speaking the least relevant aspect.
% I would prefer focus on 2. pluriformity and 2. elusiveness.
%\section{Modeling from a Language-Action Perspective}

\section{Meeting the challenge}
\label{meeting}

This section aims to discuss the domain modeling process with respect to three of the identified levels of ambition- \emph{singular}, \emph{elusive} and \emph{pluriform}. We will structure our discussion by using the framework of activity streams for domain modeling as introduced in the previous section.

\subsection{Modeling a singular domain}
At this level of ambition we are only interested in the modeling of a single environment of discourse based on complete input. In terms of the above framework for domain modeling, this ambition level assumes that-
\begin{itemize}
  \item No (further) scoping of the environment of discourse is needed
  \item The domain has been assessed and raw material is available
  \item Concept integration only needs to take place within the given
  environment of discourse
\end{itemize}
Natural language driven modeling approaches like NIAM~\cite{1989-Nijssen-NIAM} and ORM~\cite{2001-Halpin-ORM} concern elaborately described ways of executing a domain modeling process at this ambition level. For example, the modeling procedure as described in ORM~\cite{2001-Halpin-ORM} identifies the following steps:
\begin{description}
  \item[Step 1 -- Transform familiar examples into elementary facts] This step involves the verbalization in natural language of samples take from the domain.
  \item[Step 2 -- Draw the fact types and apply a population check] In this step, a first version of the schema is drawn. The plausibility of the schema is validated by adding a sample population to the schema.
  \item[Step 3 -- Trim schema and note basic derivations] In this step, the schema is checked to see if any of the identified concepts are basically the same, and should essentially be combined. Furthermore, derivable concepts (e.g.\ sales-price $=$ retail-price $+$ mark-up) are identified.
  \item[Step 4 -- Add uniqueness constraints and check the arity of fact types] At this point, it is determined how many times an instance of an identified concept can play specific roles. For example, is a \emph{person} allowed to \emph{own} more than one \emph{car}?
  \item[Step 5 -- Add mandatory role constraints and check for logical derivations] This step completes the basic set of arity constraints on the relationships in the schema, by stating wether or not instances of a concept \emph{should} play a role. For example, for each \emph{car}, the \emph{year of construction} should be specified.
  \item[Step 6 -- Add value, set-comparison, and subtyping constraints] The ORM diagramming technique provides a rich set of graphical constraints. This step is aimed at specifying these constraints.
  \item[Step 7 -- Add other constraints, and perform final checks] Finally, there may be some constraints in the domain that cannot be expressed graphically. In this last step, these constraints can be specified and
\end{description}
In terms of our framework for domain modeling processes, this procedure constitutes a rather specific way of executing the \emph{concept specification} stream of activities. It is really geared towards the (conceptual) analysis of a domain in order to design a database, rather than a general analysis of concepts playing a role in a domain. The procedure presented above is not applicable to all situations and all modelers.  

Even though the above order is very explicit, and therefore well suited for educational purposes, a goal-bounded approach to domain modeling requires a more refined view. The key question concerns the \emph{goal} for which a domain is modeled. During the \emph{definition} phase of the software development life-cycle, when the main goal is to support requirements engineering activities, the seven steps as described above are likely to be overkill. In such a context, modelers are likely to skip steps 6 and 7. The modeling procedure as discussed in~\cite{2001-Halpin-ORM}, also requires modelers to identify how concepts (such as car, co-workers, patient, etc.) are identified in a domain (e.g.\ by means of a registration number, employee number, patient number, etc.). During the definition phase, these identification mechanisms are not likely to be relevant (\emph{yet}).

During the \emph{design} phase of a software system most of the seven identified steps are indeed needed. However, experienced modelers are also likely to merge steps 1-3, steps 4-5, as well as steps 6-7, into three big steps. The resulting three steps will generally be executed consecutively on a `per fact' base. In other words:
\begin{enumerate}
  \item For each fact type, execute 1-3
  \item For each fact type, execute 4-5
  \item For each fact type, execute 6-7
\end{enumerate}
Some more empirical background to this, experience based observation, can be found in e.g.~\cite[page 161]{1993-Verhoef-ModellingSupport}.
\begin{quote}
  The order in which the various modeling tasks are performed differs to a large extent. A clear distinction exists between prescribed modeling knowledge and applied modeling knowledge, in this respect. Whereas an almost strictly \emph{linear} order of performing modeling tasks is prescribed, a very \emph{opportunistic} order is actually used. This order seems to be determined by at least two essentially different factors- the problem domain and the information engineer.
\end{quote}
Note that when an initial domain model already exists, e.g.\ as produced in the definition phase in support of requirements engineering, this will have to be used as a starting point for completion. In other words, in practice, a domain model is likely to develop incrementally along with the software development life cycle.

ORM is not the only modeling approach that is based on analysis of natural language. However, providing a full survey of such approaches is beyond the scope of this article. Nevertheless, two approaches are worth mentioning here. In~\cite{1992-Embley-OOSA} the Object-Oriented Systems Analysis method is presented. It uses a natural-language based approach to produce an Object-Relationship Model (accidently also abbreviated as ORM) that serves as a basis for further analysis. The \emph{way of working} used is not unlike that of ORM. Its \emph{way of modeling}, however, has a more sketchy nature and has been worked out to a lesser degree.  The KISS approach, as reported in~\cite{1994-Kristen-KISS}, also uses natural language analysis as its basis. It provides some support in terms of a \emph{way of working}, but does this in a rather prescriptive fashion that presumes some very particular (and limited) intermediary goals. A wide spectrum of modeling concepts are introduced (\emph{way of modeling}) covering a wide range of diagraming techniques (not unlike the UML~\cite{1999-Booch-UML}).

Independent of the approach used, a modeling process always needs to be flanked by a continuous communication process with the stakeholders \cite{2003-VeldhuijzenVanZanten-Rational}. Communication brings along the aspect of documentation. Modeling itself can hardly do without face-to-face discussions; however, the (intermediate) results need to be recorded in such a way that they can be communicated effectively to the stakeholder community~\cite{2002-Frederiks-Infogrammars,1997-Frederiks-InformationGrammars}. In this respect we could argue that any modeling approach also needs a \emph{way of communication/documenting}. Since documentation serves the purpose of communication, the documentation \emph{language} should align with the accepted language concepts in the domain. In practice it turns out that graphical notations such as ORM or UML diagrams are not the most obvious way to communicate a model to stakeholders, since most domain stakeholders do not comprehend this kind of ``IT language''. Often, it is better to use more intuitively readable diagrams and natural language to communicate concepts and their relationships and constraints, while occasionally, a more mathematical or algorithmic style may be useful in certain expert domains.

%What intellectual capacities are required from the modeler? And by the
%domain expert? Which roles can be discerned anyway? Zie ook
%artikel Paul \& Theo.
%They assume the standard two roles of Domain Expert and Analyst. They
%distinguish modeling competencies (skills) required for each role- see their
%Table 1. The names of the skills as they present them are not very meaningful
%without considerable extra explanation. Perhaps we should rephrase them? Else
%create a really tight summary.
%How do these roles map on roles and responsibilities in commercial projects?

%Which viewpoints should be used when modeling? Suitable for whom/what?
%Euuuh, da's wel een hele grote vraag. Ik stel voor dat we dat even
%parkeren. Maar wel aanstippen.  What is the state of the art?
%Verwijzing naar Archimate.

%\subsection{Modeling from a language-action perspective}


==> wsm07.tex <==
\Chapter{Natural-Language Foundations of Information-Systems Modeling}{natural-language-work-systems}
\Version{12-05-05}
In this chapter, we will essentially use the ORM philosophy to model key aspects of information-systems. This requires the immediate introduction of some new concepts into our ontology, such as: agentive, experiencing , circumstantial and predicative role, action, predication, agent, subject and context elements. These concepts allow us to reason about such things as: \emph{when} does something happens (triggering), \emph{what} happens (action), \emph{who}/\emph{what} makes it happen (agentr),  \emph{who}/\emph{what} does it happen \emph{to} (subject) in \emph{which}/\emph{what} circumstances (context).

With these new concepts, we can typically take ORM domain models and ``annotate'' them in terms of the refined concepts. We will base this process of annotation on linguistic foundations, much in the same vein as the modeling approach from the \emph{Domain Modeling} course. Based on these annotated ORM models, we will be able to mechanically derive process models in a modeling notation (ArchiMate~\cite{2005-Lankhorst-ArchiMate}) that is particularly suited for the modeling of business processes. This will be the focus of the \emph{next} chapter.

\section{Classes of roles}
We consider \PDN{organizational-system}, i.e.\ \OAS or work-systems:
\begin{itemize}
   \item So there is activity going on.
   \item In other words, there are active elements.
   \item A specific class of \PDN{concept} should therefore be: actions.
   \item Even more, these actions are performed by \emph{agents}, and are performed on \emph{subjects}. We want to be able to `talk' about these these agents and subjects.
   \item In other words, we actually need three additional classes of \PDN{concept}:
   actions, agents and subjects.
\end{itemize}
Let us now analyze this closer from a natural language perspective. Consider, once again, the following domain:
\begin{quote} \sffamily \scriptsize
  A person with name Erik is writing a letter to his loved one, at the desk in a romantically lit 
  room, on a mid-summer's day, using a pencil, while the cat is watching.
\end{quote}
with elementary facts:
\begin{quote} \sffamily \scriptsize
  A person is writing a letter\\
  This person has the name Erik\\
  This letter has a romantic nature\\
  This letter has intended recipient Erik's loved one\\
  The writing of this letter by Erik, occurs on a mid-summer's day\\ 
  The writing of this letter by Erik, is done using a pencil\\
  The writing of this letter by Erik, is done while the cat is watching\\
  The writing of this letter by Erik, is taking place at a desk\\
  This desk is located in a room\\
  This room is romantically lit
\end{quote}
As mentioned before, within these elementary facts, several \emph{players} can be discerned. In the above example, we can isolate the players and facts as follows:
\begin{quote} \sffamily \scriptsize
  [A person] is writing [a letter]\\{}
  [This person] has [the name Erik]\\{}
  [This letter] has a [romantic nature]\\{}
  [This letter] has intended recipient [Erik's loved one]\\{}
  [The writing of this letter by Erik], occurs on a [mid-summer's day]\\{} 
  [The writing of this letter by Erik], is done using [a pencil]\\{}
  [The writing of this letter by Erik], is done while [the cat] is watching\\{}
  [The writing of this letter by Erik], is taking place at [a desk]\\{}
  [This desk] is located in [a room]\\{}
  [This room] is lit in [a romantic] way
\end{quote}
The writing of the letter is the central fact in the above domain. All players in the facts describing the above domain are players in this domain. What are the actions, agents and subjects? Several degrees of activeness exist with regards to the role  player plays in a fact/domain:
\begin{itemize}
 \item Some roles will be more active than others.
 \item This is where we find inspiration in theories regarding verbs and the `things' that may play a (functional) role in these verbs.
 \item We limit ourselves to those classes that are indeed relevant when considering activity in systems.
\end{itemize}
In decreasing scale of activity:
\begin{description}
  \DefItem[Agentive role] A role where the player is regarded as carrying out an activity.

  In the example domain: {\sf The person}.
  
  Two sub-classes may be identified:
  \begin{description}
     \DefItem[Initiating role] An agentive role, where the player is regarded as being the initiator of the activity.
     \DefItem[Reactive role] A non-initiating agentive role.
  \end{description}

  \DefItem[Experiencing role] A role where the player is regarded as experiencing/undergoing an activity.

  In the example domain: {\sf a letter}, {\sf a loved one} and {\sf the cat}.
           
  Three sub-classes may be identified:
  \begin{description}
     \DefItem[Patientive role] An experiencing role, where the player is regarded as purposely undergoing changes (including its very creation)
     \DefItem[Receptive role] An experiencing role, where the player is regarded as the beneficiary/recipient of the results of the activity
     \DefItem[Observative role] An experiencing role, where the player is regarded as observing/witnessing the activity
  \end{description}
  
  \DefItem[Contextual role] A role where the player is regarded as being a part of the context in which the activity takes place.
  
  Four sub-classes may be identified:
  \begin{description}
     \DefItem[Instrumental role] A role where the player is regarded as being an instrument in an activity.

     In the example domain: {\sf a desk} and {\sf a pencil}.
  
     \DefItem[Locative role] A role, where the player is regarded as being the location of an activity, in terms of a spatial or temporal orientation.

     In the example domain: {\sf the desk}, {\sf the room} and {\sf mid-summer's day}
  
     \DefItem[Catalysing role] A role, where the presence of the player is regarded as being beneficial (either in a positive or a negative way) to an activity.

     In the example domain: {\sf the room lit in a romantic way}.
  \end{description}
  
  \DefItem[Predicative role] A role where the player is regarded as being a predicate on some other player.
  
  In the example domain: {\sf the name Erik}.
\end{description}
The choice between these different levels of role is subjective. It depends on the viewer. The players of the four main classes of roles are regarded as \emph{agents}, \emph{subjects}, \emph{context elements}, and \emph{predicators} respectively.

\Comment{We should turn to the LAP literature to try and hammer this down more fundamentally!!}

In the example domain, the {\sf writing of the letter by the person} can be regarded as a key activity in the domain. In other words, {\sf writing} is an action, while the {\sf person} is the agent and the {\sf letter} is the subject. We may regard the {\sf cat} and the {\sf loved one} as a subject as well. What about the {\sf pen}, the {\sf name Erik}, the {\sf desk}, etc? They are really players in \emph{predications} over the other players. The fact that a pen is used by the person to write the letter is a \emph{predication} of the writing \emph{action}.

If we were to zoom in on a sub-domain of the above sketched domain, we could actually find that what was a subject in the super-domain is an agent in the sub-domain. Consider, for example, the sub-domain:
\begin{quote} \sffamily
  [The writing of this letter by Erik], is done while [the cat] is watching
\end{quote}
When considered in isolation, one may quite easily argue that the primary action here is the {\sf watching}, which is something that is being done by the {\sf cat}. This really makes the {\sf cat} into an agent rather than the subject, while the thing that is being watched (the {\sf writing}) becomes the subject. This really means that our notions of agent, subject, action and predication are really to be taken \emph{relative} to the domain under consideration, which is in line with the subjective approach to modeling as taken in this textbook.

Formally, we presume the existance of sets $\AgentiveRoles, \ExperiencingRoles, \ContextualRoles, \PredicativeRoles \subseteq \Roles$ with agent and subject \emph{roles} respectively. These classes of roles form a partition of the roles:
\begin{Axiom}{S}
   $\AgentiveRoles$, $\ExperiencingRoles$, $\ContextualRoles$ and $\PredicativeRoles$ are a partition of $\Roles$.
\end{Axiom}
With this we can also define the sets of actions and predications, respectively, as:
\begin{eqn}
   \Actions      \EQ \Set{\Fact(r)}{r \in \AgentiveRoles}\\
   \Predications \EQ \Facts \SetMinus \Actions
\end{eqn}
In other words, all facts that have an agentive role are regarded as actions. The other facts are (pure) predications.

Typing should adhere our refined ontology. In other words:
\begin{Axiom}{S}
   For all $X \in \setje{\Facts, \Roles, \Players}$ we have:
   \[ x \HasType y \implies (x \in X \iff y \in X) \]
\end{Axiom}
All experiencing roles must be involved in some action:
\begin{Axiom}{S}
   $\Al{d \in \ExperiencingRoles}{\Fact(d) \in \Actions}$
\end{Axiom}

For the example given above, we would have:
\begin{quote} \sffamily \scriptsize
   Action: [Agent: A person] is writing [Subject: a letter]\\{}
   Predication: [This person] has [the name Erik]\\{}
   Predication: [This letter] has a [romantic nature]\\{}
   Predication: [This letter] has intended recipient [Erik's loved one]\\{}
   Predication: [The writing of this letter by Erik], occurs on a [mid-summer's day]\\{} 
   Predication: [The writing of this letter by Erik], is done using [a pencil]\\{}
   Predication: [The writing of this letter by Erik], is done while [the cat] is watching\\{}
   Predication: [The writing of this letter by Erik], is taking place at [a desk]\\{}
   Predication: [This desk] is located in [a room]\\{}
   Predication: [This room] is lit in [a romantic] way
\end{quote}
  
Finally, a word of warning:
\begin{itemize}
   \item Natural language also harbors `conceptual prejudice'
   \item Most, if not all, Indo-European languages are rather state oriented: `Charles the bold' stands on `the floor'
   \item Some North-American native languages are activity oriented: `Dances with wolves' stands on `what supports us when walking'
   \item Imagine the impact on the way we view \& design systems/organizations: Is nature state oriented or a continuous flow of activities?
\end{itemize}

\section{Activity types}
Based on the above discussions regarding actions and predications, we can identify which roles are of which class, and mark this in the ORM model. For the example from \SmartRef{doctor-visit5}, we have the situation as depictedin \SmartRef{doctor-visit6}.

\Image{7cm}{Compact model of a visit to a Doctor with alternative semantics}{doctor-visit6}
Those state-sequence types which comprise a number of action types (or other activity types) are considered to be (complex) \emph{activity} types. Action types on their own are (atomic) \emph{activity} types.

\QuestionsInChapter

\ChapterBib


==> wsm08.tex <==
\Chapter{Perspectives on work-systems}{perspectives-on-work-systems}
Note: In het huidige dictaat en de outline staat een stukje over
de relatie tussen de strategie van een organisatie en haar inrichting.
Die wil ik eigenlijk "in" de bespreking van actoren betrekken. Een
"organisatie" is een complexe actor. Een actor/agent heeft eventueel
een intend/missie/visie. Die geeft richting aan de inrichting. Hetzij
door de actor/agent zelf (reflexie!) hetzij door een externe partij.

\section{Our perspective on work-systems}
%% Meer uit "van Aken" halen. Met name de bespreking van onderzoek.
When studying/researching the phenomenon of \PDN{work-system}, one may do so
from different perspectives~\cite{1994-VanAken-Organisaties}:
\begin{description}
   \DefItem[Actors] The role of actors beings in \PDN{organization}.
   \DefItem[Structure] The structure of an \DN{organization}. Both formal and informal structures.
   \DefItem[Management] Managing an \DN{organization}'s operations as well as
   its further evolution and/or development.
   \DefItem[Functions] Organizational functions such as marketing, innovation, production, etc.
   \DefItem[Formal] Treating \PDN{organization} as an entity that can be formalized using an appropriate mathematical formalism.
\end{description}

The focus of this course will be on \emph{formal models} of
\PDN{information-intensive-organization}, in particular their structures. In
doing so, we will take a fundamental approach. 

% And of course the white-box/black-box perspective. This is also mentioned in
% chapter 2.

% Also: social/physical/symbolical perspectives






==> wsm09.tex <==
\Chapter{Activity Modeling}{activity-modeling}
\Version{14-04-05}

\Comment{It's probably a good idea to have an appendix with some case descriptions. Before the answers appendix. The questions in the chapters can then refer to these cases.}

\Comment{This should be based more on YAWL and ArchiMate. Study the underlying documents.}

Suitability! The situation as depicted in \SmartRef{doctor-visit4} and \SmartRef{doctor-visit5} may be highly explicit, but one may wonder if the resulting diagrams are still communicatable. Do they still convey the message?
% Relate back to viewpoints discussion in chapter 4.

\section{Introduction}
What do we model?
         \begin{itemize}
              \item Who are involved: Actor domain
              \item What activities do they perform: Activity domain
              \item What (information) objects are used/created: Actand domain
              \item AND: the coherence between these three domains
         \end{itemize}

Modeling domains:
\begin{itemize}
  \item Actor domain
          \begin{itemize}
	     \item Who is involved?
             \item What are possible interactions?
             \item Roles, resources, business functions, ...
          \end{itemize} 
    \item Activity domain
          \begin{itemize}
             \item Activities
             \item Interactions
             \item Relationships 
             \item Structure/decomposition
          \end{itemize}
    \item Actand domain
          \begin{itemize}
	     \item See ORM/DM
	     \item Advanced/complex types
	  \end{itemize}
\end{itemize}

Core concepts:
\begin{description}
   \item[Use-case:] An activity which is triggered by an external trigger.
          
          ``Paying the first month of Mr. Jones' pension.''

   \item[Trigger:] A change in the environment, 
          that initiates a use-case.

          ``Mr. Jones from Bristol turns 65 years of age.''

   \item[Use-case type:] A class of similar use-cases.

          ``Paying the first month of people's pension.''

   \item[Trigger type:] A class of business triggers with similar treatment.
 
          ``People turning 65 years of age.''

   \item[Actor] An organizational entity that is capable of
     performing behavior

     Delivers services to its environment

     ``The NIII providing courses to students''

   \item[Collaboration] A temporary configuration of two or more
     actors resulting in a collective behavior

     ``Insured person and insurance company submitting/receiving a claim''
     
     Can be regarded as a temporary of two role-playing actors into
     an ad-hoc actor, that plays a role providing the behavior of the
     collaboration
\end{description}

\section{Basic modeling language}
The notation is primarily inspired by ArchiMate~\cite{2005-Lankhorst-ArchiMate}. However, as ArchiMate (which aims at an architectural level) does not provide enough detail about process triggering, we have extended the triggering notation with the symbols used by YAWL~\cite{2005-Aalst-YAWL}. 

The ArchiMate language is actually set up such that `local' specializations can be made quite easily. In our case. a specialization is called for that honors our natural language and conception based approach. 
\Comment{Why not just use YAWL all the way, and combine thus with swimming lanes to represent actors? Mapping to UML and ArchiMate models can still be done (in ADISE lecture notes).}

\Image{12cm}{Activity modeling notation}{notation}

\Comment{Discuss the fact that we start at workflow level, and move on to BPR level, and then to architecting level.}

\Comment{More explicitly discuss YAWL patterns.}

A legend of the symbols used is depicted in \SmartRef{notation}. When taking the example from \SmartRef{doctor-visit5} and~\ref{doctor-visit6} and using this new notation, we obtain the situation as depicted in \SmartRef{doctor-visit7} and~\ref{doctor-visit8} respectively.
\Image{14cm}{Visit to a Doctor in activity modeling notation}{doctor-visit7}

\Image{14cm}{Visit to a Doctor with alternative semantics}{doctor-visit8}

\section{Composed activities}
Activities may be composed of yet other activities. This is illustrated in \SmartRef{claim-handling}.
\Image{\textwidth}{Claim handling}{claim-handling}

\Comment{More YAWL patterns.}

%\section{Functions}
\Comment{Also: Coordination \& Control}

%\section{Syntax}
% Refine ontology.

\section{Petri-net based semantics}
\Comment{Reference to Petri!!! Since YAWL refers to transitions as tasks, it probably makes sense to invert the use of states and transitions in the mapping to petri-nets. In other words, next time around we should flip the role of these two.}

In order to gain a more precise understanding of activity models, we will discuss their mapping to simple petri-nets.
In doing so we will, however, loose out on some semantic details. The exercise we undertake in this section is purely for educational purposes. See e.g.\ YAWL~\cite{2005-Aalst-YAWL} for a more detailed formalization.

In \SmartRef{nets} the working of petri-nets are illustrated.
\Image{\textwidth}{Petri-nets}{nets}

In \SmartRef{net-mapping}, the mapping from complex triggering in activity models to petri nets is given. Note that the resulting petri-net will only be applicable for \emph{one} run of the activity.
\Image{\textwidth}{Mapping activity models to Petri-nets}{net-mapping}

An example translation is given in \SmartRef{translation1}.
\Image{\textwidth}{Example mapping of activity models to Petri-nets}{translation1}

\Image{\textwidth}{Mapping participation scopes}{scope-mapping1}
Mapping the semantics of participations of participants (be it actors, actands, or others) to petri-nets can be done as illustrated in \SmartRef{scope-mapping1} and~\ref{scope-mapping2}. In this mapping we have actually used an extended version of petri-nets, called \emph{colored} petri-nets. Note the subtle difference between the two versions with regards to the size of the scope and its impact on the mapping. 
\Image{\textwidth}{Looping and participation scopes}{scope-mapping2}

\section{Quantative semantics}
The petri-net based semantics of activity models focuses on the flow of specific cases through the activity. In addition to the petri-net based semantics, we identify a quantitative semantics. This is illustrated in \SmartRef{nets-prob}. The earlier used claim handling example can be made quantitative as depicted in \SmartRef{claim-handling-prob}.
\Image{\textwidth}{Quantitative analysis of activities}{nets-prob}

\Image{\textwidth}{Claim handling with quantitative information}{claim-handling-prob}

Uses for quantative analysis:
\begin{itemize}
   \item Performance analysis.
   \item Optimization of design.
   \item Critical path analysis.
\end{itemize}

\section{Mapping to UML 2.0 activity diagrams}
In this section we look at the relationship between the activity modeling using the (enriched) ArchiMate notation and the activity diagrams from UML 2.0~\cite{2003-OMG-UML2.0}. UML activity diagrams focus on the flow of activities. Involvement of actors is represented by means of swimming lanes. The claim handling example from \SmartRef{claim-handling} can be represented by means of UML activity diagrams as illustrated in \SmartRef{claim-handling-ad}.
\Image{\textwidth}{Claim handling as an UML 2.0 activity diagram}{claim-handling-ad}

The doctor visit example from \SmartRef{doctor-visit7} and \ref{doctor-visit8} respectively can be represented as the activity diagrams depicted in \SmartRef{doctor-visit9} and \ref{doctor-visit10}
\Image{5cm}{Doctor visit as an UML 2.0 activity diagram}{doctor-visit9}

\Image{10cm}{Doctor visit as an UML 2.0 activity diagram}{doctor-visit10}


\section{Modeling approach}
% Hoe past dit nu bij de aanpak uit H3 en H4??

Outline
\begin{enumerate}
  \item Identify key use cases
  \item Describe key use cases
  \item Compose initial model
  \item Detail model
  \item Re-examine models
  \item Identify phases of activity
\end{enumerate}

\subsection{Identify key use cases}
\begin{enumerate}
  \item Determine the key entity types in UoD
  \item Define for each of the key entity types, the key use case
\end{enumerate}

\subsection{Describe key use cases}
\begin{enumerate}
  \item Verbalise each use case
  \item Single-out: predications, actions, actors, actands and activities.
\end{enumerate}

\subsection{Compose initial model}
\begin{enumerate}
   \item Relate actions, actors and actands. Use graphical notation. 
   \item Introduce activities as composed actions when needed.
\end{enumerate}

\subsection{Detail model}
\begin{enumerate}
  \item Select areas of intest
  \item Gather detailed verbalisations
  \item Compose detailed diagrams
\end{enumerate}

\subsection{Re-examine models}
Re-examine the models in order to:
\begin{enumerate}
  \item Identify and resolve unclear parts
  \item Restructure processes/actors to better resemble the UoD
\end{enumerate}

\subsection{Identify phases of activity}
\begin{enumerate}
  \item Improve clarity of the models by introducing a higher
        level perspective on the domain.
\end{enumerate}


\QuestionsInChapter

\ChapterBib


==> wsm10.tex <==
\Chapter{Resource Modeling}{resource-modeling}

\Comment{Activity-role = grouping of fact roles played by a (typerel) common player in an activity. A business role is really a business-activity role}

\section{Actor modeling}
As discussed before, we have the following modeling domains:
\begin{itemize}
  \item Actor domain
          \begin{itemize}
	     \item Who is involved?
             \item What are possible interactions?
             \item Roles, resources, business functions, ...
          \end{itemize} 
    \item Activity domain
          \begin{itemize}
             \item Activities
             \item Interactions
             \item Relationships 
             \item Structure/decomposition
          \end{itemize}
    \item Actand domain
          \begin{itemize}
	     \item See ORM/DM
	     \item Advanced/complex types
	  \end{itemize}
\end{itemize}
The previous chapter focussed on the activity domain. This chapter promissed to discuss the actor and actand domains. Thus far, however, we have been ``sharpening our axe'' by discussing complex types. Actors and actands are usually complex types from a domain modeling perspective. 

\Comment{Next year this should be made more archimate-like.}
For the actor domain, we (re-)introduce the following core concepts:
\begin{description}
   \item[Actor --] An entity that performs behavior. I.e.\ it is actively involved in an activity.
   \item[Actor type --] An entity that performs behavior. I.e.\ it is actively involved in an activity.
   \item[Use-case (instance) --] An activity which is triggered by an external trigger.
   \item[Use-case type --] A class of similar use-cases.
   \item[Process --] Synonym for use-case type.
   \item[Business use-case (instance) --] A use-case which an organisation/business executes to fulfill a service to the outside world.  
   \item[Business use-case type --] A class of similar business use-cases.
   \item[Business process --] Synonym for business use-case type.
   \item[Business role (type) --] A named specific contribution that an actor (type) may provide to a business use-case (type). 
   
   Is a special kind of role (type). Such a role is usually defined by functional responsibilities.
   
   \item[(Business) role-player (type) --] An actor (type) playing a (business) role (type).
   
   \item[Business function --] A virtual or idealised organisation within a business/organisation.

   Identification can be based on different criteria: knowledge/skills required, use of resources, type of functional behaviour, etc.
   
   \item[(Business) collaboration (type)] A temporary configuration of two or more
   actors (types) resulting in a collective behavior. 

   ``Insured person and insurance company submitting/receiving a claim''
     
   Can be regarded as a temporary of two role-playing actors into
   an ad-hoc actor, that plays a role providing the behavior of the
   collaboration
\end{description}

\Image{\textwidth}{Claim handling process with business-roles}{claim-handling2}
\SmartRef{claim-handling2} shows an example activity model with associated actor types and role types. The underlying ORM domain model is depicted in \SmartRef{claim-handling2-map}.
\Image{0.5\textwidth}{Claim handling process with business roles mapped to ORM}{claim-handling2-map}

\Image{0.5\textwidth}{Claim handling process with business-functions}{claim-handling3}
\SmartRef{claim-handling3} shows an example activity model where the business-function within the insurer is shown wich is responsible for the actual claim handling. The underlying ORM domain model is depicted in \SmartRef{claim-handling2-map}. The refined ORM domain model is depicted in \SmartRef{claim-handling3-map}.
\Image{0.5\textwidth}{Claim handling process with business-functions mapped to ORM}{claim-handling3-map}

\section{Actand modeling}
For the detailed modeling of actands, we essentially use ORM. This is illustrated in \SmartRef{claim-handling4-map}.
\Image{0.5\textwidth}{Refining actands for claim handling process}{claim-handling4-map}

%Structural actors

%%% Check slides van vorig jaar!!!


\QuestionsInChapter

\ChapterBib


==> wsm11.tex <==
\Chapter{Service modeling}{service-modeling}
\Version{24-05-05}

% ArchiMate decoupling of events.

\section{Service}

\begin{itemize}
   \item Service: The net effect (added value) of an actor's behaviour that is
   regarded to be useful (value!) by at least one actor.
   
   Examples:
   \begin{itemize} 
     \item Service your car
     \item Provide you with a mortgage
     \item Do yourself a favor, and ....
   \end{itemize}
   
   \item Service offering: The potential of an actor to be engaged in an
   activity, where this engagement may be perceived as usefull by some other
   actor. 
   
   Note: both of these actors might be complete (open active) systems!

   Is at the type level!

   \item Service delivery: The actual engagement.

   At the instance level!

   \item An information system can be regarded as a service providing actor:
   \begin{itemize}
      \item Environment $\Rightarrow$ Consumes services
      \item System $\Rightarrow$ Delivers services
   \end{itemize}
   
   \item The system may use services offered by other systems in order to deliver the service. This ``other system'' then become ``infrastructure'' to the original system. 
   
   The latter system is adding value to the basic services offered by the ``infrastructural system''.

   \item Regarding a system as a service-providing entity allows us to regard this system as a \emph{black box}.
   
   \item If some part of a system domain is viewed as an information system by some viewer, then this information system {\em may} be regarded as a black-box which interacts with its environment.

   \item The activity and resource modeling as discussed in the previous chapters basically took a \emph{white box} approach to a system. We were looking inside the system to see what activities take place, who the actors are that execute the activities, etc.

   \item When regarding a system as a black box, we obtain \emph{service information hiding}, in other words, we do not see the way a service delivery is actually implemented.

   \item Service information hiding as defined by A.P. Barros:

   A technique (for business modeling) should allow the formulation of service requests to be independent of their actual processing.
   
   In other words, we should be able to talk about service independent of the (business) processes that implement them
   
   \item Why information hiding?
   \begin{itemize}
      \item One: description of a service
      \item Many: ways to implement/deliver
      \item Useful for:
            \begin{itemize}
                \item Software
                \item Organisations
                \item ... any system that is purposely designed
	    \end{itemize}
   \end{itemize}
\end{itemize}
 
\section{Modeling services}
  
\begin{itemize}
   \item A service delivery can be regarded as moving through a number of states and transitions.
      
   We do not want to ``see'' the details of the transition, but do want to see the overall states of the service delivery as they are experienced by the service consumer.
   
   We will focus on the interaction between the consumer and offerer of the service.
   
   \item A service can be regarded as a collaborative activity between the provider of the service (e.g.\ an organisation), the consumer of the service, and potentially some additional parties.
    
   \item As such, a service can be modeled as any other activity, however, in this case the system providing the service is treated as a black-box.
   
   \item An example is shown below:
   
   \ImageBox{10cm}{claim-handling5}

   \item Focus on added value of services
   \item Focus on interactions needed (between the supplying and consuming actors) in the service delivery 
   \item Do not (yet) focus on the processes needed to deliver the actual service 
\end{itemize}

\section{Quality of service}
% Keep in sync with ADISE

The functional behavior of a service can be modeled by means of an activity model focusing on the interaction between the service provider and the consumer of the service. However, there is more to services than their ``functional'' behavior. Services may occur at different levels of \emph{quality}. We now provide a brief discussion of the notion of quality, basing ourselves on \cite{1991-ISO-Quality,1996-ISO-KSP}. The essence of \DN{quality} of a \DN{system} is captured in the following
definition:
\begin{Definitions}
  \DefinitionItem{quality}
\end{Definitions}

\Comment{Check Quality definition against ISPL}

The \PDN{quality} we referred to, are really an abbreviation of \PDN{quality-property},
which are a special class of \PDN{systemic-property}:
\begin{Definitions}
  \DefinitionItem{quality-property}
\end{Definitions}
These quality properties can be used to judge a service offered by a system, or express a desired quality level.

In \cite{1991-ISO-Quality,1996-ISO-KSP} a range of key classes of \PDN{quality-property} are identified. These classes are referred to as \PDN{quality-attribute}:
\begin{Definitions}
  \DefinitionItem{quality-attribute}
\end{Definitions}
Each \DN{quality-attribute} may also have a number of sub-characteristics, zooming in on specific quality characteristics. In \cite{1991-ISO-Quality,1996-ISO-KSP} the following \PDN{quality-attribute} have been identified: 
\begin{Definitions}
  \DefinitionItem{efficiency}
  \DefinitionItem{functionality}
  \DefinitionItem{reliability}
  \DefinitionItem{maintainability}
  \DefinitionItem{portability}
  \DefinitionItem{usability}
\end{Definitions}
From the consumer of a service offered by a system, mainly the \emph{functionality}, \emph{reliability} and \emph{usability} attributes will be of interest.

The repeated consumption of a service from one actor by another actor may be governed by a (formal or informal) contract. Such a contract defines the actual service (i.e.\ its functional behavior), as well as the non-functional quality properties that it should exhibit. For example: \emph{after lodging an insurance claim, the client will be informed of the outcome within 10 work-days}. Such contracts make explicit the mutual committments/responsibilities of the actors involved in a service delivery.

\section{Information systems as event-driven machines}
\begin{itemize}
   \item When viewing a system/organisation as a black box, its (model!) becomes a machine that ``eats'' input
   and ``produces'' output.

   In the case of an information system, the input/output consists of data representing information.
   
   \item Formally, we can model this as: $s: (\TimePoints \PartFunc \Elements) \Func (\TimePoints \PartFunc \Elements)$.
   
   When observing system $s$, a viewer has a conception of $s$ where in the course of time ``things'' are fed into the system, while the system produces yet other ``things''. These ``things'' are \emph{elements} from the viewer's conception.

   \item If $s(I) = O$, then system $s$ converts input stream $I$ into stream $O$.

   \item If $s(I)$ and $\DefinedAt{I}{t}$, then one can say that for system $s$ an event occurs at $t$, being the reception of $I(t)$.

   \item In the case of an information system, we could have:

         {\sf ADD Person `Erik' works for department `IRIS'}

         and

         {\sf LIST People who work for department `IRIS'} 

         as inputs. The output might be:

         {\sf accept}

         and

         {\sf Erik, Stijn, Theo}

         respectively
\end{itemize}

\ChapterBib


==> wsm13.tex <==
\section{Organizational metaphors}
\SmartLabel{Section}{metaphors}

In civil and military architecture it has become an accepted practice to copy
patterns from constructions in nature and use them in our own constructions.
Consider for instance the construction of an airplane.
Construction patterns are borrowed from biology in an attemtp to combine
flexibility, strength and low weight.  In line with this practice, it makes
perfect sense to see if we can use patterns and properties of other systems,
such as systems that occur in nature, in the design of information systems. For
instance, the way in which the development and design of software agents is
approached, draws more and more on the way biological organisms interact and
grow \cite{2000-Odell-Agents1,2000-Odell-Agents2,2000-Wooldridge-GAIA}. In the
field of complex-adaptive systems \cite{1995-Holland-HiddenOrder}, even more
inspiration may be gained on the development of information systems that are
better equipped to deal with complexity and evolution of their environment.

When modeling/developing \PDN{organization}, one may regard these
\PDN{organization} from the perspective of different metaphors:
\begin{quote} \it
   ``All theories of organization and management are based on implicit images
   or metaphors that persuade us to see, understand, and imagine situations in
   partial ways. Metaphors create insight. But they also distort. They have
   strengths. But they also have limitations. In creating ways of seeing, they
   create ways of not seeing. Hence there can be no single theory or metaphor
   that gives an all-purpose point of view. There can be no 'correct theory'
   for structuring everything we do.''
\end{quote}
In \cite{1998-Morgan-OrganisationParadigms}, the following eight well-known
methaphors are discussed:
%% Check Morgan!!
\begin{description}
   \DefItem[Machines] Efficiency, waste, maintenance, order, clockwork, cogs in
   a wheel, programmers, inputs and outputs, standardization, production,
   measurement and control, design 
   \DefItem[Organisms] Living systems, environmental conditions, adaptation,
   life cycles, recycling, needs, homeostasis, evolution, survival of the
   fittest, health, illness
   \DefItem[Brains] Learning, parallel information processing, distributed
   control, mindsets, intelligence, feedback, requisite variety, knowledge,
   networks
   \DefItem[Cultures] Society, values, beliefs, laws, ideology, rituals,
   diversity, traditions, history, service, shared vision and mission,
   understanding, qualities, families
   \DefItem[Political Systems] Interests and rights, power, hidden agendas and
   back room deals, authority, alliances, party-line, censorship, gatekeepers,
   leaders, conflict management
   \DefItem[Psychic Prisons] Conscious \& unconscious processes, repression \&
   regression, ego, denial, projection, coping \& defense mechanisms, pain \&
   pleasure principle, disfunction, workaholic
   \DefItem[Flux and Transformation] Constant change, dynamic equilibrium,
   flow, self-organization, systemic wisdom, attractors, chaos, complexity,
   butterfly effect, emergent properties, dialectics, paradox
   \DefItem[Instruments of Domination] Alienation, repression, imposing values,
   compliance, charisma, maintenance of power, force, exploitation, divide and
   rule, discrimination, corporate interest
\end{description}

%\S[
%  \T[Organisational metaphors (Morgan)]T
%  \I[ 
%     \item Organisations as Machines
%     \item Organisations as Organisms
%     \item Organisations as Brains
%     \item ...
%  ]I
%]S

%\S[
%  \T[Organisations as machines]T
%  \I[
%     \item Organizing is engineering
%     \item Military style of organisation
%     \item Fixed division of tasks
%     \item Hierarchical supervision
%     \item Detailed rules \& regulations
%  ]I
%]S

%\S[
%  \T[Organisations as Organisms]T
%  \I[
%     \item Open systems
%     \item Homeostasis
%     \item Evolution
%  ]I
%]S

%\S[
%  \T[Organisations as Brains]T
%  \I[
%     \item Learning abilities
%     \item Distribution of intelligence
%     \item Learning organisations
%  ]I
%]S




==> wsmma.tex <==
\chapter{Mathematical Notations}
\label{ch:Math}

The mathematical notations used in the \DaVinci\ series are explained
briefly in this appendix.

\section{Sets}
In addition to the set operations: $\union, \intersect, \setminus, \subseteq$
with their usual meaning, we also define:
\begin{eqnarray*}
   A \subset B     & \Eq & A \subseteq B \land A \neq B \\
   A \not\subset B & \Eq & \lnot A \subset B \\
%   A \SubElem x    & \Eq & A \setminus \setje{x} \index{$\SubElem$}\\
%   X \AddElem x    & \Eq & A \union    \setje{x} \index{$\AddElem$}\\
\end{eqnarray*}

The power set of a set $A$, i.e.\ the set of all subsets of $A$,
is denoted as $\Powerset(A)$, where:
\[ \Powerset(A) \EQ \Set{B}{B \subseteq A} \]

%Some sets will have a total ordering, for a finite set $X$ with a total 
%ordering $< ~\subseteq X \times X$ we can define the extremes:
%\begin{eqnarray*}
%   \Max(X) & \Eq & x \in X \mbox{\bf ~such that~} \Al{a \in X}{a < x \lor a=x} \\
%   \Min(X) & \Eq & x \in X \mbox{\bf ~such that~} \Al{a \in X}{x < a \lor a=x}
%\end{eqnarray*}


\section{Functions}
A partial function $f$ from $A$ to $B$ is defined by $f: A \PartFunc B$.
Formally, it is a relation $f \subseteq A \times B$ such that $\tuple{a,b} \in
f \land \tuple{a,c} \in f \implies b=c$.  This property makes it possible to
write $f(a) = b$ instead of $\tuple{a,b} \in f$.

A function $f$ is a set of binary tuples.  The first and second values of these
binary tuples are identified as:
\begin{eqnarray*}
   \Proj_1(f) & \Eq & \Set{a}{\tuple{a,b} \in f}\\
   \Proj_2(f) & \Eq & \Set{b}{\tuple{a,b} \in f}
\end{eqnarray*}
The following abbreviations are used for (partial) functions:
\begin{eqnarray*}
   \FuncDom(f)      & \Eq & \Proj_1(f)\\
   \FuncRan(f)      & \Eq & \Proj_2(f)\\
   \Defined{f(a)}   & \Eq & a \in \FuncDom(f)\\
   \UnDefined{f(a)} & \Eq & a \not\in \FuncDom(f)\\
\end{eqnarray*}
For unary functions, we will write $\DefinedAt{f}{a}$, and
$\UnDefinedAt{f}{a}$, instead of $\Defined{f(a)}$, and $\UnDefined{f(a)}$
respectively. Further, $\DefinedAt{\Vector{f}{n}}{\Vector{a}{m}}$ is employed
as an abbreviation for: 
   $\All{1 \leq i \leq n}\Al{1 \leq j \leq m}{\DefinedAt{f_i}{a_j}}$.

A total function $f$ from $A$ to $B$ is defined by $f: A \Func B$.  Formally,
$f: A \PartFunc B$ for which $\FuncDom(f) = A$.

%The (partial or total) function $\Restr{f}{A'}$ is the function $f$ 
%restricted to a subdomain $A' \subseteq \FuncDom(f)$.
%This function is defined by:
%\begin{eqnarray*}
%   \Restr{f}{A'} & \Eq & \Set{\tuple{a,b} \in f}{a \in A'} 
%\end{eqnarray*}

%A notational shorthand for denoting
%tuples of functions is used in this thesis: $\tuple{p,a} \Eq \FnElem{p}{a}$.
%As an example consider a function $f$ such that 
%$f = \setje{\tuple{p,a},\tuple{q,b}}$.
%This function will alternatively be denoted as 
%$\setje{\FnElem{p}{a},\FnElem{q}{b}}$.
%For a function $f$ we define:
%\begin{eqnarray*}
%   f \ChangeElem \FnElem{x}{y} & \Eq & 
%     \Set{\FnElem{v}{w} \in f}{v \not= x} \AddElem \FnElem{x}{y}
%\end{eqnarray*}

%In some cases, functions have to be denoted as an expression,
%for this purpose we apply lambda calculus (\cite{Book:84:Barendregt:LamdaCalculus}).
%An example is: $f=\LambdaFun{x}{\SIf{x = 0}{0}{1/x}}$.
%In the definition of functions, we will use $\Undefined$ to indicate that
%the function is not defined for a particular value.
%Sometimes we will also use \mbox{\bf error} instead of $\Undefined$, 
%to indicate that the function/operation leads to an error situation.

%The inverse of a function, or relation, $R$ is defined as:
%$\Inverse{f} \Eq \Setje{\FnElem{y}{x}}{\FnElem{x}{y} \in f}$.
%The inverse $\Inverse{f}$ of a function, is a function if $f$ is an
%injection (and thus a bijection on $\FuncDom(f)$).
%Functions $f$ and $g$ can be composed, if
%   $\FuncRan(g) \subseteq \FuncDom(f)$
%by $\FuncComp$ as follows: 
%   $f \FuncComp g \Eq \LambdaFun{x}{f(g(x))}$.
%Relations can be composed by $\Conc$ as:
%$R \Conc S \Eq 
%   \Setje{\tuple{x,z}}{\tuple{x,y} \in R \land \tuple{y,z} \in S}$. 
%
%If $h$ is a function $h: X \PartFunc Y$, and $X$ is an ordered domain, then 
%the last and first value to which a value has been assigned is identified by:
%\begin{eqnarray*}
%   \Last(h)  & \Eq & \Max \FuncComp \FuncDom(h) \index{$\Last$}\\
%   \First(h) & \Eq & \Min \FuncComp \FuncDom(h) \index{$\First$}
%\end{eqnarray*}

%\section{Proofs}
%In proofs, the $\!\!\!\!\Therefore$ symbol stands for a logical deduction
%step, and a logical equivalence in a proof is denoted by $\!\!\!\!\EqTo$.
%The motivation for a deduction step or equivalence is provided in
%parenthesis: $\Explain{motivation of the step}$.


%\section{Tuples}
%Finally, for tuples over any domain, three operators exists:
%\begin{eqnarray*}
%   \SFOp{Head}(\tuple{\Vector{x}{n}}) & \Eq & 
%      x_1                                 \index{$\SFOp{Head}$} \\ 
%   \SFOp{Tail}(\tuple{\Vector{x}{n}}) & \Eq & 
%      \tuple{x_2,\ldots,x_n} \index{$\SFOp{Tail}$} \\
%   \tuple{\Vector{x}{n}} +\!\!+ \tuple{\Vector{y}{n}} & \Eq & 
%      \tuple{\Vector{x}{n},\Vector{y}{n}} \index{$+\!\!+$}
%\end{eqnarray*}
%for these operators we have:
%%$\tuple{\SFOp{Head}(x)} +\!\!+ \SFOp{Tail}(x) = x$

\section{Relations}
If $R \subseteq X \times X$ is a relation, then
we will use: 
  $x \MT{R} y \MT{R} z$ 
as an abbreviation of:
  $x \MT{R} y \land y \MT{R} z$.


==> wsmpr.tex <==
\Preface
\Version{17-01-06}

In 2006, the course ``Modeling of Organizations'' is taught for the third 
time. This third time will be the second time we will use the new
lecture notes ``Work Systems Modelling'' from the \DaVinci\
series. These lecture notes, however, will be evolved further hand-in-hand with
the actual process of lecturing. In the academic year 2005/2006, a second
incarnation of these lecture notes will be created, where the aim is to
deliver these lecture notes in three increments.

An important step that will be taken in this academic year is the integration
of the ICIS Work Systems Modelling lecture notes with the NICI course on
Organisational Dynamics. The first results of this integration will start to
appear in the second and third trimester.

Needless to say that any feedback from either students or colleagues is more
than welcome.

The priority of this initial version of this textbook is on completeness of the
topics that need to be covered, rather than readability and completeness of
text. Students are advised to make notes during lectures.

Special thanks go out to the students attending the ``Information Intensive
Organizations'' course in 2004/2005. They where the guinea pigs for the new
Lecture Notes, pointing out several major shortcomings. Also thanks go out to
Arnoud Vermeij, for adding several questions and answers, as well as commenting
on draft versions of these lecture notes.


